Credit Scores: Performance and Equity

Credit scores are critical for allocating consumer debt in the United States, yet little evidence is available on their performance. We benchmark a widely used credit score against a machine learning model of consumer default and find significant misclassification of borrowers, especially those with low scores. Our model improves predictive accuracy for young, low-income, and minority groups due to its superior performance with low quality data, resulting in a gain in standing for these populations. Our findings suggest that improving credit scoring performance could lead to more equitable access to credit.

==> New_Parts/Racial_Disparities_-_Submission/Sections/background.tex <==

\section{Background Information}\label{sec:information}

The debt collection industry in the United States is large and growing.  According to a 2018 annual report by the Consumer Financial Protection Bureau, debt collection is a \$10.9 billion industry that employs nearly 120,000 people across approximately 8,000 collection agencies in the United States.  In 2010 alone, U.S. businesses placed \$150 billion in debt with collection agencies.  When the debt is unsecured, the owner of the debt can either negotiate with the debtor to bring their debt to current, write off the debt, or file a debt collection lawsuit.  This section will summarize the key institutional details surrounding debt collection lawsuits and the laws regulating the debt collection industry.  

\subsection{Debt Collection Litigation Process}

Debt collection litigation typically begins when a creditor files a ``Summons and Complaint'' in a state civil court.\footnote{These courts have many different names, including municipal court, superior court, justice court, county court, etc.}  This document names the parties involved and states the amount owed (including interest and, in some cases, attorney fees and court costs).  The summons is served to the defendant to notify them of the lawsuit.  It also provides the defendant with additional information, including the deadline for which the debtor must file a formal response to the court.  If the debtor does not meet this deadline, the creditor will usually ask the court to enter a default judgment, at which point the defendant is obligated to abide by the court's ruling and is subject to the punishments requested by the court.  

For most routine debt collection lawsuits, if the debtor files a formal response to the lawsuit, a trial date will be requested and set by the court.  In some courts, settlement conferences are held to provide both parties with the opportunity to settle the case before the trial.  Once the creditor obtains a judgment, the creditor might request a ``debtor's examination,'' which would require the debtor to appear in court and answer questions about their finances.  This process informs the creditor how it can collect the judgment.  The most common methods for enforcing the judgments are to garnish wages or bank accounts.\footnote{Courts can also seize and sell the debtor's personal property, though this is relatively uncommon.}  If a dispute is settled before trial, the creditor gives up the ability to collect on the debt by garnishing the debtor's bank accounts or wages, and therefore creditors often require a one-time lump sum payment to drop the suit. 

\subsection{Laws Regulating Debt Collection}

Debtors are granted some protections throughout the debt collection process. The 1977 Fair Debt Collection Practices Act (FDCPA) is the primary federal law governing debt collection practices. The statute's stated purposes are as follows: to eliminate the abusive practices used to collect consumer debts, such as calling the debtor at all hours of the night and showing up to their place of employment, to promote fair debt collection, and to provide consumers with an avenue for disputing and obtaining validation of debt information to ensure the information's accuracy.  

The Consumer Credit Protection Act (CCPA) of 1968 restricts the amount of earnings that creditors can garnish from defendants' weekly disposable income to 25\% or the amount by which disposable earnings are greater than 30 times the minimum wage. State laws can increase the share of wages protected from debt collection garnishments. For example, a creditor in Missouri can only garnish 10\% of after-tax wages if the debtor is the head of their household. However, the burden to assert these protections is typically on the debtor, and take-up is relatively low. No federal law limits the amount of savings that can be seized from a debtor's bank accounts.    

While not directly related to debt collection, other protections have been put in place to protect consumers in the credit market. For example, the Equal Credit Opportunity Act (ECOA), enacted in 1974, makes it illegal for creditors to discriminate against any applicant based on race, color, religion, national origin, sex, marital status, age, or participation in a public assistance program.\footnote{This law is enforced by the Federal Trade Commission (FTC).} The law applies to everyone who regularly participates in a credit decision, including banks, retail and department stores, bankcard companies, finance companies, and credit unions. The ECOA applies to the decision to grant credit and set credit terms. 

Furthermore, the Fair Credit Reporting Act (FCRA) of 1970 promotes the accuracy, fairness, and privacy of consumer information contained in the files of consumer reporting agencies. The law protected consumers from including inaccurate information in their credit reports. The Credit Card Accountability Responsibility and Disclosure (CARD) Act of 2009 established fair and transparent credit card practices. Key provisions include giving consumers enough time to pay their bills, prohibiting retroactive rate increases, making it easier to pay down debt, eliminating ``fee harvester cards'', and eliminating excessive marketing to young people. Despite these protections, abusive debt collection practices still exist, and, as we will show, black and Hispanic borrowers are disproportionately impacted by debt collection judgments.  


==> New_Parts/Racial_Disparities_-_Submission/Sections/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

We find that Black or Hispanic individuals are 39\% more likely to accumulate debt collection judgment on their credit report, even after controlling for credit score and other credit characteristics.  The debt collection gap does not appear to be driven by states with high levels of racial bias, but does correlate with areas with a high number of payday lenders, many income-less households, and lower shares of tertiary education. We use a second dataset containing zip codes in Missouri to explore potential explanations for the disparity in debt collection judgments and conclude that the racial disparity in judgments is unlikely to be driven by strategic decisions of creditors based on the likelihood of attorney representation or the outcomes of previous cases.  

Given that differences in state-level variation in taste-based discrimination, the likelihood of attorney representation, and previous case outcomes do not appear to be driving our results, we conclude that the persisting disparities in judgment rates may be indicative of systemic racism resulting in financial hardships that are not reflected in the credit report data. Keil and Waldman (2015) quote Lance LeCombs, the Metropolitan St. Louis Sewer District's spokesman, who claims his company has no demographic data on its customers and treats them all the same. He said the racial disparity in its suits was the result of ``broader ills in our community that are outside of our scope and exceed our abilities and authority to do anything about." One such broader ill is the average difference in wealth across black and white households. Estimates provided by the United States Census Bureau in 2016 suggest that the average black household has a net worth of \$12,920, contrasting sharply with the typical white household's net worth of \$114,700 - a staggering wealth gap of \$101,780. This significant disparity in wealth could critically affect a household's ability to weather negative income shocks. Back of the envelope calculations suggest that closing the wealth gap would help to close the judgment gap.  

As the number of debt collection cases rises, it is crucial to identify the extent to which racial disparities exist and how they enter the debt collection system. Future research should explore policies meant to provide more protection to consumers and their impact on the racial disparity in debt collection judgments. For example, such reforms could require debt-buying companies to prove they own the debt before they can sue a debtor, preventing companies from winning judgments when the statute of limitations has expired on a debt\footnote{In most states, the law currently requires defendants to know that the statute of limitations has expired, and raise it as a defense in court.}, or require collection attorneys to prove they have a legal right to collect attorney fees and provide an itemized list of their work on the case to win an attorney's fee through a default judgment\footnote{Currently when companies sue, they often request such fees, which are usually granted and passed on to the debtor as part of the judgment. For example, in Missouri, the fees are typically set at 15 percent of the debt owed, even though attorneys may spend only a few minutes on a suit.}. When states provide legal protections for debtors, such as allowing those with children to keep more of their pay under a head of family exemption, the burden is typically on the debtor to assert these protections. Another policy reform could require a clear notice that these are provided to debtors.


==> New_Parts/Racial_Disparities_-_Submission/Sections/data.tex <==
\section{Data} \label{sec:data}

This paper uses two different datasets to explore racial differences in debt collection judgments. The first is an individual-level panel dataset that combines financial information from individuals' Experian credit reports with demographic data from the Home Mortgage Disclosure Act (HMDA) database. This dataset is used to document the racial disparities in debt collections judgments and to identify where the disparity is the largest.  The second is a zipcode-level panel dataset containing debt collection court cases filed in Missouri between 2004 and 2013, along with other neighborhood characteristics.  This dataset is used to explore the extent to which neighborhood debt collection characteristics are driving the racial gap in judgments.

\subsection{Credit Report/HMDA Individual Level Panel}

To construct the Credit Report/HMDA matched panel, we start with a panel data set of credit bureau records. The Credit Report data is an anonymous, nationally representative, individual-level panel dataset from 2004Q1 to 2017Q2 with quarterly observations. This data contains a random draw of over half a million individuals with an Experian credit report and consists of over 200 variables that allow us to track all aspects of individuals' financial liabilities, detailed delinquencies, various types of debt with the number of accounts and balances, credit score, and an imputed income estimate. Importantly, this data also indicates the number of judgments outstanding against a given individual in a given quarter from 2013Q1 to 2017Q2.  Also included is where a judgment has been petitioned or satisfied. 

While this data does include an individuals age and zipcode, the Equal Credit Opportunity Act (ECOA) generally prohibits a creditor from inquiring about the race, color, religion, national origin, or sex of an applicant. As such, many data sets, including the Experian credit report data, lack information about an applicant's race. To obtain this information, we match the Experian credit report data with demographic information from the Home Mortgage Disclosure Act (HMDA) database.  The Home Mortgage Disclosure Act mandates that almost all mortgage lenders report comprehensive information on the applications they receive and whether they approve the loan.\footnote{Exceptions are granted only for very small or strictly rural lenders (\cite{butler2022racial}). Approximately 95\% of all first-lien mortgages are reported to the HMDA database (\cite{avery2017profile}), with the coverage rate likely being higher for properties in MSAs.} Mortgage lenders submit applicants' racial and ethnic background, personal attributes, and loan application details, such as the requested loan size, income, loan purpose (purchase, refinancing, improvement), co-applicants, loan priority (first or second lien), and the census tract location of the property, to the HMDA database. If a loan is granted, any loan sale is reported, along with an indicator for sale to any quasi-government entity. Our HMDA data ranges from 2007 to 2017.

Both the credit bureau and HMDA data are anonymized, with no unique identifier linking the two datasets; however, the detailed information on originated mortgages in both datasets allows mortgages to be matched based on their features (\cite{butler2022racial}). Following \cite{butler2022racial}, we first apply a set of filters to the mortgages from our credit bureau data. We require the mortgage to be the borrower's only first lien mortgage at the time to ensure that the borrower's location in the credit bureau data will match the property location in the HMDA data. We also require that the person lives in an MSA directly following the loan origination and that they were the only applicant on the loan. We also follow the approach of \cite{butler2022racial} for processing the HMDA data. We concentrate on home purchase and refinancing loans (excluding home improvement loans due to their less defined nature in both datasets). We mandate mortgages to be on owner-occupied properties to ensure that the property location aligns with the borrower's location in the credit bureau data. We also stipulate that the mortgage must be a first lien and the property must be situated within an MSA (where HMDA data is most comprehensive). Lastly, we require that the mortgage have only one applicant/borrower, so the demographic data directly applies to the matched individual in the credit bureau data.  

After applying the filters to both the HMDA and credit bureau data, the target population for the matched sample comprises borrowers obtaining a home purchase or refinance loan individually (no co-applicant), for their primary residence located within an MSA, between 2007 and 2017. We matched the credit bureau data to HMDA records following the procedure outlined in \cite{butler2022racial}, with slight modifications. Because our Experian credit report data only reports an individuals zip code, we first matched our zip code level credit bureau data to Census 5-Digit Zip Code Tabulation Areas (ZCTA5s) using the Missouri Census Data Center's Census Tract - ZIP/ZCTA crosswalk files.\footnote{USPS zip codes are not areal features used by the Census but a collection of mail delivery routes that identify the individual post office or metropolitan area delivery station associated with mailing addresses. ZIP Code Tabulation Areas (ZCTAs) are generalized areal representations of United States Postal Service (USPS) ZIP Code service areas. HMDA data reports 2010 census tracts starting in 2013. For loans originated from 2003 to 2012, HMDA data uses the 2000 census tracts. We successfully matched ZCTAs for 96.3\% of Census Tracts in the HMDA data. Crosswalk URL:  \url{https://mcdc.missouri.edu/applications/geocorr2014.html}.} This process increased our HMDA sample from 28.4M to 50.7M observations as it assigns each individual to all potential ZCTA5s.

We matched mortgages in the credit bureau data to HMDA data based on six characteristics: origination year, ZCTA5, loan amount, loan purpose (purchase or refinancing), mortgage type (conventional, FHA, or VA), and if/to which quasi-government entity the loan is sold. We implement an exact matching algorithm, as opposed to using nearest matches or propensity scores, to ensure the highest accuracy for our matched dataset.\footnote{In our analysis of home purchase loans, we focus on borrowers without an outstanding first-lien mortgage balance from the previous two quarters. To mitigate the impact of integer-based origination balances in HMDA data, we consider credit bureau data origination balances within a specific range. By allowing neighboring integer values, we prevent inaccuracies caused by rounding discrepancies. All other matching variables are exact matches.}  Replacing ZCTA5 with census tracts, 90.4\% of originated mortgages in the HMDA data are unique based on these characteristics. Before expanding census tracts to ZCTA5, we removed duplicate entries. After expanding the census tracts to ZCTA5 and prior to merging with credit bureau data, we filtered out observations with identical race, gender, ethnicity, and mortgage origination details. These entries appear because we expanded our census tract data to the ZIP code level. This filter and the removal of duplicates based on our matching variables result in a sample of 39.7M observations. 

\cite{butler2022racial} identifies two potential sources of error when matching HMDA with credit bureau data. First, a data error in one of the matching variables might lead to a mismatch. Second, HMDA-reporting and non-reporting lenders may originate identical, otherwise unique mortgages. They argue that such mismatches should not introduce bias in estimates beyond pure noise. Our matching process, which expands HMDA data from census tract to ZIP code level, introduces two additional error sources. First, copies created by assigning an individual from a given census tract to multiple zipcodes may find a matching observation in the incorrect zip code. This would be a severe problem if the correct loan was not observed in our HMDA data. However, the HMDA data covers 90\% of unique mortgages at the census tract level, and hence we likely observe the correct loan as well. Second, two loans from different census tracts with identical matching variables could be copied to the same ZIP code. This issue affects 34\% of HMDA observations. This is slightly more likely in census tracts with diverse populations. We demonstrate this in Figure \ref{fig:deletion_by_majority_share}, which shows the probability of having duplicated observations along our match variables after expanding the census tract level data to ZCTA5. To address this problem, we remove observations with conflicting protected attribute information at the match level.

We report the match rate as well as summary statistics on the match in Table \ref{table:1}. Panel A displays the match rate for home purchase mortgages, refinance loans, and both types of loans combined. We find a corresponding HMDA mortgage for 45.6\% of the mortgages in the credit bureau data with a slightly higher match rate for refinance loans as opposed to home purchase loans. Given that HMDA covers 95\% of mortgages, 90\% are unique at the census tract level, 96\% of census tracts are merged to ZCTA5, and 66\% of observations are unique based on our matching variables, the best achievable match rate is approximately 54.2\%. In other words, our algorithm successfully found matches in roughly 83.9\% (0.455/0.542) of the potential cases. 

The summary statistics in panels B and C of Table \ref{table:1} assess whether our matched sample is representative of the original population for home purchase loans and refinance loans respectively. Panel B reveals that the successfully matched home purchase mortgage sample is largely representative of the initial population of credit bureau mortgages. Similarly, Panel C demonstrates that the matched sample of refinance loans accurately represents the starting sample from the credit bureau data.

Since our study focuses on the impact of race on debt collection judgments, it is essential to determine if minorities are underrepresented in the data or if a specific type of minority borrower, such as high or low income, is underrepresented. Following \cite{butler2022racial}, we investigate whether race plays a role in the likelihood of matching originated mortgages from the HMDA database to our sample of credit bureau records. The regressions in Table \ref{table:2} assess the probability of successfully matching a loan based on borrower race. The coefficients on Black and Hispanic, and the interaction terms Black X log(Income) and Hispanic X log(Income) in column (1) are insignificant. 
While there is a slight indication of selection bias through the combination of race and income for Hispanic applicants seeking refinance mortgages, we can control for variables from both databases, which mitigates concerns about selection bias.

Table \ref{table:3} provides summary statistics for our individual-level panel data starting in 2013Q1 and ending in 2017Q2.\footnote{While a larger sample of data is used to match credit report and HMDA data, we limit our sample for our regression analysis as judgment data isn't reliably available in every quarter of the credit report data.} Similar to patterns identified in \cite{butler2022racial}, Columns 1 and 2 indicate that individuals within the matched data set generally exhibit higher credit scores, are relatively younger, and have a higher likelihood of holding a mortgage compared to the average U.S. resident who has a credit history. These patterns are anticipated, as individuals must either obtain a new mortgage or refinance an existing one between 2007 and 2017 to qualify for inclusion in the matched panel. Columns 3–5 demonstrate that the White borrowers in the matched panel have higher credit scores and incomes in comparison to minority (non-Asian) borrowers. 

We supplement our matched Credit Bureau/HMDA panel with data on racial biases in U.S. states based on the Google Search Volume for racial slurs, adopting the approach of \cite{stephens2014cost}. We also use Census ZIP Code Business Patterns (ZCBP) data to access the number of banks and payday lenders in each zip code. Following \cite{Bhutta2014}, we use the following two North American Industrial Classification System (NAICS) codes to capture payday lending establishments:  non-depository consumer lending (establishments primarily engaged in making unsecured cash loans to consumers) and other activities related to credit intermediation (establishments primarily engaged in facilitating credit intermediation, including check cashing services and money order issuance services).\footnote{\cite{Barthetal2016} discuss how this proxy could likely overstate the number of payday lenders. We adjust these measures to correct for states that prohibit payday lending to help reduce this bias.}  For each zip code, we use ArcGIS to create a weighted average (based on land area) of the number of banks and payday lenders within a five-mile radius of each zip code's centroid. Lastly, we add data from the 2009-2013 American Community Survey to control for population, education, and income at the zip code level.

\subsection{Missouri Neighborhood-Level Panel}

Our second dataset is a panel dataset containing zip codes in Missouri.\footnote{The Missouri court data was generously provided by Kiel and Waldman (2015). They acquired individual court case data from the state court administration. Their white paper focuses on three jurisdictions: Cook County, Illinois (composed of Chicago and surrounding suburbs), St. Louis City and St. Louis County, Missouri, and Essex County, New Jersey (composed of Newark and suburbs). The court data included basic case information such as the plaintiff, the defendant, and the defendant’s address. The defendant’s race is not reported. See Appendix section \ref{appendixa1} for additional data details.}  Aside from the fact that Missouri has a centralized database of cases tried in different circuit courts, we focus on Missouri due to it's representative nature in terms of collection (\cite{Ratcliffeetal2014}; \cite{Chengetal2019}). More specifically, Missouri is representative regarding the percentage of delinquent consumers and the average amount of debt in collections (\cite{Ratcliffeetal2014}). Missouri is also not particularly exceptional regarding its law surrounding collections, its share of black residents, or its level of inequality (\cite{Chengetal2019}).\footnote{We have additional debt collection judgment data from New Jersey and Cook County, Illinois (composed of Chicago and surrounding suburbs); however, it is less detailed than the Missouri data. While this data includes the number of cases filed in a five-year window from 2008-2012, it is not broken down by type of judgment (default, consent, contested), defendants' names, or representing attorney. As such, all of our main specifications use data from Missouri due to its representative nature, high level of detail, and to keep our sample consistent across specifications. However, analogous analysis is provided in the appendix when comparable information is available.} 

This dataset includes debt collection court cases filed in Missouri between 2004 and 2013, along with other neighborhood characteristics.  For each zip code in our sample, we know the number of debt collection lawsuits filed and the number of judgments arising from these lawsuits. We also see the number of cases that resulted in a default judgment (meaning the debtor did not show up to court), a consent judgment (meaning the debtor showed up to court and admitted to owing the debt), and the number of cases that were contested (meaning that some aspect of the debt was disputed). We know if the defendant was represented by an attorney and the plaintiff type (categorized into the following groups: auto, debt buyer, high-cost lender, major bank, medical, utility, and miscellaneous).

The Missouri court data is merged with Experian credit report data aggregated to the zip code-level to control median credit score, the average number of delinquent accounts, and other neighborhood-level credit measures for each zip code in our sample. Zip code tabulation data from the IRS from 2004 - 2018 is used to control for the average income and the fraction of all filers with income under \$25,000, \$25,000-50,000, \$50,000-75,000, \$75,000-100,000 and over \$100,000.  Also included is zip code tabulation data from the 2009-2013 American Community Survey to control for population, racial composition, the unemployment rate, and other socioeconomic variables of interest at the zip code-level. 

For our neighborhood-level analysis, our outcome variable of interest is the number of judgments per 100 people. Neighborhood racial composition is our primary independent variable of interest. More specifically, we classify a zip code as a majority-black if more than 50\% of its residents are black.\footnote{Section A.2.6 in the appendix shows that our results are robust to other measures of neighborhood racial composition, including using the share of the population that is black.} Throughout our analysis, we control for other neighborhood-level characteristics that may be driving the racial gap in debt collection judgments. For example, we document the share of cases in which an attorney was present as well as the share of cases in which the debt was contested.  

We limit our sample to only observations with common support over observables (\cite{crump2009dealing}).\footnote{Details regarding the creation of this sample are discussed in the section \ref{appendixa1} of the appendix. See Table \ref{tab:sample_restrictions} in the appendix for sample size restrictions based on data availablity and restricting the sample to the common support.} Table \ref{tab:summary_statistics} summarizes neighborhood-level data from over 800 Missouri zip codes from 2004-2013. This data shows that majority-black neighborhoods have higher judgment rates (2.7 per 100 people) than majority non-black neighborhoods (1.3 per 100 people). The data also suggests that majority-black neighborhoods have lower incomes and credit scores, higher past-due debt balances, more default judgments, fewer attorney-represented defendants, more payday lenders, lower house values, lower homeownership rates, higher unemployment rates, and higher divorce rates. Most differences are significant at the 1\% level. 


==> New_Parts/Racial_Disparities_-_Submission/Sections/figures.tex <==
\newpage

\section*{Figures}

\begin{figure}[!h]    
\footnotesize
\begin{center}
	\includegraphics[scale=0.6]{Figures/judgment_black.pdf}
	\caption{Judgments and Demographic Composition}\label{fig:demographics}
\end{center}
\begin{flushleft}
	\scriptsize{Notes: This figure plots a linear regression that examines the correlation between black population and the judgment rate. The sample includes Missouri zip codes in the common support sample.  Zip codes were sorted into 100 groups based on their black population share. The graph displays each group's average black population share against their average judgment rate. The bubble size corresponds to the data quantity in each group, and the regression line shows the weighted relationship between the judgment rate and the black population share.}
\end{flushleft}
\end{figure}


\begin{figure}[!h]
\footnotesize
\begin{center}
	\begin{subfigure}{0.45\textwidth}  % Adjusted width to make two figures fit side by side
		\centering
		\includegraphics[width=\textwidth]{Figures/regplot_income.pdf}
		\caption{Median Income and Judgment Rate}
	\end{subfigure}
    \hfill  % Added horizontal fill to ensure some space between the figures
	\begin{subfigure}{0.45\textwidth}  % Adjusted width to make two figures fit side by side
		\centering
		\includegraphics[width=\textwidth]{Figures/regplot_credit.pdf}
		\caption{Median Credit Score and Judgment Rate}
	\end{subfigure} \\
\end{center}
	\caption{Income, Credit Scores, and Judgment Rate}\label{fig:cs_vs_income}   
\begin{flushleft}
\scriptsize{Notes: Panel (a) of this figure plots the relationship between median income and the judgment rate and Panel (b) plots the relationship between median credit score and the judgment rate. The sample includes Missouri zip codes in the common support sample. The green line represents the non-parametric locally weighted regression line (LOESS) showing the smoothed fit curve of the data. Income is top coded at \$200K USD to mitigate the impact of outliers.}
\end{flushleft} 
\end{figure}


\begin{figure}[!h]
\footnotesize
	\centering
		\includegraphics[width=.5\textwidth]{Figures/judgmentsdisparity_overtime.pdf}
		\caption{Disparity over Time}\label{fig:time_series}
		\begin{flushleft}
		 \scriptsize{Notes: This figure plots in gray is the estimated coefficient and 95\% confidence interval from a regression which estimates the racial disparity in judgments by year. The sample includes Missouri zip codes in the common support sample. The red dashed lined shows the average number of judgments per 100 individuals for majority black neighborhoods while the blue solid line shows the average number of judgments per 100 individuals for neighborhoods with less than 50\% of black residents.}
		\end{flushleft}
\end{figure}

\newpage

==> New_Parts/Racial_Disparities_-_Submission/Sections/introduction.tex <==
\section{Introduction} \label{sec:introduction}

Debt collection court cases have significant financial implications for debtors. For instance, a guilty verdict, referred to as a judgment, can result in wage garnishments and seizures of bank accounts. These consequences, particularly when compounded with interest and legal fees, hinder debtors' ability to achieve financial stability and limit their ability to accumulate wealth. Moreover, judgments disproportionately occur in predominantly Black neighborhoods, even after controlling for income differences across neighborhoods (Keil and Waldman, 2019).\footnote{More specifically, the risk of judgment is twice as high in majority-Black neighborhoods than in non-majority Black neighborhoods with similar income levels (Keil and Waldman, 2019).} 

In this paper, we document a racial disparity in the likelihood of receiving a debt collection judgment after accounting for potential confounding factors including credit scores, debt levels, and other debt characteristics.  To do so, we create a nationally representative individual-level panel dataset spanning from 2013Q1 to 2017Q2 containing both individuals demographic information as well as a comprehensive set of their credit report characteristics.  Credit information comes from Experian credit reports and includes indicators for if an individual has any outstanding judgments. While credit reports do not contain information about an individual's race, following the methodology in \cite{butler2022racial}, we merge credit report data with information from the Home Mortgage Disclosure Act (HMDA) database to uncover borrowers' race and ethnicity. We find that the judgment rate is 39\% higher for black and Hispanic borrowers, controlling for credit scores, debt levels, and other debt characteristics.  This disparity is not correlated with measures of racial bias, but is instead driven by locations with a high number of payday lenders, a high share of income-less households, and low levels of tertiary education. Conditional on a judgment being issued, we find no statistical difference in the likelihood a judgment is petitioned or satisfied across minority and non-minority borrowers, suggesting limited evidence that collectors are focusing their collection efforts based on the probability a debt will be petitioned or that the account will be brought to current.    

We further examine potential mechanisms through which this disparity could permeate the debt collection system. One potential explanation for the gap in judgments is differences in neighborhood-level characteristics that impact the probability of success and profitability of collecting on a debt. When dealing with unpaid balances on unsecured debt, creditors have two main options if negotiating with the borrower has proved unsuccessful: they can write off the debt or take the debt to collections. Several factors drive this decision, including the likelihood the debtor will ultimately repay the debt and the cost of collecting on the debt. While creditors are legally prohibited from using race as a factor when making decisions related to credit, they may use neighborhood characteristics to gather information about a debtor’s ability to repay debt or to estimate the potential cost of collecting the debt. For example, it could be the case that defendants from black neighborhoods are less likely to hire an attorney or to contest the debt in court, making it less costly for debt collectors to obtain judgments in black neighborhoods. While creditors do not know this information a priori for any given individual, they could estimate the likelihood of such situations based on historical outcomes in a given zip code. 

To analyze the extent to which such mechanisms are driving the racial disparity, we create a zip code-level panel dataset spanning from 2004 to 2013 that links the number of debt collection judgments in each zip code in Missouri with data from Experian credit reports and the American Community Survey. Controlling for a comprehensive set of financial variables derived from the credit report data to account for all aspects of neighborhoods' financial liabilities, we find that debt collection court cases are 56\% more common in black neighborhoods compared to non-black neighborhoods. Using this data, we find no statistical difference in the share of contested judgments across black and non-black communities, and controlling for attorney representation has a limited effect on the judgment gap. 

Another potential mechanism that could explained the racial gap in debt collection judgments results from the broader disadvantages experienced by black communities. According to estimates provided by the United States Census Bureau in 2016, the typical black household has a net worth of \$12,920, while that of a typical white household is \$114,700 - this is a \$101,780 difference in wealth that could have important implications for a household’s ability to mitigate negative financial shocks. About \$35,000 of this wealth gap is not driven by home equity and would not be captured in our current analysis. By translating this wealth gap into differences in annual income and using our estimates of the relationship between income and judgments from our matched credit bureau data, we calculate that a wealth gap of this size would explain the judgment gap.\footnote{Our estimated racial judgment gap suggests black and Hispanic individuals are 0.0496 percentage points more likely to have a new judgment on their credit report, holding credit score, income, and other credit characteristics constant. We computed the difference in annual savings needed over a 40-year horizon to generate a wealth gap of \$35,000. We found that an annual difference of \$2,910 is sufficient to generate the wealth gap in net present value. For the interest rate, we applied the stock market’s historical return, which between 1957 through 2018 is roughly 8\%. Consistent with estimates from the U.S. Bureau of Economic Analysis, we assume an 8\% personal savings rate. Under these assumptions, this wealth gap translates into an annual income difference of \$36,375. Using our estimated regression equation, we conclude that increasing the imputed income of minority individuals by this amount would eliminate the judgment gap, while increasing the HMDA income by this amount would explain 77\% of the judgment gap.}

This paper contributes to an extensive literature that documents the role that race plays in the legal, financial, and criminal justice system. For example, black individuals are more likely to be searched for contraband (\cite{antonovicsknight2009}), to have biased bail hearings (\cite{Arnoldetal2018}), and to be charged with a serious offense (\cite{MaritStarr2014}). Black and Hispanic borrowers are less likely to get approved for an auto loan, even after controlling for creditworthiness (\cite{butler2022racial}), and  African American zip codes are less likely to receive financial restitution from complaints submitted to the Consumer Financial Protection Bureau (\cite{haendler2021financial}).  Discrimination in the labor and housing-related market has also been well documented (e.g., \cite{bartlett2019consumer}, \cite{ritter2011racial}, \cite{bertrand2004emily}, and \cite{turner2002discrimination}). Such disparities have contributed to racial differences in wealth, and a growing literature explores how the racial wealth gap was generated and how it has persisted over time (e.g., \cite{mckernan2014racial}; \cite{akbar2019racial}; \cite{derenoncourt2022wealth}). While much attention has been given to racial disparities in general, this is the first economic analysis to empirically document racial disparities in debt collection judgments.  

Aside from the literature documenting racial disparities and discrimination, this paper also contributes to a growing literature about the debt collection industry.\footnote{See \cite{hunt2007} for an overview of the debt collection industry and details about its institutional structure and regulatory environment.}  We know that consumers whom creditors and debt collectors sue are drawn predominantly from lower-income areas (\cite{hynes2008}).  Other more recent studies have investigated the role of information technology in the collection of consumer debts (\cite{drozd}), documented the link between debt collection regulations and the supply of consumer credit (\cite{Fedasseyeu2015}), and determined if consumers are made better or worse off by settling their debt outside of court (\cite{Chengetal2019}).  Interpreted broadly, the literature has documented the impacts of the debt collection process on consumer outcomes; however, racial disparities in debt collection have not been rigorously explored.    

The rest of our paper is outlined as follows:  Section 2 discusses the typical debt collection litigation process in the United States, as well as the laws regulating access to credit and debt collection procedures; Section 3 describes our data; Section 4 discusses our empirical approach; Section 5 documents the racial gap in debt collection judgments and explores potential mechanisms that may be driving the disparity; Section 6 concludes.  

==> New_Parts/Racial_Disparities_-_Submission/Sections/methods.tex <==
\section{Empirical Methods} \label{sec:methods}

Focusing first on the individual-level matched credit bureau data, we investigate racial disparities in debt collection by regressing judgment outstanding on minority, an indicator for the person being Black or Hispanic. Our empirical specification is given by the following equation:

\begin{equation}
    y_{izt}=\alpha + \beta M_{iz} + \theta X_{izt} + \gamma_z + \lambda_{st} + \epsilon_{izt}
\end{equation}

\noindent
where $y_{izt}$ is a binary variable indicating if individual i in zipcode z has a new judgment on their credit score in quarter t, $M_{iz}$ is an indicator variable equal to one if individual i in zipcode z is Black or Hispanic, and $X_{izt}$ is a vector of other controls for individual i in zipcode z in quarter t. Such controls include credit score, measures of debt balances by type of debt (credit card, mortgage loans, student loans, etc.), debt composition (type of debt as a share of total debt balances), delinquent balances by the length of delinquency (30 days, 60 days, 90 days), and bankruptcy/collection flags and indicators for the timing relative to the borrower's credit bureau/HMDA match, and imputed income/HMDA income wherever applicable. In addition, our main specification includes zipcode fixed effects to control for time-invariant differences across zipcodes and state-by-quarter fixed effects to control for any time-varying changes that impact all individuals within a state. 

We run a similar specification using our neighborhood level dataset from Missouri. Our outcome of interest becomes the number of judgments per every 100 people in zip code i in county c in year t.  Our control variable of interest is an indicator variable for if the neighborhood is a majority black neighborhood (defined as a neighborhood where the black population is greater than 50\%). We control for neighborhood-level income and credit score measures, measures of debt balances by type of debt, debt composition, delinquent balances by the length of delinquency, and bankruptcy/collection flags. We also control for other neighborhood level observable characteristics such as the Gini index, unemployment rate, median housing values, education levels, and divorce rate. All regressions include county and year fixed effects. To better understand the mechanisms driving the racial disparity in debt collection judgments, we include a number of additional control variables at the neighborhood level. Such control variables include the previous share of cases in which an attorney was present as well as the previous share of cases in which the debt was contested. All regressions are weighted by population in our neighborhood-level analysis. Standard errors are clustered at the county-year level and we report the p-values from a wild cluster bootstrap for inference due to the small number of clusters (Cameron and Miller, 2015).



==> New_Parts/Racial_Disparities_-_Submission/Sections/results.tex <==

\section{Results} \label{sec:result}

In section \ref{mainresults} we document a racial disparity in debt collection judgments using our Credit Report/HMDA individual-level panel. We conclude that debt collection judgments are 39\% more common among black and Hispanic individuals. We then present our neighborhood-level results to better understand potential mechanisms that could be driving this disparity.

\subsection{Racial Disparity in Judgements}\label{mainresults}

We begin by estimating equation (1) to determine the extent to which there is a racial disparity in debt collection judgments.  Table \ref{table:4a} presents these regression results.  Column (2) of Table \ref{table:4a} shows that minority individuals experience a 0.1156 percentage point increase in the probability of having a new judgment on their credit report after controlling for state-by-quarter fixed effects, zip code fixed effects, and demographic information. After adding credit report controls to the previous specification, we find that minority individuals are 0.0496 percentage points more likely to accumulate judgments (Column (3)); this is a 39\% increase from the judgment rate among white borrowers.  These results highlight both a substantial gap that cannot be solely explained by differences in credit characteristics as well as the importance of including measures of credit quality in our analysis. This unexplained difference in judgments is roughly the same size as we would see from a 21-point (24\% of a standard deviation) reduction in credit score. In column (4) we include imputed income derived from the credit bureau data and income from HMDA.  The coefficient on minority only decreases by 10\%.  

The information presented in columns (5) and (6) of Table \ref{table:4a} indicate that minorities tend to accrue new judgments more frequently as subprime borrowers in absolute terms, but not proportionately. The coefficient pertaining to minorities who are prime borrowers is borderline insignificant, suggesting a potential judgment rate that is twice that of non-minority borrowers. This particular observation carries significant weight. The decision-making process for subprime borrower approval typically involves a higher degree of discretion by loan officers. This can lead to a reduction in the marginal cost associated with decisions that have potential discriminatory implications.

In Panels A and B of Table \ref{table:4bc} we change our dependent variable to whether or not a judgment was reported as being petitioned or satisfied, respectively. We find no statistically significant racial disparities in the number of judgments petitioned or satisfied once conditioning on having an outstanding judgment in the previous quarter. These findings suggest that debt collectors have no incentive to target specific segments of the population based on their likelihoods to petition or satisfy their judgment.

We next explore where racial disparities in debt collection judgments are most pronounced. Initially, we investigate if these discrepancies are more significant in states with high racial bias, similar studies by \cite{charles2008prejudice} and \cite{butler2022racial}. We measure racial biases by adopting the methodology of \cite{stephens2014cost}, which uses the volume of Google Search for racial slurs. A crucial advantage of leveraging Google searches is that they reveal attitudes individuals typically hide in survey responses. In column (2) of Table \ref{table:5}, we find that the interaction between minority status and a binary variable for high racial bias is not statistically significant. This implies that the racial disparities observed in debt collection judgments cannot be attributed to state-level taste-based discrimination. 

Our next cross-sectional test is based on the prevalence of non-bank lending in the ZIP code where the applicant lives. In column (3) of Table \ref{table:5}, we find that the effect of race on judgment rates is significantly different for applicants in zip codes in the top quartile of bank lending share (i.e., areas with less reliance on non-bank lending, like payday lenders) compared to the remaining ZIP codes. This finding suggests that racial disparities in judgment rates are more prevalent in areas with a higher fraction of payday lenders. It is important to note that payday lenders are often located in areas with high financial hardship, serving communities where traditional banking services may be less accessible, and people may have limited financial options. This tends to disproportionately affect minority communities, potentially contributing to the disparities observed in judgment rates. High judgment rates and the prevalence of payday lenders are likely symptoms of underlying socioeconomic disparities, rather than the presence of payday lenders causing higher judgment rates among minorities. 

Viewing the issue from a different perspective, Column (4) looks at ZIP codes that fall within the top quartile of households without income and discovers that the disparity originates from individuals residing in these areas. Conversely, Column (5) examines individuals living in ZIP codes in the top quartile of tertiary education rates and finds no observable disparities within these regions. 

\subsection{Neighborhood Level Mechanisms}\label{mechanisms}

Why are minorities more likely to experience a debt collection judgment than white individuals, despite having similar credit characteristics? It could be that creditors are using neighborhood-level information to help determine the profitability of their debt collection efforts\footnote{Creditors can legally factor proxy variables into their decision-making if there is a legitimate business necessity, such as scoring credit risk, even if these tactics cause disparate outcomes across space (\cite{bartlett2021consumer}).} For example, they may focus their collection efforts in neighborhoods where defendants are less likely to hire an attorney or to contest the debt in court. This section uses neighborhood-level data from Missouri to explore if and to what extent neighborhood-level characteristics can explain the racial disparity in debt collection judgments. We begin by replicating the findings from the individual analysis, which used nationally representative judgment data from Experian, with judgment data from Missouri aggregated to the zip code level. We then explore neighborhood-level characteristics that could drive the relationship between neighborhood racial composition and debt collection judgments. 

We start by documenting the racial disparity in judgments across black and non-black neighborhoods.  Figure \ref{fig:demographics} uses Missouri neighborhood data, grouping zip codes into 100 bins by the share of black residents. The figure plots the average black population share against the average judgment rate per bin, with bubble size denoting the number of zip codes per bin. The regression line, weighted by observation count, shows a positive correlation between judgment rate and black population share.

Figure \ref{fig:cs_vs_income} explores the correlation between racial composition, median income, credit scores, and debt judgments in neighborhoods. Panel (a) indicates a negative correlation between judgment rate and median income, even when comparing neighborhoods of similar income levels, with higher judgment rates seen in majority-black neighborhoods. Panel (b) shows a negative correlation between judgment rate and median credit scores, with higher judgment rates in majority-black neighborhoods despite similar credit scores. This suggests differences in income and credit scores may not be the primary mechanism driving the racial disparity in debt collection cases.  

We next regress the number of judgments per 100 people on an indicator for if a neighborhood is majority black, as well as average ZIP code level income and the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles and median credit score to the baseline specification, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density. Results are presented in Table \ref{tab:debt_composition}. Our preferred specification is given in column (5) and includes all our controls for individuals debt portfolios, although the coefficient is positive and statistically significant across each specification. Column (5) suggests there are approximately 0.70 more judgments per 100 people in majority black zip codes compared to majority non-black neighborhoods; this translates in a 56\% higher judgment rate.

One potential difference in the cost of collecting debt across black and non-black neighborhoods is the likelihood that an attorney represents a given debtor. While this is not known a priori, creditors could theoretically estimate these likelihoods when deciding which delinquent accounts to bring to court. To explore how differences in attorney representation drive our results, we explore the disparity in attorney representation and investigate whether this impacts our main findings. These results are presented in Columns (1) and (2) of Table \ref{tab:judgment_type}.  Each specification in this table includes the income, credit score, and baseline controls discussed above, as well as county and year fixed effects. The outcome variable in Column (1) is the share of debt collection court cases where an attorney represented the defendant; this result shows that defendants in majority-black neighborhoods are less likely to have an attorney represent them in a debt collection court case. However, as seen in Column (2), where our dependent variable is once again judgments per 100 people, controlling for the share of cases in which an attorney represents defendants cannot explain the racial disparity in debt collection cases.\footnote{This does not imply that attorney representation is not meaningful or important in debt collection court cases. Debt collection laws often place the burden on asserting various legal protections, including the share of the debtor's wages that can be garnished as the result of a judgment on the debtor. Thus, attorney representation is important in protecting debtors' rights throughout the debt collection process, even if such cases ultimately end in judgments.} 

It could be the case that debt collectors target their collection efforts in areas where defendants are less likely to show up to court, resulting in a default judgment, or in areas where defendants do not tend to contest the debt in court. In other words, debt collectors might avoid collecting in areas where defendants tend to argue some aspect of the debt owed, which could result in the plaintiff exerting more effort or spending more money to collect the debt.  

To explore how differences in the share of contested versus uncontested cases could drive our result, we document the impact of neighborhood racial composition on the share of different types of judgments. Our outcome variable in Column (3) Table \ref{tab:judgment_type} is the share of cases in which the defendant admitted to owing the debt, and our outcome variable in Column (4) is the share of cases that were contested. We see no racial differences along these dimensions. Columns (6), (7), and (8) explore the share of cases that resulted in default judgments, were dismissed, or were settled, respectively. We see that a larger share of cases in black neighborhoods resulted in default judgments or was dismissed, while a smaller share was settled before court.

Given that the rank order preference of case outcomes is not apparent, we explore how these differences could impact the judgment gap by including the lagged share of case outcomes into our main specification, where our outcome variable is judgments per 100 people.  Including lagged case outcomes does not mitigate the judgment gap across black and non-black neighborhoods. These results suggest that previous differences in case outcomes across neighborhoods and plaintiffs' potential strategic decisions to exploit this information for cost savings measures do not explain why judgments are more common in black neighborhoods.\footnote{Section \ref{appendixa2} in the appendix contains a multitude of additional analysis and robustness checks. For example, we show the racial gap in debt collection judgments exists for every plaintiff type (albeit at different magnitudes) except medical lenders in Appendix section \ref{appendixa22} and use various different measures of neighborhood racial composition in Appendix section \ref{appendixa26}.  Results are consistent with the conclusions presented above.}  

Figure \ref{fig:time_series} plots the evolution of the racial disparity from 2004-2013 and shows that while the racial disparity is present over our whole sample period, it increases dramatically during the Great Recession. This pattern could be taken as evidence that majority-black neighborhoods were less able to mitigate the negative shocks associated with the recession or that the recession disproportionately impacted these neighborhoods.  According to estimates provided by the United States Census Bureau in 2016, the typical black household has a net worth of \$12,920, while that of a typical white household is \$114,700 - this is a \$101,780 difference in wealth that could have important implications for a household's ability to mitigate adverse income shocks. About \$35,000 of this wealth gap is not driven by home equity. By translating this wealth gap into a difference in annual income and using our estimates of the relationship between income and the likelihood of receiving a judgment on your credit score, we calculate that a wealth gap of this size would explain the racial judgment gap.  



==> New_Parts/Racial_Disparities_-_Submission/Sections/tables.tex <==
\newpage

\input{Tables/tab_1}

\input{Tables/tab_2}

\input{Tables/tab_3}

\input{Tables/Tables_neighborhood/summary_tab1}

\input{Tables/table4_a}

\input{Tables/table_4_bc}

\input{Tables/tab_5}

\input{Tables/Tables_neighborhood/results_debt_portfolio_neighborhood}

\input{Tables/Tables_neighborhood/results_judgment_type_neighborhood}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/dml.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\footnotesize
\caption{Judgments and Double Machine Learning\label{tab:dml}}
\begin{tabular}{l*{5}{c}} \hline \hline
 & R2: Y Model & R2: T Model & Estimates & T-values \\ \hline 
 & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
T: Majority Black & 0.5121 & 0.9877 & 1.020 & 1.824 \\
 & [0.0069] & [0.0022] & [0.2682] & [0.4028] \\ \hline \hline
% & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
%T: Continuous & 0.5121 &  0.9904 & 3.909 & 6.8267 \\
% & [0.0069] & [0.0015] & [0.4592] & [1.3375] \\ \hline \hline 
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes: We use five-fold cross-validation in the first stage. Features used correspond to Column (5) of Table \ref{tab:creditworthiness}. For the classification tasks, we use Gradient Boosted Trees, while for the regression tasks, we use Random Forest.  We repeat the estimation with different seeds 1,000 times with distinct train-test splits and the statistics reported are the averages obtained from this exercise. Standard deviations are in brackets.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_alternative_credit_risk_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Credit Score\label{tab:pp}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.6061\sym{***}&      1.2321\sym{***}&      0.9537\sym{***}&      0.8287\sym{***}&      1.0213\sym{***}\\
                    &    (0.1885)         &    (0.1717)         &    (0.1961)         &    (0.1764)         &    (0.0360)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &           X         &                     \\
Income              &                     &                     &           X         &           X         &                     \\
Default Probability &                     &           X         &           X         &           X         &           X         \\
Lagged Baseline Controls&                     &                     &                     &                     &           X         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &       .0007         &           0         \\
Observations        &   5909      &   5909      &   5909      &   5625      &   4738      \\
$R^2$               &      0.5977         &      0.6319         &      0.6813         &      0.7001         &      0.7291         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications. Default probabilities are used as control variables in place of credit scores. Column (5) controls for lagged default probability instead of default probability. Default probability data is available starting in 2006. All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_alternative_dependent_neighborhood.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Alternative Dependent Variables\label{tab:judgment_alternative}}
\begin{tabular}{l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
&\multicolumn{1}{c}{Judgments/Cases}&\multicolumn{2}{c}{Judgment: Low Income}&\multicolumn{2}{c}{Judgment: Low Credit }&\multicolumn{2}{c}{Judgment: Winsorized} \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &    0.028\sym{***} &       2.843\sym{***}&       2.649\sym{***}&       0.503\sym{***}&       0.492\sym{***} &      0.708\sym{***}&       0.666\sym{***}\\
              &     (0.010)                   &     (0.704)         &     (0.570)         &     (0.122)         &     (0.115)     &     (0.165)         &     (0.138)         \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Population Weighted &                   &             X       &                  &                X     &                 &          X           &                     \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Boostrap p-value   &       .0111        &       .0011         &           0         &        .003         &       .0005          &       .0008         &       .0002       \\
Observations        &    7019         &    7019         &    7019              &    6999         &    6999      &    7019       &    7019         \\
$R^2$         &       0.173                &       0.660         &       0.548         &       0.744         &       0.576         &       0.686         &       0.512        \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item  Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics, where the judgment rate is normalized in various ways.  The sample includes Missouri zip codes in the common support sample.  For Column (1) our dependent variable is the fraction of cases that result in a judgment, for Columns (2-3), our outcome variable is judgments per 100 individuals with tax filings under \$25,000 USD, for Columns (4-5) our outcome variable is judgments per 100 individuals with subprime credit, and for Columns (6-7) we winsorize our main outcome variable, judgments per 100 individuals, at the 99th percentile. Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, year fixed effects, and attorney representation are included in all specifications.  Only columns (2), (4), and (6) are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_credit_markets_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Access to Credit Markets\label{tab:access_to_credit}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.0910\sym{***}&      1.0897\sym{***}&      1.0914\sym{***}&      0.9375\sym{***}&      0.9417\sym{***}\\
                    &    (0.1398)         &    (0.1394)         &    (0.1399)         &    (0.1099)         &    (0.1135)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Broadband           &                     &      0.0565\sym{**} &                     &                     &                     \\
                    &                     &    (0.0222)         &                     &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Unscored            &                     &                     &      0.1838         &                     &                     \\
                    &                     &                     &    (0.2691)         &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (5 miles)     &                     &                     &                     &     -0.0056\sym{***}&                     \\
                    &                     &                     &                     &    (0.0011)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (5 miles)&                     &                     &                     &      0.0177\sym{***}&                     \\
                    &                     &                     &                     &    (0.0028)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (10 miles)    &                     &                     &                     &                     &     -0.0025\sym{***}\\
                    &                     &                     &                     &                     &    (0.0003)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (10 miles)&                     &                     &                     &                     &      0.0098\sym{***}\\
                    &                     &                     &                     &                     &    (0.0013)         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &           0         \\
\hline 
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &   4183      &   4183      &   4183      &   4183      &   4183      \\
$R^2$               &      0.8181         &      0.8186         &      0.8181         &      0.8279         &      0.8295         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications. All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_debt_portfolio_individual.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios (Individual Data)\label{tab:individual_portfolio_prob}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Probability of Being Black      &      0.0072\sym{***}&      0.0073\sym{***}&      0.0082\sym{***}&      0.0047\sym{***}&      0.0040\sym{***}\\
                    &    (0.0006)         &    (0.0006)         &    (0.0006)         &    (0.0006)         &    (0.0006)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\ \hline 
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &12939752      &12939752      &12939752      &12939752      &12939752      \\
$R^2$               &      0.0638         &      0.0631         &      0.0614         &      0.0711         &      0.0727         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment. County and quarter fixed effects are included in all specifications. Observations from the Experian sample, data available from 2013 until 2018Q2. We use the individuals age and ZIP code to infer their probability of being black.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_debt_portfolio_individual_zip.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios (Individual Data): ZIP\label{tab:individual_portfolio_zip}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP     &      0.0065\sym{***}&      0.0066\sym{***}&      0.0072\sym{***}&      0.0054\sym{***}&      0.0048\sym{***}\\
                    &    (0.0005)         &    (0.0005)         &    (0.0005)         &    (0.0005)         &    (0.0005)         \\
\hline
Observations        &12935791       &12935791       &12935791       &12935791       &12935791       \\
$R^2$               &      0.0638         &      0.0632         &      0.0615         &      0.0711         &      0.0728         \\ \hline \hline
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\ \hline 
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]

\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment. County and quarter fixed effects are included in all specifications. Observations from the Experian common support sample, data available from 2013 until 2018Q2. 
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_debt_portfolio_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios\label{tab:debt_composition}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      0.6910\sym{***}&      0.7134\sym{***}&      0.7070\sym{***}&      0.7095\sym{***}&      0.6962\sym{***}\\
                    &    (0.1616)         &    (0.1657)         &    (0.1650)         &    (0.1579)         &    (0.1511)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0012         &       .0009         &       .0009         &       .0005         &       .0004         \\
Observations        &   7019      &   7019      &   7019      &   7019      &   7019      \\
$R^2$               &      0.6877         &      0.6860         &      0.6854         &      0.6876         &      0.6926         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_debt_portfolio_neighborhood_bisg.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Debt Portfolios\label{tab:debt_composition_bisg}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
\hline
Black Majority: BISG&      0.6222\sym{***}&      0.6329\sym{***}&      0.6264\sym{***}&      0.6302\sym{***}&      0.6266\sym{***}\\
                    &    (0.1308)         &    (0.1349)         &    (0.1343)         &    (0.1274)         &    (0.1229)         \\
\hline
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
Wild Cluster Bootstrap p-value&       .0004         &       .0004         &       .0005         &       .0002         &       .0002         \\
Observations        &   7015       &   7015        &   7015      &   7015        &   7015        \\
$R^2$               &      0.6893         &      0.6869         &      0.6861         &      0.6884         &      0.6940         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item  This table presents results of a regression of the judgment rate on neighborhood racial composition (as defined using the BISG algorithm) and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_debt_portfolio_neighborhood_other_areas.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Debt Portfolios (NJ and IL Data)\label{tab:debt_composition_nj_il}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
  
\hline
Black Majority:  ZIP     &      0.2748\sym{***}&      0.2753\sym{***}&      0.2876\sym{***}&      0.2840\sym{***}&      0.2592\sym{***}\\
                    &    (0.0858)         &    (0.0850)         &    (0.0871)         &    (0.0924)         &    (0.0870)         \\
\hline
Wild Cluster Bootstrap p-value&       .0012         &       .0011         &       .0012         &       .0018         &       .0033         \\
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
Observations        &   3103        &   3103        &   3103        &   3103        &   3103        \\
$R^2$               &      0.9105         &      0.9113         &      0.9101         &      0.9110         &      0.9145         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes New Jersey and Illinois zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_housing_market_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Local Housing Markets\label{tab:access_to_housing}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                       &\multicolumn{4}{c}{Judgment Rate}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      0.9451\sym{***}&      0.8416\sym{***}&      0.7136\sym{***}&      0.6891\sym{***}\\
                    &    (0.1581)         &    (0.1453)         &    (0.1610)         &    (0.1584)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA: Share Rejected&                     &      1.0981\sym{***}&                     &                     \\
                    &                     &    (0.3638)         &                     &                     \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Zillow: Single Family House&                     &                     &                     &     -0.0060\sym{***}\\
                    &                     &                     &                     &    (0.0013)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA Available      &           X         &           X         &                     &                     \\
Zillow Available    &                     &                     &           X         &           X         \\ \hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &       .0006         &       .0005         \\
Observations        &   3846         &   3846         &   5231         &   5231         \\
$R^2$               &      0.7593         &      0.7628         &      0.6767         &      0.6861         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics, including information on local housing markets.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications.  All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_judgment_type_neighborhood.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Attorney Representation and Judgment Type\label{tab:judgment_type}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Attorney}&\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Consent}&\multicolumn{1}{c}{Contested}&\multicolumn{1}{c}{Default}&\multicolumn{1}{c}{Dismissed}&\multicolumn{1}{c}{Settle}&\multicolumn{1}{c}{Judgments}\\
\hline
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
\hline
Black Majority: ZIP &      -0.015\sym{***}&       0.707\sym{***}&       0.003         &       0.001         &       0.013\sym{**} &       0.014\sym{*}  &      -0.022\sym{***} & 0.768\sym{***} \\
                    &     (0.004)             &     (0.165)         &     (0.005)         &     (0.004)         &     (0.006)         &     (0.007)         &     (0.006)     & (0.165)   \\
\hline
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Attorney Representation & & X & X&X&X&X&X&X \\
Lagged Case Outcomes & & & & & & & & X \\ \hline 
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0001         &       .0007         &       .0008         &        .601         &        .709         &       .0558         &       .0702         &       .0036         \\
Observations        &    7019       &    7019       &    7019       &    7019       &    7019       &    7019       &    7019       &    7019       \\
$R^2$               &       0.448         &       0.700         &       0.685         &       0.470         &       0.438         &       0.395         &       0.651         &       0.615         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item This table explores the extent to which attorney representation or previous case outcomes can explain the racial gap in judgments.  The sample includes Missouri zip codes in the common support sample. The outcome variable in Column (1) is the share of debt collection court cases where an attorney represented the defendant.  The outcome variable in columns (2) and (8) are judgments per 100 people.  The outcome variables in Columns (3)-(7) are the share of cases resulting in a consent judgment, a contested judgment, a default judgment, the case being dismissed, and the case being settled, respectively.  All regressions are weighted by population. Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications. Aside from Column (1), all specifications control for the share of cases with attorney representation.  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_judgments_individual.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (Individual Judgment Data) \label{tab:individual}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Probability of Being Black    &      0.0479\sym{***}&      0.0469\sym{***}&      0.0088\sym{***}&      0.0084\sym{***}\\
                    &    (0.0018)         &    (0.0018)         &    (0.0018)         &    (0.0018)         \\
\hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Income &                            &     X &                     &    X\\
Credit Score                     &                     &                     &     X&     X\\
\hline & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &12939752        &12939752        &12939752        &12939752        \\
$R^2$               &      0.0303         &      0.0307         &      0.0611         &      0.0612         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment.  County and quarter fixed effects are included in all specifications. Observations from the Experian common support sample, data available from 2013 until 2018Q2. We use the individuals age and ZIP code to infer their probability of being black.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_judgments_individual_zip.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (Individual Data): ZIP \label{tab:individual_zip}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP    &      0.0262\sym{***}&      0.0258\sym{***}&      0.0075\sym{***}&      0.0073\sym{***}\\
                    &    (0.0014)         &    (0.0014)         &    (0.0014)         &    (0.0014)         \\ \hline
& & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Income &                            &     X &                     &    X\\
Credit Score                     &                     &                     &     X&     X\\
\hline & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &12935791    &12935791    &12935791    &12935791    \\
$R^2$               &      0.0294         &      0.0298         &      0.0611         &      0.0612         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-quarter level are in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Indicator variable of having a judgment.  County and quarter fixed effects are included in all specifications. Observations from the Experian common support sample, data available from 2013 until 2018Q2. 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_judgments_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores \label{tab:creditworthiness}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                       &\multicolumn{6}{c}{Judgment Rate}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.4356\sym{***}&      0.8629\sym{***}&      1.0786\sym{***}&      0.7939\sym{***}&      0.7084\sym{***}&      0.8384\sym{***}\\
                    &    (0.1873)         &    (0.1917)         &    (0.1658)         &    (0.1807)         &    (0.1662)         &    (0.0356)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income      &                     &           X         &                     &           X         &           X         &                     \\
Credit Score    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0005         &       .0009         &           0         \\
Observations        &   7365      &   7365      &   7019      &   7019      &   7019      &   6105      \\
$R^2$               &      0.5961         &      0.6617         &      0.6279         &      0.6684         &      0.6851         &      0.6770         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Income controls include average zip code-level income and the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000; credit controls include credit score quintiles and median credit score; baseline controls include total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density. All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_judgments_neighborhood_bisg.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Creditworthiness\label{tab:creditworthiness_bisg}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: BISG&      1.2637\sym{***}&      0.7413\sym{***}&      0.9180\sym{***}&      0.6791\sym{***}&      0.6283\sym{***}&      0.6899\sym{***}\\
                    &    (0.1571)         &    (0.1505)         &    (0.1290)         &    (0.1401)         &    (0.1347)         &    (0.0310)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income Details      &                     &           X         &                     &           X         &           X         &                     \\
Credit Quintiles    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\ 
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0001         &       .0005         &           0         \\
Observations        &   7361        &   7361        &   7015       &   7015        &   7015        &   6103       \\
$R^2$               &      0.5799         &      0.6585         &      0.6207         &      0.6661         &      0.6860         &      0.6739         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_judgments_neighborhood_other_areas.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (NJ and IL Data) \label{tab:creditworthiness_nj_il}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                       &\multicolumn{6}{c}{Judgment Rate}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP  &      0.9667\sym{***}&      0.8630\sym{***}&      0.3650\sym{***}&      0.5833\sym{***}&      0.2981\sym{***}&      0.3978\sym{***}\\
                    &    (0.1297)         &    (0.1058)         &    (0.0940)         &    (0.0876)         &    (0.0885)         &    (0.0844)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income      &                     &           X         &                     &           X         &           X         &                     \\
Credit Score   &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &           0         &       .0008         &           0         \\
Observations        &   3397        &   3397        &   3103        &   3103        &   3103        &   2118        \\
$R^2$               &      0.8733         &      0.8994         &      0.8909         &      0.9034         &      0.9089         &      0.9119         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 30.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_other_races_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Other Demographic Groups\label{tab:race_other}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                       &\multicolumn{6}{c}{Judgment Rate}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      2.2881\sym{***}&      1.5574\sym{***}&      1.9195\sym{***}&      1.4544\sym{***}&      1.4865\sym{***}&      1.6260\sym{***}\\
                    &    (0.2748)         &    (0.3184)         &    (0.2505)         &    (0.2955)         &    (0.2777)         &    (0.0610)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Asian: ZIP    &     -5.6745\sym{***}&     -3.3050\sym{***}&     -4.8311\sym{***}&     -3.1980\sym{***}&     -1.6851\sym{**} &     -3.6100\sym{***}\\
                    &    (0.9938)         &    (0.9074)         &    (0.9953)         &    (0.8989)         &    (0.7889)         &    (0.4954)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Hispanic: ZIP &      1.0901\sym{***}&     -0.3160\sym{***}&      0.7415\sym{***}&     -0.3814\sym{***}&      0.5452\sym{***}&     -0.3274\sym{*}  \\
                    &    (0.1345)         &    (0.1217)         &    (0.1357)         &    (0.1297)         &    (0.1421)         &    (0.1820)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income     &                     &           X         &                     &           X         &           X         &                     \\
Credit Score  &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\ \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p$_{\text{Black}}$&           0         &           0         &           0         &           0         &           0         &           0         \\
Wild Cluster Bootstrap p$_{\text{Hispanic}}$&           0         &       .0137         &       .0001         &        .008         &       .0003         &       .1084         \\
Wild Cluster Bootstrap p$_{\text{Asian}}$&           0         &       .0031         &       .0002         &       .0026         &       .0552         &           0         \\
Observations        &   7365        &   7365        &   7019        &   7019        &   7019        &   6105        \\
$R^2$               &      0.6496         &      0.6796         &      0.6618         &      0.6841         &      0.6973         &      0.6952         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_plaintiff_type_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Plaintiff Type\label{tab:plaintiff_type}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Debt Buyer}&\multicolumn{1}{c}{Major Bank}&\multicolumn{1}{c}{Medical}&\multicolumn{1}{c}{High-Cost }&\multicolumn{1}{c}{Misc.}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &       0.708\sym{***}&       0.217\sym{***}&       0.058\sym{**} &       0.045         &       0.119\sym{***}&       0.321\sym{***}\\
                    &     (0.166)         &     (0.051)         &     (0.029)         &     (0.055)         &     (0.024)         &     (0.082)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Mean                &       1.253         & .568       &        .453         &        .297         &        .076         &        .139         \\
Effect Size         &56.5         &        38.2         &        12.8         &        15.1         &       156.3         &         231         \\ \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0009         &       .0006         &       .0652         &       .5694         &           0         &       .0001         \\
Observations        &    7019        &    7019        &    7019        &    7019        &    7019        &    7019        \\
$R^2$               &       0.685         &       0.699         &       0.725         &       0.613         &       0.602         &       0.533         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate for specific types of debt collectors on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable in Column (1) is judgments per 100 individuals.  The dependent variables in Columns (2)-(6) are judgements by debt buyers per 100 individuals, judgments by major banks per 100 individuals, judgments by medical lenders per 100 individuals, judgments by high-cost lenders per 100 individuals, and judgments by other miscellaneous lenders per 100 individuals. Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications. All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/results_race_proxies_neighborhood.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Proxy for Race\label{tab:race_proxies}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                       &\multicolumn{4}{c}{Judgment Rate}\\
\hline
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      1.4731\sym{***}&                     &                     &                     \\
                    &    (0.2865)         &                     &                     &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &                     &      0.7084\sym{***}&                     &                     \\
                    &                     &    (0.1662)         &                     &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: BISG   &                     &                     &      1.3776\sym{***}&                     \\
                    &                     &                     &    (0.2563)         &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: BISG&                     &                     &                     &      0.6283\sym{***}\\
                    &                     &                     &                     &    (0.1347)         \\
\hline
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0001         &       .0009         &           0         &       .0005         \\
Observations        &   7019         &   7019         &   7015         &   7015         \\
$R^2$               &      0.6965         &      0.6851         &      0.6981         &      0.6860         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition (where racial composition is measured in various ways) and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications.  All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/summary_tab1.tex <==
\begin{table}[!h]\centering
  \begin{threeparttable}
 \footnotesize 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics for Neighborhood Level Judgment Data\label{tab:summary_statistics}}
\begin{tabular}{l*{3}{cc}}
\hline\hline
                    &\multicolumn{1}{c}{Black}&\multicolumn{1}{c}{Non-Black}&\multicolumn{1}{c}{Difference}\\
\hline
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textbf{Panel A: Judgments and Financial Characteristics } & & & \\
 \textcolor{white}{...}Judgments per 100 People       &        2.71&        1.26&       -1.46\sym{***}\\
                    &      (1.29)&      (0.75)&                     \\
 \textcolor{white}{...}Share of Default Judgments            &        0.45&        0.37&       -0.08\sym{***}\\
                    &      (0.07)&      (0.13)&                     \\
 \textcolor{white}{...}Share of Consent Judgments            &        0.16&        0.17&       0.01\sym{*}\\
                    &      (0.07)&      (0.11)&                     \\
 \textcolor{white}{...}Share of Dismissed Judgments           &        0.11&        0.15&        0.04\sym{***}\\
                    &      (0.11)&      (0.13)&                     \\
 \textcolor{white}{...}Share of  Contested Judgments       &        0.05&        0.05&       -0.01\sym{*}  \\
                    &      (0.04)&      (0.07)&                     \\
 \textcolor{white}{...}Share of  Settled Cases              &        0.19&        0.2&        0.01\sym{*}\\
                    &      (0.09)&      (0.13)&                     \\
 \textcolor{white}{...}Share w/ Attorney            &        0.04&        0.10&        0.06\sym{***}\\
                    &      (0.02)&      (0.08)&                     \\
 \textcolor{white}{...}Mean Household Income from IRS (in 000s) &       29.21&       38.68&        9.47\sym{***}\\
                    &      (9.75)&      (9.88)&                     \\
 \textcolor{white}{...}Median Credit Score &    587.59&      686.36&       98.77\sym{***}\\
                  &     (49.83)&     (72.68)&                     \\
 \textcolor{white}{...}90+ DPD Debt Balances             &     3237.66&     1405.79&    -1831.87\sym{***}\\
 &   (2629.86)&   (3768.89)&                     \\
\textbf{Panel B: Neighborhood Characteristics} & & & \\ 
 \textcolor{white}{...}GINI Index &        0.46&        0.41&       -0.05\sym{***}\\
                    &      (0.05)&      (0.05)&                     \\

 \textcolor{white}{...}Unemployment Rate   &        0.12&        0.05&       -0.06\sym{***}\\
                    &      (0.03)&      (0.03)&                     \\
 \textcolor{white}{...}Divorce Rate&        0.13&        0.12&       -0.01\sym{***}\\
                    &      (0.02)&      (0.04)&                     \\
 \textcolor{white}{...}Fraction with Bachelors Degree&        0.16&        0.16&       -0.00         \\
                    &      (0.10)&      (0.10)&                     \\
\textcolor{white}{...}Median Gross Rent  &        0.76&        0.62&       -0.14\sym{***}\\
                    &      (0.14)&      (0.16)&                     \\
\textcolor{white}{...}Home Ownership Rate &        0.50&        0.74&        0.25\sym{***}\\
                    &      (0.16)&      (0.12)&                     \\
 %\textcolor{white}{...}Banks (5 miles)     &       88.10&       11.91&      -76.19\sym{***}\\
 %                   &     (39.71)&     (30.19)&                     \\
 %\textcolor{white}{...}Payday Lenders (5 miles)&       30.64&        3.58&      -27.07\sym{***}\\
 %                   &      (9.23)&      (8.17)&                     \\
 %\textcolor{white}{...}Zillow: Single Family House (in 000s) &       90.28&      113.32&       23.04\sym{***}\\
 %                   &     (54.39)&     (43.23)&                     \\
 %\textcolor{white}{...}HMDA: Share Rejected, Black - White&        0.19&        0.14&       -0.05\sym{***}\\
 %                   &      (0.11)&      (0.31)&                     \\
\hline
Zip codes       &         247&        6640&            \\
Average Population    &    18451.03&     7036.03&   \\
\hline\hline
\end{tabular}

   \begin{tablenotes}
     \scriptsize
    \item Notes:  This table presents summary statistics for the Missouri neighborhood level data from 2004-2013.  The sample includes only observations on the common support.  Column 1 displays the sample means and standard deviations for neighborhoods in which at least 50\% of the population is black and column 2 displays sample means and standard deviations for neighborhoods in which less than 50\% is black.  The third column reports the difference in means across the two samples. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)
    \end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/summary_tab1_individual.tex <==
\begin{table}[th]\centering
  \begin{threeparttable}
 \small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics for Individual Level Experian Data\label{tab:summary_statistics_individual}}
\begin{tabular}{l*{3}{cc}}
\hline\hline
                    &\multicolumn{1}{c}{Black}&\multicolumn{1}{c}{Non-Black}&\multicolumn{1}{c}{Difference}\\
\hline
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textcolor{white}{...}Share with Judgments           &        0.06&        0.03&       -0.03\sym{***}\\
                    &      (0.23)&      (0.16)&                     \\
 \textcolor{white}{...}Household Income   &       43.82&       51.61&        7.79\sym{***}\\
                    &     (71.09)&     (52.32)&                     \\
 \textcolor{white}{...}Credit Score      &      610.87&      684.70&       73.83\sym{***}\\
                    &    (120.38)&    (113.25)&                     \\
 \textcolor{white}{...}90+ DPD Debt Balances    &     3933.21&     2109.77&    -1823.44\sym{***}\\
                    &  (31475.04)&  (23339.70)&                     \\
 \textcolor{white}{...}Age &       47.92&       49.01&        1.09\sym{***}\\
                    &     (16.34)&     (16.54)&                     \\
    \hline
Observations     &      707919&    12229556&    12937475         \\
\hline\hline
\end{tabular}

   \begin{tablenotes}
     \small
    \item Notes:  Individual level common support sample. Standard deviations are in parenthesis. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)
   \end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_neighborhood/summary_tab1_other_areas.tex <==
\begin{table}[b]
\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics: IL \& NJ\label{tab:summary_statistics_il_nj}}
\begin{tabular}{l*{3}{cc}}
\hline\hline
                    &\multicolumn{1}{c}{Black}&\multicolumn{1}{c}{Non-Black}&\multicolumn{1}{c}{Difference}\\
\hline
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textbf{Panel A: Judgments and Financial Characteristics} & & & \\
 \textcolor{white}{...}Judgments per 100 People &        2.70&        1.72&       -0.98\sym{***}\\
                    &      (2.00)&      (1.79)&                     \\
 \textcolor{white}{...}Median Credit Score  &      588.98&      707.15&      118.17\sym{***}\\
                    &     (36.72)&     (54.62)&                     \\
 \textcolor{white}{...}90+ DPD Debt Balances &     7135.13&     4260.03&    -2875.10\sym{***}\\
                    &   (6609.97)&   (6448.52)&                     \\
\textbf{Panel B: Additional Neighborhood Characteristics } & & & \\ 
 \textcolor{white}{...}GINI Index       &        0.46&        0.41&       -0.06\sym{***}\\
                    &      (0.05)&      (0.05)&                     \\
 \textcolor{white}{...}Unemployment Rate  &        0.12&        0.07&       -0.06\sym{***}\\
                    &      (0.03)&      (0.02)&                     \\
 \textcolor{white}{...}Divorce Rate  &        0.11&        0.10&       -0.02\sym{***}\\
                    &      (0.02)&      (0.03)&                     \\
 \textcolor{white}{...}Fraction with Bachelors Degree&        0.18&        0.30&        0.11\sym{***}\\
                    &      (0.10)&      (0.14)&                     \\
 \textcolor{white}{...}Gross Rent: Median   &        0.97&        1.06&        0.09\sym{***}\\
                    &      (0.25)&      (0.29)&                     \\
 \textcolor{white}{...}Home Ownership Rate      &        0.51&        0.71&        0.20\sym{***}\\
                    &      (0.20)&      (0.17)&                     \\
 \textcolor{white}{...}Banks (5 miles)  &      166.92&      113.30&      -53.63\sym{***}\\
                    &    (138.48)&    (170.14)&                     \\
 \textcolor{white}{...}Payday Lenders (5 miles)&       33.65&       11.84&      -21.81\sym{***}\\
                    &     (39.86)&     (25.73)&                     \\
 \textcolor{white}{...}Zillow: Single Family House&        176.37&      189.89&       13.53         \\
                    &     (92.22)&    (116.21)&                     \\
 \textcolor{white}{...}HMDA: Share Rejected, Black - White  &      175.91&      252.34&       76.43\sym{***}\\
                    &     (90.21)&    (123.72)&                     \\
 \textcolor{white}{...}Mean Household Income (IRS) &        0.16&        0.13&       -0.03\sym{***}\\
                    &      (0.11)&      (0.19)&                     \\
\hline
Observations        &         200&         705&         905         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
        \scriptsize
        \item Notes:  This table presents summary statistics for the Illinois and New Jersey neighborhood level data from 2004-2013.  The sample includes only observations on the common support.  Column 1 displays the sample means and standard deviations for neighborhoods in which at least 50\% of the population is black and column 2 displays sample means and standard deviations for neighborhoods in which less than 50\% is black.  The third column reports the difference in means across the two samples. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)
\end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_alternative_credit_risk_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Credit Score: Entire Sample\label{tab:pp_off_common}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.7143\sym{***}&      1.2269\sym{***}&      0.9769\sym{***}&      0.8158\sym{***}&      1.0181\sym{***}\\
                    &    (0.2216)         &    (0.1776)         &    (0.1921)         &    (0.1734)         &    (0.0332)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &           X         &                     \\
Income              &                     &                     &           X         &           X         &                     \\
Default Probability &                     &           X         &           X         &           X         &           X         \\
Lagged Baseline Controls&                     &                     &                     &                     &           X         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &       .0005         &           0         \\
Observations        &   6666       &   6666       &   6352       &   6017       &   5275       \\
$R^2$               &      0.5779         &      0.6325         &      0.6991         &      0.7230         &      0.7388         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. County and year fixed effects included in all specifications. Column (5) controls for lagged default probability instead of default probability.  Default probability data is available from 2006.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_alternative_dependent_neighborhood_off_common_support.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Alternative Dependent Variables: Entire Sample\label{tab:judgment_alternative_off_common}}
\begin{tabular}{l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
&\multicolumn{1}{c}{Judgments/Cases}&\multicolumn{2}{c}{Judgment: Low Income}&\multicolumn{2}{c}{Judgment: Low Credit }&\multicolumn{2}{c}{Judgment: Winsorized} \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &       0.026\sym{**}&       2.830\sym{***}&       2.607\sym{***}&       0.506\sym{***}&       0.499\sym{***} &       0.707\sym{***}&       0.693\sym{***}\\
                  &     (0.010)           &     (0.680)         &     (0.615)         &     (0.117)         &     (0.121)      &     (0.160)         &     (0.150)            \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Population Weighted &                 &             X        &                    &             X        &                 &    X                 &                     \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Boostrap p-value &       .0146        &       .0004         &       .0002         &       .0016         &        .001             &       .0004         &       .0002     \\
Observations        &    7484        &    7484        &    7484        &    7484        &    7464        &    7464        &    7484        \\
$R^2$               &       0.185           &       0.671         &       0.551         &       0.754         &       0.576      &       0.702         &       0.519          \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects, attorney representation included in all specifications. For Column (1) our dependent variable is the fraction of cases that result in a judgment, for Columns (2-3), our outcome variable is judgments per 100 individuals with tax filings under \$25,000 USD, for Columns (4-5) our outcome variable is judgments per 100 individuals with subprime credit, and for Columns (6-7) we winsorize our main outcome variable, judgments per 100 individuals, at the 99th percentile.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_credit_markets_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Access to Credit Markets: Entire Sample\label{tab:access_to_credit_off_common}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.0704\sym{***}&      1.0699\sym{***}&      1.0706\sym{***}&      0.9528\sym{***}&      0.9185\sym{***}\\
                    &    (0.1436)         &    (0.1434)         &    (0.1437)         &    (0.1256)         &    (0.1279)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Broadband           &                     &      0.0374\sym{*}  &                     &                     &                     \\
                    &                     &    (0.0214)         &                     &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Unscored            &                     &                     &      0.1337         &                     &                     \\
                    &                     &                     &    (0.2643)         &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (5 miles)     &                     &                     &                     &     -0.0047\sym{***}&                     \\
                    &                     &                     &                     &    (0.0008)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (5 miles)&                     &                     &                     &      0.0161\sym{***}&                     \\
                    &                     &                     &                     &    (0.0026)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (10 miles)    &                     &                     &                     &                     &     -0.0021\sym{***}\\
                    &                     &                     &                     &                     &    (0.0003)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (10 miles)&                     &                     &                     &                     &      0.0083\sym{***}\\
                    &                     &                     &                     &                     &    (0.0009)         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &           0         \\
\hline 
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &   4488       &   4488       &   4488       &   4488       &   4488       \\
$R^2$               &      0.8248         &      0.8250         &      0.8248         &      0.8335         &      0.8344         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_debt_portfolio_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios: Entire Sample\label{tab:debt_composition_off_common}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      0.6926\sym{***}&      0.7086\sym{***}&      0.7058\sym{***}&      0.6957\sym{***}&      0.6871\sym{***}\\
                    &    (0.1549)         &    (0.1599)         &    (0.1594)         &    (0.1558)         &    (0.1476)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0004         &       .0005         &       .0005         &       .0004         &       .0003         \\
Observations        &   7484        &   7484        &   7484        &   7484        &   7484        \\
$R^2$               &      0.7037         &      0.7021         &      0.7020         &      0.7038         &      0.7079         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition and other neighborhood-level characteristics.  The sample includes the entire Missouri zip code sample.  The dependent variable is judgments per 100 individuals.  Baseline controls include average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density.  Baseline controls, county fixed effects, and year fixed effects are included in all specifications, and all regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_housing_market_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Local Housing Markets: Entire Sample\label{tab:access_to_housing_off_common}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      0.9253\sym{***}&      0.8022\sym{***}&      0.7012\sym{***}&      0.6903\sym{***}\\
                    &    (0.1591)         &    (0.1401)         &    (0.1590)         &    (0.1563)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA: Share Rejected&                     &      1.2362\sym{***}&                     &                     \\
                    &                     &    (0.3948)         &                     &                     \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Zillow: Single Family House&                     &                     &                     &     -0.0040\sym{***}\\
                    &                     &                     &                     &    (0.0007)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA Available      &           X         &           X         &                     &                     \\
Zillow Available    &                     &                     &           X         &           X         \\ \hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &       .0003         &       .0002         &       .0001         \\
Observations        &   4171      &   4171      &   5679      &   5679      \\
$R^2$               &      0.7764         &      0.7806         &      0.6960         &      0.7018         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_judgment_type_neighborhood_off_common_support.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Attorney Representation and Judgment Type: Entire Sample\label{tab:judgment_type_off_common}}
\begin{tabular}{l*{9}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}\\
                    &\multicolumn{1}{c}{Attorney}&\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Consent}&\multicolumn{1}{c}{Contested}&\multicolumn{1}{c}{Default}&\multicolumn{1}{c}{Dismissed}&\multicolumn{1}{c}{Settle}&\multicolumn{1}{c}{Judgments}\\
\hline
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      -0.016\sym{***}&       0.685\sym{***}&       0.706\sym{***}&       0.004         &       0.001         &       0.014\sym{***}&       0.010         &      -0.022\sym{***} &       0.752\sym{***}\\
                    &     (0.003)         &     (0.155)         &     (0.160)         &     (0.005)         &     (0.004)         &     (0.005)         &     (0.007)         &     (0.006)    & (0.162)     \\
\hline
&&&&& & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Attorney Representation & & X & X&X&X&X&X&X&X \\
Lagged Case Outcomes & & & & & & & & & X \\ \hline 
&&&&& & & & S \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &       .0004         &       .0004         &       .4475         &       .8498         &       .0096         &       .1681         &       .0036    & 0.0008     \\
Observations        &    7484       &    7484       &    7484       &    7484       &    7484       &    7484       &    7484       &    7484    & 6701   \\
$R^2$               &       0.440         &       0.715         &       0.702         &       0.479         &       0.407         &       0.389         &       0.654         &       0.643     & 0.732    \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table explores the extent to which attorney representation or previous case outcomes can explain the racial gap in judgments.  The sample includes the entire Missouri zip code level sample. The outcome variable in Column (1) is the share of debt collection court cases where an attorney represented the defendant.  The outcome variable in columns (2) and (8) are judgments per 100 people.  The outcome variables in Columns (3)-(7) are the share of cases resulting in a consent judgment, a contested judgment, a default judgment, the case being dismissed, and the case being settled, respectively.  All regressions are weighted by population. Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications. Aside from Column (1), all specifications control for the share of cases with attorney representation. Column (8) controls for the share of default judgments. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_judgments_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores: Entire Sample \label{tab:creditworthiness_off_common}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &      1.5127\sym{***}&      0.8940\sym{***}&      1.0934\sym{***}&      0.8200\sym{***}&      0.7071\sym{***}&      0.8402\sym{***}\\
                    &    (0.2148)         &    (0.1912)         &    (0.1741)         &    (0.1816)         &    (0.1612)         &    (0.0325)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income Details      &                     &           X         &                     &           X         &           X         &                     \\
Credit Quintiles    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0006         &       .0005         &           0         \\
Observations        &   9788     &   9020     &   7837     &   7527     &   7484     &   6737     \\
$R^2$               &      0.5805         &      0.6694         &      0.6304         &      0.6814         &      0.7016         &      0.6903         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_other_races_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Other Demographic Groups: Entire Sample\label{tab:race_other_off_common}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      2.3723\sym{***}&      1.5447\sym{***}&      1.9561\sym{***}&      1.4328\sym{***}&      1.4930\sym{***}&      1.5590\sym{***}\\
                    &    (0.3076)         &    (0.3300)         &    (0.2724)         &    (0.3088)         &    (0.2859)         &    (0.0557)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Asian: ZIP    &     -5.1481\sym{***}&     -2.9361\sym{***}&     -4.4323\sym{***}&     -2.8328\sym{***}&     -0.9491\sym{*}  &     -3.0248\sym{***}\\
                    &    (0.9695)         &    (0.6906)         &    (1.0057)         &    (0.7438)         &    (0.5175)         &    (0.3856)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Hispanic: ZIP &      1.3980\sym{***}&     -0.3906\sym{***}&      0.8922\sym{***}&     -0.4970\sym{***}&      0.4932\sym{***}&     -0.4124\sym{**} \\
                    &    (0.1707)         &    (0.1407)         &    (0.1666)         &    (0.1541)         &    (0.1589)         &    (0.1670)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income    &                     &           X         &                     &           X         &           X         &                     \\
Credit Score    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\ \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p$_{\text{Black}}$&           0         &           0         &           0         &       .0006         &           0         &           0         \\
Wild Cluster Bootstrap p$_{\text{Hispanic}}$&           0         &       .0098         &       .0002         &       .0038         &       .0036         &       .0298         \\
Wild Cluster Bootstrap p$_{\text{Asian}}$&           0         &       .0001         &       .0013         &       .0018         &        .092         &           0         \\
Observations        &   9788       &   9020       &   7837       &   7527       &   7484       &   6737       \\
$R^2$               &      0.6472         &      0.6868         &      0.6692         &      0.6968         &      0.7138         &      0.7068         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_plaintiff_type_neighborhood_off_common_support.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Plaintiff Type: Entire Sample\label{tab:plaintiff_type_off_common}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Debt Buyer}&\multicolumn{1}{c}{Major Bank}&\multicolumn{1}{c}{Medical}&\multicolumn{1}{c}{High-Cost }&\multicolumn{1}{c}{Misc.}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &       0.707\sym{***}&       0.220\sym{***}&       0.052\sym{*}  &       0.045         &       0.116\sym{***}&       0.322\sym{***}\\
                    &     (0.161)         &     (0.050)         &     (0.029)         &     (0.052)         &     (0.022)         &     (0.077)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Mean                &       1.325         &        .584         & 0.489         &        .304         &        .079         &        .152         \\
Effect Size         &53.4        &        37.6         &        10.7         &          15         &         146         &       211.3         \\ \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0005         &       .0003         &       .1048         &.5348         &           0         &       .0001         \\
Observations        &    7484        &    7484        &    7484        &    7484        &    7484        &    7484        \\
$R^2$               &       0.702         &       0.710         &       0.734         &       0.623         &       0.607         &       0.534         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/results_race_proxies_neighborhood_off_common_support.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Proxy for Race: Entire Sample\label{tab:race_proxies_off_common}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      1.4731\sym{***}&                     &                     &                     \\
                    &    (0.2890)         &                     &                     &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: ZIP &                     &      0.7071\sym{***}&                     &                     \\
                    &                     &    (0.1612)         &                     &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: BISG   &                     &                     &      1.3774\sym{***}&                     \\
                    &                     &                     &    (0.2604)         &                     \\
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Black Majority: BISG&                     &                     &                     &      0.6305\sym{***}\\
                    &                     &                     &                     &    (0.1284)         \\
\hline
& & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0001         &       .0005         &       .0001         &       .0002         \\
Observations        &   7484        &   7484        &   7479        &   7479        \\
$R^2$               &      0.7133         &      0.7016         &      0.7147         &      0.7027         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.8. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the entire Missouri sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_noncommon/summary_tab1_off_common_support.tex <==
\begin{table}[b]\centering
  \begin{threeparttable}
 \footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics: Entire Sample\label{tab:summary_statistics_off_common}}
\begin{tabular}{l*{3}{cc}}
\hline\hline
                    &\multicolumn{1}{c}{Black}&\multicolumn{1}{c}{Non-Black}&\multicolumn{1}{c}{Difference}\\
\hline
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textbf{Panel A: Judgments and Finacial Characteristics} & & & \\
 \textcolor{white}{...}Judgments per 100 People      &        2.65&        1.32&       -1.32\sym{***}\\
                    &      (1.35)&      (1.53)&                     \\
 \textcolor{white}{...}Share of Default Judgments     &        0.45&        0.37&       -0.08\sym{***}\\
                    &      (0.07)&      (0.17)&                     \\
 \textcolor{white}{...}Share of Consent Judgments          &        0.16&        0.17&        0.02\sym{***}\\
                    &      (0.07)&      (0.14)&                     \\
 \textcolor{white}{...}Share of Dismissed Judgments    &        0.12&        0.15&        0.03\sym{***}\\
                    &      (0.11)&      (0.15)&                     \\
 \textcolor{white}{...}Share of  Constested Judgments        &        0.05&        0.05&       -0.01\sym{*}  \\
                    &      (0.05)&      (0.09)&                     \\
 \textcolor{white}{...}Share of  Settled Cases        &        0.19&        0.21&        0.02\sym{***}\\
                    &      (0.09)&      (0.17)&                     \\
 \textcolor{white}{...}Share w/ Attorney   &        0.04&        0.10&        0.06\sym{***}\\
                    &      (0.02)&      (0.11)&                     \\
 \textcolor{white}{...}Median Credit Score &      586.65&      688.71&      102.06\sym{***}\\
                    &     (50.98)&     (76.50)&                     \\
 \textcolor{white}{...}90+ DPD Debt Balances       &     3193.18&     1416.45&    -1776.73\sym{***}\\
                    &   (2676.72)&   (4253.49)&                     \\
\textbf{Panel B: Additional Neighborhood Characteristics} & & & \\ 
 \textcolor{white}{...}GINI Index &        0.46&        0.40&       -0.06\sym{***}\\
                    &      (0.05)&      (0.07)&                     \\

 \textcolor{white}{...}Unemployment Rate  &        0.12&        0.05&       -0.07\sym{***}\\
                    &      (0.05)&      (0.04)&                     \\
 \textcolor{white}{...}Divorce Rate&        0.13&        0.12&       -0.01\sym{***}\\
                    &      (0.03)&      (0.06)&                     \\
 \textcolor{white}{...}Fraction with Bachelors Degree&              0.16&        0.17&        0.00         \\
                    &      (0.10)&      (0.13)&                     \\
\textcolor{white}{...}Home Ownership Rate &        0.47&        0.76&        0.29\sym{***}\\
                    &      (0.19)&      (0.14)&                     \\
\textcolor{white}{...}Banks (5 miles)     &       85.44&       11.88&      -73.56\sym{***}\\
                    &     (40.79)&     (30.95)&                     \\
 \textcolor{white}{...}Payday Lenders (5 miles)&       29.98&        3.23&      -26.75\sym{***}\\
                    &      (9.86)&      (7.76)&                     \\
 \textcolor{white}{...}Zillow: Single Family House (in 000s) &       90.15&      122.26&       32.11\sym{***}\\
                    &     (54.29)&     (68.87)&                     \\
 \textcolor{white}{...}HMDA: Share Rejected, Black - White&        0.19&        0.15&       -0.04\sym{***}\\
                    &      (0.11)&      (0.31)&                     \\
 \textcolor{white}{...}Mean Household Income from IRS (in 000s) &       28.67&       41.01&       12.34\sym{***}\\
                    &     (10.00)&     (24.25)&                     \\

\hline
Zip Codes       &         258&        9530&           \\
Population &    17697 &     5808 &   \\
\hline\hline
\end{tabular}
   \begin{tablenotes}
     \scriptsize
    \item Notes:  This table presents summary statistics for the entire Missouri neighborhood level data from 2004-2013. Column 1 displays the sample means and standard deviations for neighborhoods in which at least 50\% of the population is black and column 2 displays sample means and standard deviations for neighborhoods in which less than 50\% is black.  The third column reports the difference in means across the two samples. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)
   \end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_alternative_credit_risk_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and an Alternative Credit Score: Share Black\label{tab:pp_share_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP &      1.6996\sym{***}&      0.8755\sym{***}&      0.9238\sym{***}&      0.7283\sym{***}&      0.8163\sym{***}\\
                    &    (0.2524)         &    (0.1223)         &    (0.1388)         &    (0.1754)         &    (0.0525)         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &           X         &                     \\
Income              &                     &                     &           X         &           X         &                     \\
Default Probability &                     &           X         &           X         &           X         &           X         \\
Lagged Baseline Controls&                     &                     &                     &                     &           X         \\
\hline
& & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0095         &       .0015         &       .0159         &           0         &           0         \\
Observations        &   2088        &   2088        &   2088        &   2088        &   1611        \\
$R^2$               &      0.6071         &      0.7032         &      0.7434         &      0.7623         &      0.8124         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. County and year fixed effects included in all specifications. Column (5) controls for lagged default probability instead of default probability.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_alternative_dependent_neighborhood_share_black.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Alternative Dependent Variables: Share Black\label{tab:judgment_alternative_share_black}}
\begin{tabular}{l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
&\multicolumn{1}{c}{Judgments/Cases}&\multicolumn{2}{c}{Judgment: Low Income}&\multicolumn{2}{c}{Judgment: Low Credit }&\multicolumn{2}{c}{Judgment: Winsorized} \\
\hline
& & & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP &       0.072\sym{***}   &       6.160\sym{***}&       4.467\sym{***}&       1.002\sym{***}&       0.747\sym{***} &       1.476\sym{***}&       1.096\sym{***}\\
                 &     (0.015)               &     (1.226)         &     (0.815)         &     (0.210)         &     (0.175)  &     (0.283)         &     (0.204)             \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Population Weighted &                  &                  X         &                     &         X           &                    &     X  &                  \\
\hline
& & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Boostrap p-value&           0                 &           0         &       .0004         &       .0003         &           0     &           0         &           0     \\

Observations        &    7019      &    7019      &    7019         &    6999      &    6999      &    7019     &    7019    \\
$R^2$           &       0.174               &       0.671         &       0.551         &       0.752         &       0.576     &       0.697         &       0.514           \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Regressions are weighted by population only in Columns (2), (4), and (6). Observations on the entire Missouri sample. Baseline controls, county, year fixed effects, and attorney representation included in all specifications. For Column (1) our dependent variable is the fraction of cases that result in a judgment, for Columns (2-3), our outcome variable is judgments per 100 individuals with tax filings under \$25,000 USD, for Columns (4-5) our outcome variable is judgments per 100 individuals with subprime credit, and for Columns (6-7) we winsorize our main outcome variable, judgments per 100 individuals, at the 99th percentile.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_credit_markets_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Access to Credit Markets: Share Black \label{tab:access_to_credit_share_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      2.1184\sym{***}&      2.1157\sym{***}&      2.1185\sym{***}&      1.9213\sym{***}&      2.0197\sym{***}\\
                    &    (0.2550)         &    (0.2546)         &    (0.2551)         &    (0.2065)         &    (0.2115)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Broadband           &                     &      0.0531\sym{**} &                     &                     &                     \\
                    &                     &    (0.0223)         &                     &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Unscored            &                     &                     &      0.0927         &                     &                     \\
                    &                     &                     &    (0.2716)         &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (5 miles)     &                     &                     &                     &     -0.0053\sym{***}&                     \\
                    &                     &                     &                     &    (0.0010)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (5 miles)&                     &                     &                     &      0.0116\sym{***}&                     \\
                    &                     &                     &                     &    (0.0028)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Banks (10 miles)    &                     &                     &                     &                     &     -0.0019\sym{***}\\
                    &                     &                     &                     &                     &    (0.0003)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Payday Lenders (10 miles)&                     &                     &                     &                     &      0.0028\sym{**} \\
                    &                     &                     &                     &                     &    (0.0014)         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &           0         \\
\hline 
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &   4183       &   4183       &   4183       &   4183       &   4183       \\
$R^2$               &      0.8371         &      0.8375         &      0.8371         &      0.8447         &      0.8460         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_debt_portfolio_neighborhood_other_areas_share_black.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Debt Portfolios: Share Black (NJ and IL Data)\label{tab:debt\_composition\_share\_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                    &\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}&\multicolumn{1}{c}{judgments}\\
\hline
fraction\_black      &      0.6786\sym{***}&      0.6632\sym{***}&      0.7179\sym{***}&      0.6930\sym{***}&      0.6875\sym{***}\\
                    &    (0.1541)         &    (0.1522)         &    (0.1568)         &    (0.1596)         &    (0.1565)         \\
\hline
Wild Cluster Bootstrap p-value&           0         &       .0001         &       .0001         &           0         &       .0001         \\
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
Observations        &   3103         &   3103         &   3103         &   3103         &   3103         \\
$R^2$               &      0.9113         &      0.9121         &      0.9111         &      0.9118         &      0.9153         \\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{6}{l}{\footnotesize Observations on the common support sample; estimated by Gradient Boosted Treed with five-fold cross-validation. Since the effective number of clusters is small, Wild Cluster Bootstrap p-values are reported for our main parameter of interest. Baseline controls, county, and year fixed effects included in all specifications.}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_debt_portfolio_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Debt Portfolios: Share Black\label{tab:debt_composition_share_black}}
\begin{tabular}{l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                       &\multicolumn{5}{c}{Judgment Rate}\\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      1.4651\sym{***}&      1.4758\sym{***}&      1.4727\sym{***}&      1.5054\sym{***}&      1.4915\sym{***}\\
                    &    (0.2789)         &    (0.2851)         &    (0.2850)         &    (0.2750)         &    (0.2655)         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Debt Levels         &           X         &                     &                     &                     &           X         \\
Monthly Payment and Utilization&                     &           X         &                     &                     &           X         \\
Debt Composition    &                     &                     &           X         &                     &           X         \\
Delinquency/Bankruptcy/Collections&                     &                     &                     &           X         &           X         \\
\hline
& & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &       .0001         &           0         &           0         &           0         \\
Observations        &   7019        &   7019        &   7019        &   7019        &   7019        \\
$R^2$               &      0.6995         &      0.6973         &      0.6968         &      0.6995         &      0.7045         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results of a regression of the judgment rate on neighborhood racial composition (as measured by the share of black residents) and other neighborhood-level characteristics.  The sample includes Missouri zip codes in the common support sample.  The dependent variable is judgments per 100 individuals.  Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications.  All regressions are weighted by population. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 36.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_housing_market_neighborhood_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Local Housing Markets: Share Black\label{tab:access_to_housing_share_black}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      1.8918\sym{***}&      1.8166\sym{***}&      1.5111\sym{***}&      1.4096\sym{***}\\
                    &    (0.2836)         &    (0.2818)         &    (0.2957)         &    (0.3001)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA: Share Rejected&                     &      0.3642         &                     &                     \\
                    &                     &    (0.3448)         &                     &                     \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Zillow: Single Family House&                     &                     &                     &     -0.0046\sym{***}\\
                    &                     &                     &                     &    (0.0013)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
HMDA Available      &           X         &           X         &                     &                     \\
Zillow Available    &                     &                     &           X         &           X         \\ \hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &           0         &       .0001         &       .0001         \\
Observations        &   3846        &   3846        &   5231        &   5231        \\
$R^2$               &      0.7765         &      0.7768         &      0.6898         &      0.6953         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. Baseline controls, county, and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}



==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_judgment_type_neighborhood_share_black.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Attorney Representation and Judgment Type: Share Black\label{tab:judgment_type_share_black}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Attorney}&\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Consent}&\multicolumn{1}{c}{Constested}&\multicolumn{1}{c}{Default}&\multicolumn{1}{c}{Dismissed}&\multicolumn{1}{c}{Settle}&\multicolumn{1}{c}{Judgments}\\
\hline
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &      -0.036\sym{***}&       1.409\sym{***}&       1.474\sym{***}&       0.014         &       0.011\sym{*}  &       0.045\sym{***}&       0.010         &      1.575\sym{***}\\
                    &     (0.006)         &     (0.282)         &     (0.283)         &     (0.011)         &     (0.006)         &     (0.009)         &     (0.011)         &     (0.289)         \\
\hline
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Attorney Representation & & X & X&X&X&X&X&X \\
Lagged Case Outcomes & & & & & & & & X \\ \hline 
&&&&& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&           0         &       .0002         &           0         &       .2137         &       .0987         &           0         &       .3535         &           0.0001         \\
Observations        &    7019      &    7019      &    7019      &    7019      &    7019      &    7019      &    7019      &    6093     \\
$R^2$               &       0.450         &       0.710         &       0.697         &       0.470         &       0.438         &       0.397         &       0.650         &       0.730         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  This table explores the extent to which attorney representation or previous case outcomes can explain the racial gap in judgments, using the share of black residents in a zip code as our measure for racial composition.  The sample includes Missouri zip codes in the common support sample. The outcome variable in Column (1) is the share of debt collection court cases where an attorney represented the defendant.  The outcome variable in columns (2) and (8) are judgments per 100 people.  The outcome variables in Columns (3)-(7) are the share of cases resulting in a consent judgment, a contested judgment, a default judgment, the case being dismissed, and the case being settled, respectively.  All regressions are weighted by population. Baseline controls (average zip code-level income, the fraction of IRS filings under \$25,000, between \$25,000-50,000, \$50,000-75,000, \$75,000-100,000, and over \$100,000, credit score quintiles, median credit score, total delinquent debt balances, unemployment rate, median house value, the fraction of the population with a college education, the divorce rate, and population density), county fixed effects, and year fixed effects are included in all specifications. Aside from Column (1), all specifications control for the share of cases with attorney representation. Column (8) controls for the share of default judgments. Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_judgments_neighborhood_fraction_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores: Share Black \label{tab:creditworthiness_share_black}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\
Share Black: ZIP    &      2.4081\sym{***}&      1.6669\sym{***}&      1.9877\sym{***}&      1.5634\sym{***}&      1.4731\sym{***}&      1.7233\sym{***}\\
                    &    (0.2939)         &    (0.3308)         &    (0.2640)         &    (0.3064)         &    (0.2865)         &    (0.0583)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income      &                     &           X         &                     &           X         &           X         &                     \\
Credit Score   &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &       .0001         &       .0001         &           0         \\
Observations        &   7365        &   7365        &   7019        &   7019        &   7019        &   6105        \\
$R^2$               &      0.6403         &      0.6769         &      0.6559         &      0.6816         &      0.6965         &      0.6921         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_judgments_neighborhood_other_areas_share_black.tex <==
\begin{table}[htbp] \centering
\begin{threeparttable}
\small 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments, Income, and Credit Scores (NJ and IL Data): Share Black \label{tab:creditworthiness_nj_il_share_black}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP      &      1.4889\sym{***}&      1.3818\sym{***}&      0.6564\sym{***}&      1.0221\sym{***}&      0.6958\sym{***}&      0.7178\sym{***}\\
                    &    (0.2252)         &    (0.1722)         &    (0.1593)         &    (0.1408)         &    (0.1581)         &    (0.1508)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]

Baseline Controls   &                     &                     &                     &                     &           X         &                     \\
Income    &                     &           X         &                     &           X         &           X         &                     \\
Credit Score    &                     &                     &           X         &           X         &           X         &                     \\
Lagged Baseline Controls&                     &                     &                     &                     &                     &           X         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt] \hline 
Wild Cluster Bootstrap p-value&           0         &           0         &           0         &           0         &       .0001         &           0         \\
Observations        &   3397         &   3397         &   3103         &   3103         &   3103         &   2118         \\
$R^2$               &      0.8815         &      0.9031         &      0.8919         &      0.9051         &      0.9097         &      0.9125         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\small
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.6. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample; estimated by Gradient Boosted Treed with five-fold cross-validation. County and year fixed effects included in all specifications.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/Tables_share/results_plaintiff_type_neighborhood_share_black.tex <==
\begin{sidewaystable}[htbp] \centering
\begin{threeparttable}
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Judgments and Plaintiff Type: Share Black\label{tab:plaintiff_type_share_black}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Judgments}&\multicolumn{1}{c}{Debt Buyer}&\multicolumn{1}{c}{Major Bank}&\multicolumn{1}{c}{Medical}&\multicolumn{1}{c}{High-Cost }&\multicolumn{1}{c}{Misc.}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Share Black: ZIP    &       1.473\sym{***}&       0.483\sym{***}&       0.104\sym{**} &       0.024         &       0.277\sym{***}&       0.645\sym{***}\\
                    &     (0.286)         &     (0.096)         &     (0.051)         &     (0.079)         &     (0.044)         &     (0.144)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Wild Cluster Bootstrap p-value&       .0001         &           0         &       .0604         &       .8287         &           0         &           0         \\
Observations        &    7019        &    7019        &    7019        &    7019        &    7019        &    7019        \\
$R^2$               &       0.697         &       0.706         &       0.726         &       0.612         &       0.625         &       0.547         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes:  Robust standard errors clustered at the county-year level are in parentheses. Effective number of clusters: 28.0. Wild Cluster Bootstrap p-values are reported for our main parameter of interest. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Dependent variable: Judgments per 100 individuals.  All regressions are weighted by population. Observations on the common support sample. Baseline controls, county, and year fixed effects included in all specifications. Effect size computed for going from 0\% share black to 100\%.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/tab_1.tex <==
\begin{table}[!ht]
\footnotesize
    \centering
    \begin{threeparttable}
        \caption{Descriptive Statistics of Matching Data from Credit Bureau with HMDA}  
        \label{table:1}
        \begin{tabular}{l c c c c c}  \hline \hline
            \multicolumn{6}{l}{\textbf{Panel A: Match rate}} \\ \hline
            & Credit bureau   & Matched to  & Match rate (\%) & & \\
            &  sample &  HMDA &  & & \\
            Home purchase mortgages & 42,296 & 18,611 & 44.00 & &  \\
            Refinance loans & 30,483 & 14,551 & 47.73 & & \\
            All loans & 72,779 & 33,162 & 45.57 & & \\ \hline
            & & & & &  \\[\dimexpr-\normalbaselineskip+2pt]
            \multicolumn{6}{l}{\textbf{Panel B: Home purchase mortgages}} \\ \hline
             & Credit bureau  & Matched to  & Unmatched & \multicolumn{2}{c}{\underline{Matched vs. Unmatched}} \\
             &  sample &  HMDA &  & Norm. diff. & t-stat  \\
            \underline{Match criteria} & & & & & \\
            & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            Conventional & 0.658 & 0.612 & 0.694 & -0.17 & -17.70 \\
            FHA-insured & 0.278 & 0.320 & 0.244 & 0.17 & 17.54 \\
            VA-guaranteed & 0.065 & 0.068 & 0.063 & 0.02 & 2.20 \\
            Fannie Mae & 0.145 & 0.121 & 0.164 & -0.12 & -12.44 \\
            Freddie Mac & 0.090 & 0.065 & 0.110 & -0.16 & -15.91 \\
            Loan amount & 196,397 & 185,076 & 205,293 & -0.12 & -11.83 \\
            & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            \underline{Non-match characteristics} & & & & & \\
            & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            Credit score t-1 & 714 & 709 & 718 & -0.13 & -13.09 \\
            Age & 41 & 39 & 42 & -0.18 & -17.77 \\
            Have mortgage t-1 & 0.120 & 0.084 & 0.148 & -0.20 & -20.31 \\
            Total debt t-1 & 30,034 & 25,899 & 33,283 & -0.11 & -10.87 \\
            Past due debt t-1 & 107 & 103 & 110 & -0.00 & -0.29 \\ \hline
            Observations &  42,313 &  18,618 & 23,695 &  &  \\ \hline \hline
            & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            \multicolumn{6}{l}{\textbf{Panel C: Refinance loans}} \\  \hline
             & Credit bureau  & Matched to & Unmatched & \multicolumn{2}{c}{\underline{Matched vs. Unmatched}} \\
              &  sample & HMDA &  &  Norm. diff & t-stat   \\
             \underline{Match criteria} & & & & & \\
             & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            Conventional & 0.864 & 0.850 & 0.877 & -0.08 & -6.91 \\
            FHA-insured & 0.095 & 0.106 & 0.085 & 0.07 & 6.03 \\
            VA-guaranteed & 0.041 & 0.044 & 0.037 & 0.03 & 3.02 \\
            Fannie Mae & 0.132 & 0.135 & 0.129 & 0.02 & 1.61 \\
            Freddie Mac & 0.087 & 0.081 & 0.092 & -0.04 & -3.37 \\
            Loan amount & 219,642 & 204,014 & 233,916 & -0.17 & -14.99 \\
            & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            \underline{Non-match characteristics} & & & & & \\
            & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
            Credit score t-1 & 732 & 731 & 733 & -0.03 & -2.61 \\
            Age & 48 & 49 & 48 & 0.05 & 3.99 \\
            Have mortgage t-1 & 1.000 & 1.000 & 1.000 & & \\
            Total debt t-1 & 236,565 & 221,709 & 250,134 & -0.15 & -13.41 \\
            Past due debt t-1 & 992 & 557 & 1,389 & -0.05 & -4.24 \\ \hline 
            Observations    & 30,495 & 14,554 & 15,941 &  & \\
                \hline \hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes: This table provides an overview of the credit bureau and the Home Mortgage Disclosure Act (HMDA) data matching. The initial sample of credit bureau mortgages comprises both home purchase mortgages and refinance loans issued between 2007 and 2017. Loan applicants must apply individually (excluding joint applications), reside within a metropolitan statistical area after loan origination, and have the mortgage as their sole first-lien mortgage. The matching process is described in Section 3.1. Panel A illustrates the success rate of the matching methodology. Panel B summarizes loan and borrower features for home purchase mortgages in the credit bureau data, the subset successfully matched to HMDA, and the unmatched loans. The final two columns display the normalized difference and the outcome of a t-test comparing the mean of the matched sample to the mean of the unmatched sample. Panel C offers comparable summary statistics for refinance loans. 
\end{tablenotes}
\end{threeparttable}
\end{table}
  

==> New_Parts/Racial_Disparities_-_Submission/Tables/tab_2.tex <==
\begin{table}[!ht]
\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\footnotesize
\begin{threeparttable}
\caption{Does borrower race affect the Credit Bureau/HMDA match?}
\label{table:2}
\begin{tabular}{lccc}
\hline \hline
& \multicolumn{1}{c}{Full sample} & \multicolumn{1}{c}{Home purchase mortgages} & \multicolumn{1}{c}{Refinance loans} \\
& (1) & (2) & (3) \\
\hline
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textbf{Match criteria} & & & \\
& & & \\[\dimexpr-\normalbaselineskip+2pt]
FHA loan & -0.02*** & -0.0002*** & -0.0009*** \\
& (0.002085) & (0.00002209) & (0.00003341) \\
VA loan & -0.04*** & -0.0004*** & -0.0007*** \\
& (0.002849) & (0.0000323) & (0.00005913) \\
Purchased by Fannie Mae & -0.09*** & -0.0009*** & -0.0011*** \\
& (0.001643) & (0.00001675) & (0.0000215) \\
Purchased by Freddie Mac & -0.10*** & -0.0010*** & -0.0012*** \\
& (0.001827) & (0.0000186) & (0.0000234) \\
log(Loan amount) & -0.02*** & -0.000074*** & 0.000005067 \\
& (0.001294) & (0.00001641) & (0.00002054) \\ 
& & & \\[\dimexpr-\normalbaselineskip+2pt]
\textbf{Non-match characteristics} & & & \\
& & & \\[\dimexpr-\normalbaselineskip+2pt]
Black & -0.0079 & -0.0006 & -0.0006 \\
& (0.006207) & (0.0005) & (0.0006) \\
Hispanic & -0.0049 & -0.0004 & -0.0013* \\
& (0.006786) & (0.0004) & (0.0006) \\
Black X log(Income) & -0.0006 & 0.00004069 & 0.00004955 \\
& (0.000594) & (0.00004432) & (0.00005803) \\
Hispanic X log(Income) & 0.0001 & 0.0000278 & 0.0001* \\
& (0.0006371) & (0.00003903) & (0.00005155) \\
log(Income) & 0.0030*** & -0.0002*** & -0.00009514*** \\
& (0.000243) & (0.00001564) & (0.00001952) \\ \hline 
& & & \\[\dimexpr-\normalbaselineskip+2pt]
Census tract-by-year FE & Yes & Yes & Yes \\ 
& & & \\[\dimexpr-\normalbaselineskip+2pt]
R-squared & 0.01 & 0.0002 & 0.0003 \\
Observations & 25,902,188 & 12,713,700 & 12,596,574 \\ \hline  \hline
\end{tabular}
\begin{tablenotes}
\scriptsize
\item Notes: This table presents regression analyses investigating the factors influencing the matching of a mortgage from the Home Mortgage Disclosure Act (HMDA) data to a credit bureau record. The sample includes all first-lien home purchase mortgages and refinance loans for owner-occupied properties in metropolitan statistical areas between 2007 and 2017 with reported income. Only single-applicant loans are considered, excluding joint applications. The dependent variable is a binary indicator representing a successful HMDA mortgage match to a credit bureau record, while the independent variables are loan and borrower attributes from the HMDA data. Columns 1, 2, and 3 display the results for the entire sample, home purchase mortgages, and refinance loans, respectively. The coefficients are reported in percentage point units. Standard errors are clustered by census tract-year. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{table}

==> New_Parts/Racial_Disparities_-_Submission/Tables/tab_3.tex <==
\begin{table}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Summary Statistics for the Credit Bureau/HMDA Matched Panel}\label{table:3}
\begin{tabular}{lcccccc}
\hline \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
 & \multicolumn{1}{p{1.5cm}}{\centering Full credit sample} & \multicolumn{1}{p{1.5cm}}{\centering Matched sample} & \multicolumn{1}{p{1.5cm}}{\centering White} & \multicolumn{1}{p{1.5cm}}{\centering Black} & \multicolumn{1}{p{1.5cm}}{\centering Hispanic}& \multicolumn{1}{p{1.5cm}}{\centering Asian}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit score (t-1) & 678.52 & 712.03 & 718.29 & 668.04 & 686.65 & 733.54 \\
 & (113.98) & (87.67) & (85.52) & (94.40) & (88.29) & (76.98)\\
 & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Household income & 77.76 & 94.98 & 97.17 & 78.80 & 81.35 & 112.32 \\
 & (50.31) & (52.79) & (53.09) & (42.10) & (46.69) & (61.57)\\
 & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age & 50.29 & 46.04 & 46.19 & 46.99 & 44.55 & 45.19 \\
 & (19.14) & (14.16) & (14.33) & (14.06) & (13.49) & (12.77)\\
 & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Have mortgage (t-1) & 0.27 & 0.70 & 0.72 & 0.65 & 0.63 & 0.66 \\
 & (0.44) & (0.46) & (0.45) & (0.48) & (0.48) & (0.47)\\
 & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total debt (t-1) & 62,464 & 155,939 & 157,842 & 127,641 & 133,802 & 207,858 \\
 & (142,691) & (176,230) & (178,632) & (123,868) & (150,118) & (226,610)\\
 & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past due debt (t-1) & 2,040.78 & 2,606.64 & 2,157.72 & 5,615.54 & 3,731.79 & 2,441.48 \\
 & (23,461.18) & (24,735.67) & (21,408.84) & (32,312.05) & (29,969.48) & (40,222.92)\\
 & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
New judgment outstanding & 0.1698 &  0.1428 &  0.1308 &  0.3189 &  0.1416 &  0.0583  \\
 & (4.1171) & (3.7762) & (3.6143) & (5.6378) & (3.7602) & (2.4136) \\
  & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
New judgment petitioned & 0.0827 & 0.0702 & 0.0648 & 0.1728 & 0.0527 & 0.0276  \\
 &  (2.8745) & (2.6478) & (2.5444) & (4.1535) & (2.2960) & (1.6605) \\
  & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
New judgment satisfied & 0.0283 & 0.0304 & 0.0278 & 0.0741 & 0.0243 & 0.0138  \\
 & (1.6811) & (1.7435) & (1.6682) & (2.7205) & (1.5601) & (1.1742) \\
\hline
Observations  & 769,995  & 28,361  & 21,658  & 2,276  & 2,789 & 1,638 \\ \hline \hline
\end{tabular}
\begin{tablenotes}
\item \scriptsize{This table provides descriptive statistics for the Credit Bureau/HMDA matched panel. Column 1 outlines the sample means and standard deviations for the entire credit bureau dataset; column 2 portrays these statistics for the Credit Bureau/HMDA matched panel; and columns 3–6 display these statistics for the White, Black, Hispanic, Asian borrowers within the matched dataset, respectively. The sample spans 2013Q1 to 2017Q2.  }
\end{tablenotes}
\end{threeparttable}
\end{table}


==> New_Parts/Racial_Disparities_-_Submission/Tables/tab_4.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and Judgments}\label{table:4}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{5}{c}{Judgment Outstanding}&\multicolumn{1}{c}{Judgment Petitioned}&\multicolumn{1}{c}{Judgment Satisfied}\\

\hline
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female           &      0.0080         &      0.0037         &      0.0086         &      0.0397         &     -0.0059         &      0.0036         &      0.0063         \\
                    &    (0.0111)         &    (0.0138)         &    (0.0136)         &    (0.0571)         &    (0.0067)         &    (0.0098)         &    (0.0061)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority         &      0.1237\sym{***}&      0.1156\sym{***}&      0.0496\sym{**} &      0.1373\sym{*}  &      0.0194         &      0.0220         &      0.0120         \\
                    &    (0.0202)         &    (0.0246)         &    (0.0238)         &    (0.0756)         &    (0.0122)         &    (0.0178)         &    (0.0103)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age                 &     -0.0017\sym{***}&     -0.0018\sym{***}&      0.0008\sym{*}  &      0.0025         &      0.0003         &     -0.0002         &     -0.0003         \\
                    &    (0.0003)         &    (0.0004)         &    (0.0004)         &    (0.0020)         &    (0.0002)         &    (0.0003)         &    (0.0002)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$  &                     &                     &     -0.0024\sym{***}&     -0.0044\sym{***}&     -0.0004\sym{***}&     -0.0013\sym{***}&     -0.0002\sym{***}\\
                    &                     &                     &    (0.0002)         &    (0.0005)         &    (0.0001)         &    (0.0001)         &    (0.0000)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$            &                     &                     &      0.0019\sym{***}&      0.0011         &      0.0019         &      0.0011\sym{**} &     -0.0002         \\
                    &                     &                     &    (0.0006)         &    (0.0008)         &    (0.0020)         &    (0.0004)         &    (0.0002)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$           &                     &                     &     -0.0002\sym{***}&     -0.0006\sym{***}&     -0.0000         &     -0.0001\sym{***}&     -0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0002)         &    (0.0000)         &    (0.0000)         &    (0.0000)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Judgment Outstanding$_{t-1}$      &                     &                     &      0.0216         &     -0.8370\sym{***}&     -0.2061         &     -0.0466         &      0.6217\sym{***}\\
                    &                     &                     &    (0.0991)         &    (0.1410)         &    (0.1615)         &    (0.0639)         &    (0.0775)         \\
& & & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.1956\sym{***}&      0.2067\sym{***}&      1.8568\sym{***}&      3.0859\sym{***}&      0.3312\sym{***}&      0.9873\sym{***}&      0.1673\sym{***}\\
                    &    (0.0171)         &    (0.0219)         &    (0.1186)         &    (0.3127)         &    (0.0621)         &    (0.0794)         &    (0.0353)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469015       & 468754       & 468753       & 122640       & 345323       & 468753       & 468753       \\
Mean of DV (Minority=0)           &      0.1258         &      0.1258         &      0.1258         &      0.4817         &      0.0187         &      0.0615         &      0.0249         \\
$R^2$               &      0.0044         &      0.0362         &      0.0385         &      0.0744         &      0.0339         &      0.0356         &      0.0379         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\item This table tests a regression of judgments on race, individual characteristics, and ZIP code fixed effects. The dependent variable is a binary indicator denoting having a new judgment outstanding (column 1-5), petitioned (column 6) or satisfied (column 7). The sample is quarterly credit report data. Columns 4 and 5 focus specifically on applicants with subprime and prime credit scores, respectively. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/tab_5.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Where are racial disparities in debt collection highest?}\label{table:5}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{5}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                    &\multicolumn{5}{c}{Judgment Outstanding}\\

\hline
& & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority            &      0.0496\sym{**} &      0.0472\sym{*}  &      0.0883\sym{***}&      0.0213         &      0.0674\sym{**} \\
                    &    (0.0238)         &    (0.0271)         &    (0.0314)         &    (0.0244)         &    (0.0273)         \\
& & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority $\times$ High Racial Bias &                     &      0.0107         &                     &                     &                     \\
                    &                     &    (0.0594)         &                     &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority $\times$ Low Non-Bank Financing&                     &                     &     -0.1096\sym{**} &                     &                     \\
                    &                     &                     &    (0.0468)         &                     &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority $\times$ High Households without Income &                     &                     &                     &      0.1455\sym{**} &                     \\
                    &                     &                     &                     &    (0.0719)         &                     \\
& & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority $\times$ High Tertiary Education&                     &                     &                     &                     &     -0.0888\sym{*}  \\
                    &                     &                     &                     &                     &    (0.0477)         \\
\hline
Credit Report Controls&           X         &           X         &           X         &           X         &           X         \\
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &           X         &           X         &           X         &           X         &           X         \\
Observations        & 468753        & 468641        & 463959        & 464026        & 464076        \\
Mean of DV (Minority=0)          &      0.1258         &      0.1258         &      0.1258         &      0.1258         &      0.1258         \\
$R^2$               &      0.0385         &      0.0385         &      0.0385         &      0.0385         &      0.0385         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table presents results from regression analyses examining debt collection judgments as a function of race, individual attributes, zip code fixed effects, and state-by-quarter fixed effects. The individual-level data are sourced from a combined dataset of credit bureau records and Home Mortgage Disclosure Act records. This dataset incorporates credit bureau records spanning the years from 2013 through 2018. The dependent variable is a binary indicator reflecting new outstanding debt collection judgment. Each specification controls for age, gender, minority status, state by quarter fixed effects, zip code fixed effects, and credit report controls. The reported coefficients are in percentage points. Standard errors are calculated using clustering by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/tab_6.tex <==
\begin{sidewaystable}[!h]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and Judgments using ZCTA5 Demographics}\label{table:4}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{3}{c}{Judgment Outstanding} \\ 
                    & \underline{Full Sample} & \underline{Mortgagor} & \underline{Non-Mortgagor}\\

\hline
& & & \\[\dimexpr-\normalbaselineskip+3pt]
ZIP Minority Share        &      0.1646\sym{***}&      0.1821\sym{***}&      0.1470\sym{***}\\
                    &    (0.0139)         &    (0.0163)         &    (0.0144)         \\
\hline
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         \\
Observations        &12,137,175         &3,284,329         &8,852,845         \\
Mean of DV          &      0.1707         &      0.1188         &      0.1899         \\
$R^2$               &      0.0020         &      0.0014         &      0.0025         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table provides a robustness test for our main findings by substituting borrowers' race with ZCTA5 demographic data, as opposed to our method of matching with HMDA. The robustness tests follow our main specification (Column (3)) of Table \ref{table:4}. Columns (1-3) show the results for the full sample, mortgagors, and non-mortgagors, respectively (mortgagors are anyone with a mortgage at some point in our data). The coefficients represent the effect (in percentage point units) of changing from a ZCTA5 with zero minority population share to one with 100\% minority residents. The data comprises credit bureau records from 2013–2017. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/table4_a.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and New Outstanding Judgments}\label{table:4a}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{6}{c}{Outstanding Judgment}\\

\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female         &      0.0114         &      0.0037         &      0.0086         &      0.0111         &      0.0397         &     -0.0059         \\
                    &    (0.0111)         &    (0.0138)         &    (0.0136)         &    (0.0139)         &    (0.0571)         &    (0.0067)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority             &      0.0974\sym{***}&      0.1156\sym{***}&      0.0496\sym{**} &      0.0470\sym{*}  &      0.1373\sym{*}  &      0.0194         \\
                    &    (0.0202)         &    (0.0246)         &    (0.0238)         &    (0.0245)         &    (0.0756)         &    (0.0122)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age                         &     -0.0013\sym{***}&     -0.0018\sym{***}&      0.0008\sym{*}  &      0.0004         &      0.0025         &      0.0003         \\
                    &    (0.0003)         &    (0.0004)         &    (0.0004)         &    (0.0005)         &    (0.0020)         &    (0.0002)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$  &                     &                     &     -0.0024\sym{***}&     -0.0026\sym{***}&     -0.0044\sym{***}&     -0.0004\sym{***}\\
                    &                     &                     &    (0.0002)         &    (0.0002)         &    (0.0005)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$      &                     &                     &      0.0019\sym{***}&      0.0022\sym{***}&      0.0011         &      0.0019         \\
                    &                     &                     &    (0.0006)         &    (0.0007)         &    (0.0008)         &    (0.0020)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$          &                     &                     &     -0.0002\sym{***}&     -0.0004\sym{***}&     -0.0006\sym{***}&     -0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0001)         &    (0.0002)         &    (0.0000)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Outstanding Judgment$_{t-1}$   &                     &                     &      0.0216         &     -0.0020         &     -0.8370\sym{***}&     -0.2061         \\
                    &                     &                     &    (0.0991)         &    (0.1008)         &    (0.1410)         &    (0.1615)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.1831\sym{***}&      0.2067\sym{***}&      1.8568\sym{***}&      1.9283\sym{***}&      3.0859\sym{***}&      0.3312\sym{***}\\
                    &    (0.0193)         &    (0.0219)         &    (0.1186)         &    (0.1270)         &    (0.3127)         &    (0.0621)         \\
\hline
Borrowers  &  All    &   All  &  All  &   All  &   Subprime  &  Prime  \\
State X Quarter Fixed Effects&                     &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469020         & 468754         & 468753         & 445530         & 122640         & 345323         \\
Mean of DV (Minority = 0)           &      0.1258         &      0.1258         &      0.1258         &      0.1258         &      0.4817         &      0.0187         \\
$R^2$               &      0.0001         &      0.0362         &      0.0385         &      0.0399         &      0.0744         &      0.0339         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table reports results from a regression of judgments on race, individual characteristics, zip code fixed effects, and state-by-quarter fixed effects. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. The dependent variable is a binary indicator denoting having a new judgment outstanding. The sample is quarterly credit report data. Column 1 includes no fixed effects and controls for age, gender, and minority status. Column 2 adds fixed effects, and Column 3 includes credit report controls.  Column 4 adds imputed credit bureau income, as well as HMDA income to the controls used in Column 3. Columns 5 and 6 focus specifically on applicants with subprime and prime credit scores, respectively, using the specification from Column 3. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/table_4_b.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and New Petitioned Judgments}\label{table:4b}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{6}{c}{Petitioned Judgment}\\

\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female               &      0.0078         &      0.0014         &      0.0036         &      0.0050         &      0.0185         &     -0.0019         \\
                    &    (0.0082)         &    (0.0098)         &    (0.0098)         &    (0.0104)         &    (0.0399)         &    (0.0049)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority             &      0.0464\sym{***}&      0.0555\sym{***}&      0.0220         &      0.0192         &      0.0575         &      0.0031         \\
                    &    (0.0132)         &    (0.0180)         &    (0.0178)         &    (0.0186)         &    (0.0572)         &    (0.0077)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age               &     -0.0009\sym{***}&     -0.0015\sym{***}&     -0.0002         &     -0.0005         &     -0.0009         &      0.0001         \\
                    &    (0.0002)         &    (0.0003)         &    (0.0003)         &    (0.0003)         &    (0.0014)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$  &                     &                     &     -0.0013\sym{***}&     -0.0014\sym{***}&     -0.0025\sym{***}&     -0.0002\sym{***}\\
                    &                     &                     &    (0.0001)         &    (0.0001)         &    (0.0004)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$          &                     &                     &      0.0011\sym{**} &      0.0013\sym{**} &      0.0008         &      0.0001         \\
                    &                     &                     &    (0.0004)         &    (0.0005)         &    (0.0006)         &    (0.0002)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$          &                     &                     &     -0.0001\sym{***}&     -0.0002\sym{***}&     -0.0004\sym{***}&     -0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0000)         &    (0.0001)         &    (0.0000)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Outstanding Judgment$_{t-1}$  &                     &                     &     -0.0466         &     -0.0639         &     -0.4568\sym{***}&      0.0137         \\
                    &                     &                     &    (0.0639)         &    (0.0658)         &    (0.0904)         &    (0.1340)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.1005\sym{***}&      0.1293\sym{***}&      0.9873\sym{***}&      1.0548\sym{***}&      1.8057\sym{***}&      0.1843\sym{***}\\
                    &    (0.0125)         &    (0.0160)         &    (0.0794)         &    (0.0862)         &    (0.2271)         &    (0.0428)         \\
\hline
State X Quarter Fixed Effects&                     &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469020         & 468754         & 468753         & 445530         & 122640         & 345323         \\
Mean of DV (Minority = 0)           &      0.0615         &      0.0615         &      0.0615         &      0.0615         &      0.2370         &      0.0087         \\
$R^2$               &      0.0001         &      0.0343         &      0.0356         &      0.0366         &      0.0707         &      0.0277         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table tests a regression of judgments on race, individual characteristics, and ZIP code fixed effects. The dependent variable is a binary indicator denoting having a new judgment petitioned. The sample is quarterly credit report data. Column 1 includes no fixed effects and controls for age, gender, and minority status. Column 2 adds fixed effects, while Column 3 includes credit report controls.  Column 4 adds imputed credit bureau income, as well as HMDA income to the controls used in Column 3. Columns 6 and 7 focus specifically on applicants with subprime and prime credit scores, respectively, using the specification from Column 3. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/table_4_bc.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and Judgments Petitioned or Satisfied}\label{table:4bc}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
\textbf{Panel A:  New Petitioned Judgment}  & & & & & & \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority             &      0.0464\sym{***}&      0.0555\sym{***}&      0.0220         &      0.0192         &      0.0575         &      0.0031         \\
                    &    (0.0132)         &    (0.0180)         &    (0.0178)         &    (0.0186)         &    (0.0572)         &    (0.0077)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
\hline
\textbf{Panel B:  New Satisfied Judgment}  & & & & & & \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority      &      0.0222\sym{**} &      0.0282\sym{***}&      0.0120         &      0.0068         &      0.0152         &      0.0062         \\
                    &    (0.0091)         &    (0.0106)         &    (0.0103)         &    (0.0106)         &    (0.0253)         &    (0.0090)         \\ \hline
Borrowers  &  All    &   All  &  All  &   All  &   Subprime  &  Prime  \\
Credit Controls  &      &   &  X  &   X  &   X  &  X  \\
State X Quarter Fixed Effects&                     &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469020         & 468754         & 468753         & 445530         & 122640         & 345323         \\
Mean of DV (Minority = 0)           &      0.0615         &      0.0615         &      0.0615         &      0.0615         &      0.2370         &      0.0087         \\
$R^2$               &      0.0001         &      0.0343         &      0.0356         &      0.0366         &      0.0707         &      0.0277         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table tests a regression of judgments on race, individual characteristics, zip code fixed effects, and state-by-quarter fixed effects. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. The dependent variable in Panel A is a binary indicator denoting having a new petitioned judgment, and the dependent variable in Panel B is a binary variable denoting having a new satisfied judgment. The sample is quarterly credit report data. Column 1 includes no fixed effects and controls for age, gender, and minority status. Column 2 adds fixed effects, while Column 3 includes credit report controls.  Column 4 adds imputed credit bureau income, as well as HMDA income to the controls used in Column 3. Columns 6 and 7 focus specifically on applicants with subprime and prime credit scores, respectively, using the specification from Column 3. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> New_Parts/Racial_Disparities_-_Submission/Tables/table_4_c.tex <==
\begin{sidewaystable}[!ht]
\footnotesize
\centering
\begin{threeparttable}
\caption{Race and New Satisfied Judgments}\label{table:4c}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{6}{c}{Satisfied Judgment}\\

\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Female          &            0.0080         &      0.0046         &      0.0063         &      0.0065         &     -0.0140         &      0.0090\sym{*}  \\
                    &    (0.0053)         &    (0.0060)         &    (0.0061)         &    (0.0064)         &    (0.0213)         &    (0.0050)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Minority      &      0.0222\sym{**} &      0.0282\sym{***}&      0.0120         &      0.0068         &      0.0152         &      0.0062         \\
                    &    (0.0091)         &    (0.0106)         &    (0.0103)         &    (0.0106)         &    (0.0253)         &    (0.0090)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Age              &     -0.0006\sym{***}&     -0.0005\sym{**} &     -0.0003         &     -0.0003         &     -0.0012         &      0.0000         \\
                    &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0007)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Credit Score$_{t-1}$ &                     &                     &     -0.0002\sym{***}&     -0.0002\sym{***}&     -0.0003\sym{**} &     -0.0001\sym{**} \\
                    &                     &                     &    (0.0000)         &    (0.0001)         &    (0.0002)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Past Due Debt$_{t-1}$  &                     &                     &     -0.0002         &     -0.0004\sym{**} &     -0.0003         &     -0.0001         \\
                    &                     &                     &    (0.0002)         &    (0.0001)         &    (0.0002)         &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Total Debt$_{t-1}$      &                     &                     &     -0.0000         &     -0.0000         &     -0.0001         &      0.0000         \\
                    &                     &                     &    (0.0000)         &    (0.0000)         &    (0.0001)         &    (0.0000)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Outstanding Judgment$_{t-1}$    &                     &                     &      0.6217\sym{***}&      0.6125\sym{***}&      0.5891\sym{***}&      1.1462\sym{***}\\
                    &                     &                     &    (0.0775)         &    (0.0786)         &    (0.0920)         &    (0.2722)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+3pt]
Constant            &      0.0494\sym{***}&      0.0449\sym{***}&      0.1673\sym{***}&      0.1784\sym{***}&      0.2965\sym{***}&      0.0897\sym{**} \\
                    &    (0.0086)         &    (0.0089)         &    (0.0353)         &    (0.0384)         &    (0.1065)         &    (0.0383)         \\
\hline
State X Quarter Fixed Effects&                     &           X         &           X         &           X         &           X         &           X         \\
ZIP Fixed Effects   &                     &           X         &           X         &           X         &           X         &           X         \\
Observations        & 469020         & 468754         & 468753         & 445530         & 122640         & 345323         \\
Mean of DV (Minority = 0)         &      0.0249         &      0.0249         &      0.0249         &      0.0249         &      0.0830         &      0.0073         \\
$R^2$               &      0.0001         &      0.0334         &      0.0379         &      0.0392         &      0.0762         &      0.0373         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes:  This table tests a regression of judgments on race, individual characteristics, and ZIP code fixed effects. The dependent variable is a binary indicator denoting having a new judgment satisfied. The sample is quarterly credit report data. Column 1 includes no fixed effects and controls for age, gender, and minority status. Column 2 adds fixed effects, while Column 3 includes credit report controls.  Column 4 adds imputed credit bureau income, as well as HMDA income to the controls used in Column 3. Columns 6 and 7 focus specifically on applicants with subprime and prime credit scores, respectively, using the specification from Column 3. The data comprises credit bureau records from 2013–2017, which have been merged with Home Mortgage Disclosure Act records. Reported coefficients are in percentage point units. Standard errors are clustered by state-quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Regressions/summary_tab1.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics}
\begin{tabular}{l*{9}{cc}}
\hline\hline
            &\multicolumn{1}{c}{Age < 30}&\multicolumn{1}{c}{Age >= 30}&\multicolumn{1}{c}{t-test}&\multicolumn{1}{c}{p20}&\multicolumn{1}{c}{>p20}&\multicolumn{2}{c}{t-test}        &\multicolumn{1}{c}{Minority}&\multicolumn{1}{c}{Non-Minority}&\multicolumn{2}{c}{t-test}        \\
            &     mean/sd&     mean/sd&           b         &     mean/sd&     mean/sd&     mean/sd&           b         &     mean/sd&     mean/sd&     mean/sd&           b         \\
\hline
outcome     &        0.24&        0.23&       -0.01\sym{***}&        0.45&        0.20&            &       -0.24\sym{***}&        0.38&        0.20&            &       -0.19\sym{***}\\
            &      (0.42)&      (0.42)&                     &      (0.50)&      (0.40)&            &                     &      (0.49)&      (0.40)&            &                     \\
pp\_percentile&       47.88&       55.39&        7.51\sym{***}&       33.02&       56.37&            &       23.35\sym{***}&       42.42&       56.29&            &       13.87\sym{***}\\
            &     (20.46)&     (25.39)&                     &     (18.77)&     (24.10)&            &                     &     (24.19)&     (24.04)&            &                     \\
cs\_percentile&       47.89&       57.58&        9.69\sym{***}&       32.89&       58.38&            &       25.48\sym{***}&       45.65&       57.71&            &       12.06\sym{***}\\
            &     (20.39)&     (24.95)&                     &     (18.34)&     (23.60)&            &                     &     (24.25)&     (23.90)&            &                     \\
all5030     &       58.50&      164.32&      105.82\sym{***}&       30.03&      156.54&            &      126.51\sym{***}&      119.19&      147.54&            &       28.35\sym{***}\\
            &     (95.33)&    (185.70)&                     &     (62.09)&    (180.71)&            &                     &    (144.46)&    (182.03)&            &                     \\
all5048     &        1.52&        4.18&        2.65\sym{***}&        3.01&        3.72&            &        0.71\sym{***}&        7.00&        2.91&            &       -4.09\sym{***}\\
            &     (18.62)&     (35.95)&                     &     (21.04)&     (34.37)&            &                     &     (44.24)&     (30.21)&            &                     \\
income\_insight\_score&       50.07&       98.78&       48.70\sym{***}&       30.57&       95.86&            &       65.30\sym{***}&       72.90&       92.26&            &       19.36\sym{***}\\
            &     (27.53)&     (57.56)&                     &      (6.31)&     (55.65)&            &                     &     (44.89)&     (57.96)&            &                     \\
age         &       24.79&       47.24&       22.45\sym{***}&       29.51&       44.27&            &       14.76\sym{***}&       42.25&       42.70&            &        0.46\sym{***}\\
            &      (3.05)&     (11.64)&                     &     (10.69)&     (13.30)&            &                     &     (13.47)&     (13.93)&            &                     \\
\hline
\(N\)       &      227638&      878641&     1106279         &      118475&      984190&     1102665&                     &      195031&      911248&     1106279&                     \\
\hline\hline
\end{tabular}
\end{table}


==> Regressions/summary_tab1_full_sample.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics}
\begin{tabular}{l*{9}{cc}}
\hline\hline
            &\multicolumn{1}{c}{Age < 30}&\multicolumn{1}{c}{Age >= 30}&\multicolumn{1}{c}{t-test}&\multicolumn{1}{c}{p20}&\multicolumn{1}{c}{>p20}&\multicolumn{2}{c}{t-test}        &\multicolumn{1}{c}{Minority}&\multicolumn{1}{c}{Non-Minority}&\multicolumn{2}{c}{t-test}        \\
            &     mean/sd&     mean/sd&           b         &     mean/sd&     mean/sd&     mean/sd&           b         &     mean/sd&     mean/sd&     mean/sd&           b         \\
\hline
outcome     &        0.42&        0.31&       -0.11\sym{***}&        0.65&        0.26&            &       -0.39\sym{***}&        0.51&        0.30&            &       -0.21\sym{***}\\
            &      (0.49)&      (0.46)&                     &      (0.48)&      (0.44)&            &                     &      (0.50)&      (0.46)&            &                     \\
pp\_percentile&       39.05&       52.76&       13.71\sym{***}&       24.68&       56.12&            &       31.44\sym{***}&       37.09&       52.91&            &       15.81\sym{***}\\
            &     (23.34)&     (29.82)&                     &     (18.51)&     (28.00)&            &                     &     (26.66)&     (28.91)&            &                     \\
cs\_percentile&       37.12&       53.24&       16.12\sym{***}&       22.68&       56.65&            &       33.97\sym{***}&       37.85&       52.74&            &       14.88\sym{***}\\
            &     (23.40)&     (29.56)&                     &     (17.97)&     (27.48)&            &                     &     (27.31)&     (28.86)&            &                     \\
all5030     &       26.32&       91.37&       65.05\sym{***}&       10.42&       95.02&            &       84.61\sym{***}&       53.65&       83.85&            &       30.20\sym{***}\\
            &     (67.85)&    (187.99)&                     &     (37.33)&    (188.21)&            &                     &    (125.45)&    (181.25)&            &                     \\
all5048     &        1.44&        3.71&        2.27\sym{***}&        2.10&        3.54&            &        1.45\sym{***}&        4.74&        2.92&            &       -1.82\sym{***}\\
            &     (14.76)&     (37.10)&                     &     (14.79)&     (37.04)&            &                     &     (36.95)&     (33.08)&            &                     \\
income\_insight\_score&       42.81&       88.57&       45.76\sym{***}&       29.48&       91.51&            &       62.03\sym{***}&       62.34&       83.35&            &       21.01\sym{***}\\
            &     (27.26)&     (57.36)&                     &      (6.55)&     (55.78)&            &                     &     (43.29)&     (57.59)&            &                     \\
age         &       24.13&       51.52&       27.39\sym{***}&       32.52&       49.38&            &       16.86\sym{***}&       44.23&       46.42&            &        2.19\sym{***}\\
            &      (3.17)&     (13.53)&                     &     (12.84)&     (15.39)&            &                     &     (15.81)&     (16.49)&            &                     \\
\hline
\(N\)       &     4719309&    18784855&    23504164         &     4527455&    18865186&    23392641&                     &     4310064&    19194100&    23504164&                     \\
\hline\hline
\end{tabular}
\end{table}


==> Regressions/vulnerable_full_sample.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
minority=0          &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1          &     -0.8878\sym{***}&     -0.6892\sym{***}&     -0.4657\sym{***}&     -2.0599\sym{***}&     -2.2121\sym{***}&     -1.8899\sym{***}\\
                    &    (0.0204)         &    (0.0223)         &    (0.0410)         &    (0.0426)         &    (0.0329)         &    (0.0384)         \\
[1em]
young=0             &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1             &      1.3640\sym{***}&      0.7891\sym{***}&      2.5074\sym{***}&      0.7732\sym{***}&     -0.3274\sym{***}&     -1.3637\sym{***}\\
                    &    (0.0300)         &    (0.0281)         &    (0.0720)         &    (0.0392)         &    (0.0415)         &    (0.0521)         \\
[1em]
low\_income\_p20=0    &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1    &      2.1560\sym{***}&      3.7466\sym{***}&      1.6403\sym{***}&     -1.6414\sym{***}&     -1.3764\sym{***}&     -5.4656\sym{***}\\
                    &    (0.0324)         &    (0.0486)         &    (0.0514)         &    (0.0577)         &    (0.0516)         &    (0.1419)         \\
[1em]
outcome=0           &                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &                     &     -3.9528\sym{***}&     -8.4918\sym{***}&    -11.8653\sym{***}&    -11.6279\sym{***}&     -8.0743\sym{***}\\
                    &                     &    (0.0407)         &    (0.0390)         &    (0.0612)         &    (0.0796)         &    (0.0544)         \\
[1em]
minority=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1 $\times$ outcome=1&                     &      0.7920\sym{***}&      0.5293\sym{***}&      0.7552\sym{***}&      0.6151\sym{***}&      0.2024\sym{*}  \\
                    &                     &    (0.0416)         &    (0.0425)         &    (0.0638)         &    (0.0903)         &    (0.1168)         \\
[1em]
young=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1 $\times$ outcome=1&                     &      0.8815\sym{***}&     -1.2491\sym{***}&      2.5169\sym{***}&      4.4637\sym{***}&      3.7470\sym{***}\\
                    &                     &    (0.0234)         &    (0.0629)         &    (0.0435)         &    (0.0527)         &    (0.2158)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=1&                     &     -0.3114\sym{***}&     -0.3757\sym{***}&      0.4674\sym{***}&      3.0389\sym{***}&      2.2234\sym{***}\\
                    &                     &    (0.0433)         &    (0.0462)         &    (0.0478)         &    (0.0623)         &    (0.7574)         \\
[1em]
Constant            &     -0.5685\sym{***}&      0.4200\sym{***}&      8.5217\sym{***}&      6.5220\sym{***}&      1.3454\sym{***}&     -2.3688\sym{***}\\
                    &    (0.0114)         &    (0.0148)         &    (0.0390)         &    (0.0230)         &    (0.0135)         &    (0.0038)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &23392641.0000         &23392641.0000         &6317929.0000         &3349410.0000         &7878288.0000         &5847014.0000         \\
$R^2$               &      0.0162         &      0.0354         &      0.1432         &      0.2143         &      0.0923         &      0.0281         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize }\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_full_sample_black_indicator.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
black\_indicator=0   &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
black\_indicator=1   &      0.3114\sym{***}&     -0.3040\sym{***}&      0.0888\sym{***}&     -0.6573\sym{***}&     -1.9095\sym{***}&     -2.3004\sym{***}&     -2.2300\sym{***}&     -2.2493\sym{***}&     -2.0131\sym{***}&     -1.9958\sym{***}\\
                    &    (0.0196)         &    (0.0278)         &    (0.0189)         &    (0.0443)         &    (0.0331)         &    (0.0494)         &    (0.0314)         &    (0.0361)         &    (0.0401)         &    (0.0405)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.6711\sym{***}&     -2.7394\sym{***}&     -9.0750\sym{***}&     -9.1464\sym{***}&    -11.1257\sym{***}&    -11.1715\sym{***}&    -10.3225\sym{***}&    -10.3275\sym{***}&     -8.0022\sym{***}&     -7.9861\sym{***}\\
                    &    (0.0347)         &    (0.0353)         &    (0.0336)         &    (0.0353)         &    (0.0645)         &    (0.0667)         &    (0.0795)         &    (0.0813)         &    (0.0525)         &    (0.0525)         \\
[1em]
black\_indicator=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
black\_indicator=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
black\_indicator=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
black\_indicator=1 $\times$ outcome=1&                     &      1.0693\sym{***}&                     &      0.8614\sym{***}&                     &      0.7183\sym{***}&                     &      0.0868         &                     &     -0.3605\sym{*}  \\
                    &                     &    (0.0386)         &                     &    (0.0493)         &                     &    (0.0741)         &                     &    (0.0973)         &                     &    (0.2076)         \\
[1em]
Constant            &      0.8783\sym{***}&      0.9003\sym{***}&     10.0983\sym{***}&     10.1563\sym{***}&      6.0681\sym{***}&      6.0875\sym{***}&      0.9091\sym{***}&      0.9098\sym{***}&     -2.5397\sym{***}&     -2.5401\sym{***}\\
                    &    (0.0113)         &    (0.0115)         &    (0.0273)         &    (0.0286)         &    (0.0273)         &    (0.0282)         &    (0.0107)         &    (0.0110)         &    (0.0016)         &    (0.0016)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &23504164.0000         &23504164.0000         &6358871.0000         &6358871.0000         &3377487.0000         &3377487.0000         &7919800.0000         &7919800.0000         &5848006.0000         &5848006.0000         \\
$R^2$               &      0.0168         &      0.0169         &      0.1348         &      0.1349         &      0.2069         &      0.2069         &      0.0856         &      0.0856         &      0.0255         &      0.0255         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_full_sample_hispanic_indicator.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
hispanic\_indicator=0&      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
hispanic\_indicator=1&     -0.2581\sym{***}&     -0.4344\sym{***}&      0.1049\sym{***}&     -0.3341\sym{***}&     -1.5172\sym{***}&     -1.8472\sym{***}&     -2.0683\sym{***}&     -2.2599\sym{***}&     -2.0377\sym{***}&     -2.0931\sym{***}\\
                    &    (0.0321)         &    (0.0436)         &    (0.0316)         &    (0.0598)         &    (0.0443)         &    (0.0809)         &    (0.0494)         &    (0.0557)         &    (0.0710)         &    (0.0729)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.6424\sym{***}&     -2.6742\sym{***}&     -9.0728\sym{***}&     -9.1295\sym{***}&    -11.1483\sym{***}&    -11.2132\sym{***}&    -10.3223\sym{***}&    -10.4110\sym{***}&     -7.9923\sym{***}&     -8.0739\sym{***}\\
                    &    (0.0342)         &    (0.0312)         &    (0.0336)         &    (0.0327)         &    (0.0649)         &    (0.0582)         &    (0.0800)         &    (0.0713)         &    (0.0524)         &    (0.0534)         \\
[1em]
hispanic\_indicator=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
hispanic\_indicator=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
hispanic\_indicator=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
hispanic\_indicator=1 $\times$ outcome=1&                     &      0.3820\sym{***}&                     &      0.5380\sym{***}&                     &      0.6795\sym{***}&                     &      0.9858\sym{***}&                     &      1.1908\sym{***}\\
                    &                     &    (0.0701)         &                     &    (0.0602)         &                     &    (0.1208)         &                     &    (0.1596)         &                     &    (0.1528)         \\
[1em]
Constant            &      0.9055\sym{***}&      0.9158\sym{***}&     10.0950\sym{***}&     10.1414\sym{***}&      6.1011\sym{***}&      6.1287\sym{***}&      0.9619\sym{***}&      0.9738\sym{***}&     -2.5126\sym{***}&     -2.5106\sym{***}\\
                    &    (0.0119)         &    (0.0110)         &    (0.0266)         &    (0.0261)         &    (0.0265)         &    (0.0238)         &    (0.0117)         &    (0.0105)         &    (0.0030)         &    (0.0030)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &23504164.0000         &23504164.0000         &6358871.0000         &6358871.0000         &3377487.0000         &3377487.0000         &7919800.0000         &7919800.0000         &5848006.0000         &5848006.0000         \\
$R^2$               &      0.0168         &      0.0168         &      0.1348         &      0.1348         &      0.2066         &      0.2067         &      0.0860         &      0.0860         &      0.0259         &      0.0259         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_full_sample_low_income_p20.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
low\_income\_p20=0    &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1    &      4.0810\sym{***}&      4.1462\sym{***}&      1.8645\sym{***}&      2.6902\sym{***}&     -0.6546\sym{***}&     -1.2599\sym{***}&     -0.7079\sym{***}&     -1.6375\sym{***}&     -5.9741\sym{***}&     -6.1828\sym{***}\\
                    &    (0.0418)         &    (0.0592)         &    (0.0311)         &    (0.0854)         &    (0.0575)         &    (0.0640)         &    (0.0591)         &    (0.0589)         &    (0.1423)         &    (0.1409)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -3.7478\sym{***}&     -3.7223\sym{***}&     -8.9552\sym{***}&     -8.5298\sym{***}&    -11.2017\sym{***}&    -11.5304\sym{***}&    -10.3760\sym{***}&    -11.0479\sym{***}&     -8.0208\sym{***}&     -8.0277\sym{***}\\
                    &    (0.0405)         &    (0.0442)         &    (0.0331)         &    (0.0388)         &    (0.0636)         &    (0.0655)         &    (0.0796)         &    (0.0879)         &    (0.0524)         &    (0.0526)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=1&                     &     -0.1155\sym{***}&                     &     -1.0032\sym{***}&                     &      1.3905\sym{***}&                     &      5.5265\sym{***}&                     &      3.4387\sym{***}\\
                    &                     &    (0.0443)         &                     &    (0.0733)         &                     &    (0.0433)         &                     &    (0.0720)         &                     &    (0.7620)         \\
[1em]
Constant            &      0.4252\sym{***}&      0.4185\sym{***}&      9.0680\sym{***}&      8.7271\sym{***}&      6.1030\sym{***}&      6.2443\sym{***}&      0.8868\sym{***}&      0.9771\sym{***}&     -2.5811\sym{***}&     -2.5809\sym{***}\\
                    &    (0.0123)         &    (0.0141)         &    (0.0245)         &    (0.0370)         &    (0.0259)         &    (0.0274)         &    (0.0111)         &    (0.0123)         &    (0.0013)         &    (0.0013)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &23392641.0000         &23392641.0000         &6317929.0000         &6317929.0000         &3349410.0000         &3349410.0000         &7878288.0000         &7878288.0000         &5847014.0000         &5847014.0000         \\
$R^2$               &      0.0337         &      0.0337         &      0.1385         &      0.1389         &      0.2067         &      0.2072         &      0.0851         &      0.0874         &      0.0249         &      0.0249         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_full_sample_minority.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
minority=0          &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1          &     -0.0198         &     -0.4015\sym{***}&      0.0612\sym{***}&     -0.5944\sym{***}&     -1.7614\sym{***}&     -2.1128\sym{***}&     -2.1147\sym{***}&     -2.2140\sym{***}&     -1.8855\sym{***}&     -1.8938\sym{***}\\
                    &    (0.0216)         &    (0.0238)         &    (0.0180)         &    (0.0420)         &    (0.0262)         &    (0.0434)         &    (0.0307)         &    (0.0334)         &    (0.0379)         &    (0.0386)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.6501\sym{***}&     -2.8234\sym{***}&     -9.0751\sym{***}&     -9.2759\sym{***}&    -11.0759\sym{***}&    -11.2354\sym{***}&    -10.2388\sym{***}&    -10.3479\sym{***}&     -7.9340\sym{***}&     -7.9665\sym{***}\\
                    &    (0.0341)         &    (0.0306)         &    (0.0338)         &    (0.0345)         &    (0.0651)         &    (0.0582)         &    (0.0798)         &    (0.0692)         &    (0.0522)         &    (0.0535)         \\
[1em]
minority=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
minority=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
minority=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
minority=1 $\times$ outcome=1&                     &      0.8156\sym{***}&                     &      0.7843\sym{***}&                     &      0.7173\sym{***}&                     &      0.5280\sym{***}&                     &      0.1994\sym{*}  \\
                    &                     &    (0.0418)         &                     &    (0.0459)         &                     &    (0.0668)         &                     &    (0.0924)         &                     &    (0.1167)         \\
[1em]
Constant            &      0.8927\sym{***}&      0.9448\sym{***}&     10.0903\sym{***}&     10.2527\sym{***}&      6.3092\sym{***}&      6.3748\sym{***}&      1.1322\sym{***}&      1.1461\sym{***}&     -2.4150\sym{***}&     -2.4142\sym{***}\\
                    &    (0.0123)         &    (0.0112)         &    (0.0265)         &    (0.0273)         &    (0.0263)         &    (0.0234)         &    (0.0124)         &    (0.0111)         &    (0.0039)         &    (0.0040)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &23504164.0000         &23504164.0000         &6358871.0000         &6358871.0000         &3377487.0000         &3377487.0000         &7919800.0000         &7919800.0000         &5848006.0000         &5848006.0000         \\
$R^2$               &      0.0167         &      0.0169         &      0.1348         &      0.1350         &      0.2085         &      0.2086         &      0.0876         &      0.0877         &      0.0273         &      0.0273         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_full_sample_young.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
young=0             &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1             &      2.7164\sym{***}&      2.3447\sym{***}&      2.2733\sym{***}&      3.9645\sym{***}&      1.1445\sym{***}&      0.0059         &      0.0338         &     -0.6429\sym{***}&     -1.3190\sym{***}&     -1.4245\sym{***}\\
                    &    (0.0399)         &    (0.0445)         &    (0.0390)         &    (0.1027)         &    (0.0506)         &    (0.0485)         &    (0.0485)         &    (0.0457)         &    (0.0523)         &    (0.0517)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.8675\sym{***}&     -3.0742\sym{***}&     -8.9926\sym{***}&     -8.3547\sym{***}&    -11.1110\sym{***}&    -11.7988\sym{***}&    -10.3781\sym{***}&    -11.5197\sym{***}&     -8.0376\sym{***}&     -8.1673\sym{***}\\
                    &    (0.0344)         &    (0.0372)         &    (0.0317)         &    (0.0366)         &    (0.0629)         &    (0.0668)         &    (0.0783)         &    (0.0880)         &    (0.0526)         &    (0.0535)         \\
[1em]
young=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
young=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
young=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
young=1 $\times$ outcome=1&                     &      0.9341\sym{***}&                     &     -2.0891\sym{***}&                     &      2.9145\sym{***}&                     &      5.5399\sym{***}&                     &      3.6611\sym{***}\\
                    &                     &    (0.0283)         &                     &    (0.0872)         &                     &    (0.0389)         &                     &    (0.0635)         &                     &    (0.2154)         \\
[1em]
Constant            &      0.4166\sym{***}&      0.4814\sym{***}&      9.3904\sym{***}&      8.8643\sym{***}&      5.6606\sym{***}&      5.9703\sym{***}&      0.8232\sym{***}&      0.9890\sym{***}&     -2.5457\sym{***}&     -2.5425\sym{***}\\
                    &    (0.0117)         &    (0.0130)         &    (0.0226)         &    (0.0340)         &    (0.0229)         &    (0.0243)         &    (0.0103)         &    (0.0110)         &    (0.0019)         &    (0.0019)         \\
\hline
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &23504164.0000         &23504164.0000         &6358871.0000         &6358871.0000         &3377487.0000         &3377487.0000         &7919800.0000         &7919800.0000         &5848006.0000         &5848006.0000         \\
$R^2$               &      0.0253         &      0.0255         &      0.1452         &      0.1466         &      0.2071         &      0.2094         &      0.0846         &      0.0881         &      0.0251         &      0.0252         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_hmda.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
female=0            &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
female=1            &     -0.6597\sym{***}&     -0.7317\sym{***}&     -0.2980         &      0.1152         &     -0.6105\sym{***}&     -0.2963\sym{**} \\
                    &    (0.0348)         &    (0.0389)         &    (0.4769)         &    (0.2990)         &    (0.0760)         &    (0.1172)         \\
[1em]
minority=0          &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1          &     -0.8571\sym{***}&     -0.6146\sym{***}&     -1.5145\sym{***}&     -1.7234\sym{***}&     -1.4824\sym{***}&     -0.1805         \\
                    &    (0.0524)         &    (0.0609)         &    (0.5329)         &    (0.3778)         &    (0.1193)         &    (0.2311)         \\
[1em]
young=0             &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1             &      1.5119\sym{***}&      1.2657\sym{***}&      1.8342\sym{***}&      0.8869\sym{**} &      0.3126\sym{***}&     -1.0329\sym{***}\\
                    &    (0.0443)         &    (0.0497)         &    (0.5738)         &    (0.3722)         &    (0.0866)         &    (0.2497)         \\
[1em]
low\_income\_p20=0    &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1    &      1.6958\sym{***}&      2.4339\sym{***}&      2.1370\sym{***}&     -2.0029\sym{***}&     -1.1577\sym{***}&     -3.2750\sym{*}  \\
                    &    (0.0580)         &    (0.0753)         &    (0.5789)         &    (0.4186)         &    (0.1342)         &    (1.8491)         \\
[1em]
outcome=0           &                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &                     &     -3.2372\sym{***}&     -7.4010\sym{***}&     -8.9737\sym{***}&     -9.0899\sym{***}&     -6.5594\sym{***}\\
                    &                     &    (0.0672)         &    (0.4468)         &    (0.3862)         &    (0.1864)         &    (0.6347)         \\
[1em]
female=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
female=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
female=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
female=1 $\times$ outcome=1&                     &      0.2395\sym{***}&     -0.4921         &     -0.7735         &      0.0726         &     -0.8612         \\
                    &                     &    (0.0846)         &    (0.5412)         &    (0.4920)         &    (0.2455)         &    (0.9531)         \\
[1em]
minority=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1 $\times$ outcome=1&                     &      0.2410\sym{**} &      0.7804         &      0.3127         &      0.2573         &     -1.4416         \\
                    &                     &    (0.0983)         &    (0.5651)         &    (0.5314)         &    (0.2935)         &    (1.4373)         \\
[1em]
young=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1 $\times$ outcome=1&                     &      0.2231\sym{**} &     -0.5102         &      1.0166         &      3.3383\sym{***}&      4.7955\sym{***}\\
                    &                     &    (0.1056)         &    (0.6510)         &    (0.6243)         &    (0.3137)         &    (1.7487)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=1&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=0&                     &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &                     &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=1&                     &     -0.1520         &     -1.7890\sym{***}&      0.8770         &      1.5978\sym{***}&      1.8480         \\
                    &                     &    (0.1180)         &    (0.6451)         &    (0.6658)         &    (0.4104)         &    (4.2607)         \\
[1em]
Constant            &     -1.8354\sym{***}&     -1.1741\sym{***}&      7.0119\sym{***}&      4.9036\sym{***}&     -0.5295\sym{***}&     -4.5593\sym{***}\\
                    &    (0.0195)         &    (0.0238)         &    (0.3746)         &    (0.2007)         &    (0.0452)         &    (0.0597)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &1102665.0000         &1102665.0000         & 156842.0000         & 172220.0000         & 504534.0000         & 269069.0000         \\
$R^2$               &      0.3862         &      0.3931         &      0.8260         &      0.8274         &      0.5941         &      0.6803         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize }\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_hmda_female.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
female=0            &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
female=1            &     -0.7173\sym{***}&     -0.7842\sym{***}&     -0.7250\sym{***}&     -0.4268         &     -0.2283         &      0.0862         &     -0.6155\sym{***}&     -0.6166\sym{***}&     -0.3193\sym{***}&     -0.2974\sym{**} \\
                    &    (0.0347)         &    (0.0390)         &    (0.2251)         &    (0.4848)         &    (0.2390)         &    (0.2967)         &    (0.0722)         &    (0.0758)         &    (0.1171)         &    (0.1171)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.8598\sym{***}&     -2.9881\sym{***}&     -8.4211\sym{***}&     -8.2638\sym{***}&     -8.9206\sym{***}&     -8.5915\sym{***}&     -8.3168\sym{***}&     -8.3211\sym{***}&     -6.8585\sym{***}&     -6.5062\sym{***}\\
                    &    (0.0436)         &    (0.0568)         &    (0.2744)         &    (0.3566)         &    (0.2459)         &    (0.3186)         &    (0.1230)         &    (0.1622)         &    (0.4654)         &    (0.6008)         \\
[1em]
female=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
female=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
female=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
female=1 $\times$ outcome=1&                     &      0.3023\sym{***}&                     &     -0.3873         &                     &     -0.7984         &                     &      0.0102         &                     &     -0.8855         \\
                    &                     &    (0.0847)         &                     &    (0.5479)         &                     &    (0.4887)         &                     &    (0.2455)         &                     &    (0.9576)         \\
[1em]
Constant            &     -0.7843\sym{***}&     -0.7559\sym{***}&      8.2144\sym{***}&      8.0949\sym{***}&      4.5383\sym{***}&      4.4143\sym{***}&     -0.7468\sym{***}&     -0.7464\sym{***}&     -4.6263\sym{***}&     -4.6361\sym{***}\\
                    &    (0.0179)         &    (0.0194)         &    (0.2280)         &    (0.2879)         &    (0.1346)         &    (0.1515)         &    (0.0335)         &    (0.0348)         &    (0.0545)         &    (0.0545)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &1106279.0000         &1106279.0000         & 157669.0000         & 157669.0000         & 173309.0000         & 173309.0000         & 506195.0000         & 506195.0000         & 269106.0000         & 269106.0000         \\
$R^2$               &      0.3877         &      0.3877         &      0.8245         &      0.8245         &      0.8254         &      0.8255         &      0.5918         &      0.5918         &      0.6802         &      0.6802         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_hmda_low_income_p20.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
low\_income\_p20=0    &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
low\_income\_p20=1    &      3.0181\sym{***}&      3.1631\sym{***}&      1.2455\sym{***}&      2.9330\sym{***}&     -1.1546\sym{***}&     -1.6128\sym{***}&     -0.5764\sym{***}&     -1.0254\sym{***}&     -3.6520\sym{**} &     -3.9101\sym{**} \\
                    &    (0.0550)         &    (0.0704)         &    (0.2455)         &    (0.5313)         &    (0.3011)         &    (0.3733)         &    (0.1207)         &    (0.1268)         &    (1.6827)         &    (1.8278)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -3.1604\sym{***}&     -3.1080\sym{***}&     -8.1872\sym{***}&     -7.5320\sym{***}&     -8.9398\sym{***}&     -9.1504\sym{***}&     -8.3181\sym{***}&     -8.5943\sym{***}&     -6.8257\sym{***}&     -6.8352\sym{***}\\
                    &    (0.0441)         &    (0.0484)         &    (0.2729)         &    (0.3191)         &    (0.2471)         &    (0.2730)         &    (0.1234)         &    (0.1299)         &    (0.4657)         &    (0.4674)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
low\_income\_p20=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
low\_income\_p20=1 $\times$ outcome=1&                     &     -0.3578\sym{***}&                     &     -2.1934\sym{***}&                     &      1.1869\sym{*}  &                     &      3.3159\sym{***}&                     &      2.1707         \\
                    &                     &    (0.1097)         &                     &    (0.5953)         &                     &    (0.6057)         &                     &    (0.3821)         &                     &    (4.4776)         \\
[1em]
Constant            &     -1.3712\sym{***}&     -1.3817\sym{***}&      7.2888\sym{***}&      6.7822\sym{***}&      4.6376\sym{***}&      4.7209\sym{***}&     -0.9670\sym{***}&     -0.9349\sym{***}&     -4.7672\sym{***}&     -4.7668\sym{***}\\
                    &    (0.0109)         &    (0.0116)         &    (0.2185)         &    (0.2555)         &    (0.1092)         &    (0.1176)         &    (0.0177)         &    (0.0181)         &    (0.0129)         &    (0.0130)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &1102665.0000         &1102665.0000         & 156842.0000         & 156842.0000         & 172220.0000         & 172220.0000         & 504534.0000         & 504534.0000         & 269069.0000         & 269069.0000         \\
$R^2$               &      0.3913         &      0.3913         &      0.8243         &      0.8247         &      0.8263         &      0.8263         &      0.5922         &      0.5924         &      0.6800         &      0.6800         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_hmda_minority.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
minority=0          &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
minority=1          &     -0.4681\sym{***}&     -0.5296\sym{***}&     -0.9589\sym{***}&     -1.7033\sym{***}&     -1.6575\sym{***}&     -1.7603\sym{***}&     -1.4759\sym{***}&     -1.5029\sym{***}&     -0.2539         &     -0.1957         \\
                    &    (0.0524)         &    (0.0609)         &    (0.2755)         &    (0.5356)         &    (0.3049)         &    (0.3745)         &    (0.1134)         &    (0.1189)         &    (0.2288)         &    (0.2309)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.8186\sym{***}&     -2.8655\sym{***}&     -8.3877\sym{***}&     -8.6868\sym{***}&     -8.8710\sym{***}&     -8.9371\sym{***}&     -8.2604\sym{***}&     -8.2974\sym{***}&     -6.8339\sym{***}&     -6.6307\sym{***}\\
                    &    (0.0438)         &    (0.0504)         &    (0.2745)         &    (0.3349)         &    (0.2459)         &    (0.2871)         &    (0.1230)         &    (0.1391)         &    (0.4655)         &    (0.4978)         \\
[1em]
minority=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
minority=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
minority=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
minority=1 $\times$ outcome=1&                     &      0.1933\sym{**} &                     &      0.9366\sym{*}  &                     &      0.2376         &                     &      0.1774         &                     &     -1.5633         \\
                    &                     &    (0.0984)         &                     &    (0.5647)         &                     &    (0.5279)         &                     &    (0.2938)         &                     &    (1.4354)         \\
[1em]
Constant            &     -1.0145\sym{***}&     -1.0059\sym{***}&      8.1866\sym{***}&      8.4091\sym{***}&      4.8228\sym{***}&      4.8458\sym{***}&     -0.7785\sym{***}&     -0.7750\sym{***}&     -4.7470\sym{***}&     -4.7516\sym{***}\\
                    &    (0.0129)         &    (0.0137)         &    (0.2216)         &    (0.2654)         &    (0.1152)         &    (0.1252)         &    (0.0227)         &    (0.0232)         &    (0.0253)         &    (0.0254)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &1106279.0000         &1106279.0000         & 157669.0000         & 157669.0000         & 173309.0000         & 173309.0000         & 506195.0000         & 506195.0000         & 269106.0000         & 269106.0000         \\
$R^2$               &      0.3872         &      0.3872         &      0.8246         &      0.8246         &      0.8260         &      0.8260         &      0.5922         &      0.5922         &      0.6801         &      0.6801         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_hmda_race_.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
Asian               &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
Black or African American&     -0.3041\sym{***}&     -0.2670\sym{**} &     -1.7769\sym{**} &     -2.4401\sym{*}  &     -2.5383\sym{***}&     -2.0265\sym{**} &     -1.3847\sym{***}&     -1.2547\sym{***}&      0.5673         &      0.6513         \\
                    &    (0.1029)         &    (0.1167)         &    (0.7324)         &    (1.3156)         &    (0.7191)         &    (0.8714)         &    (0.2138)         &    (0.2236)         &    (0.4070)         &    (0.4077)         \\
[1em]
Hispanic or Latino  &     -0.1459         &     -0.1315         &     -1.1341         &     -1.0009         &     -2.7285\sym{***}&     -2.9767\sym{***}&     -1.3163\sym{***}&     -1.3418\sym{***}&      0.5588         &      0.5020         \\
                    &    (0.0982)         &    (0.1087)         &    (0.7348)         &    (1.3278)         &    (0.6950)         &    (0.8321)         &    (0.1978)         &    (0.2049)         &    (0.3614)         &    (0.3635)         \\
[1em]
White               &      0.2773\sym{***}&      0.3730\sym{***}&     -0.5453         &     -0.0050         &     -1.0681\sym{*}  &     -0.8717         &      0.1447         &      0.2146         &      0.9172\sym{***}&      0.8598\sym{***}\\
                    &    (0.0797)         &    (0.0848)         &    (0.6897)         &    (1.2047)         &    (0.6306)         &    (0.7443)         &    (0.1541)         &    (0.1577)         &    (0.2455)         &    (0.2434)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.8184\sym{***}&     -2.2817\sym{***}&     -8.3800\sym{***}&     -7.9949\sym{***}&     -8.8679\sym{***}&     -8.3394\sym{***}&     -8.2607\sym{***}&     -7.5627\sym{***}&     -6.8315\sym{***}&     -8.4314\sym{***}\\
                    &    (0.0439)         &    (0.2153)         &    (0.2744)         &    (1.3781)         &    (0.2459)         &    (1.2671)         &    (0.1230)         &    (0.5641)         &    (0.4655)         &    (1.8177)         \\
[1em]
Asian $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
Asian $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
Black or African American $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
Black or African American $\times$ outcome=1&                     &     -0.4287\sym{*}  &                     &      0.7314         &                     &     -1.2598         &                     &     -1.1107         &                     &     -2.4372         \\
                    &                     &    (0.2475)         &                     &    (1.5120)         &                     &    (1.4225)         &                     &    (0.6859)         &                     &    (3.1955)         \\
[1em]
Hispanic or Latino $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
Hispanic or Latino $\times$ outcome=1&                     &     -0.3376         &                     &     -0.2091         &                     &      0.4209         &                     &     -0.1501         &                     &      1.6876         \\
                    &                     &    (0.2455)         &                     &    (1.5502)         &                     &    (1.4158)         &                     &    (0.6606)         &                     &    (2.3410)         \\
[1em]
White $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
White $\times$ outcome=1&                     &     -0.6229\sym{***}&                     &     -0.7339         &                     &     -0.6232         &                     &     -0.7866         &                     &      1.9871         \\
                    &                     &    (0.2211)         &                     &    (1.4176)         &                     &    (1.2987)         &                     &    (0.5817)         &                     &    (1.8895)         \\
[1em]
Constant            &     -1.2715\sym{***}&     -1.3509\sym{***}&      8.6990\sym{***}&      8.4212\sym{***}&      5.8243\sym{***}&      5.6623\sym{***}&     -0.9122\sym{***}&     -0.9730\sym{***}&     -5.5917\sym{***}&     -5.5428\sym{***}\\
                    &    (0.0751)         &    (0.0799)         &    (0.6865)         &    (1.1607)         &    (0.6034)         &    (0.7103)         &    (0.1439)         &    (0.1473)         &    (0.2274)         &    (0.2257)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &1106279.0000         &1106279.0000         & 157669.0000         & 157669.0000         & 173309.0000         & 173309.0000         & 506195.0000         & 506195.0000         & 269106.0000         & 269106.0000         \\
$R^2$               &      0.3872         &      0.3872         &      0.8246         &      0.8247         &      0.8261         &      0.8262         &      0.5922         &      0.5922         &      0.6802         &      0.6803         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Regressions/vulnerable_hmda_young.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                    &\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}&\multicolumn{1}{c}{PP\_CS\_decile}\\
\hline
young=0             &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
young=1             &      2.0619\sym{***}&      1.9822\sym{***}&      2.0509\sym{***}&      3.3843\sym{***}&      0.6596\sym{**} &      0.1533         &      0.4605\sym{***}&      0.1092         &     -0.9414\sym{***}&     -1.0615\sym{***}\\
                    &    (0.0414)         &    (0.0464)         &    (0.2669)         &    (0.5226)         &    (0.2704)         &    (0.3251)         &    (0.0787)         &    (0.0813)         &    (0.2463)         &    (0.2481)         \\
[1em]
outcome=0           &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
outcome=1           &     -2.8483\sym{***}&     -2.9213\sym{***}&     -8.2401\sym{***}&     -7.7044\sym{***}&     -8.8832\sym{***}&     -9.2217\sym{***}&     -8.2884\sym{***}&     -9.0272\sym{***}&     -6.8356\sym{***}&     -7.0702\sym{***}\\
                    &    (0.0435)         &    (0.0494)         &    (0.2728)         &    (0.3175)         &    (0.2466)         &    (0.2830)         &    (0.1231)         &    (0.1393)         &    (0.4659)         &    (0.4815)         \\
[1em]
young=0 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
young=0 $\times$ outcome=1&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
young=1 $\times$ outcome=0&                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         &                     &      0.0000         \\
                    &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         &                     &         (.)         \\
[1em]
young=1 $\times$ outcome=1&                     &      0.3529\sym{***}&                     &     -1.8424\sym{***}&                     &      1.4430\sym{***}&                     &      3.7136\sym{***}&                     &      4.6188\sym{***}\\
                    &                     &    (0.0981)         &                     &    (0.5959)         &                     &    (0.5566)         &                     &    (0.2872)         &                     &    (1.7664)         \\
[1em]
Constant            &     -1.5144\sym{***}&     -1.4983\sym{***}&      7.2586\sym{***}&      6.8374\sym{***}&      4.2642\sym{***}&      4.4064\sym{***}&     -1.1230\sym{***}&     -1.0298\sym{***}&     -4.7206\sym{***}&     -4.7142\sym{***}\\
                    &    (0.0133)         &    (0.0142)         &    (0.2210)         &    (0.2579)         &    (0.1202)         &    (0.1320)         &    (0.0259)         &    (0.0267)         &    (0.0184)         &    (0.0185)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &1106279.0000         &1106279.0000         & 157669.0000         & 157669.0000         & 173309.0000         & 173309.0000         & 506195.0000         & 506195.0000         & 269106.0000         & 269106.0000         \\
$R^2$               &      0.3902         &      0.3902         &      0.8258         &      0.8260         &      0.8255         &      0.8256         &      0.5916         &      0.5923         &      0.6802         &      0.6803         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize }\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Sections/conflict.tex <==
\section*{Conflict-of-Interest Disclosure Statement}
\thispagestyle{empty}

\bsk


\bsk



\bsk



\noindent
\textbf{Stefania Albanesi} \\
I have nothing to disclose.






\bsk


\bsk



\bsk


\bsk


\bsk


\bsk


\bsk



\bsk


\bsk






\bsk


\bsk



\noindent
\textbf{Domonkos F. Vamossy} \\
I have nothing to disclose.


==> Sections/misclassification.tex <==
\section{Costs of Risk Profile Misclassification}\label{sec:value_added_consumers}

In Section \ref{sec:credit_score}, we showed that the credit score's lower statistical performance leads to risk profile misclassification for a large fraction of consumers, concentrated primarily at the low end of the credit score distribution. What are the costs of such risk profile misclassification? We provide an initial answer to this question by analyzing how access to credit and interest rates vary as a function of credit scores for credit cards and mortgages, the most common types of consumer loans. Our data only contains information on credit limits, balances, inquiries and originations, so we derive interest rates from independent sources.

The purpose of this exercise is  to quantify how, given current lending conditions,  access to credit and borrowing costs would change for consumers whose credit score risk profile differs from the one predicted by our model. Changing the reference credit score and its performance properties would presumably elicit equilibrium changes in lending conditions in equilibrium, and we abstract from this possible effect. However, our analysis is still informative to assess how much being placed in the wrong risk profile can affect borrowers within the current system. 

%{\red credit cards: interest rates, credit limits, mortgages: interest rates and credit limits; inquiries vs originations}


\subsection{Access to Credit}

We begin with access to credit. Table \ref{tab:misclass_desc} in Appendix \ref{app:costs}
reports summary statistics on indicators of credit demand and supply by credit score risk profile for the period 2006Q1-2016Q2. We report the dollar values as well as the ratio to household income on average for each credit score risk profile. %{\red need cutoffs for prime low and mid}
Credit limits on credit cards vary from \$7,032 on average for Deep Subprime borrowers to \$44,711 for  Superprime borrowers. Mortgage balances average to \$ 172,753 for Subprime borrowers, rising to \$ 208,992 for Prime borrowers. Additionally, though demand for credit, as approximated by inquiries, is decreasing in credit score, success at obtaining credit increases with credit score. For example. only 6.1\% of Subprime borrowers who place a credit inquiry originate a new credit card account, while 13.6\% of Prime borrowers do.  The corresponding values for mortgages are 3.9\% and 10.6\%.

These values are population averages and are also influenced by variation in characteristics, such as age and place of residence within a given credit score profile. To control for these factors, we estimate a regression of various credit demand and credit supply outcomes, where the main explanatory variable is the credit score risk profile, and we control for age, zip code fixed effects and quarter time effects interacted with an indicator for the credit score risk profile. The details of the regression specification and the full estimation results are reported in Appendix \ref{app:costs}. Table \ref{tab:crr_reg_summary} reports the average age-adjusted credit score risk profile effects for the entire sample period, estimated from these regression. Only 38\% of Subprime borrowers have a credit card, whereas 80\% of prime borrowers do. This despite the fact that 11\% of Subprime borrowers show a credit card inquiry in the previous quarter, whereas 8\% of Prime borrowers do. Only 17\% of Subprime borrowers who placed a credit card inquiry at quarter $t$ or $t-1$ display a credit card origination at $t$, while 34\% of Prime borrowers do. Additionally, average credit card balances for Subprime borrowers are \$38,150, while they are \$79,580 for Prime borrowers. These values vary monotonically across risk profiles, and suggest that though demand for credit card borrowing is higher for lower credit score borrowers, their access to credit card lending is severely restricted compared to borrowers in more favorable risk profiles.

The pattern is  similar for mortgages. Only 28\% of Subprime borrowers have a mortgage, while 66\% of Prime borrowers do. Additionally, only 5\% of Subprime borrowers submit a mortgage inquiry in a quarter, and only 3\% of them show a mortgage origination in the same or subsequent quarters. By contrast, 6\% of Prime borrowers submit a mortgage inquiry in a quarter, and 9\% of them show an origination. Consequently, average mortgage balances for Subprime borrowers are \$66,420, while they are \$28,330 for Subprime borrowers. The variation in these statistics is monotone in the risk profile.

Figure \ref{fig:ccr_te} in Appendix \ref{app:costs} displays the quarter effects interacted with the risk profiles. The time variation is interesting, as after the Great Recession, there was a tightening of standards for consumer loans, particularly mortgages. The figure shows that that gap in access to credit card and mortgage credit between borrowers at the bottom and at the top of the credit score distribution widened substantially from 2009 to 2016.

This analysis suggests that borrowers in non-Prime credit score risk profiles who should have a more favorable ranking, as suggested by our model, would have faced substantial restrictions in accessing credit card and mortgage loans. On the other hand, borrowers with Prime and Superprime scores whose default probabilities are consistent with a worse risk rating based on our model, borrowed excessively, based on current industry standards, potentially exposing their lenders to unexpected losses.

\input{Tables/credit_risk_reg_l1_summary}


%%\input{Tables/misclassification_desc}
%
%
%To examine how access to mortgage credit varies by credit score risk profile, we look at mortgage originations and inquiries. Specifically, for each quarter $t$ in our sample, we calculate the fraction of individuals who registered a new mortgage inquiry between $t-2$ and $t-1$ or secured a new mortgage origination between $t-1$ and $t$. We group borrowers by their ranking in the credit score distribution at $t-1$. Panel B of Table \ref{tab:misclass_desc}  presents the results. % then average the percentage of new originations and inquiries across credit scores and our model rankings, based on their standings from the previous quarter. 
%
%
%The first row of the table presents the average fraction of consumers that originated a mortgage for each credit score risk profile, 0.5\% for the Deep Subprime group  and 2.1\% for the Superprime group. The second row reports the fraction of consumers with new mortgage inquiries, which ranges from 4.1\% for the Superprime category to 6.9\% for the Near Prime category. The most important statistic is the fraction of consumer with a mortgage inquiry that originate a mortgage. This is only 2.3\% in the Deep Subprime group and increases with the credit score from 3.9\% for Subprime, to 7.6\% for Near Prime, to 13.4\% for Superprime borrowers.
%
%These results suggest that borrowers in the Non-Prime group are significantly less successful at obtaining a mortgage, and that some of them may be discouraged from applying. As with credit cards, being placed in the wrong risk category entails less access to mortgage credit, a cost for the borrowers. Conversely,  borrowers who are placed by the credit score in a risk category that is too favorable given their default risk may generate a cost for the lenders.


%\input{Tables/credit_risk_differences}



\subsection{Interest Costs}\label{sec:int_cost}



We now examine the monetary implications for consumers who are misclassified into an incorrect risk profile by the credit score. Specifically, we calculate the differences in interest rate costs  they would face based on a risk profile predicted by our model compared to the credit score, given  that since the introduction of credit scores, interest rates on consumer credit products vary substantially by credit score (\citeN{edelberg2006risk}).

\paragraph{Credit Cards}
Our source for interest rates on credit cards by risk profile is Table 1 in \citeN{Stroebel_2015}, based on the account level Credit Card Metrics data set assembled by the Office of the Controller of the Currency.\footnote{The data covers all credit card accounts for the 8 largest U.S. banks for  January 2008 to December 2014. This time period is a subsample of our overall analysis. We use these interest rates for our entire sample period, as credit card interest rates are mostly invariant to the costs of funds for issuers (\citeN{ausubel1991failure} and \citeN{calem1995consumer}). Appendix \ref{app:int_costs} provides some evidence in support of the stability of credit card interest rates over our sample period.} Restricting attention to consumers with a positive credit card balances, we calculate  total balances across all cards and apply these interest rates to estimate their annualized interest rate costs based on their credit score and based on their model based ranking.

Disparities between consumers' credit score ranking and our model's ranking generate differences in interest rate costs. For customers placed in higher risk categories by the credit score compared to our prediction, interest rates on credit cards are higher than they would have been if they had been classified according to our model. Thus, using our model to score consumers rather than the credit score would generate cost savings for them. For customers placed in credit score risk categories that are too low relative to the default risk predicted by our model, interest rates will be higher.  We calculate the average differences in interest rate costs for each credit score category. The results are reported in Table \ref{tab:value_consumer_savings}, where the columns correspond to credit score based risk profiles and the rows to model based risk profiles. 

%\input{Tables/misclassification_cc_cost}


\input{Tables/misclassification_cc_cost_working_version}


The most significant gains accrue to customers with non-Prime credit scores, who as shown in Section \ref{sec:credit_score},  are more likely to be attributed a more favorable risk profile by our model. Additionally, the most considerable variation in credit card interest rates occurs between non-Prime  and Prime borrowers based on \citeN{Stroebel_2015}. The annual cost savings for these borrowers ranges from \$1,127 to \$1,854, given their average balances. Our model's gains for Prime and Superprime borrowers attributed to a lower default probability are more modest, as credit card interest rates vary less with credit score for Prime and Superprime borrowers. On the other hand, Prime and Superprime credit score borrowers placed by our model in the non-Prime risk category, would face higher interest rate costs of up to \$560 per year.

%{\red RECHECK  The resulting aggregate change in interest rate costs  associated with ranking consumers based on our model instead of the credit score is \$47,214,668, averaging \$2.7 per person per year, as calculated using weights from Table \ref{tab:risk_comp}. The primary cause of the positive per capita losses is the incorrect categorization of individuals with high debt into less advantageous credit categories. The most substantial benefits are seen among non-prime borrowers, who make up less than 40\% of our sample and generally have lower balances. This implies that though individual borrowers who are placed in a worst risk category than their probability of default would imply would face lower interest costs. However, in the aggregate, scoring consumers based on our model would benefit credit card lenders, who would collect higher interest payments.}

These calculations provides us with a lower bound for the individual interest rate cost savings on credit cards for consumers ranked in a lower risk category by our model than the credit score, as they do not take into account potential behavioral responses of misclassified consumers faced with different borrowing limits and interest rates. Fees for missed payments constitute a substantial component of credit card costs for consumers, and the ability to avoid these fees would contribute to substantial cost savings for consumers (see \citeN{agarwal2014regulating}). As shown in \citeN{Stroebel_2015}, decreases in the cost of funds for lenders mainly translate into increases in credit limits exclusively for higher credit score borrowers. Therefore, being placed in a higher risk category for consumers also inhibits their ability to benefit from expansionary monetary policy. On the other hand, the higher interest rates for consumers ranked worse by our model than the credit scores would imply additional revenues for credit card lenders. This does not capture all the potential gains for lenders for this group of customers, however. Borrowers that are ranked in a worst risk category by our model compared to the credit score would face lower credit limits, which would shield lenders from losses in the case of default.

\paragraph{Mortgages}

We now examine the variation of interest rate costs for mortgages. To obtain interest rate data, we use the Freddie Mac Single Family Loan-Level Dataset, which  only includes conforming mortgages for single family homes, with credit score based on the FICO 2 model.
We further refine the sample to include only fixed-rate 30-year mortgages for primary residences.
To quantify the potential interest rate cost differences for consumers when ranked based on our model rather than the credit score, we match the Experian data with the Freddie Mac data  based on the quarter, mortgage origination balance range, and credit risk percentiles at the origination quarter. We consider only borrowers with a single, recently-acquired first mortgage in the Experian data, to ensure that the interest rate we analyze is specifically tied to this new mortgage. 

The details of our sample selection are described in Appendix \ref{app:mortgages}, and the summary statistics are reported in Panel A of Table \ref{tab:freddie_desc_stats}. 
We first translate the credit score risk profiles and our model-predicted risk profiles into percentiles of the corresponding distributions. The resulting interest rates by credit score percentiles and origination balances are presented in  Panel B of Table \ref{tab:freddie_desc_stats}. Figure \ref{fig:origination_credit_score_interest_rate} in Appendix \ref{app:int_costs} displays average interest rates by  credit score percentile group.

We also calculate the interest rate `spread`, which is the difference between the interest rate predicted by the traditional credit score and the one predicted by our model using interest rate obtained from Freddie Mac for  standard 30-year fixed mortgages. A higher spread indicates that the traditional credit score would have projected a higher interest rate than our model. Based on these interest rates, we  estimate the  monthly payment for borrowers by risk category. We then compute the difference between the monthly payments implied by the borrowers' credit score and their ranking based on our model.  The results are reported in Table \ref{tab:value_consumer_savings_mortgage}. 

%\input{Tables/misclassification_mtg_cost}

%\input{Tables/misclassification_mtg_cost_working_version}

\input{Tables/misclassification_mtg_cost_working_version_v2}

The results suggest that borrowers with a non-Prime credit score who would be placed in better risk categories by our model would face mortgage rates from 15 to 24 basis points lower. This translates into annual mortgage payments that range from \$249 to \$454 lower. These values amount to  cumulated savings of \$7200-13,680 over 30 years of  mortgage duration, or 4.98-6.24\% of mortgage balances.

Borrowers with Prime credit scores with better model-based risk profile would also experience lower interest rates and savings on monthly payments, both in dollar terms and in percentage of income. For example, Prime Low borrowers who should be in the Prime High/Superprime  risk profile based on our model would reduce their interest rates by 10 basis points, their annual payment by \$198, cumulating to 1.7\% of mortgage balances. These savings are smaller than for borrowers in the non-Prime category, as mortgage rates vary less across Prime credit scores than they do between non-Prime and Prime credit scores.
Borrowers with Prime credit scores who  fall in worse model-based risk categories would face higher interest rates and payments. For example, Prime Low borrowers with a non-Prime model-based risk profile would face interest rates that are higher by 16 basis points, increasing their annual payments by \$217, cumulating to 4\% of total balances over the duration of the mortgage .

%{\red AGGREGATE CALCULATION, BENEFITS FOR LENDERS}

To summarize, for both credit cards and mortgages, credit score misclassification into an incorrect risk category has implications for both access to credit and the cost of credit. These implications are largest for borrowers with a non-Prime credit score who would be ranked higher based on our model.




==> Tables/credit_risk_reg_updated.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Access to Credit by Risk Profile \label{tab:crr_reg}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{8}{p{0.7in}}}
\hline\hline
& \multicolumn{4}{c}{Credit Cards} & \multicolumn{4}{c}{Mortgages} \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    & \multicolumn{1}{c}{Any Credit } & \multicolumn{1}{c}{Credit}\multicolumn{1}{c}{Inquiries}&\multicolumn{1}{c}{Originations if} & \multicolumn{1}{c}{Any First Mortgage} & \multicolumn{1}{c}{First Mortgage} & \multicolumn{1}{c}{Inquiries}&\multicolumn{1}{c}{Originations if}  \\
                   &\multicolumn{1}{c}{Limit} &\multicolumn{1}{c}{Limit}  &\multicolumn{1}{c}{} &\multicolumn{1}{c}{Inquired}   &\multicolumn{1}{c}{Balances} &\multicolumn{1}{c}{Balances}   &\multicolumn{1}{c}{} &\multicolumn{1}{c}{Inquired}     \\
\hline
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime        &      -0.092\sym{***}&   -7917.347\sym{***}&       0.037\sym{***}&      -0.011\sym{**} &       0.012\sym{***}&   20126.692\sym{***}&       0.033\sym{***}&      -0.031\sym{***}\\
                    &     (0.001)         &   (130.652)         &     (0.001)         &     (0.005)         &     (0.002)         &   (494.724)         &     (0.001)         &     (0.005)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Near Prime       &      -0.176\sym{***}&  -14383.424\sym{***}&       0.115\sym{***}&      -0.047\sym{***}&      -0.043\sym{***}&    9405.433\sym{***}&       0.073\sym{***}&      -0.055\sym{***}\\
                    &     (0.002)         &   (173.008)         &     (0.001)         &     (0.006)         &     (0.002)         &   (646.995)         &     (0.001)         &     (0.005)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Subprime      &      -0.481\sym{***}&  -28332.291\sym{***}&       0.143\sym{***}&      -0.189\sym{***}&      -0.189\sym{***}&  -18646.570\sym{***}&       0.050\sym{***}&      -0.093\sym{***}\\
                    &     (0.002)         &   (121.641)         &     (0.001)         &     (0.005)         &     (0.002)         &   (420.904)         &     (0.001)         &     (0.005)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime        &      -0.598\sym{***}&  -31015.469\sym{***}&       0.183\sym{***}&      -0.282\sym{***}&      -0.237\sym{***}&  -24759.575\sym{***}&       0.040\sym{***}&      -0.120\sym{***}\\
                    &     (0.003)         &   (127.105)         &     (0.003)         &     (0.005)         &     (0.002)         &   (505.414)         &     (0.002)         &     (0.005)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
30-39               &       0.068\sym{***}&    9685.490\sym{***}&       0.008\sym{***}&      -0.001         &       0.215\sym{***}&   48881.809\sym{***}&       0.037\sym{***}&      -0.002\sym{***}\\
                    &     (0.001)         &    (70.860)         &     (0.000)         &     (0.001)         &     (0.001)         &   (417.223)         &     (0.000)         &     (0.001)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
40-49               &       0.081\sym{***}&   15675.728\sym{***}&       0.002\sym{***}&      -0.005\sym{***}&       0.291\sym{***}&   65633.694\sym{***}&       0.032\sym{***}&      -0.009\sym{***}\\
                    &     (0.001)         &   (108.016)         &     (0.000)         &     (0.001)         &     (0.001)         &   (608.152)         &     (0.000)         &     (0.001)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
50-59               &       0.082\sym{***}&   18744.131\sym{***}&      -0.009\sym{***}&      -0.012\sym{***}&       0.269\sym{***}&   53565.830\sym{***}&       0.019\sym{***}&      -0.013\sym{***}\\
                    &     (0.001)         &   (123.438)         &     (0.000)         &     (0.001)         &     (0.001)         &   (601.340)         &     (0.000)         &     (0.001)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
60-69               &       0.061\sym{***}&   17673.841\sym{***}&      -0.021\sym{***}&      -0.013\sym{***}&       0.166\sym{***}&   32022.654\sym{***}&       0.006\sym{***}&      -0.018\sym{***}\\
                    &     (0.001)         &   (134.698)         &     (0.000)         &     (0.001)         &     (0.001)         &   (541.962)         &     (0.000)         &     (0.001)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
70+                 &      -0.002         &    7636.702\sym{***}&      -0.042\sym{***}&      -0.021\sym{***}&      -0.008\sym{***}&     -30.810         &      -0.015\sym{***}&      -0.033\sym{***}\\
                    &     (0.001)         &   (123.213)         &     (0.000)         &     (0.001)         &     (0.001)         &   (404.867)         &     (0.000)         &     (0.001)         \\
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &       0.870\sym{***}&   26760.235\sym{***}&       0.057\sym{***}&       0.353\sym{***}&       0.183\sym{***}&   11335.228\sym{***}&       0.014\sym{***}&       0.159\sym{***}\\
                    &     (0.001)         &   (127.299)         &     (0.001)         &     (0.005)         &     (0.001)         &   (526.828)         &     (0.001)         &     (0.004)         \\
\hline
& & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &26,147,712       &26,147,712       &26,147,712       & 3,761,219    &26,147,712       &26,147,712       &26,147,712       & 2,235,063        \\
$R^2$               &       0.313         &       0.252         &       0.030         &       0.071         &       0.178         &       0.124         &       0.021         &       0.030       \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports estimated for equation \ref{reg:access_spec} for credit cards (columns 1 to 4), and mortgages (columns 5 to 8). Column (1) is credit limits for credit cards, while Column (5) is first mortgage balances for mortgages. Column (4) and (8) restrict the sample to individuals who inquired in the current or previous quarter and estimates the coefficients for origination. Credit risk profiles based on previous quarter. Standard errors are clustered by ZIP code.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/feature_attribution_vulnerable.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Feature Attribution Differences by Protected Group Status}\label{tab:feature_protected}
\footnotesize
\begin{tabular}[c]{p{1.5in}p{0.75in}p{0.75in}p{0.75in}p{0.75in}p{0.75in}p{0.75in}}
& & & & & &\\
 & \multicolumn{6}{c}{\underline{Group Status}} \\ 
Feature Group  & Age $\le$ 30 & Age $>$ 30 & Income $\le$ p20 & Income $>$ p20 & Minority & Non-Minority   \\ \hline
& & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Payment History  & 0.3357 & 0.3379 & 0.3342 & 0.3380 & 0.3367 & 0.3375 \\
Amounts Owed  & 0.4895 & 0.4889 & 0.4904 & 0.4887 & 0.4893 & 0.4890 \\
Length of Credit History  & 0.0753 & 0.0754 & 0.0755 & 0.0754 & 0.0753 & 0.0754 \\
Credit Mix  & 0.0458 & 0.0450 & 0.0459 & 0.0450 & 0.0453 & 0.0452 \\
New Credit  & 0.0536 & 0.0529 & 0.0539 & 0.0529 & 0.0533 & 0.0530 \\
\hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: SHAP values for five feature groups by protected group status. For each prediction window, we compute the SHAP value for 100,000 randomly sampled observations and for each feature. We then calculate the sum of the absolute value for each feature, aggregate it across the feature groups, and report the results for the group. We normalized the results so that for each model the five groups sum up to 1. Feature groups are defined in Table \ref{tab:features} in Appendix \ref{app:model_details}. Source: Authors' calculations based on Experian data.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/feature_groups.tex <==
\begin{table}[htbp]\centering
\footnotesize
\begin{threeparttable}
\caption{Feature Groups}\label{tab:feature_corr} 
\begin{tabular}{p{3in}p{3in}} \hline 
& \\
\underline{Total debt balances*} & \underline{Monthly pmt on mortgage debt*} \\
Total debt balances & Monthly pmt on joint mortgage trades \\
Credit amt on open trades & Monthly pmt on first mortgage trades \\
 &  \\
\underline{Balance on revolving debt*} & \underline{Monthly pmt on debt*} \\
Credit amt on HELOC trades & Monthly pmt on debt \\
Balance on HELOC trades & Monthly pmt on joint install. trades \\
Credit amt on revolving trades &  \\
 & \underline{Balance on 90-180 days late install. loans*} \\
\underline{Balance on auto loans*} & Amt past due on install. trades 90+ dpd \\
Balance on open auto loan trades & Balance on install. trades 90+ dpd \\
No. of auto loan trades &  \\
 & \underline{Fraction of 90+ days delinquent debt*} \\
\underline{No. of credit cards*} & Fraction of 90+ days delinquent debt \\
Credit amt on open credit card trades & Worst current status on an open trade \\
No. of credit \& bankcards &  \\
 & \underline{90 days late credit card debt*} \\
\underline{Balance on collections*} & Amt past due on credit card trades 90+ dpd \\
Balance on collections & Balance on bankcard revolving 90+ dpd \\
Balance on collections, last 24 m &  \\
 & \underline{Mo. since recent 30-180days delinquency*} \\
\underline{No. of collections*} & Mo. since recent 30-180 days delinquency on credit card \\
No. of collections & Mo. since recent 30-180 days delinquency \\
Unsatisfied collections &  \\
 &  \underline{Mortgage debt*}\\
\underline{No. of bankruptcies*} & Mortgage to total debt \\
Public record bankruptcies &  No. of open mortgage trades\\
Public record discharged bankruptcies &   Mo. since recently opened first mortgage\\
 & Mo. since recent closed/refinanced first mortgage \\
\underline{Worst status on credit card trades*} &  \\
Worst current status on a trade excl. collections & \underline{Worst status on any trades*} \\
Worst current status on a credit card &  Worst current status on a trade\\
 &  Worst ever status on a trade in last 24 m\\
 \hline  \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: Amt=Amount, pmt=Payment, dpd=Days past due, install.=Installment, HELOC=Home equity line of credit, Mo.=Months, m=Months, No.=Number.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/freddie_sum_stats.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Freddie Mac Single Family Loan-Level Data}\label{tab:freddie_desc_stats}
\footnotesize
\begin{tabular}{l*{8}{c}}
\multicolumn{6}{l}{\textbf{Panel A: Descriptive Statistics}} \\ \hline 
Variable & Mean & Std. Dev. & Min &  25\% & 50\% & 75\% & Max   \\ \hline 
&&&&&&& \\[\dimexpr-\normalbaselineskip+2pt]
Credit Score & 750.254 & 44.734 & 620 & 720 & 760 & 787 & 850 \\
Credit Score Percentile & 63.781 & 18.685 & 27 & 53 & 67 & 77 & 100 \\
Original Payment Balance & 221,453.162 & 114,718.231 & 8,000 & 133,000 & 200,000 & 293,000 & 1,403,000 \\
Interest Rate & 4.939 & 1.034 & 2.49 & 4.125 & 4.625 & 5.875 & 9.875 \\
First Time Homebuyer & 0.366 & 0.482 & 0 & 0 & 0 & 1 & 1 \\
Combined Loan-to-Value (CLTV) & 81.528 & 14.248 & 6 & 80 & 80 & 95 & 200 \\
Debt-to-Income & 34.989 & 10.316 & 1 & 28 & 35 & 42 & 65 \\
Loan-to-Value (LTV) & 79.956 & 14.032 & 6 & 78 & 80 & 90 & 105 \\ \hline  
Observations & 3,884,908 & & & & & & \\ \hline \hline 
\end{tabular}
\begin{tabular}{l*{5}{c}}
\multicolumn{6}{l}{\textbf{Panel B: Interest Rate (\%) by Credit Score and Original Payment Balance}} \\ \hline 
&&&&& \\[\dimexpr-\normalbaselineskip+2pt]
& \multicolumn{5}{c}{\textbf{Original Payment Balance}} \\ \cline{2-6}
&&&&& \\[\dimexpr-\normalbaselineskip+2pt]
\textbf{FICO2 Percentile Range} & $<$ \$100k & \$100-200k & \$200-300k & \$300k-400k & \$400k+ \\ \hline
&&&&& \\[\dimexpr-\normalbaselineskip+2pt]
22-26.99 & 6.073 & 5.984 & 5.886 & 5.759 & 5.499 \\
27-30.99 & 5.864 & 5.790 & 5.702 & 5.547 & 5.323 \\
31-35.99 & 5.691 & 5.620 & 5.471 & 5.332 & 5.147 \\
36-41.99 & 5.406 & 5.285 & 5.112 & 5.006 & 4.891 \\
42-46.99 & 5.302 & 5.160 & 4.978 & 4.891 & 4.790 \\
47-52.99 & 5.195 & 5.022 & 4.843 & 4.759 & 4.662 \\
53-58.99 & 5.147 & 4.964 & 4.775 & 4.685 & 4.617 \\
59-66.99 & 5.129 & 4.934 & 4.750 & 4.667 & 4.610 \\
67-76.99 & 5.085 & 4.874 & 4.696 & 4.621 & 4.583 \\
77-100 & 5.039 & 4.815 & 4.656 & 4.580 & 4.549 \\
\hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: Data sourced from the Freddie Mac Single Family Loan-Level Dataset. The sample has been refined based on the following criteria: properties classified as primary residences; credit scores within the valid range of 620 to 850 to ensure data consistency; loans designated for purchase; valid entries for original debt-to-income ratio, original combined loan-to-value (CLTV), and original loan-to-value; and a loan term fixed at 360 months, limiting the dataset to fixed-rate mortgages. Data spans 2006Q1 to 2016Q2.

\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/misclassification_cc_cost.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Credit Cards}\label{tab:value_consumer_savings}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.5in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
Non-Prime & 0.00 & -40.36 & -50.81 & -72.72 \\
Prime Low & 92.57 & 0.00 & -26.52 & -41.30 \\
Prime Mid & 145.12 & 50.11 & 0.00 & -24.22 \\
Prime High-Superprime & 122.22 & 88.92 & 35.08 & 0.00 \\
                         &                     &                     &        &        \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Income (\%)}} \\
Non-Prime & 0.00 & -0.05 & -0.06 & -0.08 \\
Prime Low & 0.10 & 0.00 & -0.03 & -0.04 \\
Prime Mid & 0.14 & 0.05 & 0.00 & -0.02 \\
Prime High-Superprime & 0.13 & 0.08 & 0.03 & 0.00 \\
                         &                     &                     &        &        \\
 \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Total Debt (\%)}} \\
Non-Prime & 0.00 & -0.18 & -0.28 & -0.35 \\
Prime Low & 0.23 & 0.00 & -0.13 & -0.23 \\
Prime Mid & 0.40 & 0.16 & 0.00 & -0.15 \\
Prime High-Superprime & 0.75 & 0.44 & 0.27 & 0.00 \\
 \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports consumers' average interest rate cost savings by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Non-Prime: credit score up to 659. Prime Low: credit score 660-700. Prime Mid: credit score 701-740. Prime High-Superprime: credit scores greater than 741. Rankings based on previous quarter. Interest rates by credit score from Table 1 \citeN{Stroebel_2015}.  Time period 2006Q2-2016Q2. Sample: 17,865,452 borrowers with non-zero credit card limit. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}



==> Tables/misclassification_cc_cost_vulnerable.tex <==
%\begin{sidewaystable}[htbp]\centering
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Credit Cards}\label{tab:value_consumer_savings}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\multicolumn{5}{l}{Panel A: Age $\le$ 30} \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
\text{Non-Prime} & 0.00 & -377.12 & -262.20 & -309.30 \\
\text{Prime Low} & 662.78 & 0.00 & 55.80 & 10.46 \\
\text{Prime Mid} & 475.69 & -81.51 & 0.00 & -29.72 \\
\text{Prime High-Superprime} & 428.53 & -21.19 & 46.76 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel B: Age $>$ 30} \\
\text{Non-Prime} & 0.00 & -890.49 & -551.56 & -595.69 \\
\text{Prime Low} & 2295.15 & 0.00 & 162.82 & 25.12 \\
\text{Prime Mid} & 1871.69 & -285.67 & 0.00 & -84.75 \\
\text{Prime High-Superprime} & 1367.75 & -55.03 & 127.64 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel C: Income $\le$ p20} \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
\text{Non-Prime} & 0.00 & -259.23 & -191.42 & -312.77 \\
\text{Prime Low} & 242.85 & 0.00 & 29.19 & 5.99 \\
\text{Prime Mid} & 191.39 & -27.44 & 0.00 & -14.72 \\
\text{Prime High-Superprime} & 294.41 & -9.45 & 14.25 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel D: Income $>$ p20} \\
\text{Non-Prime} & 0.00 & -861.73 & -522.61 & -567.42 \\
\text{Prime Low} & 2172.81 & 0.00 & 145.97 & 23.10 \\
\text{Prime Mid} & 1717.38 & -262.92 & 0.00 & -74.47 \\
\text{Prime High-Superprime} & 1329.23 & -51.36 & 113.90 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel E: Non-Minority} \\
\text{Non-Prime} & 0.00 & -795.96 & -501.61 & -574.15 \\
\text{Prime Low} & 1946.04 & 0.00 & 134.18 & 22.78 \\
\text{Prime Mid} & 1602.34 & -249.49 & 0.00 & -73.43 \\
\text{Prime High-Superprime} & 1199.13 & -50.68 & 113.23 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel F: Minority} \\
\text{Non-Prime} & 0.00 & -630.11 & -430.72 & -498.70 \\
\text{Prime Low} & 1361.10 & 0.00 & 112.67 & 20.15 \\
\text{Prime Mid} & 961.86 & -180.96 & 0.00 & -64.94 \\
\text{Prime High-Superprime} & 690.28 & -32.65 & 82.26 & 0.00 \\
 \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports consumers' average interest rate cost savings by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Non-Prime: credit score up to 659. Prime Low: credit score 660-700. Prime Mid: credit score 701-740. Prime High-Superprime: credit scores greater than 741. Rankings based on previous quarter. Interest rates by credit score from Table 1 \citeN{Stroebel_2015}.  Time period 2006Q2-2016Q2. Sample: 15,970,651 borrowers with non-zero credit card balances. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}

% Panel A: -34408235.07 or -11.62691767 per person
% Panel B: -140355870 or -10.78723626 per person
% Panel C: -28656717.57 or -16.43383738 per person
% Panel D: -146107387.5 or -10.26980655 per person
% Panel E: -107220888.9 or -7.914568319 per person
% Panel F: -67543216.18 or -27.87161847 per person





==> Tables/misclassification_cc_cost_working_version.tex <==
%\begin{sidewaystable}[htbp]\centering
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Credit Cards}\label{tab:value_consumer_savings}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
% \multicolumn{5}{c}{Panel A: Borrowers with Credit Limit} 
%    &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt]     
%\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
%\text{Non-Prime} & 0.00 & -698.3 & -446.8 & -507.2 \\
%\text{Prime Low} & 1691.8 & 0.00 & 118.8 & 20.3 \\
%\text{Prime Mid} & 1295.0 & -213.7 & 0.00 & -65.6 \\
%\text{Prime High-Superprime} & 885.8 & -39.6 & 88.4 & 0.00 \\
%                         &                     &                     &        &        \\
% \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Credit Card Balances (\%)}} \\
%\text{Non-Prime} & 0.00 & -5.13 & -4.28 & -4.93 \\
%\text{Prime Low} & 5.13 & 0.00 & 0.85 & 0.2 \\
%\text{Prime Mid} & 4.28 & -0.85 & 0.00 & -0.65 \\
%\text{Prime High-Superprime} & 4.93 & -0.2 & 0.65 & 0.00 \\
%
%                         &                     &                     &        &        \\
% \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Imputed Income (\%)}} \\
%\text{Non-Prime} & 0.00 & -0.92 & -0.56 & -0.55 \\
%\text{Prime Low} & 1.85 & 0.00 & 0.14 & 0.02 \\
%\text{Prime Mid} & 1.23 & -0.21 & 0.00 & -0.06 \\
%\text{Prime High-Superprime} & 0.91 & -0.04 & 0.08 & 0.00 \\
%
%  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
% \multicolumn{5}{c}{Panel B: Borrowers with Credit Card Balances} 
%    &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt]  
%\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Interest Rate Spread (\%)}} \\
%\text{Non-Prime} & 0.00 & -5.13 & -4.28 & -4.93 \\
%\text{Prime Low} & 5.13 & 0.00 & 0.85 & 0.20 \\
%\text{Prime Mid} & 4.28 & -0.85 & 0.00 & -0.65 \\
%\text{Prime High-Superprime} & 4.93 & -0.20 & 0.65 & 0.00 \\
%                        &                     &                     &        &        \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
\text{Non-Prime} & 0.00 & -762.53 & -487.55 & -559.78 \\
\text{Prime Low} & 1853.52 & 0.00 & 130.76 & 22.37 \\
\text{Prime Mid} & 1504.94 & -240.20 & 0.00 & -72.32 \\
\text{Prime High-Superprime} & 1126.87 & -48.50 & 109.52 & 0.00 \\
                         &                     &                     &        &        \\
 \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Credit Card Balances (\%)}} \\
\text{Non-Prime} & 0.00 & -5.13 & -4.28 & -4.93 \\
\text{Prime Low} & 5.13 & 0.00 & 0.85 & 0.20 \\
\text{Prime Mid} & 4.28 & -0.85 & 0.00 & -0.65 \\
\text{Prime High-Superprime} & 4.93 & -0.20 & 0.65 & 0.00 \\
                         &                     &                     &        &        \\
% \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Imputed Income (\%)}} \\
%\text{Non-Prime} & 0.00 & -1.01 & -0.62 & -0.61 \\
%\text{Prime Low} & 2.02 & 0.00 & 0.15 & 0.02 \\
%\text{Prime Mid} & 1.43 & -0.23 & 0.00 & -0.07 \\
%\text{Prime High-Superprime} & 1.16 & -0.04 & 0.10 & 0.00 \\
 \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports consumers' average interest rate cost savings by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Non-Prime: credit score up to 659. Prime Low: credit score 660-700. Prime Mid: credit score 701-740. Prime High-Superprime: credit scores greater than 741. Rankings based on previous quarter. Interest rates by credit score from Table 1 \citeN{Stroebel_2015}.  Time period 2006Q2-2016Q2. Sample: 17,865,452 borrowers with non-zero credit card limit; 15,970,651 with non-zero credit card balances. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}




==> Tables/misclassification_mtg_cost.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Mortgages}\label{tab:value_consumer_savings_mortgage}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.5in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Interest Rate Spread (\%)}} \\
Non-Prime & -0.041 & -0.117 & -0.151 & -0.167 \\
Prime Low & 0.076 & -0.002 & -0.047 & -0.067 \\
Prime Mid & 0.086 & 0.040 & 0.001 & -0.022 \\
Prime High-Superprime & 0.120 & 0.055 & 0.020 & -0.002 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Saving (\$)}} \\
Non-Prime & -4.118 & -13.037 & -17.703 & -23.797 \\
Prime Low & 10.840 & 0.386 & -5.646 & -9.708 \\
Prime Mid & 12.397 & 6.205 & 0.236 & -3.274 \\
Prime High-Superprime & 19.608 & 8.670 & 3.316 & -0.335 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Savings / Monthly Income (\%)}} \\
Non-Prime & -0.090 & -0.252 & -0.320 & -0.360 \\
Prime Low & 0.152 & -0.006 & -0.103 & -0.145 \\
Prime Mid & 0.191 & 0.084 & -0.005 & -0.048 \\
Prime High-Superprime & 0.446 & 0.143 & 0.038 & -0.004 \\
\hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the average monthly payment cost savings on mortgages and interest rate spread for consumers by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Interest rates are calibrated using Freddie Mac Single Loan Data.  Time period 2006Q2-2016Q2. Sample: 159,552 borrowers with only one first mortgage originated in the past 9 months. Rankings based on the previous quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


%NOTE: WE HAVE DEEP SUBPRIME SINCE THE FICO CUTOFF IS THE 22ND PERCENTILE. WE DO HAVE SUBPRIME BORROWERS BETWEEN 22ND AND 27TH PERCENTILE.

==> Tables/misclassification_mtg_cost_vulnerable.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Mortgages}\label{tab:value_consumer_savings_mortgage}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\multicolumn{5}{l}{Panel A: Age $\le$ 30} \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
\text{Non-Prime} & 0.00 & -193.76 & -317.96 & -439.05 \\
\text{Prime Low} & 193.06 & 0.00 & -96.11 & -154.62 \\
\text{Prime Mid} & 384.84 & 96.25 & 0.00 & -47.76 \\
\text{Prime High-Superprime} & 362.77 & 186.62 & 57.64 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel B: Age $>$ 30} \\
\text{Non-Prime} & 0.00 & -231.44 & -376.31 & -484.19 \\
\text{Prime Low} & 251.32 & 0.00 & -121.11 & -189.86 \\
\text{Prime Mid} & 396.94 & 130.40 & 0.00 & -58.37 \\
\text{Prime High-Superprime} & 471.07 & 217.86 & 75.68 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel C: Income $\le$ p20} \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
\text{Non-Prime} & 0.00 & -156.11 & -235.82 & -336.62 \\
\text{Prime Low} & 162.23 & 0.00 & -73.05 & -117.50 \\
\text{Prime Mid} & 262.12 & 64.59 & 0.00 & -35.37 \\
\text{Prime High-Superprime} & 431.39 & 134.61 & 38.61 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel D: Income $>$ p20} \\
\text{Non-Prime} & 0.00 & -231.27 & -373.75 & -481.07 \\
\text{Prime Low} & 247.51 & 0.00 & -118.06 & -184.72 \\
\text{Prime Mid} & 411.73 & 127.80 & 0.00 & -56.60 \\
\text{Prime High-Superprime} & 459.42 & 216.87 & 73.48 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel E: Non-Minority} \\
\text{Non-Prime} & 0.00 & -225.35 & -364.45 & -489.94 \\
\text{Prime Low} & 242.64 & 0.00 & -115.39 & -185.11 \\
\text{Prime Mid} & 406.46 & 126.63 & 0.00 & -56.24 \\
\text{Prime High-Superprime} & 456.12 & 214.42 & 73.02 & 0.00 \\
                         &                     &                     &        &        \\
\multicolumn{5}{l}{Panel F: Minority} \\
\text{Non-Prime} & 0.00 & -209.16 & -353.09 & -393.44 \\
\text{Prime Low} & 210.72 & 0.00 & -108.72 & -164.96 \\
\text{Prime Mid} & 316.05 & 106.71 & 0.00 & -55.28 \\
\text{Prime High-Superprime} & 451.59 & 205.66 & 69.01 & 0.00 \\
 \hline \hline 
\hline \hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the average monthly payment cost savings on mortgages and interest rate spread for consumers by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Interest rates are calibrated using Freddie Mac Single Family Loan Data.  Time period 2006Q2-2016Q2. Sample: 247,776 borrowers with only one first mortgage originated in the past 9 months. Rankings based on the previous quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}

% Panel A: -1934262 or -47.43 per person
% Panel B:  -7742813 or -37.41 per person
% Panel C: -419343 or -35.29 per person
% Panel D: -9257732 or -39.25 per person
% Panel E: -8416946 or -37.93 per person
% Panel F: -1260130 or -48.72 per person

==> Tables/misclassification_mtg_cost_working_version.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Mortgages}\label{tab:value_consumer_savings_mortgage}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.5in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Interest Rate Spread (\%)}} \\
\text{Non-Prime} & 0.000 & -0.157 & -0.247 & -0.275 \\
\text{Prime Low} & 0.163 & 0.000 & -0.076 & -0.109 \\
\text{Prime Mid} & 0.241 & 0.074 & 0.000 & -0.034 \\
\text{Prime High-Superprime} & 0.271 & 0.103 & 0.035 & 0.000 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Saving (\$)}} \\
\text{Non-Prime} & 0.000 & -18.088 & -28.843 & -37.708 \\
\text{Prime Low} & 20.713 & 0.000 & -9.442 & -14.939 \\
\text{Prime Mid} & 33.677 & 10.079 & 0.000 & -4.741 \\
\text{Prime High-Superprime} & 37.828 & 16.482 & 5.251 & 0.000 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Savings / Mortgage Balances (\%)}} \\
\text{Non-Prime} & 0.000 & -0.011 & -0.016 & -0.017 \\
\text{Prime Low} & 0.014 & 0.000 & -0.005 & -0.007 \\
\text{Prime Mid} & 0.015 & 0.005 & 0.000 & -0.003 \\
\text{Prime High-Superprime} & 0.017 & 0.007 & 0.002 & 0.000 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Savings / Monthly Income (\%)}} \\
\text{Non-Prime} & 0.000 & -0.346 & -0.517 & -0.573 \\
\text{Prime Low} & 0.352 & 0.000 & -0.160 & -0.221 \\
\text{Prime Mid} & 0.575 & 0.146 & 0.000 & -0.066 \\
\text{Prime High-Superprime} & 0.804 & 0.258 & 0.067 & 0.000 \\
\hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the average monthly payment cost savings on mortgages and interest rate spread for consumers by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Interest rates are calibrated using Freddie Mac Single Family Loan Data.  Time period 2006Q2-2016Q2. Sample: 159,552 borrowers with only one first mortgage originated in the past 9 months. Rankings based on the previous quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


%NOTE: WE HAVE DEEP SUBPRIME SINCE THE FICO CUTOFF IS THE 22ND PERCENTILE. WE DO HAVE SUBPRIME BORROWERS BETWEEN 22ND AND 27TH PERCENTILE.

==> Tables/misclassification_mtg_cost_working_version_v2.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification- Mortgages}\label{tab:value_consumer_savings_mortgage}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Non-Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Interest Rate Spread (\%)}} \\
\text{Non-Prime} & 0.00 & -0.158 & -0.251 & -0.282 \\
\text{Prime Low} & 0.146 & 0.00 & -0.076 & -0.109 \\
\text{Prime Mid} & 0.212 & 0.071 & 0.00 & -0.033 \\
\text{Prime High-Superprime} & 0.238 & 0.100 & 0.038 & 0.00 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Annual Cost Saving (\$)}} \\
\text{Non-Prime} & 0.00 & -222.79 & -362.81 & -477.79 \\
\text{Prime Low} & 238.60 & 0.00 & -114.61 & -182.72 \\
\text{Prime Mid} & 394.58 & 124.60 & 0.00 & -56.15 \\
\text{Prime High-Superprime} & 455.49 & 213.43 & 72.67 & 0.00 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Cumulated Cost Savings / Mortgage Balances (\%)}} \\
\text{Non-Prime} & 0.00 & -3.96 & -5.67 & -6.21 \\
\text{Prime Low} & 4.98 & 0.00& -1.68 & -2.55 \\
\text{Prime Mid} & 5.34 & 1.65 & 0.00 & -1.14 \\
\text{Prime High-Superprime} & 6.24 & 2.4 & 0.78 & 0.00 \\
                         &                     &                     &        &        \\
\hline \hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the average monthly payment cost savings on mortgages and interest rate spread for consumers by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Interest rates are calibrated using Freddie Mac Single Family Loan Data.  Time period 2006Q2-2016Q2. Sample: 247,776 borrowers with only one first mortgage originated in the past 9 months. Rankings based on the previous quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/new_credit.tex <==
\begin{sidewaystable}[htbp]
\begin{center}
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{New Credit \label{tab:new_credit}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}p{1.1in}*{10}{p{0.55in}}}
\hline\hline
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
\multicolumn{11}{l}{DV: Our Model Ranking - Credit Score Ranking}\\
\hline
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
New Mortgage      &     -4.6845\sym{***}&     -1.6591\sym{***}&                     &                     &                     &                     &                     &                     &                     &                     \\
                    &    (0.1371)         &    (0.1054)         &                     &                     &                     &                     &                     &                     &                     &                     \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
New First Mortgage &                     &                     &     -5.4561\sym{***}&     -2.1796\sym{***}&                     &                     &                     &                     &                     &                     \\
                    &                     &                     &    (0.1326)         &    (0.1155)         &                     &                     &                     &                     &                     &                     \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
New Cards         &                     &                     &                     &                     &     -7.8649\sym{***}&     -7.5024\sym{***}&                     &                     &                     &                     \\
                    &                     &                     &                     &                     &    (0.0706)         &    (0.0592)         &                     &                     &                     &                     \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
CC Inquiry          &                     &                     &                     &                     &                     &                     &     -7.4470\sym{***}&     -6.4609\sym{***}&                     &                     \\
                    &                     &                     &                     &                     &                     &                     &    (0.0634)         &    (0.0536)         &                     &                     \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Mortgage Inquiry  &                     &                     &                     &                     &                     &                     &                     &                     &     -7.4589\sym{***}&     -5.6067\sym{***}\\
&                     &                     &                     &                     &                     &                     &                     &                     &    (0.0962)         &    (0.0708)         \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Default           &                     &     -5.1337\sym{***}&                     &     -5.1537\sym{***}&                     &     -5.2457\sym{***}&                     &     -4.7114\sym{***}&                     &     -5.0500\sym{***}\\
                    &                     &    (0.0325)         &                     &    (0.0325)         &                     &    (0.0332)         &                     &    (0.0340)         &                     &    (0.0348)         \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Age                 &                     &     -0.3845\sym{***}&                     &     -0.4033\sym{***}&                     &     -0.3662\sym{***}&                     &     -0.3973\sym{***}&                     &     -0.3857\sym{***}\\
                    &                     &    (0.0055)         &                     &    (0.0057)         &                     &    (0.0055)         &                     &    (0.0056)         &                     &    (0.0055)         \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Age$^2$           &                     &      0.0038\sym{***}&                     &      0.0040\sym{***}&                     &      0.0036\sym{***}&                     &      0.0038\sym{***}&                     &      0.0038\sym{***}\\
                    &                     &    (0.0001)         &                     &    (0.0001)         &                     &    (0.0001)         &                     &    (0.0001)         &                     &    (0.0001)         \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Total Debt             &                     &     -0.0121\sym{***}&                     &     -0.0121\sym{***}&                     &     -0.0114\sym{***}&                     &     -0.0118\sym{***}&                     &     -0.0113\sym{***}\\
                    &                     &    (0.0007)         &                     &    (0.0007)         &                     &    (0.0007)         &                     &    (0.0007)         &                     &    (0.0007)         \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
90 DPD+ Debt             &                     &     -0.0064\sym{***}&                     &     -0.0063\sym{***}&                     &     -0.0081\sym{***}&                     &     -0.0068\sym{***}&                     &     -0.0059\sym{***}\\
                    &                     &    (0.0005)         &                     &    (0.0005)         &                     &    (0.0005)         &                     &    (0.0005)         &                     &    (0.0005)         \\
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Constant            &      0.0330\sym{***}&     10.4128\sym{***}&      0.0714\sym{***}&     10.8895\sym{***}&      0.8568\sym{***}&     10.8199\sym{***}&      0.6655\sym{***}&     11.3627\sym{***}&      0.4026\sym{***}&     10.7639\sym{***}\\
                    &    (0.0022)         &    (0.1419)         &    (0.0017)         &    (0.1466)         &    (0.0081)         &    (0.1460)         &    (0.0057)         &    (0.1473)         &    (0.0052)         &    (0.1449)         \\
 \hline
& & & & & & & & & &\\[\dimexpr-\normalbaselineskip+2pt]
Observations        &26,135,452        &26,135,452        &26,240,879        &26,240,879        &26,135,452        &26,135,452        &26,240,879        &26,240,879        &26,240,879        &26,240,879        \\
$R^2$               &      0.0033         &      0.0454         &      0.0034         &      0.0463         &      0.0271         &      0.0681         &      0.0200         &      0.0595         &      0.0134         &      0.0524         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes: This table reports regressions of the form specified by Equation (\ref{reg:spec}). The dependent variable is the percentile ranking difference between our model and the credit score. The independent variable, "Default", is a binary indicator showing whether the individual defaulted within the next two years. "New Mortgage", "New First Mortgage", "New Cards", are binary indicators for acquiring new mortgage, first mortgage, or credit/bank cards since the previous quarter. "CC Inquiry" and "Mortgage Inquiry" are binary indicators for having a credit card or mortgage inquiry in the present quarter. We control for State x Quarter fixed effects. Standard errors are clustered by state and quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{center}
\end{sidewaystable}


==> Tables/new_credit_inquiries.tex <==
\begin{sidewaystable}[htbp]
\begin{center}
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{New Credit, Inquired Borrowers \label{tab:new_credit}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}p{1.1in}*{6}{p{0.55in}}}
\hline\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\multicolumn{7}{l}{DV: Our Model Ranking - Credit Score Ranking}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
New Mortgage      &      1.5458\sym{***}&      1.3992\sym{***}&                     &                     &                     &                     \\
                    &    (0.0931)         &    (0.0716)         &                     &                     &                     &                     \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
New First Mortgage &                     &                     &      1.2029\sym{***}&      1.0407\sym{***}&                     &                     \\
                    &                     &                     &    (0.0946)         &    (0.0805)         &                     &                     \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
New Cards        &                     &                     &                     &                     &     -2.8707\sym{***}&     -2.8557\sym{***}\\
                    &                     &                     &                     &                     &    (0.0371)         &    (0.0339)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default          &                     &     -0.5889\sym{***}&                     &     -0.6095\sym{***}&                     &     -0.2033\sym{***}\\
                    &                     &    (0.0383)         &                     &    (0.0387)         &                     &    (0.0269)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Age                 &                     &     -0.0785\sym{***}&                     &     -0.0781\sym{***}&                     &     -0.1372\sym{***}\\
                    &                     &    (0.0055)         &                     &    (0.0056)         &                     &    (0.0074)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Age$^2$             &                     &      0.0008\sym{***}&                     &      0.0008\sym{***}&                     &      0.0009\sym{***}\\
                    &                     &    (0.0001)         &                     &    (0.0001)         &                     &    (0.0001)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Total Debt             &                     &      0.0005\sym{*}  &                     &      0.0006\sym{**} &                     &      0.0005         \\
                    &                     &    (0.0003)         &                     &    (0.0003)         &                     &    (0.0004)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
90+ DPD Debt             &                     &     -0.0042\sym{***}&                     &     -0.0042\sym{***}&                     &     -0.0063\sym{***}\\
                    &                     &    (0.0004)         &                     &    (0.0004)         &                     &    (0.0005)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &     -6.9512\sym{***}&     -5.1213\sym{***}&     -6.9084\sym{***}&     -5.0927\sym{***}&     -5.5502\sym{***}&     -1.5141\sym{***}\\
                    &    (0.0083)         &    (0.1388)         &    (0.0075)         &    (0.1385)         &    (0.0101)         &    (0.1875)         \\
 \hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &2,235,207       &2,235,207       &2,235,207       &2,235,207       &3,761,440       &3,761,440       \\
$R^2$               &      0.0441         &      0.0456         &      0.0435         &      0.0450         &      0.0338         &      0.0399         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes: This table reports regressions of the form specified by Equation (\ref{reg:spec}). The dependent variable is the percentile ranking difference between our model and the credit score. The independent variable, "Default", is a binary indicator showing whether the individual defaulted within the next two years. "New Mortgage", "New First Mortgage", "New Cards", are binary indicators for acquiring new mortgage, first mortgage, or credit/bank cards since the previous quarter. Sample restricted to mortgage (Column 1-4) and credit card (Columns 5-6) inquiries only in the previous or current quarter. We control for State x Quarter fixed effects. Standard errors are clustered by state and quarter. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{center}
\end{sidewaystable}


==> Tables/old/four_categories/cc_limit.tex <==

\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Credit Cards Limits by Credit Score Risk Profile}\label{tab:cc_limits}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2in}p{1in}p{1in}p{1.75in}}
 %  \multicolumn{4}{c}{Credit Score} \\ 
   \hline \hline
      &  &  &  \\
      Deep Subprime-Near Prime &  Prime Low & Prime Mid &  Prime High-Superprime \\  \hline
        &  &  &   \\[\dimexpr-\normalbaselineskip+3pt] 
      \multicolumn{4}{c}{\textbf{\% of Borrowers}} \\
    25.247 &  11.221&  13.962 &  49.570 \\ 
      &  &  &  \\
    \multicolumn{4}{c}{\textbf{Credit Limit (\$)}} \\
        20,848.5 & 30,638.8 & 32,058.6 & 40,982.3 \\
                             &                     &                     &              \\
    \multicolumn{4}{c}{\textbf{Credit Limit / Household Income (\%)}} \\
        28.4 & 36.1 & 35.8 & 37.4 \\
                             &                     &                     &              \\
    \multicolumn{4}{c}{\textbf{\% Originated}} \\
        18.0 & 20.2 & 17.8 & 14.1 \\
                             &                     &                     &              \\
    \multicolumn{4}{c}{\textbf{\% Inquired}} \\
        18.3 & 13.7 & 10.2 & 5.5 \\
 %                      &                     &                     &        &        \\
      &  &  &  \\  \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Average credit limits, dollars and as percentage of household income by credit score risk profile, 2006Q1-2016Q2. Credit score risk profiles defined in Table \ref{tab:risk_def}. Prime Low credit scores: 660-700. Prime Mid credit scores: 701-740. Prime High credit scores: greater than 741. Sample: 18,318,847 borrowers with non-zero credit card limit. Credit risk profile based on the current quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/old/four_categories/cc_reg.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\tiny
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Credit Risk Profile and Credit Cards \label{tab:cc_reg}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}p{1in}*{12}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}&\multicolumn{1}{c}{(12)}\\
                    &\multicolumn{3}{c}{Credit Card Limit}&\multicolumn{3}{c}{Credit Card Balances}&\multicolumn{3}{c}{Credit Card Origination}&\multicolumn{3}{c}{Credit Card Inquiry}\\
\hline
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low   &   9790.3\sym{***}&   5172.9\sym{***}&   -888.0\sym{***}&   1733.9\sym{***}&   -398.6\sym{***}&    741.1\sym{***}&      0.0221\sym{***}&      0.0250\sym{***}&      0.0396\sym{***}&     -0.0463\sym{***}&     -0.0448\sym{***}&     -0.0771\sym{***}\\
                    &   (88.1)         &   (75.3)         &  (207.1)         &   (65.4)         &   (61.1)         &  (159.8)         &    (0.0004)         &    (0.0004)         &    (0.0013)         &    (0.0004)         &    (0.0004)         &    (0.0013)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid    &  11210.1\sym{***}&   4561.9\sym{***}&   1328.2\sym{***}&  -2933.0\sym{***}&  -5998.1\sym{***}&   3563.9\sym{***}&     -0.0023\sym{***}&      0.0010\sym{**} &     -0.0356\sym{***}&     -0.0804\sym{***}&     -0.0798\sym{***}&     -0.1512\sym{***}\\
                    &   (99.1)         &   (88.8)         &  (225.5)         &   (70.9)         &   (72.8)         &  (163.1)         &    (0.0004)         &    (0.0004)         &    (0.0012)         &    (0.0004)         &    (0.0004)         &    (0.0012)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime    &  20133.8\sym{***}&   1397.5\sym{***}&  18701.2\sym{***}& -10422.7\sym{***}& -18743.6\sym{***}&  12116.4\sym{***}&     -0.0390\sym{***}&     -0.0283\sym{***}&     -0.0833\sym{***}&     -0.1274\sym{***}&     -0.1188\sym{***}&     -0.1907\sym{***}\\
                    &   (98.6)         &  (108.6)         &  (241.7)         &   (72.1)         &   (95.7)         &  (161.3)         &    (0.0003)         &    (0.0004)         &    (0.0010)         &    (0.0004)         &    (0.0004)         &    (0.0011)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Age                &                     &    198.0\sym{***}&    143.2\sym{***}&                     &     80.6\sym{***}&    118.6\sym{***}&                     &     -0.0004\sym{***}&     -0.0010\sym{***}&                     &     -0.0008\sym{***}&     -0.0017\sym{***}\\
                    &                     &    (2.6)         &    (4.1)         &                     &    (1.3)         &    (3.3)         &                     &    (0.0000)         &    (0.0000)         &                     &    (0.0000)         &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Imputed Income&                     &    310.7\sym{***}&    452.6\sym{***}&                     &    134.2\sym{***}&    363.4\sym{***}&                     &     -0.0001\sym{***}&     -0.0002\sym{***}&                     &      0.0001\sym{***}&     -0.0002\sym{***}\\
                    &                     &    (1.3)         &    (3.3)         &                     &    (0.8)         &    (2.8)         &                     &    (0.0000)         &    (0.0000)         &                     &    (0.0000)         &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low$\times$ Age&                     &                     &    117.7\sym{***}&                     &                     &     28.8\sym{***}&                     &                     &     -0.0002\sym{***}&                     &                     &      0.0005\sym{***}\\
                    &                     &                     &    (5.1)         &                     &                     &    (3.7)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid $\times$ Age&                     &                     &    153.7\sym{***}&                     &                     &     15.1\sym{***}&                     &                     &      0.0006\sym{***}&                     &                     &      0.0012\sym{***}\\
                    &                     &                     &    (5.5)         &                     &                     &    (3.7)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime $\times$ Age&                     &                     &    -18.7\sym{***}&                     &                     &   -154.8\sym{***}&                     &                     &      0.0009\sym{***}&                     &                     &      0.0012\sym{***}\\
                    &                     &                     &    (4.9)         &                     &                     &    (3.4)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low$\times$ Imputed Income&                     &                     &    -10.9\sym{***}&                     &                     &    -72.9\sym{***}&                     &                     &     -0.0000\sym{***}&                     &                     &      0.0002\sym{***}\\
                    &                     &                     &    (3.4)         &                     &                     &    (2.8)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid $\times$ Imputed Income&                     &                     &    -73.6\sym{***}&                     &                     &   -179.8\sym{***}&                     &                     &      0.0002\sym{***}&                     &                     &      0.0003\sym{***}\\
                    &                     &                     &    (3.6)         &                     &                     &    (2.8)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime $\times$ Imputed Income&                     &                     &   -202.6\sym{***}&                     &                     &   -307.3\sym{***}&                     &                     &      0.0002\sym{***}&                     &                     &      0.0002\sym{***}\\
                    &                     &                     &    (3.3)         &                     &                     &    (2.8)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &  20848.5\sym{***}&  -6170.6\sym{***}& -12707.0\sym{***}&  16798.0\sym{***}&   5517.3\sym{***}& -10309.2\sym{***}&      0.1799\sym{***}&      0.2020\sym{***}&      0.2320\sym{***}&      0.1829\sym{***}&      0.2120\sym{***}&      0.2615\sym{***}\\
                    &   (94.7)         &  (133.2)         &  (206.2)         &   (77.7)         &   (77.5)         &  (167.9)         &    (0.0003)         &    (0.0005)         &    (0.0008)         &    (0.0005)         &    (0.0005)         &    (0.0010)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&                    &           X         &           X         &                    &           X         &           X         &               &           X         &           X   & & X & X      \\
Observations        &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       &18,318,847       \\
$R^2$               &      0.0472         &      0.3240         &      0.3389         &      0.0592         &      0.2474         &      0.3404         &      0.0038         &      0.0853         &      0.0858         &      0.0309         &      0.1048         &      0.1058         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\tiny
\item Notes: This table reports regressions for credit risk profile and credit cards. Prime Low, Prime Mid, and Prime High-Superprime are indicator variables for the consumer belonging to that category. Columns (1, 4, 7, 10) do not include controls. Columns (2, 5, 8, 11) controls for age, income and ZIP x Quarter fixed effects. Columns (3, 6, 9, 12) also includes interactions between credit risk profile, age and income. Income in thousands. Standard errors are clustered by ZIP code. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/old/four_categories/mortgage_originations.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Cost of  Misclassification: Mortgage Originations}\label{tab:value_consumer_savings_mortgage_originations}
\small
%\begin{tabular}{ccccc}
\begin{tabular}[c]{p{1.275in}p{1.275in}p{1.275in}p{1.275in}}
  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{4}{c}{Credit Score Risk Profile} \\ \hline \hline
   Deep Subprime-Near Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
 \multicolumn{4}{c}{\textbf{\% Originated}} \\
 1.0 & 1.6 & 2.1 & 2.1 \\
 & &      &  \\
 \multicolumn{4}{c}{\textbf{\% Inquired}} \\
 5.6 & 5.5 & 6.5 & 4.8 \\
 & &      &  \\
 \multicolumn{4}{c}{\textbf{\% Originated (Borrowers with Inquiries)}} \\
 6.6 & 12.8 & 14.5 & 17.9 \\
\hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the fraction of borrowers with mortgage originations by credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles.  Time period 2006Q2-2016Q2. Sample: 25,559,345 borrowers; 1,373,816 borrowers with a mortgage inquiry; and 404,926 borrowers with a mortgage origination. Credit risk profile and inquiries based on the previous quarter. Source: Authors' calculations based on Experian Data. 
\end{tablenotes}
\end{threeparttable}
\end{table}






==> Tables/old/four_categories/mortgage_reg.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\tiny
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Credit Risk Profile and Mortgages \label{tab:mortgage_reg}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}p{1in}*{12}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}&\multicolumn{1}{c}{(12)}\\
                    &\multicolumn{3}{c}{Mortgage Credit Limit}&\multicolumn{3}{c}{Mortgage Balances}&\multicolumn{3}{c}{Mortgage Origination}&\multicolumn{3}{c}{Mortgage Inquiry}\\
\hline
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low   &  20483.6\sym{***}&  -4271.2\sym{***}& -11994.9\sym{***}&  18534.3\sym{***}&  -2969.6\sym{***}&  -8926.2\sym{***}&      0.0052\sym{***}&      0.0036\sym{***}&      0.0102\sym{***}&     -0.0008\sym{***}&     -0.0050\sym{***}&      0.0111\sym{***}\\
                    &  (282.3)         &  (281.8)         & (1064.1)         &  (255.3)         &  (251.6)         &  (846.9)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0006)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid     &  43861.5\sym{***}&   -180.1         & -12592.0\sym{***}&  39588.4\sym{***}&   1112.8\sym{***}&  -6963.7\sym{***}&      0.0103\sym{***}&      0.0072\sym{***}&      0.0146\sym{***}&      0.0095\sym{***}&     -0.0006\sym{**} &      0.0182\sym{***}\\
                    &  (423.2)         &  (403.7)         & (1242.5)         &  (386.0)         &  (360.3)         & (1045.8)         &    (0.0001)         &    (0.0001)         &    (0.0003)         &    (0.0003)         &    (0.0003)         &    (0.0007)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime   &  50563.5\sym{***}& -37987.8\sym{***}&  52855.6\sym{***}&  41161.5\sym{***}& -35514.1\sym{***}&  56873.3\sym{***}&      0.0050\sym{***}&     -0.0006\sym{***}&      0.0188\sym{***}&     -0.0082\sym{***}&     -0.0258\sym{***}&      0.0445\sym{***}\\
                    &  (490.3)         &  (710.2)         & (1174.6)         &  (438.7)         &  (662.6)         & (1029.7)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0002)         &    (0.0003)         &    (0.0006)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Age                  &                     &   -698.5\sym{***}&   -132.8\sym{***}&                     &   -651.7\sym{***}&   -131.9\sym{***}&                     &     -0.0001\sym{***}&      0.0000\sym{***}&                     &     -0.0005\sym{***}&     -0.0000         \\
                    &                     &    (9.2)         &   (12.3)         &                     &    (8.7)         &   (11.6)         &                     &    (0.0000)         &    (0.0000)         &                     &    (0.0000)         &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Imputed Income&                     &   1542.1\sym{***}&   1659.0\sym{***}&                     &   1332.4\sym{***}&   1511.6\sym{***}&                     &      0.0001\sym{***}&      0.0002\sym{***}&                     &      0.0004\sym{***}&      0.0006\sym{***}\\
                    &                     &   (14.4)         &   (23.2)         &                     &   (13.1)         &   (21.5)         &                     &    (0.0000)         &    (0.0000)         &                     &    (0.0000)         &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low$\times$ Age&                     &                     &   -516.4\sym{***}&                     &                     &   -492.4\sym{***}&                     &                     &     -0.0002\sym{***}&                     &                     &     -0.0005\sym{***}\\
                    &                     &                     &   (14.8)         &                     &                     &   (13.2)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid $\times$ Age&                     &                     &   -368.2\sym{***}&                     &                     &   -393.4\sym{***}&                     &                     &     -0.0002\sym{***}&                     &                     &     -0.0004\sym{***}\\
                    &                     &                     &   (18.8)         &                     &                     &   (16.1)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime $\times$ Age&                     &                     &  -1304.6\sym{***}&                     &                     &  -1215.7\sym{***}&                     &                     &     -0.0003\sym{***}&                     &                     &     -0.0010\sym{***}\\
                    &                     &                     &   (16.8)         &                     &                     &   (15.6)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low$\times$ Imputed Income&                     &                     &    389.1\sym{***}&                     &                     &    335.1\sym{***}&                     &                     &     -0.0000         &                     &                     &     -0.0000\sym{**} \\
                    &                     &                     &   (24.5)         &                     &                     &   (19.7)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid $\times$ Imputed Income&                     &                     &    297.6\sym{***}&                     &                     &    236.7\sym{***}&                     &                     &     -0.0000\sym{**} &                     &                     &     -0.0001\sym{***}\\
                    &                     &                     &   (25.7)         &                     &                     &   (21.9)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime $\times$ Imputed Income&                     &                     &   -325.1\sym{***}&                     &                     &   -408.9\sym{***}&                     &                     &     -0.0001\sym{***}&                     &                     &     -0.0003\sym{***}\\
                    &                     &                     &   (21.0)         &                     &                     &   (19.2)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant               &  32950.0\sym{***}& -15843.9\sym{***}& -44640.6\sym{***}&  30800.8\sym{***}&  -9040.5\sym{***}& -39202.0\sym{***}&      0.0092\sym{***}&      0.0086\sym{***}&     -0.0000         &      0.0558\sym{***}&      0.0554\sym{***}&      0.0265\sym{***}\\
                    &  (262.5)         &  (703.0)         &  (884.5)         &  (249.2)         &  (619.6)         &  (815.7)         &    (0.0001)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0003)         &    (0.0004)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&                    &           X         &           X         &                    &           X         &           X         &               &           X         &           X   & & X & X      \\
Observations        &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       &26,240,879       \\
$R^2$               &      0.0113         &      0.1668         &      0.1725         &      0.0172         &      0.2714         &      0.2848         &      0.0009         &      0.0492         &      0.0498         &      0.0006         &      0.0577         &      0.0599         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\tiny
\item Notes: This table reports regressions for credit risk profile and mortgage access. Prime Low, Prime Mid, and Prime High-Superprime are indicator variables for the consumer belonging to that category. Columns (1, 4, 7, 10) do not include controls. Columns (2, 5, 8, 11) controls for age, income and ZIP x Quarter fixed effects. Columns (3, 6, 9, 12) also includes interactions between credit risk profile, age and income. Income in thousands. Standard errors are clustered by ZIP code. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/old/four_categories/mortgage_reg_l1.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\tiny
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Credit Risk Profile and Mortgages \label{tab:mortgage_reg_l1}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}p{1in}*{12}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}&\multicolumn{1}{c}{(12)}\\
                    &\multicolumn{3}{c}{Mortgage Credit Limit}&\multicolumn{3}{c}{Mortgage Balances}&\multicolumn{3}{c}{Mortgage Origination}&\multicolumn{3}{c}{Mortgage Inquiry}\\
\hline
& & & & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low   &  21814.9\sym{***}&  -3593.4\sym{***}& -13481.9\sym{***}&  19922.2\sym{***}&  -2103.7\sym{***}& -11221.7\sym{***}&      0.0042\sym{***}&      0.0030\sym{***}&      0.0098\sym{***}&      0.0007\sym{***}&     -0.0035\sym{***}&      0.0103\sym{***}\\
                    &  (285.4)         &  (281.1)         & (1014.5)         &  (261.0)         &  (253.2)         &  (867.3)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0002)         &    (0.0002)         &    (0.0006)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid     &  45066.4\sym{***}&   -437.8         & -13480.1\sym{***}&  40674.2\sym{***}&    981.0\sym{***}&  -7653.9\sym{***}&      0.0078\sym{***}&      0.0051\sym{***}&      0.0141\sym{***}&      0.0098\sym{***}&     -0.0005\sym{*}  &      0.0165\sym{***}\\
                    &  (431.6)         &  (412.7)         & (1306.9)         &  (390.6)         &  (366.2)         & (1066.4)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0003)         &    (0.0003)         &    (0.0007)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime   &  51471.4\sym{***}& -39277.4\sym{***}&  54388.7\sym{***}&  42046.0\sym{***}& -36386.0\sym{***}&  58135.0\sym{***}&      0.0075\sym{***}&      0.0031\sym{***}&      0.0268\sym{***}&     -0.0056\sym{***}&     -0.0230\sym{***}&      0.0489\sym{***}\\
                    &  (498.5)         &  (721.2)         & (1202.2)         &  (444.1)         &  (671.3)         & (1038.4)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0002)         &    (0.0003)         &    (0.0006)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Age                  &                     &   -736.9\sym{***}&   -221.7\sym{***}&                     &   -686.6\sym{***}&   -210.5\sym{***}&                     &     -0.0001\sym{***}&      0.0000\sym{***}&                     &     -0.0005\sym{***}&     -0.0001\sym{***}\\
                    &                     &    (9.3)         &   (13.1)         &                     &    (8.8)         &   (12.2)         &                     &    (0.0000)         &    (0.0000)         &                     &    (0.0000)         &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Imputed Income&                     &   1571.0\sym{***}&   1737.6\sym{***}&                     &   1355.5\sym{***}&   1572.7\sym{***}&                     &      0.0001\sym{***}&      0.0001\sym{***}&                     &      0.0004\sym{***}&      0.0006\sym{***}\\
                    &                     &   (14.5)         &   (24.2)         &                     &   (13.2)         &   (22.1)         &                     &    (0.0000)         &    (0.0000)         &                     &    (0.0000)         &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low$\times$ Age&                     &                     &   -477.3\sym{***}&                     &                     &   -463.9\sym{***}&                     &                     &     -0.0002\sym{***}&                     &                     &     -0.0004\sym{***}\\
                    &                     &                     &   (15.3)         &                     &                     &   (13.6)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid $\times$ Age&                     &                     &   -318.9\sym{***}&                     &                     &   -352.9\sym{***}&                     &                     &     -0.0002\sym{***}&                     &                     &     -0.0003\sym{***}\\
                    &                     &                     &   (19.5)         &                     &                     &   (16.5)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime $\times$ Age&                     &                     &  -1244.8\sym{***}&                     &                     &  -1164.3\sym{***}&                     &                     &     -0.0004\sym{***}&                     &                     &     -0.0010\sym{***}\\
                    &                     &                     &   (17.5)         &                     &                     &   (16.2)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Low$\times$ Imputed Income&                     &                     &    387.2\sym{***}&                     &                     &    357.0\sym{***}&                     &                     &     -0.0000\sym{***}&                     &                     &     -0.0000         \\
                    &                     &                     &   (24.2)         &                     &                     &   (20.2)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime Mid $\times$ Imputed Income&                     &                     &    261.6\sym{***}&                     &                     &    208.5\sym{***}&                     &                     &     -0.0000\sym{**} &                     &                     &     -0.0001\sym{***}\\
                    &                     &                     &   (27.0)         &                     &                     &   (22.4)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime High-Superprime $\times$ Imputed Income&                     &                     &   -397.2\sym{***}&                     &                     &   -465.5\sym{***}&                     &                     &     -0.0001\sym{***}&                     &                     &     -0.0003\sym{***}\\
                    &                     &                     &   (22.1)         &                     &                     &   (19.9)         &                     &                     &    (0.0000)         &                     &                     &    (0.0000)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &  32661.0\sym{***}& -15682.1\sym{***}& -45046.6\sym{***}&  30444.1\sym{***}&  -8839.7\sym{***}& -39220.9\sym{***}&      0.0086\sym{***}&      0.0096\sym{***}&     -0.0006\sym{***}&      0.0546\sym{***}&      0.0559\sym{***}&      0.0271\sym{***}\\
                    &  (259.5)         &  (705.5)         &  (887.4)         &  (245.3)         &  (621.0)         &  (808.8)         &    (0.0000)         &    (0.0001)         &    (0.0001)         &    (0.0002)         &    (0.0003)         &    (0.0004)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&                    &           X         &           X         &                    &           X         &           X         &               &           X         &           X   & & X & X      \\
Observations        &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     &25,559,345     \\
$R^2$               &      0.0115         &      0.1676         &      0.1739         &      0.0178         &      0.2745         &      0.2892         &      0.0010         &      0.0488         &      0.0496         &      0.0004         &      0.0576         &      0.0599         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\tiny
\item Notes: This table reports regressions for credit risk profile and mortgage access. Prime Low, Prime Mid, and Prime High-Superprime are indicator variables for the consumer belonging to that category. Columns (1, 4, 7, 10) do not include controls. Columns (2, 5, 8, 11) controls for age, income and ZIP x Quarter fixed effects. Columns (3, 6, 9, 12) also includes interactions between credit risk profile, age and income. Credit risk profile based on the previous quarter. Income in thousands. Standard errors are clustered by ZIP code. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/old/misclassification_old/cc_limit.tex <==

\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Credit Cards Limits by Credit Score Risk Profile}\label{tab:cc_limits}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2in}p{1in}p{1in}p{1in}p{1in}}
 %  \multicolumn{4}{c}{Credit Score} \\ 
   \hline \hline
      &  &  &  & \\
      Deep Subprime & Subprime &  Near Prime & Prime &  Superprime \\  \hline
        &  &  &   &\\[\dimexpr-\normalbaselineskip+3pt] 
 \multicolumn{5}{c}{\textbf{\% of Borrowers}} \\
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
  2.217 &  10.295 & 13.015 & 41.349 & 33.124 \\
                         &                     &                     &                     &               \\
\multicolumn{5}{c}{\textbf{Credit Limit (\$)}} \\
    8,907.6 & 14,319.0 & 28,265.1 & 32,428.2 & 44,479.7 \\
                         &                     &                     &                     &               \\
\multicolumn{5}{c}{\textbf{Credit Limit / Household Income (\%)}} \\
    14.6 & 21.5 & 36.5 & 35.2 & 39.0 \\
                         &                     &                     &                     &               \\
\multicolumn{5}{c}{\textbf{\% Originated}} \\
    10.5 & 16.4 & 20.6 & 17.0 & 14.1 \\
                         &                     &                     &                     &               \\
\multicolumn{5}{c}{\textbf{\% Inquired}} \\
    19.9 & 19.4 & 17.1 & 9.9 & 4.7 \\
 %                      &                     &                     &        &        \\
      &  &  &  \\  \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Average credit limits, dollars and as percentage of household income by credit score risk profile, 2006Q1-2016Q2. Credit score risk profiles defined in Table \ref{tab:risk_def}. Prime Low credit scores: 660-700. Prime Mid credit scores: 701-740. Prime High credit scores: greater than 741. Sample: 18,318,847 borrowers with non-zero credit card limit. Credit risk profile based on the current quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/old/misclassification_old/credit_risk_reg.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Credit Risk Profile Regressions \label{tab:crr_reg}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{Credit Limit}&\multicolumn{1}{c}{Balances}&\multicolumn{1}{c}{ Origination}&\multicolumn{1}{c}{Inquiry}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{4}{l}{\underline{Panel A: Credit Cards}}\\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Subprime           &    985.8975\sym{***}&   3231.7203\sym{***}&      0.0976\sym{***}&      0.0029         \\
                    &  (306.0130)         &  (313.3932)         &    (0.0040)         &    (0.0056)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Near Prime           &  -1843.0567\sym{***}&    902.3757\sym{***}&      0.1642\sym{***}&     -0.0606\sym{***}\\
                    &  (354.2817)         &  (345.2520)         &    (0.0040)         &    (0.0055)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime           &   1811.9908\sym{***}&   4790.2556\sym{***}&      0.0723\sym{***}&     -0.2195\sym{***}\\
                    &  (305.8879)         &  (301.7071)         &    (0.0037)         &    (0.0053)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Superprime            &  30089.6137\sym{***}&  11713.2654\sym{***}&      0.0423\sym{***}&     -0.2764\sym{***}\\
                    &  (357.9584)         &  (294.0890)         &    (0.0037)         &    (0.0052)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &  -6601.1884\sym{***}&  -9543.9801\sym{***}&      0.1362\sym{***}&      0.3410\sym{***}\\
                    &  (271.5330)         &  (292.7983)         &    (0.0035)         &    (0.0052)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &18,318,847        &18,318,847        &18,318,847        &18,318,847        \\
$R^2$               &      0.3319         &      0.3006         &      0.0288         &      0.0514         \\ \hline 
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{4}{l}{\underline{Panel B: Mortgages}}\\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Subprime        &   7574.0447\sym{***}&   9011.6209\sym{***}&      0.0089\sym{***}&      0.0208\sym{***}\\
                    & (1285.2777)         &  (975.1730)         &    (0.0006)         &    (0.0018)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Near Prime          &   4603.9812\sym{***}&   9279.0785\sym{***}&      0.0313\sym{***}&      0.0514\sym{***}\\
                    & (1617.4900)         & (1339.7821)         &    (0.0008)         &    (0.0020)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime          &  -8434.3305\sym{***}&    782.8112         &      0.0258\sym{***}&      0.0182\sym{***}\\
                    & (1647.7365)         & (1381.5282)         &    (0.0006)         &    (0.0017)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Super Prime           &  82903.9414\sym{***}&  89578.9233\sym{***}&      0.0283\sym{***}&      0.0423\sym{***}\\
                    & (1911.5932)         & (1509.9132)         &    (0.0006)         &    (0.0018)         \\
                                        & (1320.4153)         & (1069.2793)         &    (0.0005)         &    (0.0016)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            & -46118.8911\sym{***}& -42725.5638\sym{***}&     -0.0055\sym{***}&      0.0309\sym{***}\\
                    & (1320.4153)         & (1069.2793)         &    (0.0005)         &    (0.0016)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &26,240,879     &26,240,879     &26,240,879     &26,240,879     \\
$R^2$               &      0.1639         &      0.2858         &      0.0083         &      0.0233         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\small
\item Notes: This table reports regressions for credit risk profile and credit cards. Subprime, Near Prime, Prime and Superprime are indicator variables for the consumer belonging to that category. Panel A focuses on credit cards while Panel B reports mortgages. We control for interactions between credit risk profile and age, income, and quarter as well as ZIP code fixed effects. Credit risk profiles based on current quarter. Standard errors are clustered by ZIP code. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/old/misclassification_old/credit_risk_reg_l1.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Credit Risk Profile Regressions \label{tab:crr_reg}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{Credit Limit}&\multicolumn{1}{c}{Balances}&\multicolumn{1}{c}{ Origination}&\multicolumn{1}{c}{Inquiry}\\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{4}{l}{\underline{Panel A: Credit Cards}}\\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Subprime        &  -1640.9595\sym{***}&     16.3517         &      0.1055\sym{***}&      0.0491\sym{***}\\
                    &  (279.2652)         &  (292.9727)         &    (0.0045)         &    (0.0054)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Near Prime      &  -4417.9000\sym{***}&  -2466.5483\sym{***}&      0.1304\sym{***}&      0.0124\sym{**} \\
                    &  (330.0184)         &  (326.7972)         &    (0.0045)         &    (0.0054)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime       &   -277.4509         &   2427.4524\sym{***}&      0.0427\sym{***}&     -0.1240\sym{***}\\
                    &  (282.5329)         &  (284.3776)         &    (0.0043)         &    (0.0051)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Super Prime       &  27235.8444\sym{***}&   9777.2822\sym{***}&      0.0244\sym{***}&     -0.1690\sym{***}\\
                    &  (339.0496)         &  (275.4204)         &    (0.0043)         &    (0.0051)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &  -3605.0501\sym{***}&  -6268.7825\sym{***}&      0.1730\sym{***}&      0.2522\sym{***}\\
                    &  (242.5115)         &  (272.5950)         &    (0.0041)         &    (0.0050)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &17,865,452       &17,865,452       &17,865,452       &17,865,452       \\
$R^2$               &      0.3349         &      0.2783         &      0.0286         &      0.0465         \\\hline 
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{4}{l}{\underline{Panel B: Mortgages}}\\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Subprime        &   6884.5850\sym{***}&   8249.0710\sym{***}&      0.0082\sym{***}&      0.0202\sym{***}\\
                    & (1305.5592)         &  (946.8998)         &    (0.0006)         &    (0.0019)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Near Prime      &   2677.9648         &   8022.0649\sym{***}&      0.0242\sym{***}&      0.0499\sym{***}\\
                    & (1631.9227)         & (1272.8597)         &    (0.0008)         &    (0.0021)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Prime       &  -8947.5964\sym{***}&    293.8923         &      0.0248\sym{***}&      0.0129\sym{***}\\
                    & (1673.7345)         & (1362.3201)         &    (0.0006)         &    (0.0018)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Super Prime       &  85675.3348\sym{***}&  91349.7514\sym{***}&      0.0415\sym{***}&      0.0396\sym{***}\\
                    & (1928.9244)         & (1500.0278)         &    (0.0007)         &    (0.0018)         \\
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            & -44017.9984\sym{***}& -40408.4583\sym{***}&     -0.0034\sym{***}&      0.0451\sym{***}\\
                    & (1337.1248)         & (1036.3985)         &    (0.0005)         &    (0.0017)         \\
\hline
& & & & \\[\dimexpr-\normalbaselineskip+2pt]
Observations        &25,559,345       &25,559,345       &25,559,345       &25,559,345       \\
$R^2$               &      0.1651         &      0.2899         &      0.0081         &      0.0230         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\small
\item Notes: This table reports regressions for credit risk profile and credit cards. Subprime, Near Prime, Prime and Superprime are indicator variables for the consumer belonging to that category. Panel A focuses on credit cards while Panel B reports mortgages. We control for interactions between credit risk profile and age, income, and quarter as well as ZIP code fixed effects. Credit risk profiles based on previous quarter. Standard errors are clustered by ZIP code. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/old/misclassification_old/misclassification_cost.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification}\label{tab:value_consumer_savings}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.5in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Deep Subprime-Near Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving (\$)}} \\
Deep Subprime-Near Prime & 0.00 & -39.97 & -48.69 & -69.69 \\
Prime Low & 103.08 & 0.00 & -26.31 & -39.94 \\
Prime Mid & 177.43 & 52.17 & 0.00 & -24.01 \\
Prime High-Superprime & 151.87 & 97.51 & 35.36 & 0.00 \\
                         &                     &                     &        &        \\
\textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Income (\%)}} \\
Deep Subprime-Near Prime & 0.00 & -0.05 & -0.06 & -0.08 \\
Prime Low & 0.11 & 0.00 & -0.03 & -0.04 \\
Prime Mid & 0.17 & 0.05 & 0.00 & -0.02 \\
Prime High-Superprime & 0.16 & 0.09 & 0.03 & 0.00 \\
                         &                     &                     &        &        \\
 \textbf{ Model-Based} & \multicolumn{4}{c}{\textbf{Annual Average Cost Saving / Total Debt (\%)}} \\
Deep Subprime-Near Prime & 0.00 & -0.18 & -0.28 & -0.35 \\
Prime Low & 0.21 & 0.00 & -0.13 & -0.23 \\
Prime Mid & 0.34 & 0.16 & 0.00 & -0.14 \\
Prime High-Superprime & 0.69 & 0.42 & 0.27 & 0.00 \\
 \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports consumers' average interest rate cost savings by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Prime Low credit scores: 660-700. Prime Mid credit scores: 701-740. Prime High credit scores greater than 741. Interest rates by credit score from \citeN{Stroebel_2015}.  Time period 2006Q1-2016Q2. Sample: 18,318,847 borrowers with non-zero credit card limit. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}



==> Tables/old/misclassification_old/misclassification_mortgage.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Cost of Credit Risk Misclassification: Mortgages}\label{tab:value_consumer_savings_mortgage}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.5in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Deep Subprime-Near Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Interest Rate Spread (\%)}} \\
Deep Subprime-Near Prime & -0.041 & -0.117 & -0.151 & -0.167 \\
Prime Low & 0.076 & -0.002 & -0.047 & -0.067 \\
Prime Mid & 0.086 & 0.040 & 0.001 & -0.022 \\
Prime High-Superprime & 0.120 & 0.055 & 0.020 & -0.002 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Saving (\$)}} \\
Deep Subprime-Near Prime & -4.118 & -13.037 & -17.703 & -23.797 \\
Prime Low & 10.840 & 0.386 & -5.646 & -9.708 \\
Prime Mid & 12.397 & 6.205 & 0.236 & -3.274 \\
Prime High-Superprime & 19.608 & 8.670 & 3.316 & -0.335 \\
                         &                     &                     &        &        \\
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Monthly Payment Cost Savings / Monthly Income (\%)}} \\
Deep Subprime-Near Prime & -0.090 & -0.252 & -0.320 & -0.360 \\
Prime Low & 0.152 & -0.006 & -0.103 & -0.145 \\
Prime Mid & 0.191 & 0.084 & -0.005 & -0.048 \\
Prime High-Superprime & 0.446 & 0.143 & 0.038 & -0.004 \\
    
\hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the average monthly payment cost savings on mortgages and interest rate spread for consumers by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Interest rates are calibrated using Freddie Mac Single Loan Data.  Time period 2006Q2-2016Q2. Sample: 159,552 borrowers with only one first mortgage originated in the past 9 months. Rankings based on the previous quarter. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


%NOTE: WE HAVE DEEP SUBPRIME SINCE THE FICO CUTOFF IS THE 22ND PERCENTILE. WE DO HAVE SUBPRIME BORROWERS BETWEEN 22ND AND 27TH PERCENTILE.

==> Tables/old/misclassification_old/misclassification_mortgage_desc.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\caption{Descriptive Statistics for Cost of Credit Risk Misclassification: Mortgages}\label{tab:value_consumer_savings_mortgage_desc}
\small
%\begin{tabular}{lccccc}
\begin{tabular}[c]{p{2.5in}p{1in}p{1in}p{1in}p{1in}}
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
   \multicolumn{5}{c}{Risk Profile} \\ \hline \hline
  \textbf{ Credit Score } & Deep Subprime-Near Prime & Prime Low & Prime Mid &  Prime High - Superprime \\  \hline
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{\% of Borrowers}} \\
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
Deep Subprime-Near Prime & 10.186 & 7.082 & 3.215 & 0.724 \\
Prime Low & 2.080 & 5.319 & 7.522 & 4.782 \\
Prime Mid & 0.338 & 1.190 & 5.286 & 12.874 \\
Prime High-Superprime & 0.095 & 0.281 & 1.535 & 37.484 \\

  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Origination Balance / Income}} \\
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
Deep Subprime-Near Prime & 3.13 & 3.02 & 2.90 & 2.79 \\
Prime Low & 2.99 & 2.88 & 2.90 & 2.72 \\
Prime Mid & 3.40 & 2.74 & 2.78 & 2.60 \\
Prime High-Superprime & 4.18 & 3.43 & 2.70 & 2.08 \\

  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Origination Balance}} \\
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
Deep Subprime-Near Prime & 186.30 & 189.28 & 190.73 & 222.52 \\
Prime Low & 211.19 & 208.33 & 204.33 & 223.68 \\
Prime Mid & 236.63 & 229.40 & 218.15 & 228.32 \\
Prime High-Superprime & 255.50 & 259.76 & 248.86 & 235.52 \\

  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
\textbf{Model-Based} & \multicolumn{4}{c}{\textbf{Imputed Income}} \\
  &  &  &  &  \\[\dimexpr-\normalbaselineskip+3pt] 
Deep Subprime-Near Prime & 65.99 & 68.45 & 72.13 & 88.46 \\
Prime Low & 80.11 & 79.45 & 77.42 & 90.58 \\
Prime Mid & 76.11 & 92.38 & 87.23 & 96.82 \\
Prime High-Superprime & 79.71 & 88.80 & 100.85 & 123.30 \\
\hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports descriptive statistics for consumers by estimated model-based risk profile, given their credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles. Interest rates are calibrated using Freddie Mac Single Loan Data.  Time period 2006Q2-2016Q2. Sample: 159,552 borrowers with only one first mortgage originated in the past 9 months. Source: Authors' calculations based on Experian Data. Imputed income and origination balance in thousand \$s. Rankings based on previous quarter.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


%NOTE: WE HAVE DEEP SUBPRIME SINCE THE FICO CUTOFF IS THE 22ND PERCENTILE. WE DO HAVE SUBPRIME BORROWERS BETWEEN 22ND AND 27TH PERCENTILE.

==> Tables/old/misclassification_old/mortgage_originations.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}
\caption{Cost of  Misclassification: Mortgage Originations}\label{tab:value_consumer_savings_mortgage_originations}
\small
%\begin{tabular}{ccccc}
\begin{tabular}[c]{p{2in}p{1in}p{1in}p{1in}p{1in}}
 %  \multicolumn{4}{c}{Credit Score} \\ 
   \hline \hline
      &  &  &  & \\
      Deep Subprime & Subprime &  Near Prime & Prime &  Superprime \\  \hline
        &  &  &   &\\[\dimexpr-\normalbaselineskip+3pt] 
\multicolumn{5}{c}{\textbf{\% Originated}} \\
    0.5 & 0.8 & 1.6 & 1.9 & 2.1 \\
                         &                     &                     &                     &               \\
\multicolumn{5}{c}{\textbf{\% Inquired}} \\
    4.6 & 5.0 & 6.9 & 6.0 & 4.1 \\
                         &                     &                     &                     &               \\
\multicolumn{5}{c}{\textbf{\% Originated (Borrowers with Inquiries)}} \\
    2.6 & 4.7 & 9.9 & 14.5 & 19.4 \\
\hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table reports the fraction of borrowers with mortgage originations by credit score risk profile. Table \ref{tab:risk_def} defines credit score risk profiles.  Time period 2006Q2-2016Q2. Sample: 25,559,345 borrowers; 1,373,816 borrowers with a mortgage inquiry; and 404,926 borrowers with a mortgage origination. Credit risk profile and inquiries based on the previous quarter. Source: Authors' calculations based on Experian Data. 
\end{tablenotes}
\end{threeparttable}
\end{table}






==> Tables/old/regressions_detail/credit_card_reg.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{credit\_limit}&\multicolumn{1}{c}{cc\_balances}&\multicolumn{1}{c}{cc\_origination}&\multicolumn{1}{c}{inquiry}\\
\hline
cs\_bin=1            &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=2            &    985.8975\sym{***}&   3231.7203\sym{***}&      0.0976\sym{***}&      0.0029         \\
                    &  (306.0130)         &  (313.3932)         &    (0.0040)         &    (0.0056)         \\
[1em]
cs\_bin=3            &  -1843.0567\sym{***}&    902.3757\sym{***}&      0.1642\sym{***}&     -0.0606\sym{***}\\
                    &  (354.2817)         &  (345.2520)         &    (0.0040)         &    (0.0055)         \\
[1em]
cs\_bin=4            &   1811.9908\sym{***}&   4790.2556\sym{***}&      0.0723\sym{***}&     -0.2195\sym{***}\\
                    &  (305.8879)         &  (301.7071)         &    (0.0037)         &    (0.0053)         \\
[1em]
cs\_bin=5            &  30089.6137\sym{***}&  11713.2654\sym{***}&      0.0423\sym{***}&     -0.2764\sym{***}\\
                    &  (357.9584)         &  (294.0890)         &    (0.0037)         &    (0.0052)         \\
[1em]
cs\_bin=1 $\times$ age&    111.4846\sym{***}&    134.0810\sym{***}&     -0.0002\sym{***}&     -0.0013\sym{***}\\
                    &    (5.1283)         &    (5.3530)         &    (0.0000)         &    (0.0001)         \\
[1em]
cs\_bin=2 $\times$ age&     98.2982\sym{***}&     96.7873\sym{***}&     -0.0009\sym{***}&     -0.0018\sym{***}\\
                    &    (3.9102)         &    (3.4562)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=3 $\times$ age&    177.4729\sym{***}&    138.0435\sym{***}&     -0.0015\sym{***}&     -0.0017\sym{***}\\
                    &    (5.0087)         &    (4.0408)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=4 $\times$ age&    261.6173\sym{***}&    115.9333\sym{***}&     -0.0004\sym{***}&     -0.0005\sym{***}\\
                    &    (3.4766)         &    (1.7766)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=5 $\times$ age&    -25.7951\sym{***}&    -40.2351\sym{***}&     -0.0003\sym{***}&     -0.0005\sym{***}\\
                    &    (3.6728)         &    (0.7917)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=1 $\times$ income\_insight\_score&    272.7280\sym{***}&    333.2509\sym{***}&     -0.0003\sym{***}&      0.0004\sym{***}\\
                    &    (4.8245)         &    (5.7379)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=2 $\times$ income\_insight\_score&    336.9501\sym{***}&    303.7578\sym{***}&     -0.0004\sym{***}&     -0.0002\sym{***}\\
                    &    (3.6708)         &    (3.3682)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=3 $\times$ income\_insight\_score&    503.5135\sym{***}&    385.2055\sym{***}&     -0.0003\sym{***}&     -0.0001\sym{***}\\
                    &    (3.5408)         &    (2.9777)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=4 $\times$ income\_insight\_score&    359.3026\sym{***}&    157.6783\sym{***}&     -0.0000\sym{***}&      0.0001\sym{***}\\
                    &    (1.7539)         &    (1.0249)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=5 $\times$ income\_insight\_score&    204.6417\sym{***}&     39.1559\sym{***}&     -0.0001\sym{***}&      0.0000\sym{***}\\
                    &    (1.2020)         &    (0.3389)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=1 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=1 $\times$ quarter=9&   -304.2965         &   -123.3861         &      0.0298\sym{***}&     -0.0633\sym{***}\\
                    &  (192.8095)         &  (211.2999)         &    (0.0048)         &    (0.0059)         \\
[1em]
cs\_bin=1 $\times$ quarter=10&   -544.7228\sym{*}  &   -464.8922         &      0.0347\sym{***}&     -0.0638\sym{***}\\
                    &  (292.7776)         &  (316.2859)         &    (0.0047)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=11&   -769.6804\sym{***}&   -967.7485\sym{***}&      0.0274\sym{***}&     -0.0437\sym{***}\\
                    &  (258.2346)         &  (287.0423)         &    (0.0046)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=12&    477.8119\sym{*}  &    550.5430\sym{*}  &      0.0346\sym{***}&      0.0325\sym{***}\\
                    &  (254.7690)         &  (285.4040)         &    (0.0047)         &    (0.0064)         \\
[1em]
cs\_bin=1 $\times$ quarter=13&     34.3807         &    139.5987         &      0.0801\sym{***}&     -0.0205\sym{***}\\
                    &  (250.5460)         &  (284.1962)         &    (0.0048)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=14&   -481.9422\sym{**} &   -521.3947\sym{*}  &      0.0658\sym{***}&     -0.0303\sym{***}\\
                    &  (244.6975)         &  (269.9806)         &    (0.0045)         &    (0.0059)         \\
[1em]
cs\_bin=1 $\times$ quarter=15&   -553.5674\sym{**} &   -471.2748\sym{*}  &      0.0210\sym{***}&     -0.0682\sym{***}\\
                    &  (248.3952)         &  (276.3938)         &    (0.0042)         &    (0.0057)         \\
[1em]
cs\_bin=1 $\times$ quarter=16&    747.1815\sym{***}&   1131.3953\sym{***}&     -0.0216\sym{***}&     -0.0360\sym{***}\\
                    &  (250.4695)         &  (275.5455)         &    (0.0041)         &    (0.0059)         \\
[1em]
cs\_bin=1 $\times$ quarter=17&    810.9568\sym{***}&   1286.9526\sym{***}&      0.0080\sym{*}  &     -0.0858\sym{***}\\
                    &  (260.0022)         &  (289.1186)         &    (0.0042)         &    (0.0059)         \\
[1em]
cs\_bin=1 $\times$ quarter=18&    817.2819\sym{***}&   1378.1250\sym{***}&     -0.0185\sym{***}&     -0.1033\sym{***}\\
                    &  (267.3698)         &  (298.0891)         &    (0.0041)         &    (0.0058)         \\
[1em]
cs\_bin=1 $\times$ quarter=19&    766.0141\sym{***}&   1876.2325\sym{***}&     -0.0350\sym{***}&     -0.1141\sym{***}\\
                    &  (274.8228)         &  (310.2630)         &    (0.0039)         &    (0.0058)         \\
[1em]
cs\_bin=1 $\times$ quarter=20&   2842.0470\sym{***}&   4569.1550\sym{***}&     -0.0400\sym{***}&     -0.1065\sym{***}\\
                    &  (286.2705)         &  (324.6956)         &    (0.0039)         &    (0.0058)         \\
[1em]
cs\_bin=1 $\times$ quarter=21&   1870.1965\sym{***}&   3722.5989\sym{***}&     -0.0485\sym{***}&     -0.1560\sym{***}\\
                    &  (290.6300)         &  (336.0637)         &    (0.0039)         &    (0.0057)         \\
[1em]
cs\_bin=1 $\times$ quarter=22&    925.1820\sym{***}&   2547.6501\sym{***}&     -0.0483\sym{***}&     -0.1757\sym{***}\\
                    &  (289.9190)         &  (335.4954)         &    (0.0039)         &    (0.0056)         \\
[1em]
cs\_bin=1 $\times$ quarter=23&     83.4572         &   1609.1899\sym{***}&     -0.0359\sym{***}&     -0.1844\sym{***}\\
                    &  (292.1784)         &  (338.1368)         &    (0.0041)         &    (0.0056)         \\
[1em]
cs\_bin=1 $\times$ quarter=24&    344.8992         &   2072.1763\sym{***}&     -0.0537\sym{***}&     -0.1524\sym{***}\\
                    &  (291.2946)         &  (335.6919)         &    (0.0040)         &    (0.0059)         \\
[1em]
cs\_bin=1 $\times$ quarter=25&   -780.7338\sym{***}&    474.4522         &     -0.0354\sym{***}&     -0.1689\sym{***}\\
                    &  (301.3898)         &  (345.2631)         &    (0.0043)         &    (0.0060)         \\
[1em]
cs\_bin=1 $\times$ quarter=26&  -1348.9559\sym{***}&   -494.2613         &     -0.0479\sym{***}&     -0.1709\sym{***}\\
                    &  (308.7786)         &  (351.3573)         &    (0.0042)         &    (0.0060)         \\
[1em]
cs\_bin=1 $\times$ quarter=27&  -2055.4660\sym{***}&  -1368.6081\sym{***}&     -0.0314\sym{***}&     -0.1632\sym{***}\\
                    &  (314.6451)         &  (357.5774)         &    (0.0044)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=28&  -2250.9523\sym{***}&  -1933.8444\sym{***}&     -0.0211\sym{***}&     -0.1674\sym{***}\\
                    &  (290.5137)         &  (330.7026)         &    (0.0047)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=29&  -3479.1977\sym{***}&  -3471.3718\sym{***}&     -0.0307\sym{***}&     -0.1701\sym{***}\\
                    &  (293.0985)         &  (320.6905)         &    (0.0046)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=30&  -3925.7137\sym{***}&  -3938.0847\sym{***}&     -0.0244\sym{***}&     -0.1744\sym{***}\\
                    &  (285.7614)         &  (310.6330)         &    (0.0046)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=31&  -3904.2524\sym{***}&  -3946.3761\sym{***}&     -0.0260\sym{***}&     -0.1634\sym{***}\\
                    &  (283.1465)         &  (309.4419)         &    (0.0045)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=32&  -2970.8001\sym{***}&  -2878.1249\sym{***}&     -0.0361\sym{***}&     -0.1753\sym{***}\\
                    &  (276.2593)         &  (306.4265)         &    (0.0045)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=33&  -3716.8226\sym{***}&  -3996.9160\sym{***}&     -0.0217\sym{***}&     -0.1740\sym{***}\\
                    &  (273.6685)         &  (296.6547)         &    (0.0047)         &    (0.0062)         \\
[1em]
cs\_bin=1 $\times$ quarter=34&  -3898.0364\sym{***}&  -4386.0080\sym{***}&     -0.0340\sym{***}&     -0.1793\sym{***}\\
                    &  (269.1872)         &  (288.4943)         &    (0.0045)         &    (0.0061)         \\
[1em]
cs\_bin=1 $\times$ quarter=35&  -3626.6524\sym{***}&  -3874.8604\sym{***}&     -0.0342\sym{***}&     -0.1599\sym{***}\\
                    &  (256.9645)         &  (277.8057)         &    (0.0044)         &    (0.0061)         \\
[1em]
cs\_bin=1 $\times$ quarter=36&  -3629.1131\sym{***}&  -3952.3286\sym{***}&     -0.0488\sym{***}&     -0.1799\sym{***}\\
                    &  (268.4654)         &  (292.5751)         &    (0.0043)         &    (0.0061)         \\
[1em]
cs\_bin=1 $\times$ quarter=37&  -3937.9418\sym{***}&  -4330.8527\sym{***}&     -0.0344\sym{***}&     -0.1636\sym{***}\\
                    &  (273.6992)         &  (299.1916)         &    (0.0046)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=38&  -4246.5051\sym{***}&  -4742.8170\sym{***}&     -0.0019         &     -0.1632\sym{***}\\
                    &  (259.9704)         &  (281.3216)         &    (0.0049)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=39&  -4002.8992\sym{***}&  -4563.6294\sym{***}&     -0.0082\sym{*}  &     -0.1471\sym{***}\\
                    &  (267.4779)         &  (288.3837)         &    (0.0047)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=40&  -3914.1745\sym{***}&  -4518.4464\sym{***}&     -0.0319\sym{***}&     -0.1566\sym{***}\\
                    &  (274.1128)         &  (297.0836)         &    (0.0046)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=41&  -3905.4700\sym{***}&  -4415.2275\sym{***}&     -0.0120\sym{**} &     -0.1368\sym{***}\\
                    &  (275.7060)         &  (296.6596)         &    (0.0048)         &    (0.0064)         \\
[1em]
cs\_bin=1 $\times$ quarter=42&  -4028.8507\sym{***}&  -4551.5441\sym{***}&     -0.0070         &     -0.1282\sym{***}\\
                    &  (269.1180)         &  (294.8722)         &    (0.0047)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=43&  -3528.4906\sym{***}&  -4055.1431\sym{***}&      0.0066         &     -0.1159\sym{***}\\
                    &  (268.7769)         &  (294.4633)         &    (0.0049)         &    (0.0064)         \\
[1em]
cs\_bin=1 $\times$ quarter=44&  -3258.9951\sym{***}&  -3786.6389\sym{***}&     -0.0215\sym{***}&     -0.1276\sym{***}\\
                    &  (269.6931)         &  (292.1579)         &    (0.0046)         &    (0.0064)         \\
[1em]
cs\_bin=1 $\times$ quarter=45&  -3743.0473\sym{***}&  -4423.8240\sym{***}&      0.0019         &     -0.1257\sym{***}\\
                    &  (262.7766)         &  (289.4928)         &    (0.0049)         &    (0.0064)         \\
[1em]
cs\_bin=1 $\times$ quarter=46&  -3850.9676\sym{***}&  -4597.3458\sym{***}&      0.0020         &     -0.1208\sym{***}\\
                    &  (263.1559)         &  (284.4047)         &    (0.0048)         &    (0.0064)         \\
[1em]
cs\_bin=1 $\times$ quarter=47&  -3624.5693\sym{***}&  -4423.1605\sym{***}&     -0.0057         &     -0.1200\sym{***}\\
                    &  (264.6956)         &  (281.4271)         &    (0.0047)         &    (0.0063)         \\
[1em]
cs\_bin=1 $\times$ quarter=48&  -2653.4372\sym{***}&  -3203.1642\sym{***}&     -0.0061         &     -0.1153\sym{***}\\
                    &  (340.7328)         &  (355.5525)         &    (0.0048)         &    (0.0065)         \\
[1em]
cs\_bin=1 $\times$ quarter=49&  -3008.2446\sym{***}&  -3713.7711\sym{***}&      0.0137\sym{***}&     -0.1006\sym{***}\\
                    &  (279.9387)         &  (293.5416)         &    (0.0049)         &    (0.0065)         \\
[1em]
cs\_bin=2 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=2 $\times$ quarter=9&   -263.5530\sym{**} &   -206.3799\sym{**} &      0.0248\sym{***}&     -0.0318\sym{***}\\
                    &  (113.2074)         &   (92.8102)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin=2 $\times$ quarter=10&    -80.0866         &   -168.6339         &      0.0486\sym{***}&     -0.0251\sym{***}\\
                    &  (128.0614)         &  (107.0320)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=11&   -360.9570\sym{***}&   -487.0665\sym{***}&      0.0500\sym{***}&     -0.0150\sym{***}\\
                    &  (135.7303)         &  (114.8813)         &    (0.0026)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=12&   -248.5157\sym{*}  &   -303.2879\sym{***}&      0.0116\sym{***}&      0.0181\sym{***}\\
                    &  (136.0650)         &  (116.0489)         &    (0.0025)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=13&    -14.5608         &   -261.5268\sym{**} &      0.1064\sym{***}&     -0.0104\sym{***}\\
                    &  (143.7413)         &  (122.8276)         &    (0.0027)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=14&    -49.3206         &   -287.0144\sym{**} &      0.0465\sym{***}&     -0.0098\sym{***}\\
                    &  (143.3181)         &  (122.1245)         &    (0.0026)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=15&    320.6363\sym{**} &     11.1104         &      0.0307\sym{***}&     -0.0322\sym{***}\\
                    &  (152.5045)         &  (129.7175)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=16&    858.1320\sym{***}&    554.3638\sym{***}&     -0.0119\sym{***}&     -0.0243\sym{***}\\
                    &  (152.4311)         &  (129.8299)         &    (0.0024)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=17&    749.7073\sym{***}&    465.1552\sym{***}&      0.0224\sym{***}&     -0.0580\sym{***}\\
                    &  (156.1256)         &  (133.5438)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=18&    903.8155\sym{***}&    701.2213\sym{***}&     -0.0243\sym{***}&     -0.0700\sym{***}\\
                    &  (160.0638)         &  (137.2443)         &    (0.0023)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=19&    595.1366\sym{***}&    948.3481\sym{***}&     -0.0456\sym{***}&     -0.0777\sym{***}\\
                    &  (159.7596)         &  (140.7413)         &    (0.0023)         &    (0.0026)         \\
[1em]
cs\_bin=2 $\times$ quarter=20&    592.3799\sym{***}&   1294.7239\sym{***}&     -0.0702\sym{***}&     -0.0923\sym{***}\\
                    &  (160.5180)         &  (140.9690)         &    (0.0022)         &    (0.0026)         \\
[1em]
cs\_bin=2 $\times$ quarter=21&   -512.0287\sym{***}&    653.9466\sym{***}&     -0.0813\sym{***}&     -0.1197\sym{***}\\
                    &  (158.8997)         &  (141.3029)         &    (0.0022)         &    (0.0025)         \\
[1em]
cs\_bin=2 $\times$ quarter=22&  -1338.1383\sym{***}&    159.6041         &     -0.0865\sym{***}&     -0.1319\sym{***}\\
                    &  (157.0300)         &  (140.2244)         &    (0.0022)         &    (0.0025)         \\
[1em]
cs\_bin=2 $\times$ quarter=23&  -2076.5507\sym{***}&   -446.9056\sym{***}&     -0.0728\sym{***}&     -0.1331\sym{***}\\
                    &  (155.8511)         &  (138.0500)         &    (0.0023)         &    (0.0025)         \\
[1em]
cs\_bin=2 $\times$ quarter=24&  -2482.1104\sym{***}&   -764.4199\sym{***}&     -0.0962\sym{***}&     -0.1163\sym{***}\\
                    &  (156.8134)         &  (139.8218)         &    (0.0022)         &    (0.0026)         \\
[1em]
cs\_bin=2 $\times$ quarter=25&  -3592.2249\sym{***}&  -1715.4933\sym{***}&     -0.0646\sym{***}&     -0.1232\sym{***}\\
                    &  (155.7193)         &  (138.3184)         &    (0.0024)         &    (0.0026)         \\
[1em]
cs\_bin=2 $\times$ quarter=26&  -4260.4279\sym{***}&  -2380.8691\sym{***}&     -0.0713\sym{***}&     -0.1150\sym{***}\\
                    &  (157.7583)         &  (139.8896)         &    (0.0023)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=27&  -4879.9292\sym{***}&  -3045.3913\sym{***}&     -0.0496\sym{***}&     -0.1077\sym{***}\\
                    &  (157.3422)         &  (139.4228)         &    (0.0024)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=28&  -5077.6413\sym{***}&  -3410.2743\sym{***}&     -0.0590\sym{***}&     -0.1141\sym{***}\\
                    &  (156.5358)         &  (138.9652)         &    (0.0024)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=29&  -5798.8372\sym{***}&  -4167.4948\sym{***}&     -0.0428\sym{***}&     -0.0983\sym{***}\\
                    &  (154.6416)         &  (137.0414)         &    (0.0024)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=30&  -5676.8988\sym{***}&  -3924.0825\sym{***}&     -0.0289\sym{***}&     -0.1068\sym{***}\\
                    &  (161.0405)         &  (141.5531)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=31&  -5620.4230\sym{***}&  -3927.0895\sym{***}&     -0.0209\sym{***}&     -0.0990\sym{***}\\
                    &  (161.2521)         &  (141.5269)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=32&  -5306.0743\sym{***}&  -3771.3506\sym{***}&     -0.0498\sym{***}&     -0.1170\sym{***}\\
                    &  (161.5915)         &  (142.4571)         &    (0.0024)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=33&  -5330.4586\sym{***}&  -3921.1033\sym{***}&     -0.0329\sym{***}&     -0.1089\sym{***}\\
                    &  (163.7249)         &  (142.9268)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=34&  -5425.2817\sym{***}&  -4222.7876\sym{***}&     -0.0259\sym{***}&     -0.1028\sym{***}\\
                    &  (164.2211)         &  (142.3282)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=35&  -5024.5194\sym{***}&  -3829.2133\sym{***}&     -0.0179\sym{***}&     -0.0954\sym{***}\\
                    &  (162.0736)         &  (141.6302)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=36&  -5344.0445\sym{***}&  -4206.9854\sym{***}&     -0.0500\sym{***}&     -0.1082\sym{***}\\
                    &  (162.4323)         &  (142.0591)         &    (0.0024)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=37&  -5371.9441\sym{***}&  -4250.9312\sym{***}&     -0.0372\sym{***}&     -0.0975\sym{***}\\
                    &  (163.5189)         &  (142.4680)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin=2 $\times$ quarter=38&  -5089.5684\sym{***}&  -4019.3052\sym{***}&      0.0058\sym{**} &     -0.0844\sym{***}\\
                    &  (164.2649)         &  (143.3580)         &    (0.0026)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=39&  -4761.9637\sym{***}&  -3833.3629\sym{***}&      0.0486\sym{***}&     -0.0695\sym{***}\\
                    &  (166.6451)         &  (144.8494)         &    (0.0027)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=40&  -5107.4072\sym{***}&  -4259.2439\sym{***}&     -0.0265\sym{***}&     -0.0783\sym{***}\\
                    &  (167.9565)         &  (144.7961)         &    (0.0025)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=41&  -5006.2221\sym{***}&  -4193.8290\sym{***}&     -0.0071\sym{***}&     -0.0611\sym{***}\\
                    &  (168.9002)         &  (145.4149)         &    (0.0026)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=42&  -4519.2189\sym{***}&  -3849.6583\sym{***}&      0.0098\sym{***}&     -0.0507\sym{***}\\
                    &  (168.3772)         &  (144.8500)         &    (0.0026)         &    (0.0028)         \\
[1em]
cs\_bin=2 $\times$ quarter=43&  -4271.9223\sym{***}&  -3585.3669\sym{***}&      0.0330\sym{***}&     -0.0356\sym{***}\\
                    &  (165.6308)         &  (142.7664)         &    (0.0027)         &    (0.0029)         \\
[1em]
cs\_bin=2 $\times$ quarter=44&  -4773.5974\sym{***}&  -4092.8534\sym{***}&     -0.0073\sym{***}&     -0.0546\sym{***}\\
                    &  (165.0450)         &  (142.0417)         &    (0.0026)         &    (0.0029)         \\
[1em]
cs\_bin=2 $\times$ quarter=45&  -4626.5562\sym{***}&  -4018.9240\sym{***}&      0.0253\sym{***}&     -0.0384\sym{***}\\
                    &  (165.4975)         &  (142.7108)         &    (0.0027)         &    (0.0029)         \\
[1em]
cs\_bin=2 $\times$ quarter=46&  -4078.3535\sym{***}&  -3570.9316\sym{***}&      0.0223\sym{***}&     -0.0295\sym{***}\\
                    &  (167.6379)         &  (143.2678)         &    (0.0026)         &    (0.0029)         \\
[1em]
cs\_bin=2 $\times$ quarter=47&  -3599.0502\sym{***}&  -3226.4842\sym{***}&      0.0409\sym{***}&     -0.0255\sym{***}\\
                    &  (169.2719)         &  (143.4383)         &    (0.0027)         &    (0.0029)         \\
[1em]
cs\_bin=2 $\times$ quarter=48&  -3635.4598\sym{***}&  -3315.6540\sym{***}&      0.0239\sym{***}&     -0.0400\sym{***}\\
                    &  (169.1610)         &  (144.5161)         &    (0.0027)         &    (0.0029)         \\
[1em]
cs\_bin=2 $\times$ quarter=49&  -3328.6537\sym{***}&  -3078.4487\sym{***}&      0.0467\sym{***}&     -0.0181\sym{***}\\
                    &  (171.2329)         &  (146.4677)         &    (0.0027)         &    (0.0029)         \\
[1em]
cs\_bin=3 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=3 $\times$ quarter=9&   -276.5796\sym{**} &   -360.8453\sym{***}&      0.0238\sym{***}&     -0.0072\sym{***}\\
                    &  (131.4137)         &   (96.6329)         &    (0.0024)         &    (0.0021)         \\
[1em]
cs\_bin=3 $\times$ quarter=10&     41.4737         &   -290.1454\sym{**} &      0.0531\sym{***}&     -0.0028         \\
                    &  (156.1895)         &  (114.2653)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=11&    -52.2203         &   -486.4052\sym{***}&      0.0558\sym{***}&      0.0010         \\
                    &  (163.9586)         &  (120.3248)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=12&   -875.9335\sym{***}&   -813.1876\sym{***}&     -0.0148\sym{***}&      0.0142\sym{***}\\
                    &  (163.1550)         &  (121.9120)         &    (0.0023)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=13&    285.9207\sym{*}  &   -195.4081         &      0.1532\sym{***}&      0.0061\sym{***}\\
                    &  (172.3648)         &  (128.6458)         &    (0.0026)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=14&   1174.9206\sym{***}&    279.6235\sym{**} &      0.0401\sym{***}&      0.0034         \\
                    &  (180.8072)         &  (134.1814)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=15&   1517.3754\sym{***}&    677.7020\sym{***}&      0.0330\sym{***}&     -0.0185\sym{***}\\
                    &  (188.7571)         &  (140.6681)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=16&   1369.3789\sym{***}&    726.5014\sym{***}&     -0.0028         &     -0.0166\sym{***}\\
                    &  (186.3690)         &  (139.0027)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=17&   1341.2447\sym{***}&    640.1275\sym{***}&      0.0536\sym{***}&     -0.0263\sym{***}\\
                    &  (192.6006)         &  (143.1343)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=18&   1554.5341\sym{***}&   1048.0520\sym{***}&     -0.0061\sym{**} &     -0.0349\sym{***}\\
                    &  (195.5014)         &  (147.2065)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=19&    977.4750\sym{***}&   1524.0759\sym{***}&     -0.0457\sym{***}&     -0.0495\sym{***}\\
                    &  (197.5831)         &  (150.7653)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=20&    -87.8985         &   1280.3041\sym{***}&     -0.0718\sym{***}&     -0.0663\sym{***}\\
                    &  (191.4749)         &  (147.2692)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=21&  -1442.0053\sym{***}&    746.1844\sym{***}&     -0.0841\sym{***}&     -0.0778\sym{***}\\
                    &  (192.5099)         &  (150.0629)         &    (0.0022)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=22&  -2954.9281\sym{***}&    179.4975         &     -0.0929\sym{***}&     -0.0833\sym{***}\\
                    &  (189.8285)         &  (148.3172)         &    (0.0022)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=23&  -3745.1572\sym{***}&   -223.5534         &     -0.0730\sym{***}&     -0.0888\sym{***}\\
                    &  (189.8327)         &  (149.1987)         &    (0.0023)         &    (0.0021)         \\
[1em]
cs\_bin=3 $\times$ quarter=24&  -4669.2219\sym{***}&   -746.0098\sym{***}&     -0.0986\sym{***}&     -0.0794\sym{***}\\
                    &  (188.8023)         &  (149.4066)         &    (0.0022)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=25&  -5892.8202\sym{***}&  -1421.0631\sym{***}&     -0.0634\sym{***}&     -0.0797\sym{***}\\
                    &  (188.1378)         &  (148.7313)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=26&  -6797.2604\sym{***}&  -2172.1310\sym{***}&     -0.0705\sym{***}&     -0.0649\sym{***}\\
                    &  (188.6036)         &  (148.3009)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=27&  -7287.2287\sym{***}&  -2591.0303\sym{***}&     -0.0485\sym{***}&     -0.0650\sym{***}\\
                    &  (189.6187)         &  (148.5014)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=28&  -7755.7845\sym{***}&  -3133.9826\sym{***}&     -0.0536\sym{***}&     -0.0736\sym{***}\\
                    &  (190.3340)         &  (148.7704)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=29&  -8147.8653\sym{***}&  -3466.1671\sym{***}&     -0.0546\sym{***}&     -0.0575\sym{***}\\
                    &  (191.1279)         &  (148.8533)         &    (0.0023)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=30&  -8309.4792\sym{***}&  -3603.2321\sym{***}&     -0.0332\sym{***}&     -0.0544\sym{***}\\
                    &  (193.6593)         &  (150.4549)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=31&  -7947.0423\sym{***}&  -3511.4461\sym{***}&     -0.0192\sym{***}&     -0.0611\sym{***}\\
                    &  (194.5339)         &  (151.2272)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=32&  -7904.3951\sym{***}&  -3461.3942\sym{***}&     -0.0608\sym{***}&     -0.0711\sym{***}\\
                    &  (193.6858)         &  (150.0802)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=33&  -8012.8478\sym{***}&  -3647.5576\sym{***}&     -0.0445\sym{***}&     -0.0641\sym{***}\\
                    &  (194.9003)         &  (149.8195)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=34&  -7926.2812\sym{***}&  -3756.1932\sym{***}&     -0.0254\sym{***}&     -0.0601\sym{***}\\
                    &  (194.6885)         &  (149.8288)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=35&  -7630.2289\sym{***}&  -3517.3018\sym{***}&     -0.0029         &     -0.0498\sym{***}\\
                    &  (190.8868)         &  (146.9786)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin=3 $\times$ quarter=36&  -8181.9064\sym{***}&  -4094.1515\sym{***}&     -0.0444\sym{***}&     -0.0522\sym{***}\\
                    &  (194.1673)         &  (149.5697)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=37&  -8112.7651\sym{***}&  -4132.5329\sym{***}&     -0.0361\sym{***}&     -0.0440\sym{***}\\
                    &  (193.2380)         &  (148.2263)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=38&  -7955.5410\sym{***}&  -3908.5415\sym{***}&     -0.0132\sym{***}&     -0.0360\sym{***}\\
                    &  (197.7146)         &  (151.5319)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=39&  -7264.4237\sym{***}&  -3559.9293\sym{***}&      0.0837\sym{***}&     -0.0281\sym{***}\\
                    &  (196.0088)         &  (149.1760)         &    (0.0026)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=40&  -8030.2039\sym{***}&  -4313.7956\sym{***}&     -0.0323\sym{***}&     -0.0337\sym{***}\\
                    &  (196.2690)         &  (149.4524)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=41&  -7963.4935\sym{***}&  -4254.1199\sym{***}&     -0.0145\sym{***}&     -0.0192\sym{***}\\
                    &  (197.0426)         &  (150.0717)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=42&  -7319.0275\sym{***}&  -3823.2363\sym{***}&     -0.0063\sym{***}&     -0.0127\sym{***}\\
                    &  (199.2957)         &  (151.0321)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=43&  -6819.0293\sym{***}&  -3484.9757\sym{***}&      0.0159\sym{***}&     -0.0100\sym{***}\\
                    &  (197.6705)         &  (150.1069)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=44&  -7985.0951\sym{***}&  -4482.6995\sym{***}&     -0.0330\sym{***}&     -0.0213\sym{***}\\
                    &  (197.8909)         &  (150.8004)         &    (0.0023)         &    (0.0023)         \\
[1em]
cs\_bin=3 $\times$ quarter=45&  -7681.5480\sym{***}&  -4362.7581\sym{***}&     -0.0015         &     -0.0115\sym{***}\\
                    &  (198.3670)         &  (150.6893)         &    (0.0024)         &    (0.0024)         \\
[1em]
cs\_bin=3 $\times$ quarter=46&  -7061.1337\sym{***}&  -3918.1595\sym{***}&     -0.0017         &     -0.0065\sym{***}\\
                    &  (200.0539)         &  (151.9433)         &    (0.0024)         &    (0.0024)         \\
[1em]
cs\_bin=3 $\times$ quarter=47&  -6361.4578\sym{***}&  -3432.3939\sym{***}&      0.0157\sym{***}&     -0.0088\sym{***}\\
                    &  (200.5571)         &  (152.6596)         &    (0.0025)         &    (0.0024)         \\
[1em]
cs\_bin=3 $\times$ quarter=48&  -7240.6235\sym{***}&  -4209.9288\sym{***}&      0.0037         &     -0.0096\sym{***}\\
                    &  (201.9278)         &  (152.9961)         &    (0.0024)         &    (0.0024)         \\
[1em]
cs\_bin=3 $\times$ quarter=49&  -6805.1743\sym{***}&  -3958.4350\sym{***}&      0.0300\sym{***}&      0.0051\sym{**} \\
                    &  (202.6944)         &  (154.2301)         &    (0.0025)         &    (0.0024)         \\
[1em]
cs\_bin=4 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=4 $\times$ quarter=9&     77.3736         &     79.5764\sym{**} &      0.0099\sym{***}&      0.0012         \\
                    &   (52.9891)         &   (31.2454)         &    (0.0013)         &    (0.0009)         \\
[1em]
cs\_bin=4 $\times$ quarter=10&    551.9918\sym{***}&    392.8627\sym{***}&      0.0551\sym{***}&      0.0077\sym{***}\\
                    &   (64.3059)         &   (37.3423)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=11&    464.3500\sym{***}&    474.9736\sym{***}&      0.0435\sym{***}&      0.0034\sym{***}\\
                    &   (70.8505)         &   (41.1400)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=12&  -1524.1222\sym{***}&   -115.1319\sym{***}&     -0.0331\sym{***}&      0.0087\sym{***}\\
                    &   (72.6677)         &   (43.1229)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=13&    340.6877\sym{***}&    365.0915\sym{***}&      0.1622\sym{***}&      0.0088\sym{***}\\
                    &   (76.8468)         &   (45.3246)         &    (0.0015)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=14&   1115.4796\sym{***}&    561.4850\sym{***}&      0.0199\sym{***}&      0.0072\sym{***}\\
                    &   (81.4202)         &   (47.8800)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=15&   1809.0334\sym{***}&    861.4993\sym{***}&      0.0212\sym{***}&     -0.0073\sym{***}\\
                    &   (85.7762)         &   (49.5723)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=16&    333.7206\sym{***}&    358.0700\sym{***}&     -0.0030\sym{**} &     -0.0052\sym{***}\\
                    &   (84.7805)         &   (50.5511)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=17&   1025.6510\sym{***}&    391.0329\sym{***}&      0.0852\sym{***}&     -0.0049\sym{***}\\
                    &   (87.0989)         &   (50.0262)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=18&   1167.8654\sym{***}&    606.1304\sym{***}&      0.0021         &     -0.0065\sym{***}\\
                    &   (90.1518)         &   (51.2657)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=19&   -256.4082\sym{***}&    597.1558\sym{***}&     -0.0458\sym{***}&     -0.0200\sym{***}\\
                    &   (91.8412)         &   (52.6130)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=20&  -2591.5404\sym{***}&    123.5669\sym{**} &     -0.0510\sym{***}&     -0.0279\sym{***}\\
                    &   (90.0847)         &   (52.0974)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=21&  -3876.2167\sym{***}&   -112.7563\sym{**} &     -0.0459\sym{***}&     -0.0266\sym{***}\\
                    &   (91.9296)         &   (53.2300)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=22&  -4764.6778\sym{***}&   -169.7957\sym{***}&     -0.0576\sym{***}&     -0.0269\sym{***}\\
                    &   (90.9479)         &   (52.0862)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=23&  -5398.8869\sym{***}&   -316.8035\sym{***}&     -0.0434\sym{***}&     -0.0366\sym{***}\\
                    &   (92.4465)         &   (52.6406)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=24&  -6643.2464\sym{***}&   -728.7307\sym{***}&     -0.0657\sym{***}&     -0.0335\sym{***}\\
                    &   (92.5057)         &   (53.0327)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=25&  -7343.4044\sym{***}&   -787.1817\sym{***}&     -0.0415\sym{***}&     -0.0278\sym{***}\\
                    &   (93.2793)         &   (53.3791)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=26&  -7473.5738\sym{***}&   -730.5024\sym{***}&     -0.0507\sym{***}&     -0.0210\sym{***}\\
                    &   (94.3009)         &   (53.7815)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=27&  -7480.0864\sym{***}&   -691.2628\sym{***}&     -0.0339\sym{***}&     -0.0256\sym{***}\\
                    &   (94.0872)         &   (53.5579)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=28&  -8082.5158\sym{***}&  -1109.8813\sym{***}&     -0.0168\sym{***}&     -0.0257\sym{***}\\
                    &   (93.1922)         &   (53.5492)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=29&  -7910.5932\sym{***}&   -959.9131\sym{***}&     -0.0401\sym{***}&     -0.0171\sym{***}\\
                    &   (93.3617)         &   (53.2995)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=30&  -7750.3309\sym{***}&   -782.3377\sym{***}&     -0.0271\sym{***}&     -0.0172\sym{***}\\
                    &   (97.7161)         &   (54.9411)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=31&  -7009.7058\sym{***}&   -636.2007\sym{***}&     -0.0268\sym{***}&     -0.0200\sym{***}\\
                    &   (99.7303)         &   (54.5513)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=32&  -7641.0010\sym{***}&  -1037.3052\sym{***}&     -0.0512\sym{***}&     -0.0219\sym{***}\\
                    &   (99.6596)         &   (55.1030)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=33&  -7614.5620\sym{***}&   -963.9328\sym{***}&     -0.0376\sym{***}&     -0.0192\sym{***}\\
                    &  (100.7133)         &   (55.1163)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=34&  -7422.3764\sym{***}&   -935.9427\sym{***}&     -0.0214\sym{***}&     -0.0178\sym{***}\\
                    &  (101.2031)         &   (55.0199)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=35&  -7771.9841\sym{***}&  -1016.4363\sym{***}&     -0.0118\sym{***}&     -0.0135\sym{***}\\
                    &  (100.8878)         &   (54.6540)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=36&  -8184.6803\sym{***}&  -1323.1944\sym{***}&     -0.0446\sym{***}&     -0.0086\sym{***}\\
                    &  (100.6674)         &   (54.7130)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=37&  -7903.9919\sym{***}&  -1251.4862\sym{***}&     -0.0392\sym{***}&     -0.0056\sym{***}\\
                    &  (101.2310)         &   (54.8182)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=38&  -7655.2392\sym{***}&  -1118.1474\sym{***}&     -0.0345\sym{***}&     -0.0020\sym{*}  \\
                    &  (101.8143)         &   (55.2007)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=39&  -6737.4032\sym{***}&   -890.6152\sym{***}&      0.0543\sym{***}&     -0.0030\sym{***}\\
                    &  (103.5186)         &   (55.9744)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin=4 $\times$ quarter=40&  -7910.0946\sym{***}&  -1496.0201\sym{***}&     -0.0436\sym{***}&     -0.0016         \\
                    &  (103.3161)         &   (56.0487)         &    (0.0012)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=41&  -7376.8743\sym{***}&  -1213.9970\sym{***}&     -0.0324\sym{***}&      0.0032\sym{***}\\
                    &  (104.0269)         &   (56.0086)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=42&  -6850.0665\sym{***}&   -942.3860\sym{***}&     -0.0336\sym{***}&      0.0046\sym{***}\\
                    &  (104.9252)         &   (56.7611)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=43&  -6193.7874\sym{***}&   -621.8164\sym{***}&     -0.0238\sym{***}&      0.0020\sym{*}  \\
                    &  (107.0213)         &   (57.2482)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=44&  -7633.5863\sym{***}&  -1354.1249\sym{***}&     -0.0563\sym{***}&     -0.0003         \\
                    &  (107.2671)         &   (57.8646)         &    (0.0012)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=45&  -7109.3222\sym{***}&  -1157.1071\sym{***}&     -0.0382\sym{***}&      0.0064\sym{***}\\
                    &  (108.5952)         &   (58.1535)         &    (0.0012)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=46&  -6574.9018\sym{***}&   -888.5292\sym{***}&     -0.0389\sym{***}&      0.0073\sym{***}\\
                    &  (110.0393)         &   (58.9934)         &    (0.0012)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=47&  -5766.1993\sym{***}&   -598.6664\sym{***}&     -0.0273\sym{***}&      0.0033\sym{***}\\
                    &  (111.7255)         &   (59.5584)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=48&  -7042.1042\sym{***}&  -1368.2016\sym{***}&     -0.0341\sym{***}&      0.0062\sym{***}\\
                    &  (112.7194)         &   (60.3621)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin=4 $\times$ quarter=49&  -6653.4495\sym{***}&  -1215.8825\sym{***}&     -0.0048\sym{***}&      0.0143\sym{***}\\
                    &  (115.1030)         &   (61.5912)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin=5 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=5 $\times$ quarter=9&    279.3648\sym{***}&    324.0431\sym{***}&      0.0008         &      0.0014\sym{**} \\
                    &   (45.6794)         &   (14.8684)         &    (0.0014)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=10&    541.4157\sym{***}&    380.3933\sym{***}&      0.0886\sym{***}&      0.0025\sym{***}\\
                    &   (55.3238)         &   (17.2457)         &    (0.0015)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=11&    524.9519\sym{***}&    595.4557\sym{***}&      0.0688\sym{***}&      0.0043\sym{***}\\
                    &   (61.5583)         &   (18.4952)         &    (0.0016)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=12&  -2230.6516\sym{***}&     -2.4550         &     -0.0439\sym{***}&      0.0063\sym{***}\\
                    &   (65.3499)         &   (19.3600)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=13&   1135.7843\sym{***}&    476.6714\sym{***}&      0.2652\sym{***}&      0.0067\sym{***}\\
                    &   (66.9507)         &   (19.9714)         &    (0.0017)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=14&   2256.9390\sym{***}&    450.8079\sym{***}&      0.0198\sym{***}&      0.0058\sym{***}\\
                    &   (69.6008)         &   (20.4860)         &    (0.0014)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=15&   2742.0241\sym{***}&    746.1347\sym{***}&      0.0359\sym{***}&      0.0030\sym{***}\\
                    &   (73.2377)         &   (20.8674)         &    (0.0014)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=16&   1059.3805\sym{***}&    113.6432\sym{***}&     -0.0018         &      0.0035\sym{***}\\
                    &   (74.9148)         &   (21.0380)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=17&   3588.7361\sym{***}&    356.8330\sym{***}&      0.1494\sym{***}&      0.0048\sym{***}\\
                    &   (78.9574)         &   (21.4448)         &    (0.0015)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=18&   4185.2645\sym{***}&    350.3889\sym{***}&      0.0216\sym{***}&      0.0048\sym{***}\\
                    &   (82.0622)         &   (21.6096)         &    (0.0014)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=19&   1228.4561\sym{***}&    294.2195\sym{***}&     -0.0488\sym{***}&     -0.0009         \\
                    &   (82.4578)         &   (22.0921)         &    (0.0012)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=20&  -3582.4514\sym{***}&   -309.8609\sym{***}&     -0.0504\sym{***}&     -0.0028\sym{***}\\
                    &   (82.0473)         &   (21.8012)         &    (0.0012)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=21&  -4859.7028\sym{***}&    -46.3602\sym{**} &     -0.0251\sym{***}&     -0.0002         \\
                    &   (83.6693)         &   (21.7398)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=22&  -5512.7647\sym{***}&     -6.1362         &     -0.0409\sym{***}&     -0.0029\sym{***}\\
                    &   (84.6148)         &   (22.0504)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=23&  -5548.6136\sym{***}&    154.4445\sym{***}&     -0.0242\sym{***}&     -0.0067\sym{***}\\
                    &   (85.8498)         &   (22.1904)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=24&  -6476.5699\sym{***}&   -284.2848\sym{***}&     -0.0466\sym{***}&     -0.0058\sym{***}\\
                    &   (85.7242)         &   (21.8369)         &    (0.0012)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=25&  -7008.7994\sym{***}&     54.0276\sym{**} &     -0.0250\sym{***}&     -0.0031\sym{***}\\
                    &   (86.2698)         &   (22.1477)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=26&  -7022.9056\sym{***}&     71.0166\sym{***}&     -0.0381\sym{***}&     -0.0030\sym{***}\\
                    &   (87.3522)         &   (22.3663)         &    (0.0012)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=27&  -6825.8979\sym{***}&    385.4390\sym{***}&     -0.0256\sym{***}&     -0.0032\sym{***}\\
                    &   (88.6730)         &   (23.4752)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=28&  -6746.8753\sym{***}&   -177.7072\sym{***}&      0.0297\sym{***}&     -0.0028\sym{***}\\
                    &   (88.3228)         &   (22.5963)         &    (0.0015)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=29&  -6148.3195\sym{***}&    203.1829\sym{***}&     -0.0297\sym{***}&      0.0019\sym{**} \\
                    &   (89.9946)         &   (22.9815)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=30&  -5998.9657\sym{***}&    209.6040\sym{***}&     -0.0225\sym{***}&      0.0013\sym{*}  \\
                    &   (94.5653)         &   (23.9321)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=31&  -4170.2446\sym{***}&    505.7634\sym{***}&     -0.0216\sym{***}&      0.0040\sym{***}\\
                    &   (98.9921)         &   (24.0457)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=32&  -4803.2361\sym{***}&   -120.9425\sym{***}&     -0.0441\sym{***}&      0.0022\sym{***}\\
                    &   (98.7654)         &   (23.5990)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=33&  -4440.1588\sym{***}&    166.3424\sym{***}&     -0.0282\sym{***}&      0.0020\sym{***}\\
                    &  (100.4244)         &   (24.0132)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=34&  -3927.7855\sym{***}&    201.3783\sym{***}&     -0.0156\sym{***}&      0.0009         \\
                    &  (102.6946)         &   (24.3339)         &    (0.0013)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=35&  -4066.6024\sym{***}&    446.9422\sym{***}&      0.0018         &      0.0061\sym{***}\\
                    &  (102.3055)         &   (24.9459)         &    (0.0014)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=36&  -4406.9127\sym{***}&    -91.0658\sym{***}&     -0.0317\sym{***}&      0.0095\sym{***}\\
                    &  (101.6047)         &   (23.9168)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=37&  -4012.6083\sym{***}&    270.9395\sym{***}&     -0.0247\sym{***}&      0.0110\sym{***}\\
                    &  (103.1083)         &   (24.7743)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=38&  -3657.5880\sym{***}&    207.9952\sym{***}&     -0.0345\sym{***}&      0.0109\sym{***}\\
                    &  (104.5746)         &   (24.3634)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=39&  -2604.1760\sym{***}&    489.1829\sym{***}&      0.0570\sym{***}&      0.0128\sym{***}\\
                    &  (105.3863)         &   (24.7848)         &    (0.0014)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=40&  -3449.7959\sym{***}&   -152.1367\sym{***}&     -0.0382\sym{***}&      0.0110\sym{***}\\
                    &  (104.2795)         &   (24.2820)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=41&  -3022.8788\sym{***}&    283.3742\sym{***}&     -0.0295\sym{***}&      0.0116\sym{***}\\
                    &  (106.4478)         &   (24.9408)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=42&  -2916.2072\sym{***}&    234.0248\sym{***}&     -0.0376\sym{***}&      0.0103\sym{***}\\
                    &  (106.7707)         &   (24.9833)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=43&  -2432.7413\sym{***}&    649.9246\sym{***}&     -0.0283\sym{***}&      0.0113\sym{***}\\
                    &  (109.1082)         &   (25.3271)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=44&  -3638.5923\sym{***}&   -202.1248\sym{***}&     -0.0539\sym{***}&      0.0099\sym{***}\\
                    &  (108.5366)         &   (24.6234)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=45&  -3112.7577\sym{***}&    231.6255\sym{***}&     -0.0390\sym{***}&      0.0135\sym{***}\\
                    &  (110.7832)         &   (25.2975)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=46&  -2882.3282\sym{***}&    237.1496\sym{***}&     -0.0398\sym{***}&      0.0143\sym{***}\\
                    &  (111.6047)         &   (25.9248)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=47&  -2523.0063\sym{***}&    433.0314\sym{***}&     -0.0368\sym{***}&      0.0123\sym{***}\\
                    &  (112.3916)         &   (26.0762)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=48&  -3366.4456\sym{***}&   -238.3067\sym{***}&     -0.0376\sym{***}&      0.0158\sym{***}\\
                    &  (112.6912)         &   (25.3833)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=49&  -3065.5479\sym{***}&    134.8880\sym{***}&     -0.0053\sym{***}&      0.0193\sym{***}\\
                    &  (114.4161)         &   (26.2185)         &    (0.0013)         &    (0.0008)         \\
[1em]
Constant            &  -6601.1884\sym{***}&  -9543.9801\sym{***}&      0.1362\sym{***}&      0.3410\sym{***}\\
                    &  (271.5330)         &  (292.7983)         &    (0.0035)         &    (0.0052)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         \\
Observations        &18318847.0000         &18318847.0000         &18318847.0000         &18318847.0000         \\
$R^2$               &      0.3319         &      0.3006         &      0.0288         &      0.0514         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize }\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Tables/old/regressions_detail/credit_card_reg_l1.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{credit\_limit}&\multicolumn{1}{c}{cc\_balances}&\multicolumn{1}{c}{cc\_origination}&\multicolumn{1}{c}{inquiry}\\
\hline
cs\_bin\_l1=1         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=2         &  -1640.9595\sym{***}&     16.3517         &      0.1055\sym{***}&      0.0491\sym{***}\\
                    &  (279.2652)         &  (292.9727)         &    (0.0045)         &    (0.0054)         \\
[1em]
cs\_bin\_l1=3         &  -4417.9000\sym{***}&  -2466.5483\sym{***}&      0.1304\sym{***}&      0.0124\sym{**} \\
                    &  (330.0184)         &  (326.7972)         &    (0.0045)         &    (0.0054)         \\
[1em]
cs\_bin\_l1=4         &   -277.4509         &   2427.4524\sym{***}&      0.0427\sym{***}&     -0.1240\sym{***}\\
                    &  (282.5329)         &  (284.3776)         &    (0.0043)         &    (0.0051)         \\
[1em]
cs\_bin\_l1=5         &  27235.8444\sym{***}&   9777.2822\sym{***}&      0.0244\sym{***}&     -0.1690\sym{***}\\
                    &  (339.0496)         &  (275.4204)         &    (0.0043)         &    (0.0051)         \\
[1em]
cs\_bin\_l1=1 $\times$ age&     64.2037\sym{***}&     81.1534\sym{***}&     -0.0006\sym{***}&     -0.0012\sym{***}\\
                    &    (4.8318)         &    (4.6491)         &    (0.0000)         &    (0.0001)         \\
[1em]
cs\_bin\_l1=2 $\times$ age&     85.9518\sym{***}&     86.9124\sym{***}&     -0.0012\sym{***}&     -0.0017\sym{***}\\
                    &    (3.7522)         &    (3.3163)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=3 $\times$ age&    163.6333\sym{***}&    134.1379\sym{***}&     -0.0012\sym{***}&     -0.0014\sym{***}\\
                    &    (4.9066)         &    (3.9749)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=4 $\times$ age&    257.8329\sym{***}&    110.7348\sym{***}&     -0.0003\sym{***}&     -0.0005\sym{***}\\
                    &    (3.4997)         &    (1.8023)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=5 $\times$ age&    -28.2741\sym{***}&    -57.4465\sym{***}&     -0.0006\sym{***}&     -0.0007\sym{***}\\
                    &    (3.7056)         &    (0.8401)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=1 $\times$ income\_insight\_score&    210.3832\sym{***}&    269.0078\sym{***}&     -0.0004\sym{***}&      0.0004\sym{***}\\
                    &    (4.1019)         &    (4.9993)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=2 $\times$ income\_insight\_score&    319.3543\sym{***}&    288.6192\sym{***}&     -0.0006\sym{***}&     -0.0003\sym{***}\\
                    &    (3.6164)         &    (3.3134)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=3 $\times$ income\_insight\_score&    500.4224\sym{***}&    375.8657\sym{***}&     -0.0004\sym{***}&     -0.0002\sym{***}\\
                    &    (3.5315)         &    (2.9651)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=4 $\times$ income\_insight\_score&    358.5546\sym{***}&    152.4451\sym{***}&     -0.0001\sym{***}&      0.0001\sym{***}\\
                    &    (1.7693)         &    (1.0413)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=5 $\times$ income\_insight\_score&    206.2127\sym{***}&     43.6117\sym{***}&     -0.0001\sym{***}&      0.0000\sym{***}\\
                    &    (1.2161)         &    (0.3712)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=10&   -495.3119\sym{***}&   -628.2006\sym{***}&      0.0075         &     -0.0060         \\
                    &  (177.6749)         &  (222.4426)         &    (0.0052)         &    (0.0059)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=11&   -923.5037\sym{***}&  -1183.0791\sym{***}&      0.0036         &      0.0235\sym{***}\\
                    &  (204.9590)         &  (254.7389)         &    (0.0052)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=12&     75.0868         &    -33.4543         &      0.0063         &      0.0992\sym{***}\\
                    &  (216.6059)         &  (272.0399)         &    (0.0051)         &    (0.0065)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=13&    153.6353         &    -17.0452         &      0.0491\sym{***}&      0.0320\sym{***}\\
                    &  (221.0695)         &  (275.8277)         &    (0.0054)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=14&   -588.4756\sym{***}&   -727.5948\sym{***}&      0.0259\sym{***}&      0.0305\sym{***}\\
                    &  (212.0798)         &  (254.7426)         &    (0.0051)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=15&   -698.8862\sym{***}&   -610.3299\sym{**} &     -0.0175\sym{***}&     -0.0053         \\
                    &  (215.1007)         &  (264.1918)         &    (0.0047)         &    (0.0057)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=16&    143.4543         &    347.2846         &     -0.0537\sym{***}&      0.0371\sym{***}\\
                    &  (212.5558)         &  (257.6637)         &    (0.0045)         &    (0.0059)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=17&    180.8176         &    456.8231\sym{*}  &     -0.0277\sym{***}&     -0.0307\sym{***}\\
                    &  (221.6679)         &  (273.6198)         &    (0.0047)         &    (0.0057)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=18&    292.4684         &    772.9880\sym{***}&     -0.0549\sym{***}&     -0.0344\sym{***}\\
                    &  (230.4443)         &  (282.3085)         &    (0.0045)         &    (0.0057)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=19&   -216.3272         &    634.6244\sym{**} &     -0.0616\sym{***}&     -0.0384\sym{***}\\
                    &  (230.6891)         &  (289.5861)         &    (0.0045)         &    (0.0058)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=20&    782.2909\sym{***}&   2209.7670\sym{***}&     -0.0631\sym{***}&     -0.0297\sym{***}\\
                    &  (237.3026)         &  (297.7152)         &    (0.0045)         &    (0.0058)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=21&   1076.4047\sym{***}&   2674.9043\sym{***}&     -0.0662\sym{***}&     -0.0751\sym{***}\\
                    &  (249.0023)         &  (319.0452)         &    (0.0045)         &    (0.0056)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=22&    134.3564         &   1379.8763\sym{***}&     -0.0617\sym{***}&     -0.0951\sym{***}\\
                    &  (250.2835)         &  (320.3475)         &    (0.0045)         &    (0.0056)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=23&   -266.2980         &    762.0006\sym{**} &     -0.0492\sym{***}&     -0.0980\sym{***}\\
                    &  (255.2065)         &  (318.6921)         &    (0.0047)         &    (0.0056)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=24&   -177.6139         &    862.7562\sym{***}&     -0.0718\sym{***}&     -0.0742\sym{***}\\
                    &  (251.3463)         &  (312.4673)         &    (0.0044)         &    (0.0058)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=25&   -942.7902\sym{***}&    -45.3486         &     -0.0550\sym{***}&     -0.0875\sym{***}\\
                    &  (261.6400)         &  (324.5462)         &    (0.0048)         &    (0.0059)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=26&  -1552.6950\sym{***}&  -1087.2731\sym{***}&     -0.0609\sym{***}&     -0.0847\sym{***}\\
                    &  (270.3014)         &  (331.9178)         &    (0.0048)         &    (0.0060)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=27&  -1900.9599\sym{***}&  -1738.0864\sym{***}&     -0.0459\sym{***}&     -0.0847\sym{***}\\
                    &  (273.1713)         &  (329.5311)         &    (0.0050)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=28&  -1895.4058\sym{***}&  -1919.9365\sym{***}&     -0.0371\sym{***}&     -0.0920\sym{***}\\
                    &  (258.9853)         &  (312.2797)         &    (0.0052)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=29&  -2641.1964\sym{***}&  -3004.6656\sym{***}&     -0.0451\sym{***}&     -0.1018\sym{***}\\
                    &  (253.6852)         &  (297.2986)         &    (0.0052)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=30&  -3285.2458\sym{***}&  -3799.2335\sym{***}&     -0.0410\sym{***}&     -0.1000\sym{***}\\
                    &  (267.3500)         &  (302.0336)         &    (0.0052)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=31&  -3325.8278\sym{***}&  -3833.7115\sym{***}&     -0.0376\sym{***}&     -0.0942\sym{***}\\
                    &  (253.8043)         &  (289.7025)         &    (0.0052)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=32&  -2714.7926\sym{***}&  -2980.5361\sym{***}&     -0.0437\sym{***}&     -0.0985\sym{***}\\
                    &  (243.9682)         &  (289.6046)         &    (0.0052)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=33&  -2757.3041\sym{***}&  -3202.0843\sym{***}&     -0.0314\sym{***}&     -0.1017\sym{***}\\
                    &  (247.1456)         &  (285.0865)         &    (0.0054)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=34&  -3245.9117\sym{***}&  -3894.6571\sym{***}&     -0.0447\sym{***}&     -0.0992\sym{***}\\
                    &  (250.9311)         &  (288.1621)         &    (0.0052)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=35&  -3034.3876\sym{***}&  -3641.5307\sym{***}&     -0.0473\sym{***}&     -0.0874\sym{***}\\
                    &  (234.8823)         &  (271.1262)         &    (0.0051)         &    (0.0060)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=36&  -3246.7141\sym{***}&  -3837.2772\sym{***}&     -0.0667\sym{***}&     -0.1040\sym{***}\\
                    &  (233.7815)         &  (272.4260)         &    (0.0048)         &    (0.0060)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=37&  -3204.4521\sym{***}&  -3805.4208\sym{***}&     -0.0541\sym{***}&     -0.0972\sym{***}\\
                    &  (235.9948)         &  (273.9940)         &    (0.0050)         &    (0.0061)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=38&  -3638.9850\sym{***}&  -4248.7261\sym{***}&     -0.0057         &     -0.0892\sym{***}\\
                    &  (239.9691)         &  (277.1901)         &    (0.0057)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=39&  -3557.9284\sym{***}&  -4300.0372\sym{***}&     -0.0194\sym{***}&     -0.0814\sym{***}\\
                    &  (234.4736)         &  (268.3744)         &    (0.0055)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=40&  -3259.7662\sym{***}&  -4038.9211\sym{***}&     -0.0500\sym{***}&     -0.0817\sym{***}\\
                    &  (235.6895)         &  (276.4102)         &    (0.0051)         &    (0.0062)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=41&  -3349.3833\sym{***}&  -4154.2825\sym{***}&     -0.0312\sym{***}&     -0.0713\sym{***}\\
                    &  (241.0352)         &  (280.3787)         &    (0.0054)         &    (0.0064)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=42&  -3323.0490\sym{***}&  -3956.8287\sym{***}&     -0.0331\sym{***}&     -0.0620\sym{***}\\
                    &  (243.1564)         &  (285.2133)         &    (0.0054)         &    (0.0064)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=43&  -3367.4530\sym{***}&  -3974.4428\sym{***}&     -0.0153\sym{***}&     -0.0463\sym{***}\\
                    &  (239.2041)         &  (282.6778)         &    (0.0054)         &    (0.0064)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=44&  -2806.8979\sym{***}&  -3496.1684\sym{***}&     -0.0363\sym{***}&     -0.0535\sym{***}\\
                    &  (236.2002)         &  (276.9988)         &    (0.0051)         &    (0.0063)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=45&  -2832.9578\sym{***}&  -3633.2114\sym{***}&     -0.0244\sym{***}&     -0.0593\sym{***}\\
                    &  (240.5145)         &  (283.7902)         &    (0.0054)         &    (0.0064)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=46&  -3234.8786\sym{***}&  -4102.5954\sym{***}&     -0.0315\sym{***}&     -0.0571\sym{***}\\
                    &  (237.6338)         &  (274.9892)         &    (0.0052)         &    (0.0064)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=47&  -3307.4433\sym{***}&  -4129.2509\sym{***}&     -0.0343\sym{***}&     -0.0501\sym{***}\\
                    &  (235.4257)         &  (269.1847)         &    (0.0052)         &    (0.0064)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=48&  -2515.7265\sym{***}&  -3362.9647\sym{***}&     -0.0236\sym{***}&     -0.0520\sym{***}\\
                    &  (233.6875)         &  (263.9653)         &    (0.0052)         &    (0.0063)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=49&  -2416.5803\sym{***}&  -3168.0077\sym{***}&     -0.0159\sym{***}&     -0.0433\sym{***}\\
                    &  (272.4869)         &  (305.1726)         &    (0.0054)         &    (0.0065)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=10&   -266.6411\sym{**} &    -98.9215         &      0.0166\sym{***}&      0.0059\sym{**} \\
                    &  (109.3634)         &   (96.6270)         &    (0.0026)         &    (0.0024)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=11&   -245.9673\sym{**} &   -299.2256\sym{***}&      0.0221\sym{***}&      0.0181\sym{***}\\
                    &  (119.9042)         &  (102.6814)         &    (0.0026)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=12&   -301.9017\sym{**} &   -317.8845\sym{***}&     -0.0087\sym{***}&      0.0564\sym{***}\\
                    &  (122.3603)         &  (105.6280)         &    (0.0025)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=13&     57.1192         &    -65.7992         &      0.0851\sym{***}&      0.0238\sym{***}\\
                    &  (127.2001)         &  (110.2384)         &    (0.0027)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=14&    -17.5929         &    -46.3895         &      0.0216\sym{***}&      0.0261\sym{***}\\
                    &  (133.1451)         &  (116.2001)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=15&      4.6043         &     81.1588         &      0.0042\sym{*}  &      0.0005         \\
                    &  (134.9933)         &  (117.6533)         &    (0.0025)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=16&    716.7759\sym{***}&    646.8257\sym{***}&     -0.0334\sym{***}&      0.0125\sym{***}\\
                    &  (139.7027)         &  (121.0984)         &    (0.0024)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=17&    861.6841\sym{***}&    808.7250\sym{***}&      0.0045\sym{*}  &     -0.0203\sym{***}\\
                    &  (143.3465)         &  (124.6546)         &    (0.0025)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=18&    824.0533\sym{***}&    993.4895\sym{***}&     -0.0501\sym{***}&     -0.0321\sym{***}\\
                    &  (147.4910)         &  (130.1720)         &    (0.0024)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=19&    335.6225\sym{**} &   1211.7559\sym{***}&     -0.0718\sym{***}&     -0.0441\sym{***}\\
                    &  (148.6686)         &  (133.4432)         &    (0.0023)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=20&    645.5215\sym{***}&   1663.2023\sym{***}&     -0.0890\sym{***}&     -0.0508\sym{***}\\
                    &  (145.2168)         &  (132.6790)         &    (0.0023)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=21&    -44.0091         &   1318.7345\sym{***}&     -0.0995\sym{***}&     -0.0817\sym{***}\\
                    &  (149.8739)         &  (136.8799)         &    (0.0023)         &    (0.0024)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=22&  -1065.8324\sym{***}&    723.1006\sym{***}&     -0.1026\sym{***}&     -0.0916\sym{***}\\
                    &  (147.6379)         &  (135.2218)         &    (0.0023)         &    (0.0024)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=23&  -1618.1654\sym{***}&    305.3819\sym{**} &     -0.0930\sym{***}&     -0.0946\sym{***}\\
                    &  (147.6172)         &  (135.9399)         &    (0.0023)         &    (0.0024)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=24&  -2057.0819\sym{***}&   -202.3207         &     -0.1092\sym{***}&     -0.0766\sym{***}\\
                    &  (143.6331)         &  (130.6850)         &    (0.0023)         &    (0.0024)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=25&  -2822.0455\sym{***}&   -869.5176\sym{***}&     -0.0815\sym{***}&     -0.0875\sym{***}\\
                    &  (147.9308)         &  (134.2590)         &    (0.0024)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=26&  -3624.9499\sym{***}&  -1639.6641\sym{***}&     -0.0881\sym{***}&     -0.0765\sym{***}\\
                    &  (146.7106)         &  (132.8454)         &    (0.0024)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=27&  -4170.3365\sym{***}&  -2258.6288\sym{***}&     -0.0685\sym{***}&     -0.0686\sym{***}\\
                    &  (148.9730)         &  (134.0179)         &    (0.0024)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=28&  -4469.2024\sym{***}&  -2787.4630\sym{***}&     -0.0730\sym{***}&     -0.0729\sym{***}\\
                    &  (144.1100)         &  (128.7372)         &    (0.0024)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=29&  -4913.9172\sym{***}&  -3272.3011\sym{***}&     -0.0630\sym{***}&     -0.0613\sym{***}\\
                    &  (146.6156)         &  (131.2272)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=30&  -5458.5922\sym{***}&  -3845.3563\sym{***}&     -0.0435\sym{***}&     -0.0679\sym{***}\\
                    &  (147.9987)         &  (131.6839)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=31&  -5330.7641\sym{***}&  -3554.8809\sym{***}&     -0.0403\sym{***}&     -0.0647\sym{***}\\
                    &  (149.8580)         &  (132.4532)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=32&  -4698.6750\sym{***}&  -3222.1573\sym{***}&     -0.0581\sym{***}&     -0.0762\sym{***}\\
                    &  (148.9171)         &  (132.5327)         &    (0.0025)         &    (0.0025)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=33&  -4856.6349\sym{***}&  -3485.5261\sym{***}&     -0.0422\sym{***}&     -0.0698\sym{***}\\
                    &  (151.3834)         &  (133.8637)         &    (0.0026)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=34&  -4887.3611\sym{***}&  -3622.8239\sym{***}&     -0.0400\sym{***}&     -0.0668\sym{***}\\
                    &  (153.3240)         &  (134.1261)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=35&  -4877.4303\sym{***}&  -3607.1012\sym{***}&     -0.0336\sym{***}&     -0.0590\sym{***}\\
                    &  (151.1880)         &  (132.7939)         &    (0.0026)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=36&  -4869.8370\sym{***}&  -3781.9503\sym{***}&     -0.0603\sym{***}&     -0.0673\sym{***}\\
                    &  (152.8186)         &  (133.9142)         &    (0.0025)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=37&  -4853.2909\sym{***}&  -3783.5849\sym{***}&     -0.0547\sym{***}&     -0.0603\sym{***}\\
                    &  (153.5555)         &  (134.3708)         &    (0.0026)         &    (0.0026)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=38&  -4922.2083\sym{***}&  -3795.2471\sym{***}&     -0.0078\sym{***}&     -0.0492\sym{***}\\
                    &  (153.3886)         &  (134.5182)         &    (0.0027)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=39&  -4508.0341\sym{***}&  -3502.6497\sym{***}&      0.0286\sym{***}&     -0.0365\sym{***}\\
                    &  (153.6535)         &  (135.0008)         &    (0.0028)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=40&  -4627.6237\sym{***}&  -3818.3088\sym{***}&     -0.0414\sym{***}&     -0.0405\sym{***}\\
                    &  (155.0815)         &  (134.6610)         &    (0.0026)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=41&  -4620.4424\sym{***}&  -3792.5867\sym{***}&     -0.0279\sym{***}&     -0.0276\sym{***}\\
                    &  (158.9673)         &  (137.9546)         &    (0.0026)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=42&  -4402.6857\sym{***}&  -3586.9130\sym{***}&     -0.0183\sym{***}&     -0.0185\sym{***}\\
                    &  (158.8939)         &  (137.7277)         &    (0.0026)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=43&  -3987.0452\sym{***}&  -3259.6111\sym{***}&      0.0104\sym{***}&     -0.0020         \\
                    &  (158.3169)         &  (137.6768)         &    (0.0027)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=44&  -4142.9996\sym{***}&  -3551.5975\sym{***}&     -0.0251\sym{***}&     -0.0162\sym{***}\\
                    &  (155.0239)         &  (133.8229)         &    (0.0026)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=45&  -4264.7082\sym{***}&  -3645.1690\sym{***}&      0.0013         &     -0.0069\sym{**} \\
                    &  (155.1129)         &  (134.3610)         &    (0.0027)         &    (0.0028)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=46&  -4054.8755\sym{***}&  -3408.7644\sym{***}&     -0.0039         &      0.0029         \\
                    &  (157.4153)         &  (136.2834)         &    (0.0027)         &    (0.0028)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=47&  -3489.2410\sym{***}&  -2991.7359\sym{***}&      0.0123\sym{***}&      0.0041         \\
                    &  (159.0915)         &  (136.9006)         &    (0.0027)         &    (0.0028)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=48&  -3270.9761\sym{***}&  -3003.9947\sym{***}&      0.0032         &      0.0003         \\
                    &  (159.0521)         &  (135.6386)         &    (0.0027)         &    (0.0027)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=49&  -3159.6280\sym{***}&  -2863.4177\sym{***}&      0.0240\sym{***}&      0.0176\sym{***}\\
                    &  (159.2237)         &  (137.1378)         &    (0.0027)         &    (0.0028)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=10&      9.8492         &     27.7422         &      0.0330\sym{***}&      0.0085\sym{***}\\
                    &  (128.2346)         &   (96.9691)         &    (0.0024)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=11&    102.1012         &    -49.0511         &      0.0369\sym{***}&      0.0102\sym{***}\\
                    &  (153.9013)         &  (115.7205)         &    (0.0025)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=12&   -794.5263\sym{***}&   -735.1456\sym{***}&     -0.0295\sym{***}&      0.0201\sym{***}\\
                    &  (154.4353)         &  (117.9597)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=13&    289.7023\sym{*}  &    -56.0521         &      0.1392\sym{***}&      0.0133\sym{***}\\
                    &  (161.7111)         &  (123.8561)         &    (0.0026)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=14&    816.7095\sym{***}&    527.9840\sym{***}&      0.0202\sym{***}&      0.0168\sym{***}\\
                    &  (170.3412)         &  (130.6598)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=15&   1684.7851\sym{***}&   1208.9704\sym{***}&      0.0166\sym{***}&     -0.0062\sym{***}\\
                    &  (180.5055)         &  (137.3396)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=16&   1095.0081\sym{***}&    812.2244\sym{***}&     -0.0159\sym{***}&     -0.0117\sym{***}\\
                    &  (180.2382)         &  (137.8728)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=17&   1668.4864\sym{***}&   1249.6273\sym{***}&      0.0379\sym{***}&     -0.0195\sym{***}\\
                    &  (184.7796)         &  (141.3169)         &    (0.0025)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=18&   1576.8155\sym{***}&   1700.7444\sym{***}&     -0.0248\sym{***}&     -0.0264\sym{***}\\
                    &  (189.8086)         &  (145.4561)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=19&    779.6855\sym{***}&   2156.1699\sym{***}&     -0.0634\sym{***}&     -0.0378\sym{***}\\
                    &  (190.9744)         &  (150.1401)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=20&      2.6682         &   1917.4258\sym{***}&     -0.0857\sym{***}&     -0.0592\sym{***}\\
                    &  (186.4908)         &  (147.2560)         &    (0.0022)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=21&  -1256.8743\sym{***}&   1506.3536\sym{***}&     -0.1018\sym{***}&     -0.0691\sym{***}\\
                    &  (185.5393)         &  (147.2030)         &    (0.0022)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=22&  -2513.2085\sym{***}&   1103.7084\sym{***}&     -0.1121\sym{***}&     -0.0753\sym{***}\\
                    &  (185.9090)         &  (149.0906)         &    (0.0022)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=23&  -3578.0300\sym{***}&    606.2145\sym{***}&     -0.0925\sym{***}&     -0.0802\sym{***}\\
                    &  (185.8529)         &  (148.3525)         &    (0.0022)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=24&  -4748.3124\sym{***}&   -393.1944\sym{***}&     -0.1142\sym{***}&     -0.0717\sym{***}\\
                    &  (183.6770)         &  (147.0586)         &    (0.0022)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=25&  -5591.7882\sym{***}&   -765.0441\sym{***}&     -0.0801\sym{***}&     -0.0696\sym{***}\\
                    &  (184.0984)         &  (147.8149)         &    (0.0023)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=26&  -6347.0200\sym{***}&  -1201.2014\sym{***}&     -0.0897\sym{***}&     -0.0593\sym{***}\\
                    &  (184.2226)         &  (147.0122)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=27&  -7050.3248\sym{***}&  -1897.6312\sym{***}&     -0.0657\sym{***}&     -0.0583\sym{***}\\
                    &  (184.7290)         &  (146.3141)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=28&  -7892.8992\sym{***}&  -2889.0799\sym{***}&     -0.0682\sym{***}&     -0.0658\sym{***}\\
                    &  (183.2274)         &  (144.7197)         &    (0.0023)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=29&  -8009.2226\sym{***}&  -2975.6721\sym{***}&     -0.0715\sym{***}&     -0.0493\sym{***}\\
                    &  (186.3502)         &  (146.1899)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=30&  -8225.1813\sym{***}&  -3072.0917\sym{***}&     -0.0514\sym{***}&     -0.0496\sym{***}\\
                    &  (189.7395)         &  (149.1408)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=31&  -8227.5712\sym{***}&  -3138.7745\sym{***}&     -0.0404\sym{***}&     -0.0511\sym{***}\\
                    &  (189.5693)         &  (149.2796)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=32&  -7895.8885\sym{***}&  -3319.7620\sym{***}&     -0.0762\sym{***}&     -0.0644\sym{***}\\
                    &  (187.7263)         &  (147.7284)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=33&  -7944.1755\sym{***}&  -3204.4104\sym{***}&     -0.0629\sym{***}&     -0.0584\sym{***}\\
                    &  (189.8222)         &  (147.6138)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=34&  -7973.8723\sym{***}&  -3450.0084\sym{***}&     -0.0398\sym{***}&     -0.0502\sym{***}\\
                    &  (190.9467)         &  (147.3192)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=35&  -8112.5388\sym{***}&  -3466.2745\sym{***}&     -0.0236\sym{***}&     -0.0428\sym{***}\\
                    &  (188.3269)         &  (146.3780)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=36&  -8205.2025\sym{***}&  -3902.9845\sym{***}&     -0.0627\sym{***}&     -0.0467\sym{***}\\
                    &  (188.0179)         &  (146.1036)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=37&  -8045.6353\sym{***}&  -3768.1826\sym{***}&     -0.0530\sym{***}&     -0.0360\sym{***}\\
                    &  (190.4529)         &  (147.7487)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=38&  -8093.2247\sym{***}&  -3736.3696\sym{***}&     -0.0327\sym{***}&     -0.0272\sym{***}\\
                    &  (190.9853)         &  (147.8667)         &    (0.0024)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=39&  -7506.5385\sym{***}&  -3425.3178\sym{***}&      0.0645\sym{***}&     -0.0202\sym{***}\\
                    &  (193.1711)         &  (148.6452)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=40&  -8243.7888\sym{***}&  -4261.1580\sym{***}&     -0.0497\sym{***}&     -0.0262\sym{***}\\
                    &  (193.1349)         &  (147.3551)         &    (0.0023)         &    (0.0022)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=41&  -7729.3821\sym{***}&  -3879.4727\sym{***}&     -0.0280\sym{***}&     -0.0100\sym{***}\\
                    &  (192.1011)         &  (147.8204)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=42&  -7518.3946\sym{***}&  -3658.8511\sym{***}&     -0.0212\sym{***}&     -0.0016         \\
                    &  (192.5092)         &  (147.5796)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=43&  -6832.6760\sym{***}&  -3135.2961\sym{***}&     -0.0037         &     -0.0005         \\
                    &  (195.5737)         &  (149.2325)         &    (0.0025)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=44&  -7906.7331\sym{***}&  -4354.7869\sym{***}&     -0.0485\sym{***}&     -0.0114\sym{***}\\
                    &  (194.7636)         &  (149.0442)         &    (0.0023)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=45&  -7612.5609\sym{***}&  -4062.4041\sym{***}&     -0.0174\sym{***}&      0.0001         \\
                    &  (194.8881)         &  (149.5951)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=46&  -7202.7438\sym{***}&  -3719.1129\sym{***}&     -0.0187\sym{***}&      0.0034         \\
                    &  (195.1960)         &  (149.2117)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=47&  -6550.5188\sym{***}&  -3299.7504\sym{***}&     -0.0002         &      0.0038         \\
                    &  (197.8753)         &  (150.9931)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=48&  -7227.1122\sym{***}&  -4127.7475\sym{***}&     -0.0193\sym{***}&     -0.0071\sym{***}\\
                    &  (199.4873)         &  (152.2537)         &    (0.0024)         &    (0.0023)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=49&  -7109.0702\sym{***}&  -4033.7574\sym{***}&      0.0125\sym{***}&      0.0138\sym{***}\\
                    &  (199.8478)         &  (153.2396)         &    (0.0025)         &    (0.0024)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=10&    417.6959\sym{***}&    300.9385\sym{***}&      0.0472\sym{***}&      0.0049\sym{***}\\
                    &   (54.0774)         &   (35.1151)         &    (0.0014)         &    (0.0009)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=11&    397.2448\sym{***}&    496.3106\sym{***}&      0.0348\sym{***}&      0.0026\sym{***}\\
                    &   (66.4240)         &   (41.1045)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=12&  -1768.7243\sym{***}&   -465.9866\sym{***}&     -0.0446\sym{***}&      0.0047\sym{***}\\
                    &   (70.9332)         &   (44.1314)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=13&    129.0544\sym{*}  &    198.9711\sym{***}&      0.1603\sym{***}&      0.0070\sym{***}\\
                    &   (74.4011)         &   (46.3634)         &    (0.0015)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=14&    989.1069\sym{***}&    571.8294\sym{***}&      0.0090\sym{***}&      0.0055\sym{***}\\
                    &   (79.3519)         &   (49.0955)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=15&   1546.9459\sym{***}&    914.0965\sym{***}&      0.0114\sym{***}&     -0.0073\sym{***}\\
                    &   (83.3018)         &   (50.9955)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=16&    245.2549\sym{***}&     57.0422         &     -0.0128\sym{***}&     -0.0082\sym{***}\\
                    &   (85.1390)         &   (53.4998)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=17&   1112.2991\sym{***}&    230.9410\sym{***}&      0.0795\sym{***}&     -0.0072\sym{***}\\
                    &   (85.8360)         &   (51.9715)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=18&   1136.8168\sym{***}&    675.9493\sym{***}&     -0.0086\sym{***}&     -0.0082\sym{***}\\
                    &   (88.7265)         &   (53.3411)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=19&   -156.2341\sym{*}  &    928.5331\sym{***}&     -0.0553\sym{***}&     -0.0203\sym{***}\\
                    &   (90.4211)         &   (54.8570)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=20&  -2699.5641\sym{***}&     29.7156         &     -0.0606\sym{***}&     -0.0311\sym{***}\\
                    &   (90.1305)         &   (54.5163)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=21&  -3948.3873\sym{***}&   -131.1919\sym{**} &     -0.0570\sym{***}&     -0.0288\sym{***}\\
                    &   (90.8326)         &   (54.7025)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=22&  -5009.6747\sym{***}&   -180.4149\sym{***}&     -0.0704\sym{***}&     -0.0295\sym{***}\\
                    &   (91.0786)         &   (54.7737)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=23&  -5563.7174\sym{***}&   -349.0516\sym{***}&     -0.0547\sym{***}&     -0.0386\sym{***}\\
                    &   (92.0994)         &   (54.7224)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=24&  -6965.7044\sym{***}&  -1138.3539\sym{***}&     -0.0782\sym{***}&     -0.0368\sym{***}\\
                    &   (92.2068)         &   (54.8890)         &    (0.0012)         &    (0.0009)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=25&  -7741.4363\sym{***}&  -1011.7287\sym{***}&     -0.0535\sym{***}&     -0.0301\sym{***}\\
                    &   (93.3357)         &   (54.7891)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=26&  -7993.5870\sym{***}&   -944.0863\sym{***}&     -0.0637\sym{***}&     -0.0231\sym{***}\\
                    &   (94.2001)         &   (55.7938)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=27&  -7938.8142\sym{***}&   -802.1612\sym{***}&     -0.0465\sym{***}&     -0.0272\sym{***}\\
                    &   (95.2848)         &   (55.9856)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=28&  -8590.6414\sym{***}&  -1653.1467\sym{***}&     -0.0280\sym{***}&     -0.0299\sym{***}\\
                    &   (94.3491)         &   (55.6572)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=29&  -8412.1041\sym{***}&  -1251.4970\sym{***}&     -0.0525\sym{***}&     -0.0191\sym{***}\\
                    &   (94.6578)         &   (55.8638)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=30&  -8198.6193\sym{***}&   -987.7569\sym{***}&     -0.0397\sym{***}&     -0.0189\sym{***}\\
                    &   (97.6160)         &   (56.7983)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=31&  -7403.7288\sym{***}&   -636.0862\sym{***}&     -0.0377\sym{***}&     -0.0209\sym{***}\\
                    &   (99.6572)         &   (57.4912)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=32&  -8115.7272\sym{***}&  -1525.5808\sym{***}&     -0.0655\sym{***}&     -0.0258\sym{***}\\
                    &  (101.1979)         &   (57.4612)         &    (0.0012)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=33&  -8028.5044\sym{***}&  -1207.9255\sym{***}&     -0.0519\sym{***}&     -0.0211\sym{***}\\
                    &  (101.1188)         &   (57.2835)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=34&  -7894.4701\sym{***}&  -1188.6128\sym{***}&     -0.0354\sym{***}&     -0.0201\sym{***}\\
                    &  (102.0130)         &   (57.2003)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=35&  -8256.0565\sym{***}&  -1110.2878\sym{***}&     -0.0245\sym{***}&     -0.0143\sym{***}\\
                    &  (101.6250)         &   (57.7382)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=36&  -8705.6224\sym{***}&  -1873.1886\sym{***}&     -0.0581\sym{***}&     -0.0122\sym{***}\\
                    &  (101.8096)         &   (56.9938)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=37&  -8380.3759\sym{***}&  -1441.6053\sym{***}&     -0.0512\sym{***}&     -0.0069\sym{***}\\
                    &  (102.5490)         &   (57.3267)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=38&  -8123.3440\sym{***}&  -1363.2217\sym{***}&     -0.0483\sym{***}&     -0.0047\sym{***}\\
                    &  (103.3369)         &   (57.9360)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=39&  -7271.4395\sym{***}&  -1076.5992\sym{***}&      0.0445\sym{***}&     -0.0040\sym{***}\\
                    &  (103.6447)         &   (57.8378)         &    (0.0014)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=40&  -8479.7627\sym{***}&  -2160.5228\sym{***}&     -0.0559\sym{***}&     -0.0053\sym{***}\\
                    &  (104.0547)         &   (57.9610)         &    (0.0013)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=41&  -7969.4250\sym{***}&  -1517.9493\sym{***}&     -0.0446\sym{***}&      0.0017         \\
                    &  (104.6195)         &   (58.2951)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=42&  -7366.7414\sym{***}&  -1258.4778\sym{***}&     -0.0449\sym{***}&      0.0023\sym{**} \\
                    &  (105.6984)         &   (58.8831)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=43&  -6672.7087\sym{***}&   -796.5096\sym{***}&     -0.0346\sym{***}&      0.0009         \\
                    &  (106.6266)         &   (59.2486)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=44&  -8292.4752\sym{***}&  -2113.1797\sym{***}&     -0.0694\sym{***}&     -0.0054\sym{***}\\
                    &  (109.1524)         &   (59.4899)         &    (0.0012)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=45&  -7578.9881\sym{***}&  -1415.8102\sym{***}&     -0.0500\sym{***}&      0.0043\sym{***}\\
                    &  (108.7544)         &   (60.1737)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=46&  -7046.4963\sym{***}&  -1134.9121\sym{***}&     -0.0486\sym{***}&      0.0060\sym{***}\\
                    &  (110.7338)         &   (60.5652)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=47&  -6306.4926\sym{***}&   -818.8638\sym{***}&     -0.0378\sym{***}&      0.0015         \\
                    &  (112.2996)         &   (61.8577)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=48&  -7638.5915\sym{***}&  -2001.2390\sym{***}&     -0.0458\sym{***}&      0.0029\sym{***}\\
                    &  (114.3651)         &   (63.0954)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=49&  -7159.2104\sym{***}&  -1469.8791\sym{***}&     -0.0157\sym{***}&      0.0120\sym{***}\\
                    &  (115.7014)         &   (63.6915)         &    (0.0013)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=10&    536.3066\sym{***}&    152.4261\sym{***}&      0.0861\sym{***}&      0.0027\sym{***}\\
                    &   (49.6753)         &   (21.6446)         &    (0.0015)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=11&    246.7739\sym{***}&    313.1729\sym{***}&      0.0653\sym{***}&      0.0029\sym{***}\\
                    &   (58.5410)         &   (23.2925)         &    (0.0017)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=12&  -2441.6189\sym{***}&   -409.8031\sym{***}&     -0.0463\sym{***}&      0.0050\sym{***}\\
                    &   (64.6439)         &   (23.5777)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=13&   1206.0821\sym{***}&    184.5241\sym{***}&      0.2502\sym{***}&      0.0061\sym{***}\\
                    &   (67.7627)         &   (24.9693)         &    (0.0018)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=14&   2159.0946\sym{***}&    159.2272\sym{***}&      0.0194\sym{***}&      0.0047\sym{***}\\
                    &   (70.1567)         &   (24.8917)         &    (0.0014)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=15&   2768.3196\sym{***}&    506.4013\sym{***}&      0.0332\sym{***}&      0.0020\sym{**} \\
                    &   (72.7792)         &   (25.5890)         &    (0.0014)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=16&   1030.1235\sym{***}&   -326.6751\sym{***}&     -0.0054\sym{***}&      0.0016\sym{**} \\
                    &   (75.7530)         &   (25.7718)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=17&   3388.5142\sym{***}&    -47.7890\sym{*}  &      0.1397\sym{***}&      0.0035\sym{***}\\
                    &   (79.4274)         &   (25.8526)         &    (0.0015)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=18&   4095.9737\sym{***}&    -15.1382         &      0.0202\sym{***}&      0.0036\sym{***}\\
                    &   (82.1493)         &   (26.1111)         &    (0.0014)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=19&   1016.7251\sym{***}&    -51.6306\sym{*}  &     -0.0521\sym{***}&     -0.0020\sym{***}\\
                    &   (83.1080)         &   (26.4861)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=20&  -3748.2039\sym{***}&   -781.6862\sym{***}&     -0.0566\sym{***}&     -0.0046\sym{***}\\
                    &   (82.7652)         &   (26.5500)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=21&  -5104.5203\sym{***}&   -522.0061\sym{***}&     -0.0295\sym{***}&     -0.0022\sym{***}\\
                    &   (85.0193)         &   (25.9791)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=22&  -5673.1635\sym{***}&   -441.1188\sym{***}&     -0.0438\sym{***}&     -0.0045\sym{***}\\
                    &   (84.7918)         &   (26.1155)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=23&  -5749.6780\sym{***}&   -261.2053\sym{***}&     -0.0271\sym{***}&     -0.0089\sym{***}\\
                    &   (85.8662)         &   (26.4875)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=24&  -6611.5138\sym{***}&   -848.9402\sym{***}&     -0.0508\sym{***}&     -0.0088\sym{***}\\
                    &   (86.2924)         &   (26.1405)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=25&  -7040.5062\sym{***}&   -353.7408\sym{***}&     -0.0283\sym{***}&     -0.0051\sym{***}\\
                    &   (86.7593)         &   (26.2861)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=26&  -6986.1241\sym{***}&   -315.1169\sym{***}&     -0.0399\sym{***}&     -0.0045\sym{***}\\
                    &   (87.4524)         &   (26.3065)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=27&  -6783.6002\sym{***}&    -26.2020         &     -0.0274\sym{***}&     -0.0051\sym{***}\\
                    &   (88.8151)         &   (26.6663)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=28&  -6695.7336\sym{***}&   -680.7433\sym{***}&      0.0250\sym{***}&     -0.0054\sym{***}\\
                    &   (90.0249)         &   (27.2110)         &    (0.0015)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=29&  -6156.3736\sym{***}&   -220.4075\sym{***}&     -0.0318\sym{***}&     -0.0001         \\
                    &   (90.0236)         &   (26.7408)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=30&  -5872.2707\sym{***}&   -100.8022\sym{***}&     -0.0253\sym{***}&     -0.0006         \\
                    &   (95.0299)         &   (28.4506)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=31&  -3982.8014\sym{***}&    312.6180\sym{***}&     -0.0241\sym{***}&      0.0021\sym{***}\\
                    &   (99.4463)         &   (28.5712)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=32&  -4780.7422\sym{***}&   -595.0323\sym{***}&     -0.0487\sym{***}&     -0.0002         \\
                    &   (99.5058)         &   (27.8126)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=33&  -4455.8623\sym{***}&   -208.9614\sym{***}&     -0.0309\sym{***}&     -0.0003         \\
                    &  (100.3890)         &   (27.5318)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=34&  -3933.3009\sym{***}&   -154.4538\sym{***}&     -0.0197\sym{***}&     -0.0017\sym{**} \\
                    &  (102.6675)         &   (28.7520)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=35&  -3816.2097\sym{***}&    199.2813\sym{***}&      0.0003         &      0.0045\sym{***}\\
                    &  (103.5522)         &   (29.0013)         &    (0.0015)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=36&  -4302.5976\sym{***}&   -524.3364\sym{***}&     -0.0352\sym{***}&      0.0071\sym{***}\\
                    &  (102.7626)         &   (28.7229)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=37&  -3911.9872\sym{***}&    -13.5959         &     -0.0277\sym{***}&      0.0090\sym{***}\\
                    &  (103.6316)         &   (28.9609)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=38&  -3515.6280\sym{***}&    -51.2802\sym{*}  &     -0.0368\sym{***}&      0.0098\sym{***}\\
                    &  (105.0809)         &   (29.1081)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=39&  -2315.0867\sym{***}&    292.1693\sym{***}&      0.0514\sym{***}&      0.0115\sym{***}\\
                    &  (106.7401)         &   (29.6270)         &    (0.0015)         &    (0.0009)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=40&  -3257.8307\sym{***}&   -600.3285\sym{***}&     -0.0431\sym{***}&      0.0080\sym{***}\\
                    &  (106.2145)         &   (28.9163)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=41&  -2845.9407\sym{***}&     49.8640\sym{*}  &     -0.0334\sym{***}&      0.0096\sym{***}\\
                    &  (106.3670)         &   (29.5825)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=42&  -2750.0826\sym{***}&    -41.0282         &     -0.0404\sym{***}&      0.0092\sym{***}\\
                    &  (107.7315)         &   (29.1388)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=43&  -2304.3633\sym{***}&    356.3743\sym{***}&     -0.0308\sym{***}&      0.0095\sym{***}\\
                    &  (109.3394)         &   (30.1138)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=44&  -3473.4938\sym{***}&   -666.8000\sym{***}&     -0.0590\sym{***}&      0.0069\sym{***}\\
                    &  (109.8649)         &   (29.4254)         &    (0.0012)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=45&  -3052.5281\sym{***}&    -78.1383\sym{***}&     -0.0421\sym{***}&      0.0117\sym{***}\\
                    &  (110.6660)         &   (29.7871)         &    (0.0013)         &    (0.0009)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=46&  -2759.5324\sym{***}&    -64.5642\sym{**} &     -0.0437\sym{***}&      0.0130\sym{***}\\
                    &  (112.1820)         &   (30.0079)         &    (0.0013)         &    (0.0009)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=47&  -2227.2455\sym{***}&    233.1272\sym{***}&     -0.0399\sym{***}&      0.0110\sym{***}\\
                    &  (114.2914)         &   (30.6261)         &    (0.0013)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=48&  -3187.2529\sym{***}&   -664.0247\sym{***}&     -0.0411\sym{***}&      0.0136\sym{***}\\
                    &  (113.8408)         &   (30.0806)         &    (0.0013)         &    (0.0009)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=49&  -2841.1502\sym{***}&   -132.0567\sym{***}&     -0.0092\sym{***}&      0.0183\sym{***}\\
                    &  (115.1581)         &   (30.7337)         &    (0.0014)         &    (0.0009)         \\
[1em]
Constant            &  -3605.0501\sym{***}&  -6268.7825\sym{***}&      0.1730\sym{***}&      0.2522\sym{***}\\
                    &  (242.5115)         &  (272.5950)         &    (0.0041)         &    (0.0050)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         \\
Observations        &17865452.0000         &17865452.0000         &17865452.0000         &17865452.0000         \\
$R^2$               &      0.3349         &      0.2783         &      0.0286         &      0.0465         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize }\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Tables/old/regressions_detail/mortgage_reg.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{mtf5320}&\multicolumn{1}{c}{mtf5020}&\multicolumn{1}{c}{mortgage\_origination}&\multicolumn{1}{c}{mortgage\_inquiry}\\
\hline
cs\_bin=1            &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=2            &   7574.0447\sym{***}&   9011.6209\sym{***}&      0.0089\sym{***}&      0.0208\sym{***}\\
                    & (1285.2777)         &  (975.1730)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=3            &   4603.9812\sym{***}&   9279.0785\sym{***}&      0.0313\sym{***}&      0.0514\sym{***}\\
                    & (1617.4900)         & (1339.7821)         &    (0.0008)         &    (0.0020)         \\
[1em]
cs\_bin=4            &  -8434.3305\sym{***}&    782.8112         &      0.0258\sym{***}&      0.0182\sym{***}\\
                    & (1647.7365)         & (1381.5282)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=5            &  82903.9414\sym{***}&  89578.9233\sym{***}&      0.0283\sym{***}&      0.0423\sym{***}\\
                    & (1911.5932)         & (1509.9132)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ age&     61.3205\sym{***}&     60.5392\sym{***}&      0.0002\sym{***}&      0.0005\sym{***}\\
                    &   (20.6276)         &   (20.2172)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=2 $\times$ age&     97.3077\sym{***}&     88.6109\sym{***}&      0.0001\sym{***}&      0.0002\sym{***}\\
                    &   (12.4991)         &   (11.7391)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=3 $\times$ age&   -380.5481\sym{***}&   -372.8544\sym{***}&     -0.0001\sym{***}&     -0.0003\sym{***}\\
                    &   (15.3887)         &   (13.9537)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=4 $\times$ age&   -553.0468\sym{***}&   -562.2338\sym{***}&     -0.0001\sym{***}&     -0.0005\sym{***}\\
                    &   (10.7412)         &   (10.0156)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=5 $\times$ age&  -1778.9103\sym{***}&  -1631.9142\sym{***}&     -0.0003\sym{***}&     -0.0012\sym{***}\\
                    &   (16.6341)         &   (14.8799)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=1 $\times$ income\_insight\_score&   1619.0396\sym{***}&   1517.8089\sym{***}&      0.0002\sym{***}&      0.0007\sym{***}\\
                    &   (45.0946)         &   (38.4054)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=2 $\times$ income\_insight\_score&   1349.0598\sym{***}&   1227.2644\sym{***}&      0.0001\sym{***}&      0.0005\sym{***}\\
                    &   (26.0205)         &   (23.3643)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=3 $\times$ income\_insight\_score&   1928.3025\sym{***}&   1751.9511\sym{***}&      0.0001\sym{***}&      0.0006\sym{***}\\
                    &   (30.3462)         &   (27.6236)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=4 $\times$ income\_insight\_score&   1918.8989\sym{***}&   1709.1394\sym{***}&      0.0001\sym{***}&      0.0005\sym{***}\\
                    &   (17.7874)         &   (16.4908)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=5 $\times$ income\_insight\_score&   1097.4557\sym{***}&    861.2241\sym{***}&      0.0000\sym{***}&      0.0002\sym{***}\\
                    &   (12.7332)         &   (10.5008)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin=1 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=1 $\times$ quarter=9&   -758.0183\sym{**} &   -698.7301\sym{**} &      0.0003         &      0.0093\sym{***}\\
                    &  (310.7697)         &  (303.6839)         &    (0.0007)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=10&  -1025.3641\sym{***}&   -893.7653\sym{**} &     -0.0004         &      0.0148\sym{***}\\
                    &  (374.5337)         &  (363.9923)         &    (0.0006)         &    (0.0020)         \\
[1em]
cs\_bin=1 $\times$ quarter=11&  -1371.4453\sym{***}&  -1168.3198\sym{***}&      0.0003         &      0.0092\sym{***}\\
                    &  (429.1707)         &  (414.5874)         &    (0.0007)         &    (0.0019)         \\
[1em]
cs\_bin=1 $\times$ quarter=12&   2777.1024\sym{***}&   2787.2297\sym{***}&      0.0012\sym{*}  &      0.0117\sym{***}\\
                    &  (375.9534)         &  (372.3516)         &    (0.0007)         &    (0.0020)         \\
[1em]
cs\_bin=1 $\times$ quarter=13&   2871.1845\sym{***}&   2995.7597\sym{***}&      0.0014\sym{**} &      0.0095\sym{***}\\
                    &  (395.7988)         &  (390.2068)         &    (0.0007)         &    (0.0019)         \\
[1em]
cs\_bin=1 $\times$ quarter=14&   3187.2640\sym{***}&   3381.6081\sym{***}&      0.0004         &      0.0036\sym{*}  \\
                    &  (451.5136)         &  (445.6369)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin=1 $\times$ quarter=15&   2493.8330\sym{***}&   2825.2765\sym{***}&     -0.0014\sym{**} &     -0.0100\sym{***}\\
                    &  (469.9142)         &  (459.6508)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=16&   5775.4040\sym{***}&   5966.6293\sym{***}&     -0.0025\sym{***}&     -0.0073\sym{***}\\
                    &  (432.9696)         &  (430.6738)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=17&   5038.1631\sym{***}&   5388.1189\sym{***}&     -0.0017\sym{***}&     -0.0099\sym{***}\\
                    &  (459.9501)         &  (455.8296)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=18&   4398.2084\sym{***}&   4854.9169\sym{***}&     -0.0022\sym{***}&     -0.0152\sym{***}\\
                    &  (474.2289)         &  (465.7416)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=19&   3677.0774\sym{***}&   4272.8225\sym{***}&     -0.0023\sym{***}&     -0.0272\sym{***}\\
                    &  (486.3054)         &  (469.0479)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=20&   9705.2779\sym{***}&   8140.9678\sym{***}&     -0.0021\sym{***}&     -0.0294\sym{***}\\
                    & (1755.7817)         &  (482.3657)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=21&   6714.4459\sym{***}&   6836.1023\sym{***}&     -0.0012\sym{*}  &     -0.0282\sym{***}\\
                    &  (511.4514)         &  (493.0166)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=22&   5991.1767\sym{***}&   6190.5004\sym{***}&     -0.0022\sym{***}&     -0.0318\sym{***}\\
                    &  (493.3423)         &  (468.6241)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=23&   5168.2752\sym{***}&   5399.2060\sym{***}&     -0.0021\sym{***}&     -0.0351\sym{***}\\
                    &  (530.7665)         &  (504.2661)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=24&   7921.9867\sym{***}&   7887.2333\sym{***}&     -0.0008         &     -0.0350\sym{***}\\
                    &  (513.9311)         &  (500.3920)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=25&   6179.1726\sym{***}&   6183.4853\sym{***}&     -0.0014\sym{**} &     -0.0369\sym{***}\\
                    &  (477.7411)         &  (457.6316)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=26&   4943.3695\sym{***}&   5047.9898\sym{***}&     -0.0009         &     -0.0402\sym{***}\\
                    &  (470.5446)         &  (452.4222)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=27&   3451.0656\sym{***}&   3614.0865\sym{***}&     -0.0027\sym{***}&     -0.0452\sym{***}\\
                    &  (479.1821)         &  (458.0205)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=28&   5556.4533\sym{***}&   5516.8105\sym{***}&     -0.0007         &     -0.0435\sym{***}\\
                    &  (484.6856)         &  (461.0171)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=29&   4218.2504\sym{***}&   4353.2395\sym{***}&     -0.0031\sym{***}&     -0.0429\sym{***}\\
                    &  (495.6140)         &  (492.0431)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=30&   4012.2500\sym{***}&   4099.0288\sym{***}&     -0.0029\sym{***}&     -0.0436\sym{***}\\
                    &  (486.4053)         &  (472.6914)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=31&   2449.1183\sym{***}&   2463.5814\sym{***}&     -0.0031\sym{***}&     -0.0458\sym{***}\\
                    &  (498.2579)         &  (470.9434)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=32&   3621.0483\sym{***}&   3654.9238\sym{***}&     -0.0014\sym{**} &     -0.0454\sym{***}\\
                    &  (444.8537)         &  (440.2386)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=33&   1579.1952\sym{***}&   1614.8808\sym{***}&     -0.0018\sym{***}&     -0.0452\sym{***}\\
                    &  (443.1982)         &  (431.6753)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=34&   -209.8266         &   -200.5356         &     -0.0025\sym{***}&     -0.0452\sym{***}\\
                    &  (440.2766)         &  (427.1009)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=35&    585.3060         &    485.8458         &     -0.0023\sym{***}&     -0.0484\sym{***}\\
                    &  (408.8983)         &  (398.1019)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=36&   -289.6965         &   -382.3200         &     -0.0028\sym{***}&     -0.0465\sym{***}\\
                    &  (412.5154)         &  (402.1325)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=37&   -555.6622         &   -595.1757         &     -0.0001         &     -0.0451\sym{***}\\
                    &  (423.5140)         &  (412.0129)         &    (0.0007)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=38&  -1872.5692\sym{***}&  -1990.1337\sym{***}&     -0.0032\sym{***}&     -0.0472\sym{***}\\
                    &  (420.3980)         &  (405.3307)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=39&  -2841.8254\sym{***}&  -2932.9023\sym{***}&     -0.0009         &     -0.0500\sym{***}\\
                    &  (430.1490)         &  (413.9486)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=40&  -1974.5761\sym{***}&  -2108.8821\sym{***}&     -0.0020\sym{***}&     -0.0515\sym{***}\\
                    &  (409.2863)         &  (395.9903)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=41&  -2895.0583\sym{***}&  -3036.8363\sym{***}&     -0.0035\sym{***}&     -0.0494\sym{***}\\
                    &  (409.1455)         &  (393.0892)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=42&  -3588.5692\sym{***}&  -3699.5692\sym{***}&     -0.0041\sym{***}&     -0.0487\sym{***}\\
                    &  (421.5067)         &  (405.0654)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=43&  -3770.8510\sym{***}&  -3927.9149\sym{***}&     -0.0048\sym{***}&     -0.0470\sym{***}\\
                    &  (433.1690)         &  (414.0750)         &    (0.0006)         &    (0.0017)         \\
[1em]
cs\_bin=1 $\times$ quarter=44&  -4161.7703\sym{***}&  -4374.2192\sym{***}&     -0.0038\sym{***}&     -0.0466\sym{***}\\
                    &  (417.9413)         &  (400.0867)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=45&  -5431.1348\sym{***}&  -5515.6348\sym{***}&     -0.0044\sym{***}&     -0.0434\sym{***}\\
                    &  (423.2654)         &  (405.1350)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=46&  -6372.0320\sym{***}&  -6364.0931\sym{***}&     -0.0048\sym{***}&     -0.0396\sym{***}\\
                    &  (448.7618)         &  (424.7040)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin=1 $\times$ quarter=47&  -7600.9404\sym{***}&  -7540.9292\sym{***}&     -0.0044\sym{***}&     -0.0368\sym{***}\\
                    &  (467.9790)         &  (438.6911)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin=1 $\times$ quarter=48&  -6644.4546\sym{***}&  -6798.6232\sym{***}&     -0.0048\sym{***}&     -0.0369\sym{***}\\
                    &  (431.3916)         &  (407.8382)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin=1 $\times$ quarter=49&  -7064.4893\sym{***}&  -7140.9342\sym{***}&     -0.0054\sym{***}&     -0.0345\sym{***}\\
                    &  (441.5379)         &  (417.0669)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin=2 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=2 $\times$ quarter=9&   -499.0212\sym{**} &   -344.5500\sym{*}  &      0.0009\sym{*}  &      0.0109\sym{***}\\
                    &  (206.6743)         &  (202.7472)         &    (0.0005)         &    (0.0009)         \\
[1em]
cs\_bin=2 $\times$ quarter=10&  -1167.4409\sym{***}&   -851.1867\sym{***}&      0.0002         &      0.0159\sym{***}\\
                    &  (248.4383)         &  (241.4266)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=11&  -2312.7483\sym{***}&  -1817.4412\sym{***}&      0.0002         &      0.0075\sym{***}\\
                    &  (276.7081)         &  (265.4303)         &    (0.0005)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=12&   2906.1688\sym{***}&   2978.6099\sym{***}&      0.0005         &      0.0116\sym{***}\\
                    &  (258.0672)         &  (255.9205)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=13&   3105.2392\sym{***}&   3296.4188\sym{***}&      0.0002         &      0.0138\sym{***}\\
                    &  (296.6959)         &  (291.3084)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=14&   2589.8398\sym{***}&   2901.4946\sym{***}&     -0.0021\sym{***}&      0.0025\sym{**} \\
                    &  (302.4939)         &  (296.8383)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=15&   1927.9300\sym{***}&   2403.1044\sym{***}&     -0.0042\sym{***}&     -0.0125\sym{***}\\
                    &  (324.2739)         &  (314.8183)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=16&   5875.2946\sym{***}&   6009.6466\sym{***}&     -0.0062\sym{***}&     -0.0063\sym{***}\\
                    &  (299.4943)         &  (298.6541)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=17&   4396.9064\sym{***}&   4703.2803\sym{***}&     -0.0052\sym{***}&     -0.0105\sym{***}\\
                    &  (309.9842)         &  (308.3197)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin=2 $\times$ quarter=18&   3317.4060\sym{***}&   3730.4507\sym{***}&     -0.0070\sym{***}&     -0.0178\sym{***}\\
                    &  (312.0043)         &  (306.6821)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=19&   2458.1778\sym{***}&   3020.9309\sym{***}&     -0.0069\sym{***}&     -0.0304\sym{***}\\
                    &  (325.6545)         &  (316.7379)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=20&   8670.5973\sym{***}&   5844.0628\sym{***}&     -0.0072\sym{***}&     -0.0294\sym{***}\\
                    & (1419.2495)         &  (309.0157)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=21&   4670.3448\sym{***}&   4584.1121\sym{***}&     -0.0058\sym{***}&     -0.0295\sym{***}\\
                    &  (311.1951)         &  (302.3348)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=22&   2878.7377\sym{***}&   2879.3170\sym{***}&     -0.0075\sym{***}&     -0.0336\sym{***}\\
                    &  (313.6218)         &  (301.3032)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=23&    457.7013         &    562.2141\sym{*}  &     -0.0069\sym{***}&     -0.0390\sym{***}\\
                    &  (324.3263)         &  (309.1330)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=24&   3698.5141\sym{***}&   3473.0705\sym{***}&     -0.0062\sym{***}&     -0.0394\sym{***}\\
                    &  (293.8734)         &  (285.2959)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=25&   1908.2919\sym{***}&   1766.5462\sym{***}&     -0.0067\sym{***}&     -0.0397\sym{***}\\
                    &  (298.6642)         &  (289.1342)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=26&    582.6809\sym{*}  &    448.7005         &     -0.0058\sym{***}&     -0.0432\sym{***}\\
                    &  (304.4192)         &  (293.6693)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=27&  -2022.3289\sym{***}&  -2035.1050\sym{***}&     -0.0066\sym{***}&     -0.0496\sym{***}\\
                    &  (301.9415)         &  (287.9134)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=28&    565.7928\sym{**} &    294.2957         &     -0.0065\sym{***}&     -0.0473\sym{***}\\
                    &  (286.7580)         &  (279.3744)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=29&   -975.4579\sym{***}&  -1209.0830\sym{***}&     -0.0082\sym{***}&     -0.0464\sym{***}\\
                    &  (287.0198)         &  (277.1202)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=30&  -1824.6686\sym{***}&  -2089.7617\sym{***}&     -0.0084\sym{***}&     -0.0478\sym{***}\\
                    &  (304.9782)         &  (291.4553)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=31&  -4044.5164\sym{***}&  -4150.1247\sym{***}&     -0.0081\sym{***}&     -0.0514\sym{***}\\
                    &  (294.6514)         &  (281.0923)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=32&  -2103.2361\sym{***}&  -2481.5292\sym{***}&     -0.0071\sym{***}&     -0.0480\sym{***}\\
                    &  (285.7612)         &  (278.9387)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=33&  -3188.2952\sym{***}&  -3558.9756\sym{***}&     -0.0080\sym{***}&     -0.0473\sym{***}\\
                    &  (284.5078)         &  (275.0837)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=34&  -4278.5722\sym{***}&  -4635.3763\sym{***}&     -0.0080\sym{***}&     -0.0479\sym{***}\\
                    &  (296.0415)         &  (284.2971)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=35&  -4315.6987\sym{***}&  -4772.6779\sym{***}&     -0.0078\sym{***}&     -0.0513\sym{***}\\
                    &  (278.9007)         &  (269.6623)         &    (0.0004)         &    (0.0009)         \\
[1em]
cs\_bin=2 $\times$ quarter=36&  -5347.8377\sym{***}&  -5838.2902\sym{***}&     -0.0081\sym{***}&     -0.0483\sym{***}\\
                    &  (292.8672)         &  (283.3114)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=37&  -6254.3040\sym{***}&  -6661.6373\sym{***}&     -0.0066\sym{***}&     -0.0462\sym{***}\\
                    &  (290.7719)         &  (280.2638)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=38&  -7096.0201\sym{***}&  -7573.3216\sym{***}&     -0.0068\sym{***}&     -0.0505\sym{***}\\
                    &  (291.9390)         &  (277.0170)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=39&  -7175.2450\sym{***}&  -7648.7909\sym{***}&     -0.0054\sym{***}&     -0.0541\sym{***}\\
                    &  (298.2368)         &  (284.6054)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=40&  -8006.2873\sym{***}&  -8389.7174\sym{***}&     -0.0076\sym{***}&     -0.0531\sym{***}\\
                    &  (293.3329)         &  (281.4904)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=41&  -8699.8950\sym{***}&  -9053.6712\sym{***}&     -0.0086\sym{***}&     -0.0496\sym{***}\\
                    &  (303.5280)         &  (291.4251)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=42&  -8804.9311\sym{***}&  -9193.0346\sym{***}&     -0.0083\sym{***}&     -0.0498\sym{***}\\
                    &  (302.5091)         &  (289.1988)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=43&  -9219.4087\sym{***}&  -9611.7189\sym{***}&     -0.0083\sym{***}&     -0.0504\sym{***}\\
                    &  (308.3930)         &  (292.7846)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=44&  -9836.6033\sym{***}& -10194.8713\sym{***}&     -0.0090\sym{***}&     -0.0480\sym{***}\\
                    &  (304.8427)         &  (290.6437)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=45& -10652.2719\sym{***}& -11019.2309\sym{***}&     -0.0093\sym{***}&     -0.0449\sym{***}\\
                    &  (305.6196)         &  (290.2483)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=46& -10602.6453\sym{***}& -11025.6758\sym{***}&     -0.0083\sym{***}&     -0.0437\sym{***}\\
                    &  (310.0947)         &  (294.1651)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=47& -11319.5844\sym{***}& -11672.0169\sym{***}&     -0.0086\sym{***}&     -0.0461\sym{***}\\
                    &  (314.1410)         &  (296.4330)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=48& -11597.0234\sym{***}& -11887.2024\sym{***}&     -0.0086\sym{***}&     -0.0415\sym{***}\\
                    &  (313.0336)         &  (296.9155)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=2 $\times$ quarter=49& -11755.8794\sym{***}& -12015.6656\sym{***}&     -0.0099\sym{***}&     -0.0402\sym{***}\\
                    &  (318.4610)         &  (302.5056)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin=3 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=3 $\times$ quarter=9&    931.9335\sym{**} &   1030.8262\sym{**} &     -0.0005         &      0.0109\sym{***}\\
                    &  (448.2785)         &  (443.5413)         &    (0.0009)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=10&   1096.3256\sym{**} &   1300.8343\sym{***}&     -0.0027\sym{***}&      0.0136\sym{***}\\
                    &  (500.1078)         &  (493.2991)         &    (0.0008)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=11&   2539.4869\sym{***}&   2832.4199\sym{***}&     -0.0018\sym{**} &      0.0013         \\
                    &  (552.9780)         &  (543.0698)         &    (0.0009)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=12&   4521.7931\sym{***}&   4589.5292\sym{***}&     -0.0049\sym{***}&      0.0092\sym{***}\\
                    &  (527.5568)         &  (522.6395)         &    (0.0008)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=13&   5206.1714\sym{***}&   5338.6905\sym{***}&     -0.0038\sym{***}&      0.0118\sym{***}\\
                    &  (583.5046)         &  (578.8118)         &    (0.0008)         &    (0.0015)         \\
[1em]
cs\_bin=3 $\times$ quarter=14&   5798.8766\sym{***}&   6046.7327\sym{***}&     -0.0064\sym{***}&     -0.0022         \\
                    &  (609.4564)         &  (605.5043)         &    (0.0008)         &    (0.0015)         \\
[1em]
cs\_bin=3 $\times$ quarter=15&   5366.3630\sym{***}&   5637.8137\sym{***}&     -0.0108\sym{***}&     -0.0201\sym{***}\\
                    &  (602.3411)         &  (597.5768)         &    (0.0008)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=16&   5112.2767\sym{***}&   5181.8533\sym{***}&     -0.0178\sym{***}&     -0.0084\sym{***}\\
                    &  (563.6387)         &  (561.9581)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=17&   3388.5612\sym{***}&   3557.1383\sym{***}&     -0.0151\sym{***}&     -0.0129\sym{***}\\
                    &  (582.8651)         &  (578.2954)         &    (0.0008)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=18&    744.6348         &    847.0106         &     -0.0191\sym{***}&     -0.0263\sym{***}\\
                    &  (594.9579)         &  (585.3249)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=19&  -2925.1361\sym{***}&  -2798.1376\sym{***}&     -0.0192\sym{***}&     -0.0410\sym{***}\\
                    &  (626.0709)         &  (613.9168)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=20&   5935.2241\sym{**} &  -1347.0613\sym{**} &     -0.0212\sym{***}&     -0.0291\sym{***}\\
                    & (2697.4149)         &  (577.6906)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=21&  -2714.8204\sym{***}&  -3505.5219\sym{***}&     -0.0201\sym{***}&     -0.0266\sym{***}\\
                    &  (566.5908)         &  (549.8955)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=22&  -6222.2778\sym{***}&  -6970.1469\sym{***}&     -0.0211\sym{***}&     -0.0369\sym{***}\\
                    &  (584.5445)         &  (569.0498)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=23&  -7131.4985\sym{***}&  -8356.8447\sym{***}&     -0.0200\sym{***}&     -0.0467\sym{***}\\
                    &  (793.2462)         &  (598.8794)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=24&  -6540.9040\sym{***}&  -7548.6576\sym{***}&     -0.0200\sym{***}&     -0.0491\sym{***}\\
                    &  (547.3972)         &  (536.7275)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=25&  -7731.5520\sym{***}&  -8773.6609\sym{***}&     -0.0205\sym{***}&     -0.0470\sym{***}\\
                    &  (565.7910)         &  (554.0680)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=26&  -9583.7914\sym{***}& -10576.5218\sym{***}&     -0.0189\sym{***}&     -0.0478\sym{***}\\
                    &  (557.8414)         &  (546.8523)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=27&  -9750.3835\sym{***}& -10803.2664\sym{***}&     -0.0207\sym{***}&     -0.0548\sym{***}\\
                    &  (570.9189)         &  (556.9733)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=28&  -8264.5481\sym{***}&  -9614.6229\sym{***}&     -0.0206\sym{***}&     -0.0577\sym{***}\\
                    &  (556.0279)         &  (543.2169)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=29&  -9359.7469\sym{***}& -10786.5254\sym{***}&     -0.0229\sym{***}&     -0.0546\sym{***}\\
                    &  (560.4880)         &  (547.4803)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=30& -11123.7931\sym{***}& -12440.8843\sym{***}&     -0.0234\sym{***}&     -0.0520\sym{***}\\
                    &  (555.3300)         &  (541.3116)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=31& -11574.4186\sym{***}& -12958.8285\sym{***}&     -0.0218\sym{***}&     -0.0560\sym{***}\\
                    &  (573.5101)         &  (559.7322)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=32& -10566.7692\sym{***}& -12215.6193\sym{***}&     -0.0203\sym{***}&     -0.0513\sym{***}\\
                    &  (544.5477)         &  (533.1713)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=33& -11743.7868\sym{***}& -13341.1735\sym{***}&     -0.0221\sym{***}&     -0.0458\sym{***}\\
                    &  (560.8265)         &  (550.0796)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=34& -12987.1603\sym{***}& -14605.8439\sym{***}&     -0.0205\sym{***}&     -0.0468\sym{***}\\
                    &  (568.3830)         &  (548.4776)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=35& -11663.5683\sym{***}& -13523.2427\sym{***}&     -0.0200\sym{***}&     -0.0501\sym{***}\\
                    &  (561.0551)         &  (542.0700)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=36& -13504.2723\sym{***}& -15179.6907\sym{***}&     -0.0205\sym{***}&     -0.0464\sym{***}\\
                    &  (564.4812)         &  (553.2727)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=37& -14600.2599\sym{***}& -16141.8769\sym{***}&     -0.0183\sym{***}&     -0.0418\sym{***}\\
                    &  (565.0397)         &  (553.5105)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=38& -15239.5446\sym{***}& -16814.9280\sym{***}&     -0.0162\sym{***}&     -0.0493\sym{***}\\
                    &  (565.6753)         &  (553.8569)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=39& -14322.7885\sym{***}& -16097.2842\sym{***}&     -0.0146\sym{***}&     -0.0584\sym{***}\\
                    &  (561.5141)         &  (548.9264)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=40& -15486.3960\sym{***}& -17137.9655\sym{***}&     -0.0202\sym{***}&     -0.0550\sym{***}\\
                    &  (569.4692)         &  (556.9470)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=41& -16434.5636\sym{***}& -18122.7210\sym{***}&     -0.0224\sym{***}&     -0.0482\sym{***}\\
                    &  (573.5049)         &  (559.6549)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=42& -16585.2345\sym{***}& -18358.1511\sym{***}&     -0.0191\sym{***}&     -0.0506\sym{***}\\
                    &  (596.4766)         &  (579.2840)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=43& -16522.8054\sym{***}& -18340.9030\sym{***}&     -0.0200\sym{***}&     -0.0552\sym{***}\\
                    &  (594.8713)         &  (580.4863)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin=3 $\times$ quarter=44& -19403.2521\sym{***}& -21049.3079\sym{***}&     -0.0216\sym{***}&     -0.0475\sym{***}\\
                    &  (592.0783)         &  (578.3396)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=45& -19575.9240\sym{***}& -21236.6307\sym{***}&     -0.0211\sym{***}&     -0.0411\sym{***}\\
                    &  (608.2865)         &  (593.1578)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=46& -19221.6741\sym{***}& -20941.8546\sym{***}&     -0.0182\sym{***}&     -0.0437\sym{***}\\
                    &  (609.1303)         &  (596.7699)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=47& -19732.6143\sym{***}& -21202.2589\sym{***}&     -0.0202\sym{***}&     -0.0514\sym{***}\\
                    &  (632.0481)         &  (616.1843)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=48& -21579.4341\sym{***}& -23031.6291\sym{***}&     -0.0196\sym{***}&     -0.0421\sym{***}\\
                    &  (633.4633)         &  (617.1000)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=3 $\times$ quarter=49& -22402.1145\sym{***}& -23713.4037\sym{***}&     -0.0221\sym{***}&     -0.0394\sym{***}\\
                    &  (584.5689)         &  (582.7676)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin=4 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=4 $\times$ quarter=9&   2033.9787\sym{***}&   1815.7686\sym{***}&     -0.0008\sym{*}  &      0.0070\sym{***}\\
                    &  (200.5005)         &  (194.8351)         &    (0.0005)         &    (0.0006)         \\
[1em]
cs\_bin=4 $\times$ quarter=10&   3844.7110\sym{***}&   3490.1466\sym{***}&     -0.0018\sym{***}&      0.0076\sym{***}\\
                    &  (247.8417)         &  (241.0399)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=11&   4831.4448\sym{***}&   4359.5608\sym{***}&     -0.0025\sym{***}&      0.0008         \\
                    &  (276.0739)         &  (268.6316)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=12&   1394.5019\sym{***}&   1199.8695\sym{***}&     -0.0030\sym{***}&      0.0048\sym{***}\\
                    &  (287.8212)         &  (282.9339)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=13&   3733.7447\sym{***}&   3298.0697\sym{***}&      0.0005         &      0.0078\sym{***}\\
                    &  (296.9959)         &  (289.0545)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=14&   5245.9525\sym{***}&   4713.3954\sym{***}&     -0.0036\sym{***}&     -0.0016\sym{**} \\
                    &  (317.2696)         &  (309.6876)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=15&   6209.4717\sym{***}&   5457.6930\sym{***}&     -0.0058\sym{***}&     -0.0119\sym{***}\\
                    &  (330.6601)         &  (321.1199)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=16&   1367.0620\sym{***}&    920.0259\sym{***}&     -0.0113\sym{***}&      0.0024\sym{***}\\
                    &  (324.7324)         &  (318.6590)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=17&   2062.1409\sym{***}&   1519.8456\sym{***}&     -0.0071\sym{***}&     -0.0007         \\
                    &  (333.5740)         &  (325.5089)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=18&   1842.4006\sym{***}&   1198.3730\sym{***}&     -0.0120\sym{***}&     -0.0099\sym{***}\\
                    &  (346.8030)         &  (337.5697)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=19&    810.8734\sym{**} &    -33.7401         &     -0.0132\sym{***}&     -0.0121\sym{***}\\
                    &  (376.9257)         &  (366.0533)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=20&  11045.1899\sym{***}&  -1031.4778\sym{***}&     -0.0151\sym{***}&      0.0125\sym{***}\\
                    & (2045.3079)         &  (354.7940)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=21&   -261.7260         &  -1694.7729\sym{***}&     -0.0117\sym{***}&      0.0141\sym{***}\\
                    &  (354.3052)         &  (343.6036)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=22&   -894.7288\sym{**} &  -2325.0392\sym{***}&     -0.0099\sym{***}&     -0.0061\sym{***}\\
                    &  (358.4019)         &  (346.1207)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=23&  -1108.3328\sym{***}&  -2627.8879\sym{***}&     -0.0098\sym{***}&     -0.0126\sym{***}\\
                    &  (391.5651)         &  (377.5642)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=24&   -841.4398\sym{**} &  -2579.1367\sym{***}&     -0.0106\sym{***}&     -0.0137\sym{***}\\
                    &  (381.7072)         &  (367.9541)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=25&   -930.9844\sym{**} &  -2745.6455\sym{***}&     -0.0112\sym{***}&     -0.0091\sym{***}\\
                    &  (387.3640)         &  (374.3068)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=26&  -1108.5178\sym{***}&  -3078.9818\sym{***}&     -0.0090\sym{***}&     -0.0007         \\
                    &  (392.7457)         &  (378.4971)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=27&  -1866.4989\sym{***}&  -3831.7016\sym{***}&     -0.0102\sym{***}&     -0.0079\sym{***}\\
                    &  (393.4185)         &  (378.9396)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=28&  -2224.5069\sym{***}&  -4066.4000\sym{***}&     -0.0072\sym{***}&     -0.0188\sym{***}\\
                    &  (382.8120)         &  (370.4419)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=29&  -1729.3743\sym{***}&  -3730.6537\sym{***}&     -0.0117\sym{***}&     -0.0148\sym{***}\\
                    &  (388.7593)         &  (377.1004)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=30&  -2747.3312\sym{***}&  -4857.4910\sym{***}&     -0.0141\sym{***}&     -0.0085\sym{***}\\
                    &  (391.8463)         &  (379.0659)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=31&  -2846.4313\sym{***}&  -5075.9378\sym{***}&     -0.0101\sym{***}&     -0.0103\sym{***}\\
                    &  (406.6382)         &  (392.2275)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=32&  -4764.8654\sym{***}&  -6870.6346\sym{***}&     -0.0100\sym{***}&     -0.0030\sym{***}\\
                    &  (403.2975)         &  (389.8768)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=33&  -4927.8480\sym{***}&  -7136.4247\sym{***}&     -0.0098\sym{***}&      0.0033\sym{***}\\
                    &  (408.3857)         &  (394.7147)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=34&  -5130.7712\sym{***}&  -7419.1941\sym{***}&     -0.0088\sym{***}&      0.0030\sym{***}\\
                    &  (410.1142)         &  (395.8929)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=35&  -6305.2625\sym{***}&  -8355.0531\sym{***}&     -0.0069\sym{***}&     -0.0009         \\
                    &  (404.6016)         &  (392.1294)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=36&  -7017.0539\sym{***}&  -9040.2881\sym{***}&     -0.0072\sym{***}&      0.0014\sym{*}  \\
                    &  (408.0423)         &  (395.5363)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=37&  -6772.1143\sym{***}&  -8723.0651\sym{***}&     -0.0045\sym{***}&      0.0061\sym{***}\\
                    &  (410.4775)         &  (396.7054)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin=4 $\times$ quarter=38&  -5958.8488\sym{***}&  -7936.9977\sym{***}&     -0.0008         &     -0.0103\sym{***}\\
                    &  (410.1783)         &  (396.7681)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=39&  -4198.1612\sym{***}&  -6499.2277\sym{***}&     -0.0024\sym{***}&     -0.0219\sym{***}\\
                    &  (420.8948)         &  (406.4813)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=40&  -7143.4161\sym{***}&  -9073.6191\sym{***}&     -0.0099\sym{***}&     -0.0184\sym{***}\\
                    &  (416.2226)         &  (404.7900)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=41&  -7069.6322\sym{***}&  -9136.4285\sym{***}&     -0.0124\sym{***}&     -0.0111\sym{***}\\
                    &  (421.4700)         &  (409.3624)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=42&  -6638.2809\sym{***}&  -8929.2339\sym{***}&     -0.0093\sym{***}&     -0.0135\sym{***}\\
                    &  (426.1934)         &  (413.7639)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=43&  -5232.7797\sym{***}&  -7794.9967\sym{***}&     -0.0101\sym{***}&     -0.0182\sym{***}\\
                    &  (431.9350)         &  (417.9381)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=44&  -9829.9000\sym{***}& -12132.6585\sym{***}&     -0.0121\sym{***}&     -0.0092\sym{***}\\
                    &  (420.4340)         &  (409.6951)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=45&  -9641.6164\sym{***}& -11931.5928\sym{***}&     -0.0102\sym{***}&     -0.0048\sym{***}\\
                    &  (423.2588)         &  (412.8821)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=46&  -8102.9149\sym{***}& -10588.5904\sym{***}&     -0.0063\sym{***}&     -0.0100\sym{***}\\
                    &  (422.4029)         &  (411.3167)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=47&  -7144.7240\sym{***}&  -9731.4959\sym{***}&     -0.0095\sym{***}&     -0.0175\sym{***}\\
                    &  (425.7705)         &  (413.5321)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=48& -10952.8102\sym{***}& -13200.7441\sym{***}&     -0.0093\sym{***}&     -0.0100\sym{***}\\
                    &  (438.5840)         &  (427.2336)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=4 $\times$ quarter=49& -12082.0925\sym{***}& -14198.6221\sym{***}&     -0.0124\sym{***}&     -0.0022\sym{***}\\
                    &  (447.9941)         &  (435.7341)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=8&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin=5 $\times$ quarter=9&   1981.6794\sym{***}&   1459.9166\sym{***}&     -0.0001         &      0.0047\sym{***}\\
                    &  (183.2302)         &  (174.7028)         &    (0.0004)         &    (0.0005)         \\
[1em]
cs\_bin=5 $\times$ quarter=10&   4480.8901\sym{***}&   3341.7721\sym{***}&     -0.0014\sym{***}&      0.0042\sym{***}\\
                    &  (220.5187)         &  (208.8185)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=11&   7016.5379\sym{***}&   5348.2526\sym{***}&     -0.0012\sym{***}&      0.0018\sym{***}\\
                    &  (297.0813)         &  (281.1925)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=12&   2530.3869\sym{***}&   1854.3972\sym{***}&     -0.0014\sym{***}&      0.0048\sym{***}\\
                    &  (297.2166)         &  (282.5120)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=13&   6299.9623\sym{***}&   4815.4063\sym{***}&      0.0069\sym{***}&      0.0077\sym{***}\\
                    &  (310.0555)         &  (293.7052)         &    (0.0005)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=14&   9600.1537\sym{***}&   7513.5849\sym{***}&     -0.0008\sym{**} &      0.0033\sym{***}\\
                    &  (336.2955)         &  (316.7238)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=15&  11646.0877\sym{***}&   9026.9006\sym{***}&     -0.0010\sym{***}&     -0.0009         \\
                    &  (345.0582)         &  (322.4663)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=16&   6502.4160\sym{***}&   4973.6656\sym{***}&     -0.0039\sym{***}&      0.0115\sym{***}\\
                    &  (336.9512)         &  (313.4517)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=17&   8542.1996\sym{***}&   6619.0729\sym{***}&     -0.0008\sym{**} &      0.0102\sym{***}\\
                    &  (340.3094)         &  (316.6973)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=18&  10362.0014\sym{***}&   8010.1866\sym{***}&     -0.0032\sym{***}&      0.0042\sym{***}\\
                    &  (352.9660)         &  (326.4943)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=19&  11480.1197\sym{***}&   8728.8933\sym{***}&     -0.0043\sym{***}&      0.0078\sym{***}\\
                    &  (370.4505)         &  (344.9236)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=20&  29835.6238\sym{***}&   5949.9144\sym{***}&     -0.0056\sym{***}&      0.0399\sym{***}\\
                    & (3634.2711)         &  (350.1570)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=21&   7332.4790\sym{***}&   5079.3846\sym{***}&     -0.0010\sym{***}&      0.0364\sym{***}\\
                    &  (387.1660)         &  (359.2413)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=22&   7793.3592\sym{***}&   5494.8596\sym{***}&      0.0028\sym{***}&      0.0127\sym{***}\\
                    &  (451.0122)         &  (423.4533)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=23&   8434.5374\sym{***}&   5830.5956\sym{***}&      0.0000         &      0.0125\sym{***}\\
                    &  (411.6312)         &  (379.3558)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=24&   9574.2667\sym{***}&   6846.2436\sym{***}&     -0.0003         &      0.0112\sym{***}\\
                    &  (401.7395)         &  (369.2104)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=25&   9843.6088\sym{***}&   6836.5881\sym{***}&     -0.0009\sym{**} &      0.0162\sym{***}\\
                    &  (383.0725)         &  (354.2779)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=26&   9048.4819\sym{***}&   5974.1927\sym{***}&     -0.0006         &      0.0334\sym{***}\\
                    &  (401.9455)         &  (369.2644)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=27&   7350.3864\sym{***}&   4522.9365\sym{***}&      0.0019\sym{***}&      0.0273\sym{***}\\
                    &  (410.2336)         &  (374.0375)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=28&   9167.3072\sym{***}&   6751.1076\sym{***}&      0.0081\sym{***}&      0.0092\sym{***}\\
                    &  (402.9520)         &  (368.4459)         &    (0.0005)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=29&  10937.8873\sym{***}&   8251.4264\sym{***}&      0.0011\sym{***}&      0.0103\sym{***}\\
                    &  (404.6919)         &  (369.7498)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=30&  10387.3089\sym{***}&   7597.8919\sym{***}&     -0.0030\sym{***}&      0.0225\sym{***}\\
                    &  (417.5248)         &  (380.5560)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=31&   8655.2779\sym{***}&   5806.1066\sym{***}&      0.0014\sym{***}&      0.0244\sym{***}\\
                    &  (426.7923)         &  (391.3207)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=32&   6438.0328\sym{***}&   4367.0145\sym{***}&      0.0037\sym{***}&      0.0298\sym{***}\\
                    &  (435.0032)         &  (396.1086)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=33&   7048.1303\sym{***}&   4926.9524\sym{***}&      0.0049\sym{***}&      0.0333\sym{***}\\
                    &  (446.5507)         &  (407.4017)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=34&   7275.4693\sym{***}&   5129.6818\sym{***}&      0.0032\sym{***}&      0.0373\sym{***}\\
                    &  (457.0483)         &  (414.9748)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=35&   5442.3734\sym{***}&   3626.9275\sym{***}&      0.0055\sym{***}&      0.0330\sym{***}\\
                    &  (456.2595)         &  (413.3625)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin=5 $\times$ quarter=36&   5963.4132\sym{***}&   4484.9889\sym{***}&      0.0060\sym{***}&      0.0308\sym{***}\\
                    &  (458.7872)         &  (416.3857)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=37&   5526.5013\sym{***}&   4197.9642\sym{***}&      0.0081\sym{***}&      0.0308\sym{***}\\
                    &  (462.3527)         &  (419.3666)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=38&   7477.8800\sym{***}&   6011.3522\sym{***}&      0.0109\sym{***}&      0.0124\sym{***}\\
                    &  (464.1045)         &  (418.7029)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=39&   9808.7246\sym{***}&   7744.8158\sym{***}&      0.0054\sym{***}&      0.0011\sym{*}  \\
                    &  (467.0658)         &  (421.6217)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=40&  10191.5344\sym{***}&   8447.1427\sym{***}&     -0.0005         &      0.0021\sym{***}\\
                    &  (458.7640)         &  (414.8525)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=41&  10326.0652\sym{***}&   8107.3648\sym{***}&     -0.0021\sym{***}&      0.0078\sym{***}\\
                    &  (474.4906)         &  (428.9969)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=42&  12221.7187\sym{***}&   9469.4300\sym{***}&     -0.0017\sym{***}&      0.0063\sym{***}\\
                    &  (477.0721)         &  (432.7478)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=43&  13261.3038\sym{***}&  10054.2590\sym{***}&     -0.0018\sym{***}&      0.0042\sym{***}\\
                    &  (483.0248)         &  (438.3137)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=44&  11136.6770\sym{***}&   8435.3292\sym{***}&     -0.0040\sym{***}&      0.0121\sym{***}\\
                    &  (485.8565)         &  (439.2610)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=45&  10742.1705\sym{***}&   7672.2471\sym{***}&     -0.0019\sym{***}&      0.0134\sym{***}\\
                    &  (490.0525)         &  (440.9074)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin=5 $\times$ quarter=46&  12929.7468\sym{***}&   9469.5591\sym{***}&      0.0009\sym{**} &      0.0094\sym{***}\\
                    &  (502.5364)         &  (453.4254)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=47&  12753.8362\sym{***}&   9047.0667\sym{***}&     -0.0023\sym{***}&      0.0037\sym{***}\\
                    &  (512.6917)         &  (459.8282)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=48&  11228.6348\sym{***}&   7888.6957\sym{***}&     -0.0012\sym{***}&      0.0089\sym{***}\\
                    &  (516.3495)         &  (460.0428)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin=5 $\times$ quarter=49&   9840.4957\sym{***}&   6302.8376\sym{***}&     -0.0039\sym{***}&      0.0153\sym{***}\\
                    &  (517.9277)         &  (460.8587)         &    (0.0004)         &    (0.0007)         \\
[1em]
Constant            & -46118.8911\sym{***}& -42725.5638\sym{***}&     -0.0055\sym{***}&      0.0309\sym{***}\\
                    & (1320.4153)         & (1069.2793)         &    (0.0005)         &    (0.0016)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         \\
Observations        &26240879.0000         &26240879.0000         &26240879.0000         &26240879.0000         \\
$R^2$               &      0.1639         &      0.2858         &      0.0083         &      0.0233         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize }\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Tables/old/regressions_detail/mortgage_reg_l1.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{\label{tab: vulnerable\_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{mtf5320}&\multicolumn{1}{c}{mtf5020}&\multicolumn{1}{c}{mortgage\_origination}&\multicolumn{1}{c}{mortgage\_inquiry}\\
\hline
cs\_bin\_l1=1         &      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=2         &   6884.5850\sym{***}&   8249.0710\sym{***}&      0.0082\sym{***}&      0.0202\sym{***}\\
                    & (1305.5592)         &  (946.8998)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=3         &   2677.9648         &   8022.0649\sym{***}&      0.0242\sym{***}&      0.0499\sym{***}\\
                    & (1631.9227)         & (1272.8597)         &    (0.0008)         &    (0.0021)         \\
[1em]
cs\_bin\_l1=4         &  -8947.5964\sym{***}&    293.8923         &      0.0248\sym{***}&      0.0129\sym{***}\\
                    & (1673.7345)         & (1362.3201)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=5         &  85675.3348\sym{***}&  91349.7514\sym{***}&      0.0415\sym{***}&      0.0396\sym{***}\\
                    & (1928.9244)         & (1500.0278)         &    (0.0007)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ age&    -23.8209         &    -16.6207         &      0.0001\sym{***}&      0.0003\sym{***}\\
                    &   (21.3953)         &   (20.7542)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=2 $\times$ age&     10.2073         &     11.3580         &      0.0001\sym{***}&      0.0001\sym{***}\\
                    &   (13.7196)         &   (12.6268)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=3 $\times$ age&   -459.8197\sym{***}&   -444.2131\sym{***}&     -0.0000\sym{***}&     -0.0003\sym{***}\\
                    &   (15.9069)         &   (14.6178)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=4 $\times$ age&   -581.0379\sym{***}&   -588.8516\sym{***}&     -0.0001\sym{***}&     -0.0005\sym{***}\\
                    &   (10.8242)         &   (10.0400)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=5 $\times$ age&  -1831.4378\sym{***}&  -1681.0348\sym{***}&     -0.0005\sym{***}&     -0.0013\sym{***}\\
                    &   (16.9158)         &   (15.2618)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=1 $\times$ income\_insight\_score&   1613.3589\sym{***}&   1498.4217\sym{***}&      0.0002\sym{***}&      0.0007\sym{***}\\
                    &   (47.9989)         &   (39.5434)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=2 $\times$ income\_insight\_score&   1404.9415\sym{***}&   1271.2680\sym{***}&      0.0001\sym{***}&      0.0005\sym{***}\\
                    &   (26.9214)         &   (24.1587)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=3 $\times$ income\_insight\_score&   2023.5592\sym{***}&   1825.2959\sym{***}&      0.0001\sym{***}&      0.0006\sym{***}\\
                    &   (32.1534)         &   (28.6154)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=4 $\times$ income\_insight\_score&   1952.4635\sym{***}&   1735.5061\sym{***}&      0.0001\sym{***}&      0.0004\sym{***}\\
                    &   (17.9759)         &   (16.4874)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=5 $\times$ income\_insight\_score&   1097.8002\sym{***}&    863.5732\sym{***}&      0.0000\sym{***}&      0.0002\sym{***}\\
                    &   (12.7890)         &   (10.5604)         &    (0.0000)         &    (0.0000)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=10&  -1166.6875\sym{***}&  -1085.1224\sym{***}&     -0.0008         &      0.0035\sym{*}  \\
                    &  (280.8816)         &  (273.3845)         &    (0.0007)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=11&  -1444.9881\sym{***}&  -1240.8015\sym{***}&     -0.0004         &     -0.0019         \\
                    &  (348.4315)         &  (336.6366)         &    (0.0006)         &    (0.0020)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=12&   1612.6422\sym{***}&   1604.9570\sym{***}&      0.0008         &     -0.0004         \\
                    &  (344.1458)         &  (339.0056)         &    (0.0007)         &    (0.0020)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=13&   2625.9380\sym{***}&   2662.1623\sym{***}&      0.0006         &     -0.0012         \\
                    &  (363.9634)         &  (359.4848)         &    (0.0007)         &    (0.0020)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=14&   1801.2139\sym{***}&   1916.1200\sym{***}&     -0.0005         &     -0.0109\sym{***}\\
                    &  (373.0559)         &  (365.5711)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=15&   1474.2199\sym{***}&   1697.5626\sym{***}&     -0.0024\sym{***}&     -0.0232\sym{***}\\
                    &  (401.4680)         &  (390.0670)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=16&   3799.1505\sym{***}&   3961.2445\sym{***}&     -0.0029\sym{***}&     -0.0169\sym{***}\\
                    &  (388.5181)         &  (384.1942)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=17&   3783.9663\sym{***}&   4065.0349\sym{***}&     -0.0021\sym{***}&     -0.0218\sym{***}\\
                    &  (401.0175)         &  (395.1065)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=18&   3228.7385\sym{***}&   3623.7583\sym{***}&     -0.0026\sym{***}&     -0.0259\sym{***}\\
                    &  (432.5044)         &  (424.6404)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=19&   2253.1998\sym{***}&   2774.4652\sym{***}&     -0.0030\sym{***}&     -0.0388\sym{***}\\
                    &  (464.2469)         &  (448.7633)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=20&   7661.7573\sym{***}&   6126.5120\sym{***}&     -0.0031\sym{***}&     -0.0398\sym{***}\\
                    & (1769.3813)         &  (417.5696)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=21&   6047.7282\sym{***}&   6181.2001\sym{***}&     -0.0019\sym{***}&     -0.0381\sym{***}\\
                    &  (455.7142)         &  (437.2698)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=22&   4694.7312\sym{***}&   4968.2342\sym{***}&     -0.0031\sym{***}&     -0.0417\sym{***}\\
                    &  (455.1850)         &  (429.4733)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=23&   3756.2095\sym{***}&   4076.5411\sym{***}&     -0.0032\sym{***}&     -0.0447\sym{***}\\
                    &  (474.5155)         &  (443.9493)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=24&   6868.9380\sym{***}&   6977.9162\sym{***}&     -0.0023\sym{***}&     -0.0435\sym{***}\\
                    &  (489.2160)         &  (474.3826)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=25&   6424.7926\sym{***}&   6475.6200\sym{***}&     -0.0021\sym{***}&     -0.0454\sym{***}\\
                    &  (502.2322)         &  (484.2288)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=26&   4489.7433\sym{***}&   4666.3118\sym{***}&     -0.0024\sym{***}&     -0.0482\sym{***}\\
                    &  (452.1957)         &  (427.3797)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=27&   3054.5056\sym{***}&   3191.6698\sym{***}&     -0.0036\sym{***}&     -0.0539\sym{***}\\
                    &  (471.7868)         &  (435.5384)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=28&   4765.1144\sym{***}&   4861.4185\sym{***}&     -0.0027\sym{***}&     -0.0513\sym{***}\\
                    &  (443.8955)         &  (426.8697)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=29&   4622.2415\sym{***}&   4652.8951\sym{***}&     -0.0044\sym{***}&     -0.0508\sym{***}\\
                    &  (478.3655)         &  (449.1051)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=30&   3505.9269\sym{***}&   3682.9751\sym{***}&     -0.0044\sym{***}&     -0.0522\sym{***}\\
                    &  (499.7732)         &  (489.8492)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=31&   2666.3567\sym{***}&   2830.0352\sym{***}&     -0.0047\sym{***}&     -0.0551\sym{***}\\
                    &  (470.3169)         &  (451.8304)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=32&   3503.5579\sym{***}&   3549.9572\sym{***}&     -0.0035\sym{***}&     -0.0534\sym{***}\\
                    &  (438.4033)         &  (428.4970)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=33&   2490.0491\sym{***}&   2508.5823\sym{***}&     -0.0039\sym{***}&     -0.0534\sym{***}\\
                    &  (426.5889)         &  (413.1427)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=34&    900.3724\sym{**} &    948.9227\sym{**} &     -0.0039\sym{***}&     -0.0538\sym{***}\\
                    &  (438.1823)         &  (420.8992)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=35&   -176.5212         &   -164.5694         &     -0.0044\sym{***}&     -0.0570\sym{***}\\
                    &  (397.9242)         &  (384.6766)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=36&   -291.0755         &   -469.8549         &     -0.0043\sym{***}&     -0.0547\sym{***}\\
                    &  (403.3586)         &  (384.2321)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=37&   -142.7127         &   -194.4393         &     -0.0027\sym{***}&     -0.0543\sym{***}\\
                    &  (408.3265)         &  (392.8914)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=38&  -1662.5180\sym{***}&  -1889.4706\sym{***}&     -0.0047\sym{***}&     -0.0571\sym{***}\\
                    &  (437.3000)         &  (391.2335)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=39&  -2117.4298\sym{***}&  -2224.5100\sym{***}&     -0.0031\sym{***}&     -0.0593\sym{***}\\
                    &  (422.6337)         &  (400.7750)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=40&  -1810.5507\sym{***}&  -1940.5082\sym{***}&     -0.0037\sym{***}&     -0.0583\sym{***}\\
                    &  (399.0882)         &  (380.8416)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=41&  -2040.9769\sym{***}&  -2134.8428\sym{***}&     -0.0044\sym{***}&     -0.0588\sym{***}\\
                    &  (408.8737)         &  (388.0779)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=42&  -2901.6172\sym{***}&  -3007.9099\sym{***}&     -0.0046\sym{***}&     -0.0571\sym{***}\\
                    &  (400.1335)         &  (380.9925)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=43&  -3609.4687\sym{***}&  -3706.0682\sym{***}&     -0.0057\sym{***}&     -0.0566\sym{***}\\
                    &  (421.6446)         &  (399.3451)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=44&  -3395.3953\sym{***}&  -3560.0856\sym{***}&     -0.0053\sym{***}&     -0.0528\sym{***}\\
                    &  (408.6593)         &  (386.1495)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=45&  -4393.5782\sym{***}&  -4491.7454\sym{***}&     -0.0057\sym{***}&     -0.0520\sym{***}\\
                    &  (419.8112)         &  (397.7782)         &    (0.0006)         &    (0.0018)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=46&  -5279.5462\sym{***}&  -5268.5676\sym{***}&     -0.0056\sym{***}&     -0.0481\sym{***}\\
                    &  (423.8287)         &  (398.3901)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=47&  -6674.0992\sym{***}&  -6490.9454\sym{***}&     -0.0054\sym{***}&     -0.0474\sym{***}\\
                    &  (449.6949)         &  (418.9439)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=48&  -5593.3751\sym{***}&  -5638.9228\sym{***}&     -0.0052\sym{***}&     -0.0445\sym{***}\\
                    &  (429.2180)         &  (399.6882)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=1 $\times$ quarter=49&  -6361.0322\sym{***}&  -6421.7542\sym{***}&     -0.0055\sym{***}&     -0.0460\sym{***}\\
                    &  (429.9464)         &  (400.8854)         &    (0.0006)         &    (0.0019)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=10&  -1008.6833\sym{***}&   -824.4737\sym{***}&     -0.0011\sym{**} &      0.0056\sym{***}\\
                    &  (216.3067)         &  (211.6859)         &    (0.0005)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=11&  -1898.9997\sym{***}&  -1518.8063\sym{***}&     -0.0007         &     -0.0026\sym{**} \\
                    &  (254.6605)         &  (247.8255)         &    (0.0005)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=12&   1325.4728\sym{***}&   1441.1742\sym{***}&     -0.0002         &      0.0026\sym{**} \\
                    &  (244.3671)         &  (240.7021)         &    (0.0005)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=13&   2734.6564\sym{***}&   2811.4254\sym{***}&     -0.0013\sym{***}&      0.0024\sym{**} \\
                    &  (266.8192)         &  (263.9722)         &    (0.0005)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=14&   2282.2523\sym{***}&   2490.9817\sym{***}&     -0.0035\sym{***}&     -0.0075\sym{***}\\
                    &  (302.7987)         &  (296.7123)         &    (0.0005)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=15&   1155.2595\sym{***}&   1499.7849\sym{***}&     -0.0059\sym{***}&     -0.0227\sym{***}\\
                    &  (299.5268)         &  (292.8837)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=16&   3350.7034\sym{***}&   3550.3422\sym{***}&     -0.0076\sym{***}&     -0.0171\sym{***}\\
                    &  (284.9589)         &  (281.9099)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=17&   3849.7305\sym{***}&   4026.3838\sym{***}&     -0.0067\sym{***}&     -0.0212\sym{***}\\
                    &  (289.1537)         &  (287.1834)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=18&   2142.0272\sym{***}&   2477.8228\sym{***}&     -0.0083\sym{***}&     -0.0290\sym{***}\\
                    &  (307.6643)         &  (304.1798)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=19&    953.6643\sym{***}&   1428.7049\sym{***}&     -0.0083\sym{***}&     -0.0413\sym{***}\\
                    &  (305.8164)         &  (299.4285)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=20&   6137.3274\sym{***}&   3697.9437\sym{***}&     -0.0081\sym{***}&     -0.0399\sym{***}\\
                    & (1285.1379)         &  (300.1246)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=21&   3637.6266\sym{***}&   3497.2756\sym{***}&     -0.0070\sym{***}&     -0.0404\sym{***}\\
                    &  (311.5318)         &  (302.9760)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=22&   1639.1991\sym{***}&   1644.3857\sym{***}&     -0.0086\sym{***}&     -0.0441\sym{***}\\
                    &  (307.0889)         &  (296.1910)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=23&    529.6152         &    268.9027         &     -0.0083\sym{***}&     -0.0497\sym{***}\\
                    &  (444.8261)         &  (301.2812)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=24&   1910.8970\sym{***}&   1736.8622\sym{***}&     -0.0074\sym{***}&     -0.0497\sym{***}\\
                    &  (296.6797)         &  (288.0193)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=25&   1242.9876\sym{***}&   1074.3442\sym{***}&     -0.0084\sym{***}&     -0.0509\sym{***}\\
                    &  (298.2229)         &  (289.4417)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=26&   -556.0468\sym{*}  &   -642.3907\sym{**} &     -0.0071\sym{***}&     -0.0544\sym{***}\\
                    &  (302.6202)         &  (293.7263)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=27&  -1953.8981\sym{***}&  -1998.7452\sym{***}&     -0.0084\sym{***}&     -0.0594\sym{***}\\
                    &  (310.6522)         &  (299.4224)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=28&   -585.0397\sym{**} &   -827.9411\sym{***}&     -0.0081\sym{***}&     -0.0581\sym{***}\\
                    &  (291.1413)         &  (282.4437)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=29&  -1299.6162\sym{***}&  -1545.7568\sym{***}&     -0.0098\sym{***}&     -0.0566\sym{***}\\
                    &  (295.7307)         &  (287.3166)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=30&  -2989.9158\sym{***}&  -3165.4269\sym{***}&     -0.0100\sym{***}&     -0.0583\sym{***}\\
                    &  (304.4767)         &  (293.8175)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=31&  -3987.7021\sym{***}&  -4187.3270\sym{***}&     -0.0098\sym{***}&     -0.0612\sym{***}\\
                    &  (303.5837)         &  (290.3369)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=32&  -3090.6708\sym{***}&  -3460.3423\sym{***}&     -0.0084\sym{***}&     -0.0581\sym{***}\\
                    &  (288.4900)         &  (279.6994)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=33&  -3917.3695\sym{***}&  -4301.2067\sym{***}&     -0.0095\sym{***}&     -0.0573\sym{***}\\
                    &  (293.6728)         &  (285.0267)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=34&  -4866.8273\sym{***}&  -5240.8689\sym{***}&     -0.0096\sym{***}&     -0.0588\sym{***}\\
                    &  (296.2632)         &  (285.6940)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=35&  -5304.6095\sym{***}&  -5718.2702\sym{***}&     -0.0093\sym{***}&     -0.0618\sym{***}\\
                    &  (291.5471)         &  (281.8215)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=36&  -6437.2495\sym{***}&  -6846.8557\sym{***}&     -0.0098\sym{***}&     -0.0586\sym{***}\\
                    &  (285.8138)         &  (276.0359)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=37&  -6549.3848\sym{***}&  -6991.0284\sym{***}&     -0.0077\sym{***}&     -0.0565\sym{***}\\
                    &  (304.6048)         &  (296.0924)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=38&  -7981.0423\sym{***}&  -8426.8045\sym{***}&     -0.0083\sym{***}&     -0.0604\sym{***}\\
                    &  (297.1916)         &  (286.7453)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=39&  -8029.4631\sym{***}&  -8514.0407\sym{***}&     -0.0065\sym{***}&     -0.0643\sym{***}\\
                    &  (302.5527)         &  (290.2360)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=40&  -8783.0434\sym{***}&  -9135.9195\sym{***}&     -0.0092\sym{***}&     -0.0627\sym{***}\\
                    &  (300.5910)         &  (290.5315)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=41&  -9475.4881\sym{***}&  -9840.1112\sym{***}&     -0.0102\sym{***}&     -0.0598\sym{***}\\
                    &  (303.9914)         &  (292.7855)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=42&  -9811.0848\sym{***}& -10184.9505\sym{***}&     -0.0097\sym{***}&     -0.0605\sym{***}\\
                    &  (313.5075)         &  (300.7642)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=43&  -9820.3987\sym{***}& -10217.9677\sym{***}&     -0.0102\sym{***}&     -0.0606\sym{***}\\
                    &  (313.0865)         &  (299.8104)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=44& -10839.7088\sym{***}& -11187.1937\sym{***}&     -0.0101\sym{***}&     -0.0576\sym{***}\\
                    &  (312.2140)         &  (298.9894)         &    (0.0004)         &    (0.0010)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=45& -11213.3681\sym{***}& -11531.4742\sym{***}&     -0.0106\sym{***}&     -0.0545\sym{***}\\
                    &  (318.1927)         &  (305.9746)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=46& -11640.1385\sym{***}& -11996.3851\sym{***}&     -0.0102\sym{***}&     -0.0544\sym{***}\\
                    &  (315.9497)         &  (302.1492)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=47& -12305.2110\sym{***}& -12582.7934\sym{***}&     -0.0104\sym{***}&     -0.0554\sym{***}\\
                    &  (322.4110)         &  (308.1568)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=48& -12645.3125\sym{***}& -12964.2702\sym{***}&     -0.0100\sym{***}&     -0.0499\sym{***}\\
                    &  (323.9904)         &  (308.6308)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=2 $\times$ quarter=49& -12826.3756\sym{***}& -13033.9146\sym{***}&     -0.0115\sym{***}&     -0.0498\sym{***}\\
                    &  (324.3062)         &  (309.2582)         &    (0.0004)         &    (0.0011)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=10&    713.2294         &    792.3069\sym{*}  &     -0.0025\sym{***}&      0.0038\sym{***}\\
                    &  (441.5564)         &  (432.9189)         &    (0.0008)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=11&    694.7420         &    962.0687\sym{*}  &     -0.0009         &     -0.0079\sym{***}\\
                    &  (503.2565)         &  (494.9744)         &    (0.0008)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=12&   2394.5748\sym{***}&   2628.3842\sym{***}&     -0.0021\sym{***}&     -0.0023         \\
                    &  (526.4856)         &  (519.8612)         &    (0.0008)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=13&   4913.6813\sym{***}&   4991.7961\sym{***}&     -0.0016\sym{**} &      0.0003         \\
                    &  (525.8622)         &  (521.3561)         &    (0.0008)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=14&   5420.0227\sym{***}&   5602.2594\sym{***}&     -0.0045\sym{***}&     -0.0122\sym{***}\\
                    &  (584.2538)         &  (578.8994)         &    (0.0008)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=15&   4636.8950\sym{***}&   4931.7259\sym{***}&     -0.0084\sym{***}&     -0.0312\sym{***}\\
                    &  (599.1542)         &  (591.7528)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=16&   4243.3149\sym{***}&   4515.8361\sym{***}&     -0.0146\sym{***}&     -0.0211\sym{***}\\
                    &  (569.7387)         &  (567.3101)         &    (0.0007)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=17&   3960.3743\sym{***}&   4079.6838\sym{***}&     -0.0115\sym{***}&     -0.0235\sym{***}\\
                    &  (557.3307)         &  (551.9145)         &    (0.0007)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=18&   1109.7600\sym{**} &   1310.0109\sym{**} &     -0.0158\sym{***}&     -0.0375\sym{***}\\
                    &  (560.7088)         &  (553.3203)         &    (0.0007)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=19&  -1800.3773\sym{***}&  -1681.0340\sym{***}&     -0.0162\sym{***}&     -0.0511\sym{***}\\
                    &  (581.9188)         &  (571.0971)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=20&   7836.7426\sym{**} &  -2812.5460\sym{***}&     -0.0177\sym{***}&     -0.0415\sym{***}\\
                    & (3311.8047)         &  (667.8066)         &    (0.0007)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=21&  -3104.7217\sym{***}&  -3892.3547\sym{***}&     -0.0167\sym{***}&     -0.0387\sym{***}\\
                    &  (674.8913)         &  (660.2109)         &    (0.0007)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=22&  -6237.2431\sym{***}&  -6988.9001\sym{***}&     -0.0182\sym{***}&     -0.0497\sym{***}\\
                    &  (550.2152)         &  (536.6093)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=23&  -9061.2152\sym{***}&  -9758.5731\sym{***}&     -0.0165\sym{***}&     -0.0594\sym{***}\\
                    &  (684.2486)         &  (664.9017)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=24&  -8464.0435\sym{***}&  -9343.2132\sym{***}&     -0.0158\sym{***}&     -0.0613\sym{***}\\
                    &  (676.0162)         &  (662.3123)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=25&  -9004.1940\sym{***}& -10035.0817\sym{***}&     -0.0167\sym{***}&     -0.0596\sym{***}\\
                    &  (635.3493)         &  (621.8882)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=26& -10505.0348\sym{***}& -11573.0216\sym{***}&     -0.0149\sym{***}&     -0.0613\sym{***}\\
                    &  (658.7121)         &  (642.8813)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=27& -12059.3466\sym{***}& -13070.4818\sym{***}&     -0.0163\sym{***}&     -0.0683\sym{***}\\
                    &  (645.0366)         &  (631.5515)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=28& -10935.3845\sym{***}& -12090.8944\sym{***}&     -0.0163\sym{***}&     -0.0710\sym{***}\\
                    &  (638.0895)         &  (623.9014)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=29& -10964.9503\sym{***}& -12345.5731\sym{***}&     -0.0192\sym{***}&     -0.0682\sym{***}\\
                    &  (640.0740)         &  (624.7544)         &    (0.0006)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=30& -12122.9723\sym{***}& -13539.8963\sym{***}&     -0.0196\sym{***}&     -0.0661\sym{***}\\
                    &  (647.4820)         &  (631.3081)         &    (0.0006)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=31& -13975.7858\sym{***}& -15321.7895\sym{***}&     -0.0175\sym{***}&     -0.0704\sym{***}\\
                    &  (644.4576)         &  (627.9438)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=32& -13101.6519\sym{***}& -14603.9935\sym{***}&     -0.0163\sym{***}&     -0.0637\sym{***}\\
                    &  (641.3890)         &  (628.7603)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=33& -13378.7539\sym{***}& -15032.7922\sym{***}&     -0.0181\sym{***}&     -0.0600\sym{***}\\
                    &  (641.8840)         &  (627.2284)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=34& -14137.5227\sym{***}& -15840.1385\sym{***}&     -0.0170\sym{***}&     -0.0608\sym{***}\\
                    &  (665.8320)         &  (644.8906)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=35& -14943.3979\sym{***}& -16620.7814\sym{***}&     -0.0164\sym{***}&     -0.0647\sym{***}\\
                    &  (651.1517)         &  (631.8232)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=36& -16017.9767\sym{***}& -17684.8172\sym{***}&     -0.0164\sym{***}&     -0.0593\sym{***}\\
                    &  (669.8387)         &  (649.6217)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=37& -16203.6811\sym{***}& -17808.2256\sym{***}&     -0.0145\sym{***}&     -0.0547\sym{***}\\
                    &  (662.2021)         &  (647.7590)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=38& -16767.9826\sym{***}& -18374.9570\sym{***}&     -0.0116\sym{***}&     -0.0632\sym{***}\\
                    &  (660.9968)         &  (647.0576)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=39& -16520.9519\sym{***}& -18265.2914\sym{***}&     -0.0103\sym{***}&     -0.0719\sym{***}\\
                    &  (668.2572)         &  (649.9082)         &    (0.0007)         &    (0.0013)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=40& -18912.0275\sym{***}& -20382.8109\sym{***}&     -0.0160\sym{***}&     -0.0679\sym{***}\\
                    &  (671.7279)         &  (656.2555)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=41& -18240.7306\sym{***}& -19889.7920\sym{***}&     -0.0181\sym{***}&     -0.0606\sym{***}\\
                    &  (671.4417)         &  (655.3961)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=42& -18372.3238\sym{***}& -20094.7532\sym{***}&     -0.0155\sym{***}&     -0.0637\sym{***}\\
                    &  (671.1588)         &  (655.3298)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=43& -18464.4474\sym{***}& -20248.0258\sym{***}&     -0.0159\sym{***}&     -0.0681\sym{***}\\
                    &  (698.4698)         &  (678.6553)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=44& -22027.5754\sym{***}& -23531.6388\sym{***}&     -0.0178\sym{***}&     -0.0605\sym{***}\\
                    &  (713.2295)         &  (695.4416)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=45& -22283.6440\sym{***}& -23844.0035\sym{***}&     -0.0175\sym{***}&     -0.0549\sym{***}\\
                    &  (704.2598)         &  (686.2377)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=46& -21439.5797\sym{***}& -23122.5400\sym{***}&     -0.0140\sym{***}&     -0.0574\sym{***}\\
                    &  (719.0087)         &  (699.7484)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=47& -21796.5357\sym{***}& -23317.6872\sym{***}&     -0.0161\sym{***}&     -0.0646\sym{***}\\
                    &  (724.4422)         &  (706.0690)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=48& -24624.2280\sym{***}& -25790.4258\sym{***}&     -0.0152\sym{***}&     -0.0561\sym{***}\\
                    &  (758.0766)         &  (738.0153)         &    (0.0007)         &    (0.0014)         \\
[1em]
cs\_bin\_l1=3 $\times$ quarter=49& -25415.3481\sym{***}& -26520.9500\sym{***}&     -0.0187\sym{***}&     -0.0509\sym{***}\\
                    &  (754.1299)         &  (732.5584)         &    (0.0007)         &    (0.0015)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=10&   1840.0487\sym{***}&   1638.1274\sym{***}&     -0.0010\sym{**} &      0.0001         \\
                    &  (208.1737)         &  (202.9047)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=11&   3407.8362\sym{***}&   3094.0854\sym{***}&     -0.0019\sym{***}&     -0.0064\sym{***}\\
                    &  (264.7355)         &  (257.3487)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=12&  -1189.8001\sym{***}&  -1058.3271\sym{***}&     -0.0030\sym{***}&     -0.0019\sym{**} \\
                    &  (280.6951)         &  (272.6677)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=13&   1545.4507\sym{***}&   1294.0016\sym{***}&      0.0003         &      0.0011         \\
                    &  (292.3858)         &  (284.4765)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=14&   3752.8559\sym{***}&   3342.1967\sym{***}&     -0.0034\sym{***}&     -0.0083\sym{***}\\
                    &  (316.4503)         &  (306.5681)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=15&   4741.4704\sym{***}&   4232.1640\sym{***}&     -0.0053\sym{***}&     -0.0182\sym{***}\\
                    &  (334.3335)         &  (325.4075)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=16&  -1069.3005\sym{***}&  -1198.3178\sym{***}&     -0.0105\sym{***}&     -0.0040\sym{***}\\
                    &  (325.3697)         &  (316.9629)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=17&    397.1058         &     93.5859         &     -0.0073\sym{***}&     -0.0077\sym{***}\\
                    &  (331.1851)         &  (324.5194)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=18&    161.6312         &   -310.6852         &     -0.0118\sym{***}&     -0.0171\sym{***}\\
                    &  (342.8497)         &  (333.0069)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=19&   -186.1165         &   -809.2757\sym{**} &     -0.0122\sym{***}&     -0.0188\sym{***}\\
                    &  (358.8288)         &  (348.6336)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=20&  10021.5754\sym{***}&  -2565.1360\sym{***}&     -0.0143\sym{***}&      0.0062\sym{***}\\
                    & (2307.7873)         &  (367.1139)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=21&  -2521.7329\sym{***}&  -3733.6988\sym{***}&     -0.0119\sym{***}&      0.0064\sym{***}\\
                    &  (389.4370)         &  (375.2253)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=22&  -3408.0673\sym{***}&  -4620.6458\sym{***}&     -0.0105\sym{***}&     -0.0131\sym{***}\\
                    &  (370.7264)         &  (359.8070)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=23&  -3234.7583\sym{***}&  -4535.0072\sym{***}&     -0.0102\sym{***}&     -0.0191\sym{***}\\
                    &  (376.6823)         &  (364.0085)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=24&  -3598.5037\sym{***}&  -5053.9001\sym{***}&     -0.0105\sym{***}&     -0.0218\sym{***}\\
                    &  (399.8147)         &  (386.6887)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=25&  -3326.5318\sym{***}&  -4968.4852\sym{***}&     -0.0111\sym{***}&     -0.0167\sym{***}\\
                    &  (397.3230)         &  (383.1572)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=26&  -3476.7451\sym{***}&  -5158.2362\sym{***}&     -0.0087\sym{***}&     -0.0081\sym{***}\\
                    &  (406.7421)         &  (393.1972)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=27&  -4704.3547\sym{***}&  -6423.2513\sym{***}&     -0.0107\sym{***}&     -0.0157\sym{***}\\
                    &  (406.1210)         &  (392.0371)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=28&  -5161.7534\sym{***}&  -6774.5447\sym{***}&     -0.0082\sym{***}&     -0.0262\sym{***}\\
                    &  (395.9967)         &  (384.3729)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=29&  -4252.9923\sym{***}&  -6046.7591\sym{***}&     -0.0120\sym{***}&     -0.0227\sym{***}\\
                    &  (400.3954)         &  (388.1643)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=30&  -4939.8647\sym{***}&  -6875.7465\sym{***}&     -0.0135\sym{***}&     -0.0160\sym{***}\\
                    &  (402.1326)         &  (389.4907)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=31&  -5823.3907\sym{***}&  -7786.2857\sym{***}&     -0.0102\sym{***}&     -0.0175\sym{***}\\
                    &  (419.3569)         &  (406.4998)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=32&  -7998.3497\sym{***}&  -9838.2477\sym{***}&     -0.0106\sym{***}&     -0.0106\sym{***}\\
                    &  (420.6881)         &  (407.8703)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=33&  -7908.5921\sym{***}&  -9866.9005\sym{***}&     -0.0104\sym{***}&     -0.0042\sym{***}\\
                    &  (425.6645)         &  (412.3831)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=34&  -7999.8374\sym{***}& -10059.2053\sym{***}&     -0.0094\sym{***}&     -0.0036\sym{***}\\
                    &  (429.7390)         &  (415.3647)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=35&  -9102.8204\sym{***}& -11047.3410\sym{***}&     -0.0083\sym{***}&     -0.0084\sym{***}\\
                    &  (420.2480)         &  (408.3804)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=36& -11001.2559\sym{***}& -12601.8813\sym{***}&     -0.0083\sym{***}&     -0.0063\sym{***}\\
                    &  (426.1297)         &  (414.8733)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=37& -10406.1060\sym{***}& -12085.0624\sym{***}&     -0.0060\sym{***}&     -0.0015\sym{**} \\
                    &  (428.9562)         &  (416.0936)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=38&  -8960.5209\sym{***}& -10681.7699\sym{***}&     -0.0024\sym{***}&     -0.0172\sym{***}\\
                    &  (436.1684)         &  (422.0382)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=39&  -6981.0973\sym{***}&  -9062.7089\sym{***}&     -0.0036\sym{***}&     -0.0292\sym{***}\\
                    &  (431.0213)         &  (418.0653)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=40& -10258.6060\sym{***}& -11873.7478\sym{***}&     -0.0098\sym{***}&     -0.0274\sym{***}\\
                    &  (437.4113)         &  (425.6645)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=41&  -9830.4382\sym{***}& -11665.9208\sym{***}&     -0.0119\sym{***}&     -0.0193\sym{***}\\
                    &  (441.7085)         &  (429.3389)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=42&  -8870.6943\sym{***}& -10975.4554\sym{***}&     -0.0091\sym{***}&     -0.0211\sym{***}\\
                    &  (437.3893)         &  (425.2495)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=43&  -8212.5725\sym{***}& -10504.3713\sym{***}&     -0.0099\sym{***}&     -0.0258\sym{***}\\
                    &  (449.4050)         &  (435.8436)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=44& -13521.1777\sym{***}& -15471.7196\sym{***}&     -0.0118\sym{***}&     -0.0177\sym{***}\\
                    &  (452.0309)         &  (439.4596)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=45& -12778.0796\sym{***}& -14871.0226\sym{***}&     -0.0104\sym{***}&     -0.0127\sym{***}\\
                    &  (445.5401)         &  (432.9999)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=46& -11065.2634\sym{***}& -13282.4524\sym{***}&     -0.0067\sym{***}&     -0.0178\sym{***}\\
                    &  (442.9181)         &  (431.3253)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=47& -10529.3581\sym{***}& -12812.0053\sym{***}&     -0.0096\sym{***}&     -0.0252\sym{***}\\
                    &  (448.5785)         &  (435.5132)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=48& -14680.8836\sym{***}& -16638.2002\sym{***}&     -0.0092\sym{***}&     -0.0191\sym{***}\\
                    &  (468.1203)         &  (454.6590)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=4 $\times$ quarter=49& -15316.9758\sym{***}& -17192.9092\sym{***}&     -0.0118\sym{***}&     -0.0107\sym{***}\\
                    &  (470.9179)         &  (456.8615)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=9&      0.0000         &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=10&   2134.5584\sym{***}&   1608.1322\sym{***}&     -0.0009\sym{**} &     -0.0002         \\
                    &  (202.5723)         &  (194.7042)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=11&   4805.6270\sym{***}&   3691.3294\sym{***}&     -0.0009\sym{*}  &     -0.0029\sym{***}\\
                    &  (280.7730)         &  (267.1036)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=12&   1546.8631\sym{***}&   1002.5024\sym{***}&     -0.0011\sym{**} &      0.0002         \\
                    &  (293.1894)         &  (278.0688)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=13&   4128.1961\sym{***}&   3248.1708\sym{***}&      0.0081\sym{***}&      0.0028\sym{***}\\
                    &  (310.3618)         &  (294.4940)         &    (0.0005)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=14&   6879.1440\sym{***}&   5428.5073\sym{***}&     -0.0002         &     -0.0013\sym{**} \\
                    &  (331.1891)         &  (312.9948)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=15&   9945.6657\sym{***}&   7816.1974\sym{***}&     -0.0007         &     -0.0050\sym{***}\\
                    &  (344.6113)         &  (323.4246)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=16&   4430.6649\sym{***}&   3138.2751\sym{***}&     -0.0046\sym{***}&      0.0071\sym{***}\\
                    &  (337.2190)         &  (314.2767)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=17&   6458.5125\sym{***}&   5032.6028\sym{***}&     -0.0001         &      0.0066\sym{***}\\
                    &  (348.7589)         &  (322.9845)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=18&   7939.5609\sym{***}&   6131.4085\sym{***}&     -0.0034\sym{***}&      0.0005         \\
                    &  (351.8572)         &  (326.3532)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=19&   9596.8869\sym{***}&   7371.9300\sym{***}&     -0.0050\sym{***}&      0.0045\sym{***}\\
                    &  (362.0820)         &  (335.0156)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=20&  26350.7041\sym{***}&   5197.1844\sym{***}&     -0.0065\sym{***}&      0.0366\sym{***}\\
                    & (3393.8592)         &  (347.8192)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=21&   6386.5130\sym{***}&   4600.7892\sym{***}&     -0.0004         &      0.0341\sym{***}\\
                    &  (386.5832)         &  (356.4741)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=22&   6744.7145\sym{***}&   4895.1930\sym{***}&      0.0042\sym{***}&      0.0092\sym{***}\\
                    &  (394.2357)         &  (364.1052)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=23&   7681.3939\sym{***}&   5502.8602\sym{***}&      0.0014\sym{***}&      0.0086\sym{***}\\
                    &  (444.2298)         &  (415.2962)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=24&   7632.7329\sym{***}&   5189.9945\sym{***}&     -0.0002         &      0.0074\sym{***}\\
                    &  (411.6159)         &  (379.6476)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=25&   8570.3216\sym{***}&   6058.8363\sym{***}&     -0.0003         &      0.0138\sym{***}\\
                    &  (391.6498)         &  (360.8721)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=26&   8132.6972\sym{***}&   5374.3823\sym{***}&     -0.0007         &      0.0311\sym{***}\\
                    &  (399.0140)         &  (365.4819)         &    (0.0004)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=27&   6886.1664\sym{***}&   4470.1920\sym{***}&      0.0033\sym{***}&      0.0243\sym{***}\\
                    &  (405.7568)         &  (371.7318)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=28&   6808.9586\sym{***}&   4753.4656\sym{***}&      0.0106\sym{***}&      0.0049\sym{***}\\
                    &  (407.9009)         &  (371.4064)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=29&   9162.9536\sym{***}&   6934.5873\sym{***}&      0.0023\sym{***}&      0.0075\sym{***}\\
                    &  (407.5591)         &  (372.0689)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=30&   8791.1121\sym{***}&   6419.1227\sym{***}&     -0.0032\sym{***}&      0.0199\sym{***}\\
                    &  (413.0925)         &  (376.6991)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=31&   8596.1642\sym{***}&   6121.2830\sym{***}&      0.0022\sym{***}&      0.0210\sym{***}\\
                    &  (427.8659)         &  (389.2623)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=32&   4771.9775\sym{***}&   3000.6412\sym{***}&      0.0054\sym{***}&      0.0254\sym{***}\\
                    &  (437.7862)         &  (399.4950)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=33&   5834.8751\sym{***}&   4177.2300\sym{***}&      0.0067\sym{***}&      0.0303\sym{***}\\
                    &  (447.8947)         &  (407.0565)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=34&   5384.1452\sym{***}&   3753.9322\sym{***}&      0.0052\sym{***}&      0.0332\sym{***}\\
                    &  (452.2637)         &  (411.3168)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=35&   5633.8852\sym{***}&   4225.0331\sym{***}&      0.0087\sym{***}&      0.0299\sym{***}\\
                    &  (456.5739)         &  (415.0326)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=36&   4698.1447\sym{***}&   3442.5821\sym{***}&      0.0089\sym{***}&      0.0268\sym{***}\\
                    &  (461.6168)         &  (417.1566)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=37&   5307.4777\sym{***}&   4418.7964\sym{***}&      0.0114\sym{***}&      0.0276\sym{***}\\
                    &  (471.5531)         &  (428.0311)         &    (0.0005)         &    (0.0008)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=38&   6407.8275\sym{***}&   5364.1673\sym{***}&      0.0141\sym{***}&      0.0082\sym{***}\\
                    &  (464.7069)         &  (419.1127)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=39&   8905.5993\sym{***}&   7318.0338\sym{***}&      0.0078\sym{***}&     -0.0024\sym{***}\\
                    &  (471.1238)         &  (425.6304)         &    (0.0005)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=40&   7101.8385\sym{***}&   5692.5047\sym{***}&      0.0001         &     -0.0016\sym{**} \\
                    &  (473.8296)         &  (429.7554)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=41&   8985.9037\sym{***}&   7200.6250\sym{***}&     -0.0022\sym{***}&      0.0048\sym{***}\\
                    &  (473.3596)         &  (428.9086)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=42&   9582.3004\sym{***}&   7326.6877\sym{***}&     -0.0014\sym{***}&      0.0025\sym{***}\\
                    &  (481.6807)         &  (435.1868)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=43&  12153.9659\sym{***}&   9311.4294\sym{***}&     -0.0010\sym{**} &      0.0005         \\
                    &  (482.8843)         &  (437.0989)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=44&   8287.5469\sym{***}&   5899.5350\sym{***}&     -0.0038\sym{***}&      0.0075\sym{***}\\
                    &  (492.1145)         &  (443.3600)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=45&   9819.0949\sym{***}&   7257.5094\sym{***}&     -0.0008\sym{*}  &      0.0101\sym{***}\\
                    &  (497.8047)         &  (447.6786)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=46&  11111.0591\sym{***}&   8068.7891\sym{***}&      0.0023\sym{***}&      0.0062\sym{***}\\
                    &  (500.7382)         &  (452.0718)         &    (0.0005)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=47&  11940.0194\sym{***}&   8622.2227\sym{***}&     -0.0013\sym{***}&     -0.0003         \\
                    &  (518.0097)         &  (465.6739)         &    (0.0004)         &    (0.0006)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=48&   8869.0798\sym{***}&   5886.1427\sym{***}&     -0.0009\sym{**} &      0.0053\sym{***}\\
                    &  (524.7920)         &  (467.2124)         &    (0.0004)         &    (0.0007)         \\
[1em]
cs\_bin\_l1=5 $\times$ quarter=49&   8844.5333\sym{***}&   5707.3762\sym{***}&     -0.0038\sym{***}&      0.0116\sym{***}\\
                    &  (526.4818)         &  (469.7158)         &    (0.0004)         &    (0.0007)         \\
[1em]
Constant            & -44017.9984\sym{***}& -40408.4583\sym{***}&     -0.0034\sym{***}&      0.0451\sym{***}\\
                    & (1337.1248)         & (1036.3985)         &    (0.0005)         &    (0.0017)         \\
\hline
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         \\
Observations        &25559345.0000         &25559345.0000         &25559345.0000         &25559345.0000         \\
$R^2$               &      0.1651         &      0.2899         &      0.0081         &      0.0230         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize }\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
\end{table}


==> Tables/old/vulnerable_detail/vulnerable_all.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Vulnerable Populations \label{tab:vulnerable_populations}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
& & &  \multicolumn{4}{c}{\underline{Credit Score Categories}} \\
& & & Deep Subprime, & Near & & Super\\
& & &  Subprime &  Prime & Prime &  Prime \\
\multicolumn{7}{l}{DV: Our Model Ranking - Credit Score Ranking}\\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{7}{l}{\underline{Panel A: Experian Sample}}\\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority              &      0.4752\sym{***}&      1.2813\sym{***}&      0.5618\sym{***}&     -0.7801\sym{***}&     -0.7139\sym{***}&     -1.3514\sym{***}\\
                    &    (0.0309)         &    (0.0366)         &    (0.0330)         &    (0.0400)         &    (0.0431)         &    (0.0474)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young         &      0.7730\sym{***}&      0.4470\sym{***}&      1.9292\sym{***}&      2.6345\sym{***}&     -0.9181\sym{***}&     -3.3753\sym{***}\\
                    &    (0.0574)         &    (0.0620)         &    (0.0923)         &    (0.0654)         &    (0.0641)         &    (0.1369)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$    &      4.1225\sym{***}&      5.7533\sym{***}&      2.2919\sym{***}&     -2.8897\sym{***}&     -3.9764\sym{***}&     -6.3473\sym{***}\\
                    &    (0.0497)         &    (0.0551)         &    (0.0343)         &    (0.0809)         &    (0.1080)         &    (0.2123)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years           &                     &     -6.3984\sym{***}&    -13.4328\sym{***}&    -12.7350\sym{***}&    -14.3038\sym{***}&     -8.3974\sym{***}\\
                    &                     &    (0.0380)         &    (0.0449)         &    (0.0848)         &    (0.1324)         &    (0.0952)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority$\times$ Default, next 2 years &                     &     -0.7831\sym{***}&     -0.1448\sym{***}&      0.0052         &      0.0928         &     -0.2651         \\
                    &                     &    (0.0277)         &    (0.0397)         &    (0.0642)         &    (0.0944)         &    (0.1688)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young  $\times$ Default, next 2 years &                     &      0.6667\sym{***}&     -0.8691\sym{***}&      0.4428\sym{***}&      5.7245\sym{***}&     -5.8865\sym{***}\\
                    &                     &    (0.0414)         &    (0.0739)         &    (0.0806)         &    (0.1102)         &    (0.2695)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$ $\times$ Default, next 2 years&                     &     -0.5651\sym{***}&      1.5208\sym{***}&      1.8297\sym{***}&      1.9646\sym{***}&     -7.6350\sym{***}\\
                    &                     &    (0.0396)         &    (0.0433)         &    (0.0654)         &    (0.1232)         &    (1.5636)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &     -1.0441\sym{***}&     -0.2104\sym{***}&     10.0994\sym{***}&      2.9506\sym{***}&      0.7830\sym{***}&     -4.5350\sym{***}\\
                    &    (0.0228)         &    (0.0227)         &    (0.0293)         &    (0.0281)         &    (0.0314)         &    (0.0081)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         \\
Observations      &26,240,879      &26,240,879      &6,786,915      &3,721,409      &9,536,207      &6,196,348      \\
$R^2$               &      0.0149         &      0.0400         &      0.2359         &      0.1121         &      0.0417         &      0.0282         \\ \hline 
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{7}{l}{\underline{Panel B: Experian-HMDA Sample}}\\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority                 &     -0.8221\sym{***}&     -0.7597\sym{***}&     -2.3464\sym{**} &     -1.9647\sym{***}&     -1.6716\sym{***}&     -0.5946\sym{*}  \\
                    &    (0.0784)         &    (0.0852)         &    (0.9638)         &    (0.6583)         &    (0.1756)         &    (0.3583)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young                &      1.7220\sym{***}&      1.7374\sym{***}&      6.7768\sym{***}&      3.0164\sym{***}&      0.9891\sym{***}&     -3.1641\sym{***}\\
                    &    (0.0712)         &    (0.0762)         &    (1.0200)         &    (0.6597)         &    (0.1367)         &    (0.4142)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$    &      2.2421\sym{***}&      2.5849\sym{***}&      1.4098         &     -1.5736\sym{**} &     -2.4265\sym{***}&     -3.9001\sym{*}  \\
                    &    (0.0989)         &    (0.1139)         &    (1.0082)         &    (0.7117)         &    (0.2131)         &    (2.1947)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years          &                     &     -3.4841\sym{***}&     -7.4418\sym{***}&     -6.8353\sym{***}&     -7.9994\sym{***}&     -7.9168\sym{***}\\
                    &                     &    (0.1102)         &    (0.7824)         &    (0.7736)         &    (0.3882)         &    (1.6763)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority$\times$ Default, next 2 years&                     &      0.7413\sym{***}&      1.9858\sym{*}  &      0.8675         &      0.0221         &      1.8054         \\
                    &                     &    (0.1808)         &    (1.1429)         &    (1.2279)         &    (0.7000)         &    (3.1098)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young  $\times$ Default, next 2 years&                     &     -0.9243\sym{***}&     -5.8244\sym{***}&     -3.0658\sym{**} &      2.2263\sym{***}&     -2.1895         \\
                    &                     &    (0.1952)         &    (1.2581)         &    (1.4004)         &    (0.7279)         &    (4.7704)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$ $\times$ Default, next 2 years&                     &      0.3450         &      0.4788         &      1.3140         &      0.5026         &     -5.2064         \\
                    &                     &    (0.2171)         &    (1.2596)         &    (1.4607)         &    (0.9525)         &    (8.7229)         \\
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &     -5.9403\sym{***}&     -5.6027\sym{***}&      2.4714\sym{***}&     -2.7625\sym{***}&     -5.8101\sym{***}&     -7.4084\sym{***}\\
                    &    (0.0219)         &    (0.0244)         &    (0.5358)         &    (0.2651)         &    (0.0499)         &    (0.0462)         \\
\hline
& & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         \\
Observations       & 756,179      & 756,179      & 101,133      & 116,383      & 355,693      & 182,970      \\
$R^2$               &      0.4947         &      0.4984         &      0.8921         &      0.8718         &      0.6703         &      0.7645         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes: This table reports regressions of the form specified by Equation (\ref{reg:spec}).  Young is an indicator variable if the individual is under 30 years old.  Income$_{p20}$ is an indicator variable if the individual belongs to the lowest quintile of the estimated income distribution. In Panel A, the Minority indicator is based on ZIP code level Black and Hispanic population being over 50\%. In Panel B, the Minority indicator is 1 if the individual is Black or Hispanic. In Panel B, the Female indicator is 1 if the individual is female. Panel A presents the full Experian sample, while Panel B provides the matched Experian-HMDA sample results. Standard errors are clustered by state and quarter in Panel A, and by ZIP and quarter in Panel B. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/old/vulnerable_detail/vulnerable_low_income_p20.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Vulnerable Populations: Low Income \label{tab:vulnerable_populations_experian_low_income}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
& & &  \multicolumn{8}{c}{\underline{Credit Score Categories}} \\
& & & \multicolumn{2}{c}{Deep Subprime, Subprime} & \multicolumn{2}{c}{Near Prime} & \multicolumn{2}{c}{Prime} & \multicolumn{2}{c}{Super Prime}\\
\multicolumn{11}{l}{DV: Our Model Ranking - Credit Score Ranking}\\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{11}{l}{\underline{Panel A: Experian Sample}}\\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$    &      5.9378\sym{***}&      6.0673\sym{***}&      3.5516\sym{***}&      2.9046\sym{***}&     -1.2329\sym{***}&     -1.6670\sym{***}&     -4.0492\sym{***}&     -4.4634\sym{***}&     -7.9212\sym{***}&     -7.6075\sym{***}\\
                    &    (0.0694)         &    (0.0770)         &    (0.0429)         &    (0.0394)         &    (0.0803)         &    (0.0838)         &    (0.1287)         &    (0.1364)         &    (0.2154)         &    (0.2009)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years         &     -6.5285\sym{***}&     -6.3915\sym{***}&    -13.0377\sym{***}&    -13.6549\sym{***}&    -12.3362\sym{***}&    -12.7950\sym{***}&    -12.6529\sym{***}&    -13.3496\sym{***}&     -9.4018\sym{***}&     -9.3679\sym{***}\\
                    &    (0.0353)         &    (0.0383)         &    (0.0406)         &    (0.0494)         &    (0.0727)         &    (0.0795)         &    (0.1086)         &    (0.1289)         &    (0.0889)         &    (0.0883)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$ $\times$ Default, next 2 years&                     &     -0.4382\sym{***}&                     &      1.3147\sym{***}&                     &      1.8874\sym{***}&                     &      5.0388\sym{***}&                     &     -8.3064\sym{***}\\
                    &                     &    (0.0481)         &                     &    (0.0352)         &                     &    (0.0616)         &                     &    (0.1520)         &                     &    (1.6082)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &      0.0662\sym{***}&      0.0469\sym{***}&     10.2537\sym{***}&     10.5615\sym{***}&      3.1097\sym{***}&      3.2119\sym{***}&      0.4448\sym{***}&      0.4850\sym{***}&     -4.8075\sym{***}&     -4.8078\sym{***}\\
                    &    (0.0114)         &    (0.0127)         &    (0.0199)         &    (0.0217)         &    (0.0171)         &    (0.0189)         &    (0.0156)         &    (0.0168)         &    (0.0010)         &    (0.0010)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &26,240,879     &26,240,879     &6,786,915     &6,786,915     &3,721,409     &3,721,409     &9,536,207     &9,536,207     &6,196,348     &6,196,348     \\
$R^2$               &      0.0391         &      0.0391         &      0.2330         &      0.2335         &      0.1070         &      0.1074         &      0.0399         &      0.0404         &      0.0226         &      0.0226         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{11}{l}{\underline{Panel B: Experian-HMDA Sample}}\\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$   &      3.4221\sym{***}&      3.4658\sym{***}&      3.1879\sym{***}&      3.9931\sym{***}&     -0.1645         &     -0.1117         &     -1.8474\sym{***}&     -1.9400\sym{***}&     -5.7014\sym{***}&     -5.5440\sym{**} \\
                    &    (0.0926)         &    (0.1059)         &    (0.6126)         &    (0.9258)         &    (0.5813)         &    (0.6462)         &    (0.1964)         &    (0.2014)         &    (2.1110)         &    (2.1789)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years    &     -3.5648\sym{***}&     -3.5183\sym{***}&     -8.9140\sym{***}&     -8.3046\sym{***}&     -7.2454\sym{***}&     -7.1862\sym{***}&     -7.5121\sym{***}&     -7.6899\sym{***}&     -7.6957\sym{***}&     -7.6614\sym{***}\\
                    &    (0.0822)         &    (0.0922)         &    (0.5423)         &    (0.6652)         &    (0.5622)         &    (0.6321)         &    (0.3001)         &    (0.3195)         &    (1.4286)         &    (1.4435)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Income$_{p20}$$\times$ Default, next 2 years&                     &     -0.2273         &                     &     -1.8208         &                     &     -0.3016         &                     &      1.6719\sym{*}  &                     &     -2.5143         \\
                    &                     &    (0.2005)         &                     &    (1.1693)         &                     &    (1.3360)         &                     &    (0.8816)         &                     &    (8.6784)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &     -5.3917\sym{***}&     -5.3961\sym{***}&      3.7564\sym{***}&      3.4582\sym{***}&     -2.5891\sym{***}&     -2.6006\sym{***}&     -5.8294\sym{***}&     -5.8213\sym{***}&     -7.6743\sym{***}&     -7.6747\sym{***}\\
                    &    (0.0138)         &    (0.0149)         &    (0.3470)         &    (0.4292)         &    (0.1607)         &    (0.1734)         &    (0.0230)         &    (0.0235)         &    (0.0128)         &    (0.0130)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        & 756,179     & 756,179     & 101,133     & 101,133     & 116,383     & 116,383     & 355,693     & 355,693     & 182,970     & 182,970     \\
$R^2$               &      0.4969         &      0.4969         &      0.8878         &      0.8879         &      0.8702         &      0.8702         &      0.6691         &      0.6691         &      0.7632         &      0.7632         \\
\hline\hline

\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes: This table reports regressions of the form specified by Equation (\ref{reg:spec}). Income$_{p20}$ is an indicator variable if the individual belongs to the lowest quintile of the estimated income distribution. Panel A presents the full Experian sample, while Panel B provides results for the matched Experian-HMDA sample. Standard errors are clustered by state and quarter in Panel A, and by ZIP and quarter in Panel B. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/old/vulnerable_detail/vulnerable_minority.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Vulnerable Populations: Minority Status \label{tab:vulnerable_populations_minority}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
& & &  \multicolumn{8}{c}{\underline{Credit Score Categories}} \\
& & & \multicolumn{2}{c}{Deep Subprime, Subprime} & \multicolumn{2}{c}{Near Prime} & \multicolumn{2}{c}{Prime} & \multicolumn{2}{c}{Super Prime}\\
\multicolumn{11}{l}{DV: Our Model Ranking - Credit Score Ranking}\\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{11}{l}{\underline{Panel A: Experian Sample}}\\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority           &      1.6318\sym{***}&      1.8608\sym{***}&      0.7182\sym{***}&      0.6869\sym{***}&     -0.9199\sym{***}&     -0.9454\sym{***}&     -0.7753\sym{***}&     -0.7816\sym{***}&     -1.4144\sym{***}&     -1.3996\sym{***}\\
                    &    (0.0373)         &    (0.0411)         &    (0.0226)         &    (0.0353)         &    (0.0328)         &    (0.0412)         &    (0.0454)         &    (0.0444)         &    (0.0485)         &    (0.0484)         \\        
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years    &     -5.3399\sym{***}&     -5.1112\sym{***}&    -13.0977\sym{***}&    -13.1154\sym{***}&    -12.3097\sym{***}&    -12.3343\sym{***}&    -12.7894\sym{***}&    -12.8064\sym{***}&     -9.3194\sym{***}&     -9.1702\sym{***}\\
                    &    (0.0331)         &    (0.0283)         &    (0.0434)         &    (0.0416)         &    (0.0731)         &    (0.0694)         &    (0.1129)         &    (0.1033)         &    (0.0899)         &    (0.0955)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority $\times$ Default, next 2 years&                     &     -0.9018\sym{***}&                     &      0.0615         &                     &      0.1002         &                     &      0.0763         &                     &     -0.8159\sym{***}\\
                    &                     &    (0.0296)         &                     &    (0.0413)         &                     &    (0.0627)         &                     &    (0.0974)         &                     &    (0.1794)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &      0.6806\sym{***}&      0.6430\sym{***}&     11.7417\sym{***}&     11.7503\sym{***}&      3.0126\sym{***}&      3.0179\sym{***}&      0.1730\sym{***}&      0.1739\sym{***}&     -4.6819\sym{***}&     -4.6833\sym{***}\\
                    &    (0.0085)         &    (0.0082)         &    (0.0220)         &    (0.0217)         &    (0.0152)         &    (0.0149)         &    (0.0102)         &    (0.0097)         &    (0.0045)         &    (0.0045)         \\ \hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &26,240,879     &26,240,879     &6,786,915     &6,786,915     &3,721,409     &3,721,409     &9,536,207     &9,536,207     &6,196,348     &6,196,348     \\
$R^2$               &      0.0195         &      0.0196         &      0.2180         &      0.2180         &      0.1064         &      0.1064         &      0.0353         &      0.0353         &      0.0233         &      0.0233         \\\hline 
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{11}{l}{\underline{Panel B: Experian-HMDA Sample}}\\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority       &     -0.4890\sym{***}&     -0.5971\sym{***}&     -1.6528\sym{**} &     -2.7371\sym{***}&     -1.8659\sym{***}&     -2.0593\sym{***}&     -1.7130\sym{***}&     -1.7187\sym{***}&     -0.5678         &     -0.5912\sym{*}  \\
                    &    (0.0787)         &    (0.0853)         &    (0.6629)         &    (0.9810)         &    (0.5948)         &    (0.6604)         &    (0.1724)         &    (0.1756)         &    (0.3564)         &    (0.3592)         \\
                    
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years        &     -3.1657\sym{***}&     -3.3483\sym{***}&     -9.0466\sym{***}&     -9.8099\sym{***}&     -7.2165\sym{***}&     -7.4923\sym{***}&     -7.5069\sym{***}&     -7.5276\sym{***}&     -7.7121\sym{***}&     -7.9582\sym{***}\\
                    &    (0.0820)         &    (0.0958)         &    (0.5441)         &    (0.6773)         &    (0.5617)         &    (0.6688)         &    (0.2999)         &    (0.3393)         &    (1.4312)         &    (1.6468)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Minority $\times$ Default, next 2 years&                     &      0.6806\sym{***}&                     &      2.1770\sym{*}  &                     &      0.9784         &                     &      0.0985         &                     &      1.3050         \\
                    &                     &    (0.1820)         &                     &    (1.1544)         &                     &    (1.2323)         &                     &    (0.7051)         &                     &    (3.1062)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &     -4.9267\sym{***}&     -4.9097\sym{***}&      5.4393\sym{***}&      5.7862\sym{***}&     -2.1920\sym{***}&     -2.1459\sym{***}&     -5.7323\sym{***}&     -5.7315\sym{***}&     -7.6291\sym{***}&     -7.6267\sym{***}\\
                    &    (0.0159)         &    (0.0168)         &    (0.3100)         &    (0.3846)         &    (0.1715)         &    (0.1855)         &    (0.0303)         &    (0.0308)         &    (0.0363)         &    (0.0369)         \\ \hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        & 756,179     & 756,179     & 101,133     & 101,133     & 116,383     & 116,383     & 355,693     & 355,693     & 182,970     & 182,970     \\
$R^2$               &      0.4931         &      0.4932         &      0.8864         &      0.8866         &      0.8707         &      0.8707         &      0.6691         &      0.6691         &      0.7631         &      0.7631         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes: This table reports regressions of the form specified by Equation (\ref{reg:spec}). In Panel A, the Minority indicator is based on ZIP code level Black and Hispanic population being over 50\%. In Panel B, the Minority indicator is 1 if the individual is Black or Hispanic. Panel A presents the full Experian sample, while Panel B provides the matched Experian-HMDA sample results. Standard errors are clustered by state and quarter in Panel A, and by ZIP and quarter in Panel B. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}

==> Tables/old/vulnerable_detail/vulnerable_young.tex <==
\begin{sidewaystable}[htbp]\centering
\begin{threeparttable}
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Vulnerable Populations: Age \label{tab:vulnerable_populations_young}}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{10}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
& & &  \multicolumn{8}{c}{\underline{Credit Score Categories}} \\
& & & \multicolumn{2}{c}{Deep Subprime, Subprime} & \multicolumn{2}{c}{Near Prime} & \multicolumn{2}{c}{Prime} & \multicolumn{2}{c}{Super Prime}\\
\multicolumn{11}{l}{DV: Our Model Ranking - Credit Score Ranking}\\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{11}{l}{\underline{Panel A: Experian Sample}}\\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young                 &      2.5985\sym{***}&      2.3873\sym{***}&      2.7214\sym{***}&      2.7578\sym{***}&      1.6486\sym{***}&      1.3929\sym{***}&     -1.4921\sym{***}&     -1.8365\sym{***}&     -3.6072\sym{***}&     -3.4670\sym{***}\\
                    &    (0.0687)         &    (0.0743)         &    (0.0642)         &    (0.0887)         &    (0.0699)         &    (0.0719)         &    (0.0873)         &    (0.0877)         &    (0.1388)         &    (0.1369)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years     &     -5.3321\sym{***}&     -5.5850\sym{***}&    -13.0184\sym{***}&    -12.9960\sym{***}&    -12.2866\sym{***}&    -12.5804\sym{***}&    -12.8634\sym{***}&    -14.2942\sym{***}&     -9.2089\sym{***}&     -8.5743\sym{***}\\
                    &    (0.0314)         &    (0.0358)         &    (0.0412)         &    (0.0454)         &    (0.0729)         &    (0.0866)         &    (0.1125)         &    (0.1395)         &    (0.0858)         &    (0.0890)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young $\times$ Default, next 2 years&                     &      0.9832\sym{***}&                     &     -0.0748         &                     &      1.2169\sym{***}&                     &      5.9132\sym{***}&                     &     -6.0761\sym{***}\\
                    &                     &    (0.0452)         &                     &    (0.0634)         &                     &    (0.0778)         &                     &    (0.1245)         &                     &    (0.2665)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &      0.4174\sym{***}&      0.4607\sym{***}&     11.0977\sym{***}&     11.0865\sym{***}&      2.3752\sym{***}&      2.4442\sym{***}&      0.4361\sym{***}&      0.5244\sym{***}&     -4.6603\sym{***}&     -4.6664\sym{***}\\
                    &    (0.0152)         &    (0.0164)         &    (0.0228)         &    (0.0295)         &    (0.0233)         &    (0.0255)         &    (0.0245)         &    (0.0249)         &    (0.0062)         &    (0.0060)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
State X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        &26,240,879     &26,240,879     &6,786,915     &6,786,915     &3,721,409     &3,721,409     &9,536,207     &9,536,207     &6,196,348     &6,196,348     \\
$R^2$               &      0.0227         &      0.0228         &      0.2251         &      0.2251         &      0.1079         &      0.1081         &      0.0365         &      0.0376         &      0.0263         &      0.0266         \\ \hline 
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{11}{l}{\underline{Panel B: Experian-HMDA Sample}}\\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young               &      2.3697\sym{***}&      2.4245\sym{***}&      4.9860\sym{***}&      7.4363\sym{***}&      1.9623\sym{***}&      2.4083\sym{***}&      0.5685\sym{***}&      0.4841\sym{***}&     -3.2290\sym{***}&     -3.2183\sym{***}\\
                    &    (0.0665)         &    (0.0712)         &    (0.6260)         &    (0.9121)         &    (0.5340)         &    (0.5916)         &    (0.1272)         &    (0.1293)         &    (0.4113)         &    (0.4128)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Default, next 2 years  &     -3.2276\sym{***}&     -3.1028\sym{***}&     -8.5706\sym{***}&     -6.7226\sym{***}&     -7.1918\sym{***}&     -6.4933\sym{***}&     -7.5064\sym{***}&     -8.0314\sym{***}&     -7.8600\sym{***}&     -7.7803\sym{***}\\
                    &    (0.0815)         &    (0.0944)         &    (0.5348)         &    (0.6215)         &    (0.5606)         &    (0.6548)         &    (0.2999)         &    (0.3496)         &    (1.4241)         &    (1.4748)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Young $\times$ Default, next 2 years&                     &     -0.4764\sym{***}&                     &     -5.6888\sym{***}&                     &     -2.5436\sym{**} &                     &      2.1679\sym{***}&                     &     -1.7855         \\
                    &                     &    (0.1805)         &                     &    (1.1529)         &                     &    (1.2704)         &                     &    (0.6679)         &                     &    (4.8503)         \\
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &     -5.5934\sym{***}&     -5.6065\sym{***}&      2.9903\sym{***}&      2.0678\sym{***}&     -3.2251\sym{***}&     -3.3699\sym{***}&     -6.1706\sym{***}&     -6.1451\sym{***}&     -7.4681\sym{***}&     -7.4684\sym{***}\\
                    &    (0.0187)         &    (0.0197)         &    (0.3366)         &    (0.4046)         &    (0.1888)         &    (0.2051)         &    (0.0406)         &    (0.0413)         &    (0.0299)         &    (0.0300)         \\
\hline
& & & & & & & & & & \\[\dimexpr-\normalbaselineskip+2pt]
ZIP X Quarter Fixed Effects&           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         &           X         \\
Observations        & 756,179     & 756,179     & 101,133     & 101,133     & 116,383     & 116,383     & 355,693     & 355,693     & 182,970     & 182,970     \\
$R^2$               &      0.4963         &      0.4963         &      0.8900         &      0.8913         &      0.8709         &      0.8711         &      0.6686         &      0.6687         &      0.7644         &      0.7644         \\
\hline\hline
\end{tabular*}
\begin{tablenotes}
\scriptsize
\item Notes: This table reports regressions of the form specified by Equation (\ref{reg:spec}). Young is an indicator variable if the individual is under 30 years old. Panel A presents the full Experian sample, while Panel B provides the matched Experian-HMDA sample results. Standard errors are clustered by state and quarter in Panel A, and by ZIP and quarter in Panel B. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/restrictions.tex <==
\begin{table}[htbp]
\caption{Itemized Sample Restrictions}\label{tab:restrictions}
\footnotesize
\begin{center}
\begin{tabular}{lll}
 &  & Observations \\ \hline 
   &  &  \\
 Credit Report Data &  & 40,600,000 \\ \hline
     &  &  \\
  Remove & &  \\ \hline 
   &  &  \\
Deceased &  & - 756,149    \\
Age &  & - 3,051,161     \\
Residence &  & - 15,366    \\ 
Credit Score & & - 155,149  \\
2004Q1-2005Q4 \& 2016Q3-2018Q2 & &  -9,795,920   \\
Prediction Window & & - 585,376    \\
\hline 
   & & \\
Prediction Sample & & 26,240,879\\ \hline \hline 
\end{tabular}
\end{center}
\end{table}

==> Tables/risk_comp_age.tex <==
\begin{table}[!ht]
\begin{threeparttable}
\caption{Credit Score and Model Risk Profile Comparison by Age Group}\label{tab:risk_comp}
    \centering
    \small
    \begin{tabular}{l|ccccc|c}
     
    & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
     &\multicolumn{5}{c}{ Model Based Risk Profile} \\ 
            & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt] \hline
            & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
        Credit Score & Deep Subprime & Subprime & Near Prime & Prime  & Super Prime & Disagreement \\ 
        & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt] \hline
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
 \multicolumn{6}{l}{\underline{Panel A: Age $\le$ 30}} \\ 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime & 43.41 & 45.12 & 7.85 & 3.60 & 0.02 & 56.59 \\ 
Subprime & 11.26 & 52.16 & 21.77 & 14.75 & 0.07 & 47.84 \\
Near Prime & 0.71 & 34.41 & 30.05 & 33.29 & 1.54 & 69.95 \\ 
Prime & 0.08 & 3.78 & 12.60 & 72.28 & 11.26 & 27.72 \\ 
Super Prime & 0.05 & 0.16 & 0.24 & 56.24 & 43.31 & 56.69 \\
& & & & &  & \\ \hline 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
 \multicolumn{6}{l}{\underline{Panel B: Age $>$ 30}} \\ 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime & 46.08    & 42.62    & 9.53     & 1.73     & 0.04     & 53.92    \\ 
Subprime      & 16.19    & 52.95    & 22.77    & 7.99     & 0.09     & 47.05    \\ 
Near Prime    & 2.03     & 39.48    & 30.47    & 26.03    & 1.99     & 69.53    \\ 
Prime         & 0.20     & 4.67     & 12.92    & 64.32    & 17.89    & 35.68    \\ 
Super Prime   & 0.01     & 0.04     & 0.14     & 24.06    & 75.74    & 24.26    \\
\hline \hline
    \end{tabular}
        
\begin{tablenotes}
\footnotesize
\item Notes: Rows correspond to industry-defined credit score risk profiles, defined in Table \ref{tab:risk_def}. Columns are fractions in each corresponding model-based risk profile. Column ``Disagreement" reports the fraction of borrowers in each credit score risk profile that would be placed in a different risk profile by our model. All values in percentage. Total \# of observations: 26,240,879; 6,184,996 with age $\le$ 30, and 20,055,883 over 30. Time period 2006Q1-2016Q2. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/risk_comp_income.tex <==
\begin{table}[!ht]
\begin{threeparttable}
\caption{Credit Score and Model Risk Profile Comparison by Income Group}\label{tab:risk_comp}
    \centering
    \small
    \begin{tabular}{l|ccccc|c}
     
    & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
     &\multicolumn{5}{c}{ Model Based Risk Profile} \\ 
            & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt] \hline
            & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
        Credit Score & Deep Subprime & Subprime & Near Prime & Prime  & Super Prime & Disagreement \\ 
        & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt] \hline
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
 \multicolumn{6}{l}{\underline{Panel A: Income $\le$ Income$_{p20}$ }} \\ 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime & 40.43    & 47.11    & 9.94     & 2.49     & 0.03     & 59.57    \\
Subprime      & 11.02    & 54.42    & 23.62    & 10.88    & 0.05     & 45.58    \\
Near Prime    & 0.91     & 41.46    & 28.40    & 28.40    & 0.83     & 71.60    \\
Prime         & 0.16     & 6.70     & 20.08    & 70.21    & 2.85     & 29.79    \\
Super Prime   & 0.20     & 0.75     & 1.54     & 67.81    & 29.70    & 70.30    \\
& & & & &  & \\ \hline 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
 \multicolumn{6}{l}{\underline{Panel B: Income $>$ Income$_{p20}$}} \\ 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime & 53.80    & 36.89    & 6.92     & 2.36     & 0.04     & 46.20    \\
Subprime      & 17.86    & 51.22    & 21.45    & 9.37     & 0.11     & 48.78    \\
Near Prime    & 1.92     & 36.82    & 31.06    & 27.97    & 2.23     & 68.94    \\
Prime         & 0.17     & 4.13     & 11.88    & 66.01    & 17.81    & 33.99    \\
Super Prime   & 0.02     & 0.05     & 0.14     & 25.64    & 74.15    & 25.85    \\
\hline \hline
    \end{tabular}
        
\begin{tablenotes}
\footnotesize
\item Notes: Rows correspond to industry-defined credit score risk profiles, defined in Table \ref{tab:risk_def}. Columns are fractions in each corresponding model-based risk profile. Column ``Disagreement" reports the fraction of borrowers in each credit score risk profile that would be placed in a different risk profile by our model. All values in percentage. Total \# of observations: 26,240,879; 5,566,986 in the lowest quintile of the income distribution, and 20,673,893 outside. Time period 2006Q1-2016Q2. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/risk_comp_minority.tex <==
\begin{table}[!ht]
\begin{threeparttable}
\caption{Credit Score and Model Risk Profile Comparison by Minority Status}\label{tab:risk_comp}
    \centering
    \small
    \begin{tabular}{l|ccccc|c}
     
    & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
     &\multicolumn{5}{c}{ Model Based Risk Profile} \\ 
            & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt] \hline
            & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
        Credit Score & Deep Subprime & Subprime & Near Prime & Prime  & Super Prime & Disagreement \\ 
        & & & & &  & \\[\dimexpr-\normalbaselineskip+2pt] \hline
 \multicolumn{6}{l}{\underline{Panel A: ZIP Minority Population $\ge$ 50\% }} \\ 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime & 45.17    & 44.30    & 8.60     & 1.91     & 0.02     & 54.83    \\
Subprime      & 15.17    & 52.71    & 22.93    & 9.13     & 0.06     & 47.29    \\
Near Prime    & 2.13     & 42.73    & 28.49    & 25.03    & 1.62     & 71.51    \\
Prime         & 0.30     & 6.16     & 15.55    & 64.06    & 13.93    & 35.94    \\
Super Prime   & 0.03     & 0.09     & 0.26     & 32.80    & 66.82    & 33.18    \\
& & & & &  & \\ \hline 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
 \multicolumn{6}{l}{\underline{Panel B: ZIP Minority Population $<$ 50\%}} \\ 
& & & & &  & \\[\dimexpr-\normalbaselineskip+2pt]
Deep Subprime & 45.01    & 43.24    & 9.03     & 2.68     & 0.04     & 54.99    \\
Subprime      & 14.47    & 52.71    & 22.28    & 10.45    & 0.09     & 47.29    \\
Near Prime    & 1.52     & 36.74    & 30.87    & 28.94    & 1.93     & 69.13    \\
Prime         & 0.15     & 4.10     & 12.32    & 66.96    & 16.48    & 33.04    \\
Super Prime   & 0.01     & 0.04     & 0.13     & 24.96    & 74.85    & 25.15    \\
\hline \hline
    \end{tabular}
        
\begin{tablenotes}
\footnotesize
\item Notes: Rows correspond to industry-defined credit score risk profiles, defined in Table \ref{tab:risk_def}. Columns are fractions in each corresponding model-based risk profile. Column ``Disagreement" reports the fraction of borrowers in each credit score risk profile that would be placed in a different risk profile by our model. All values in percentage. Total number of observations: 26,240,879; 4,873,733 with ZIP minority population $\ge$ 50\%, and 21,367,146 with less than 50\%. Time period 2006Q1-2016Q2. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/score_comparison.tex <==
% \begin{sidewaystable}[htpb]\centering
% \begin{threeparttable}
% \caption{Decile Comparison}\label{tab:credit_score_model_deciles}
% \begin{tabular}{l*{10}{c}}\hline
% \textbf{Credit Score Decile} & \multicolumn{10}{c}{\textbf{Our Model Decile}} \\
% \hline
%  $\downarrow$ & \textbf{First} & \textbf{Second} & \textbf{Third} & \textbf{Fourth} & \textbf{Fifth} & \textbf{Sixth} & \textbf{Seventh} & \textbf{Eighth} & \textbf{Ninth} & \textbf{Tenth} \\
% \hline
% \textbf{First} & 59.26 & 30.30 & 8.29 & 1.54 & 0.43 & 0.12 & 0.03 & 0.01 & 0.01 & 0.00 \\
% \textbf{Second} & 30.07 & 35.97 & 23.45 & 7.62 & 2.04 & 0.60 & 0.17 & 0.06 & 0.03 & 0.01 \\
% \textbf{Third} & 8.83 & 22.90 & 33.91 & 21.55 & 8.54 & 2.98 & 0.88 & 0.25 & 0.14 & 0.03 \\
% \textbf{Fourth} & 1.43 & 7.72 & 21.90 & 33.82 & 21.13 & 9.84 & 3.11 & 0.64 & 0.34 & 0.06 \\
% \textbf{Fifth} & 0.29 & 1.86 & 7.84 & 21.95 & 31.25 & 23.26 & 10.35 & 2.09 & 0.92 & 0.19 \\
% \textbf{Sixth} & 0.13 & 0.97 & 3.69 & 10.60 & 23.27 & 28.85 & 22.43 & 6.99 & 2.47 & 0.60 \\
% \textbf{Seventh} & 0.02 & 0.25 & 0.83 & 2.71 & 10.59 & 24.25 & 31.45 & 18.93 & 8.40 & 2.58 \\
% \textbf{Eighth} & 0.00 & 0.01 & 0.03 & 0.16 & 2.56 & 8.57 & 22.32 & 30.23 & 24.01 & 12.11 \\
% \textbf{Ninth} & 0.00 & 0.01 & 0.01 & 0.02 & 0.18 & 1.42 & 8.13 & 29.32 & 33.04 & 27.87 \\
% \textbf{Tenth} & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.11 & 1.15 & 11.51 & 30.65 & 56.54 \\
% \hline
% \end{tabular}
% \begin{tablenotes}
% \footnotesize
% \item Notes: This table displays a comparison of score deciles across Credit Score and our model. Consumers were categorized into deciles, representing groups of 10\% of the sample. For each credit score decile, we calculate the percentage of customers that fall into each decile based on our model. The entries marked as ``0.00'' indicate the presence of some consumers, albeit in numbers so small that they round down to zero. The purpose of this classification is to provide clarity on the number of consumers who have similar scores across the models and those who have significant score discrepancies. 44\% of consumers in adjacent deciles, 37\% in matching deciles, 15\% are two deciles off, while 4\% of borrowers are three or more deciles off.


% \end{tablenotes}
% \end{threeparttable}
% \end{sidewaystable}


==> Tables/table_6_blattner_cs.tex <==
\begin{sidewaystable}[ht]
\begin{threeparttable}
    \centering
    \footnotesize
    \caption{Testing Data Bias: Credit Score}
    \label{table:bias}
    \begin{tabular}{llccccccc}
        & &  \multicolumn{3}{c}{AUC} & \multicolumn{3}{c}{Share} \\ 
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        & &  Non-Protected Group & Protected Group & Diff & Non-Protected Group & Protected Group & Diff \\ \hline 
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        \multicolumn{8}{l}{\underline{Panel A: Minority Status}} \\
   &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
Thick file: no   mortgage & 90+ DPD         & 0.792 & 0.790 & 0.002 & 0.020 & 0.033 & -0.012 \\
                          & At most 60+ DPD & 0.711 & 0.710 & 0.001 & 0.005 & 0.007 & -0.001 \\
                          & Current         & 0.863 & 0.830 & 0.033 & 0.207 & 0.147 & 0.060  \\
Thick file: with mortgage & 90+ DPD         & 0.809 & 0.799 & 0.010 & 0.017 & 0.024 & -0.007 \\
                          & At most 60+ DPD & 0.704 & 0.682 & 0.023 & 0.009 & 0.009 & 0.000  \\
                          & Current         & 0.835 & 0.803 & 0.032 & 0.267 & 0.142 & 0.126  \\
Thin file                 & 90+ DPD         & 0.641 & 0.637 & 0.003 & 0.096 & 0.187 & -0.090 \\
                          & At most 60+ DPD & 0.620 & 0.608 & 0.013 & 0.009 & 0.014 & -0.005 \\
                          & Current         & 0.764 & 0.705 & 0.058 & 0.368 & 0.438 & -0.069 \\ 
&  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        \multicolumn{8}{l}{\underline{Panel B: Age Group}} \\
&  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
Thick file: no   mortgage & 90+ DPD         & 0.791 & 0.790 & 0.001  & 0.027 & 0.009 & 0.018  \\
                          & At most 60+ DPD & 0.712 & 0.708 & 0.004  & 0.007 & 0.002 & 0.005  \\
                          & Current         & 0.863 & 0.832 & 0.031  & 0.237 & 0.064 & 0.173  \\
Thick file: with mortgage & 90+ DPD         & 0.806 & 0.821 & -0.015 & 0.024 & 0.003 & 0.021  \\
                          & At most 60+ DPD & 0.700 & 0.703 & -0.002 & 0.011 & 0.001 & 0.010  \\
                          & Current         & 0.834 & 0.813 & 0.020  & 0.310 & 0.032 & 0.278  \\
Thin file                 & 90+ DPD         & 0.636 & 0.639 & -0.003 & 0.096 & 0.170 & -0.075 \\
                          & At most 60+ DPD & 0.590 & 0.662 & -0.072 & 0.007 & 0.018 & -0.011 \\
                          & Current         & 0.762 & 0.748 & 0.014  & 0.283 & 0.701 & -0.418 \\ 
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        \multicolumn{8}{l}{\underline{Panel C: Income Group}} \\
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
Thick file: no   mortgage & 90+ DPD         & 0.789 & 0.767 & 0.022  & 0.023 & 0.023 & 0.000  \\
                          & At most 60+ DPD & 0.704 & 0.668 & 0.036  & 0.006 & 0.003 & 0.003  \\
                          & Current         & 0.855 & 0.713 & 0.142  & 0.241 & 0.029 & 0.212  \\
Thick file: with mortgage & 90+ DPD         & 0.807 & 0.769 & 0.038  & 0.022 & 0.005 & 0.018  \\
                          & At most 60+ DPD & 0.700 & 0.625 & 0.074  & 0.011 & 0.001 & 0.010  \\
                          & Current         & 0.832 & 0.725 & 0.106  & 0.308 & 0.007 & 0.301  \\
Thin file                 & 90+ DPD         & 0.657 & 0.621 & 0.036  & 0.060 & 0.309 & -0.248 \\
                          & At most 60+ DPD & 0.597 & 0.619 & -0.022 & 0.006 & 0.022 & -0.015 \\
                          & Current         & 0.759 & 0.666 & 0.093  & 0.322 & 0.601 & -0.279 \\ 
        \hline \hline 

    \end{tabular}
\begin{tablenotes}
\item Note: The table shows results from testing data bias. Each row corresponds to a subsample of observations. Categories are mutually exclusive. Share refers to the share of individuals in that subsample. AUC refers to the Area Under the Curve measure of the VantageScore 3.0 credit score. Non-protected groups: non-minority, age $>$ 30, income $>$ p20. Thin file: less than 10 years of credit history and less than 3 open accounts.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}

==> Tables/table_6_blattner_our_model.tex <==
\begin{sidewaystable}[ht]
\begin{threeparttable}
    \centering
    \footnotesize
    \caption{Testing Data Bias: Our Model}
    \label{table:bias}
    \begin{tabular}{llccccccc}
        & &  \multicolumn{3}{c}{AUC} & \multicolumn{3}{c}{Share} \\ 
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        & &  Non-Protected Group & Protected Group & Diff & Non-Protected Group & Protected Group & Diff \\ \hline 
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        \multicolumn{8}{l}{\underline{Panel A: Minority Status}} \\
   &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
Thick file: no   mortgage & 90+ DPD         & 0.858 & 0.855 & 0.003  & 0.020 & 0.033 & -0.012 \\
                          & At most 60+ DPD & 0.742 & 0.736 & 0.006  & 0.005 & 0.007 & -0.001 \\
                          & Current         & 0.871 & 0.839 & 0.032  & 0.207 & 0.147 & 0.060  \\
Thick file: with mortgage & 90+ DPD         & 0.870 & 0.864 & 0.006  & 0.017 & 0.024 & -0.007 \\
                          & At most 60+ DPD & 0.733 & 0.714 & 0.019  & 0.009 & 0.009 & 0.000  \\
                          & Current         & 0.843 & 0.809 & 0.034  & 0.267 & 0.142 & 0.126  \\
Thin file                 & 90+ DPD         & 0.858 & 0.862 & -0.003 & 0.096 & 0.187 & -0.090 \\
                          & At most 60+ DPD & 0.718 & 0.727 & -0.009 & 0.009 & 0.014 & -0.005 \\
                          & Current         & 0.837 & 0.797 & 0.040  & 0.368 & 0.438 & -0.069 \\ 
&  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        \multicolumn{8}{l}{\underline{Panel B: Age Group}} \\
&  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
Thick file: no   mortgage & 90+ DPD         & 0.859 & 0.844 & 0.015  & 0.027 & 0.009 & 0.018  \\
                          & At most 60+ DPD & 0.743 & 0.729 & 0.014  & 0.007 & 0.002 & 0.005  \\
                          & Current         & 0.871 & 0.840 & 0.031  & 0.237 & 0.064 & 0.173  \\
Thick file: with mortgage & 90+ DPD         & 0.868 & 0.862 & 0.007  & 0.024 & 0.003 & 0.021  \\
                          & At most 60+ DPD & 0.730 & 0.727 & 0.003  & 0.011 & 0.001 & 0.010  \\
                          & Current         & 0.843 & 0.818 & 0.024  & 0.310 & 0.032 & 0.278  \\
Thin file                 & 90+ DPD         & 0.863 & 0.849 & 0.013  & 0.096 & 0.170 & -0.075 \\
                          & At most 60+ DPD & 0.717 & 0.725 & -0.008 & 0.007 & 0.018 & -0.011 \\
                          & Current         & 0.847 & 0.806 & 0.041  & 0.283 & 0.701 & -0.418\\ 
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
        \multicolumn{8}{l}{\underline{Panel C: Income Group}} \\
     &  &  & & & & &\\[\dimexpr-\normalbaselineskip+3pt]
Thick file: no   mortgage & 90+ DPD         & 0.858 & 0.834 & 0.025  & 0.023 & 0.023 & 0.000  \\
                          & At most 60+ DPD & 0.735 & 0.705 & 0.029  & 0.006 & 0.003 & 0.003  \\
                          & Current         & 0.863 & 0.729 & 0.134  & 0.241 & 0.029 & 0.212  \\
Thick file: with mortgage & 90+ DPD         & 0.869 & 0.846 & 0.023  & 0.022 & 0.005 & 0.018  \\
                          & At most 60+ DPD & 0.729 & 0.681 & 0.048  & 0.011 & 0.001 & 0.010  \\
                          & Current         & 0.840 & 0.757 & 0.083  & 0.308 & 0.007 & 0.301  \\
Thin file                 & 90+ DPD         & 0.869 & 0.849 & 0.020  & 0.060 & 0.309 & -0.248 \\
                          & At most 60+ DPD & 0.706 & 0.715 & -0.009 & 0.006 & 0.022 & -0.015 \\
                          & Current         & 0.835 & 0.775 & 0.060  & 0.322 & 0.601 & -0.279 \\ 
        \hline \hline 

    \end{tabular}
\begin{tablenotes}
\item Note: The table shows results from testing data bias. Each row corresponds to a subsample of observations. Categories are mutually exclusive. Share refers to the share of individuals in that subsample. AUC refers to the Area Under the Curve measure of the VantageScore 3.0 credit score. Non-protected groups: non-minority, age $>$ 30, income $>$ p20. Thin file: less than 10 years of credit history and less than 3 open accounts.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}

==> Tables/thin_files_vulnerable.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\begin{threeparttable}
\caption{Vulnerable Status and Length of Credit History}\label{tab:vulnerable_thin_group_proportions}
\begin{tabular}{p{2in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}}
\hline
&&&& \\[\dimexpr-\normalbaselineskip+2pt]
Type & Age $\le$ 30 & Age $>$ 30 & Income $\le$ p20 & Income $>$ p20 & Non-Minority & Minority \\ \hline
&&&& \\[\dimexpr-\normalbaselineskip+2pt]
``Thick file"             & 0.1998 & 0.8195 &0.1746 & 0.8078 & 0.6973 & 0.5688  \\ 
&&&& \\[\dimexpr-\normalbaselineskip+2pt]
``Thin file"             & 	0.8002 & 0.1805 	 & 0.8254 & 0.1922 & 0.3027	& 0.4312  \\ \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Notes: This table presents the proportion of borrowers with ``thick" and ``thin" credit files across vulnerable groups. A ``thick file" refers to borrowers with a credit history over 10 years, while a ``thin file" indicates a limited or sparse credit history. The proportions reflect the distribution of credit file thickness among different groups. Source: Authors' calculations based on Experian Data.
\end{tablenotes}
\end{threeparttable}
\end{table}     

==> Tables/vulnerable_auc.tex <==
\begin{table}[!ht]
    \centering
    \caption{Performance by Demographic group} \label{tab:perf-vulnerables}
    \begin{tabular}{llllllll}
    \hline \hline
    &  &  &  &  &   & & \\[\dimexpr-\normalbaselineskip+3pt]
        AUC score & All & \multicolumn{2}{c}{Income } &  \multicolumn{2}{c}{Age } &  \multicolumn{2}{c}{Minority } \\ \hline
         &  &  &  &  &   & & \\[\dimexpr-\normalbaselineskip+3pt]
        ~ & ~ & ${<p20}$ & ${\geq p20}$ & $< 30 $& $\geq 30$ & Yes & No \\ 
        Credit Score & 0.856 & 0.735 & 0.867 & 0.824 & 0.865 & 0.802 & 0.864 \\ 
        Our model & 0.906 & 0.855 & 0.908 & 0.881 & 0.913 & 0.881 & 0.91 \\  \hline \hline
    \end{tabular}
   
\end{table}
